A new compressed cover tree for k-nearest neighbour search and the stable-under-noise mergegram of a point cloud

This thesis consists of two topics related to computational geometry and one topic related to topological data analysis (TDA), which combines fields of computational geometry and algebraic topology for analyzing data. The first part studies the classical problem of finding k nearest neighbors to m query points in a larger set of n reference points in any metric space. The second part is about the construction of a Minimum Spanning Tree (MST) on any finite metric space. The third part extends the key concept of persistence within Topological Data Analysis in a new direction.

==> Definitions/journalnames.tex <==
%% Website Name%%% Website Name%%% Full Name%%% Short Name%%% DOI abbr%%% ISSN%% \continuouspages%
%\DeclareOption{}{\gdef\@journal{}\gdef\@journalfull{}\gdef\@journalshort{}\gdef\@doiabbr{}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{acoustics}{\gdef\@journal{acoustics}\gdef\@journalfull{Acoustics}\gdef\@journalshort{Acoustics}\gdef\@doiabbr{acoustics}\gdef\@ISSN{2624-599X}\gdef\@continuouspages{yes}}
\DeclareOption{actuators}{\gdef\@journal{actuators}\gdef\@journalfull{Actuators}\gdef\@journalshort{Actuators}\gdef\@doiabbr{act}\gdef\@ISSN{2076-0825}}
%\DeclareOption{addictions}{\gdef\@journal{addictions}\gdef\@journalfull{Addictions}\gdef\@journalshort{Addictions}\gdef\@doiabbr{}\gdef\@ISSN{0006-0006}}
\DeclareOption{admsci}{\gdef\@journal{admsci}\gdef\@journalfull{Administrative Sciences}\gdef\@journalshort{Adm. Sci.}\gdef\@doiabbr{admsci}\gdef\@ISSN{2076-3387}}
\DeclareOption{adolescents}{\gdef\@journal{adolescents}\gdef\@journalfull{Adolescents}\gdef\@journalshort{Adolescents}\gdef\@doiabbr{adolescents}\gdef\@ISSN{2673-7051}\gdef\@continuouspages{yes}}
\DeclareOption{aerospace}{\gdef\@journal{aerospace}\gdef\@journalfull{Aerospace}\gdef\@journalshort{Aerospace}\gdef\@doiabbr{aerospace}\gdef\@ISSN{2226-4310}}
\DeclareOption{agriculture}{\gdef\@journal{agriculture}\gdef\@journalfull{Agriculture}\gdef\@journalshort{Agriculture}\gdef\@doiabbr{agriculture}\gdef\@ISSN{2077-0472}}
\DeclareOption{agriengineering}{\gdef\@journal{agriengineering}\gdef\@journalfull{AgriEngineering}\gdef\@journalshort{AgriEngineering}\gdef\@doiabbr{agriengineering}\gdef\@ISSN{2624-7402}\gdef\@continuouspages{yes}}
\DeclareOption{agronomy}{\gdef\@journal{agronomy}\gdef\@journalfull{Agronomy}\gdef\@journalshort{Agronomy}\gdef\@doiabbr{agronomy}\gdef\@ISSN{2073-4395}}
\DeclareOption{ai}{\gdef\@journal{ai}\gdef\@journalfull{AI}\gdef\@journalshort{AI}\gdef\@doiabbr{ai}\gdef\@ISSN{2673-2688}\gdef\@continuouspages{yes}}
\DeclareOption{algorithms}{\gdef\@journal{algorithms}\gdef\@journalfull{Algorithms}\gdef\@journalshort{Algorithms}\gdef\@doiabbr{a}\gdef\@ISSN{1999-4893}}
\DeclareOption{allergies}{\gdef\@journal{allergies}\gdef\@journalfull{Allergies}\gdef\@journalshort{Allergies}\gdef\@doiabbr{allergies}\gdef\@ISSN{2313-5786}}
\DeclareOption{analytica}{\gdef\@journal{analytica}\gdef\@journalfull{Analytica}\gdef\@journalshort{Analytica}\gdef\@doiabbr{analy}\gdef\@ISSN{2673-4532}\gdef\@continuouspages{yes}}
\DeclareOption{animals}{\gdef\@journal{animals}\gdef\@journalfull{Animals}\gdef\@journalshort{Animals}\gdef\@doiabbr{ani}\gdef\@ISSN{2076-2615}}
\DeclareOption{antibiotics}{\gdef\@journal{antibiotics}\gdef\@journalfull{Antibiotics}\gdef\@journalshort{Antibiotics}\gdef\@doiabbr{antibiotics}\gdef\@ISSN{2079-6382}}
\DeclareOption{antibodies}{\gdef\@journal{antibodies}\gdef\@journalfull{Antibodies}\gdef\@journalshort{Antibodies}\gdef\@doiabbr{antib}\gdef\@ISSN{2073-4468}}
\DeclareOption{antioxidants}{\gdef\@journal{antioxidants}\gdef\@journalfull{Antioxidants}\gdef\@journalshort{Antioxidants}\gdef\@doiabbr{antiox}\gdef\@ISSN{2076-3921}}
\DeclareOption{appliedchem}{\gdef\@journal{appliedchem}\gdef\@journalfull{AppliedChem}\gdef\@journalshort{AppliedChem}\gdef\@doiabbr{appliedchem}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{applmech}{\gdef\@journal{applmech}\gdef\@journalfull{Applied Mechanics}\gdef\@journalshort{Appl. Mech.}\gdef\@doiabbr{applmech}\gdef\@ISSN{2673-3161}\gdef\@continuouspages{yes}}
\DeclareOption{applmicrobiol}{\gdef\@journal{applmicrobiol}\gdef\@journalfull{Applied Microbiology}\gdef\@journalshort{Appl. Microbiol.}\gdef\@doiabbr{applmicrobiol}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{applnano}{\gdef\@journal{applnano}\gdef\@journalfull{Applied Nano}\gdef\@journalshort{Appl. Nano}\gdef\@doiabbr{applnano}\gdef\@ISSN{2673-3501}\gdef\@continuouspages{yes}}
\DeclareOption{applsci}{\gdef\@journal{applsci}\gdef\@journalfull{Applied Sciences}\gdef\@journalshort{Appl. Sci.}\gdef\@doiabbr{app}\gdef\@ISSN{2076-3417}}
\DeclareOption{arts}{\gdef\@journal{arts}\gdef\@journalfull{Arts}\gdef\@journalshort{Arts}\gdef\@doiabbr{arts}\gdef\@ISSN{2076-0752}}
\DeclareOption{asi}{\gdef\@journal{asi}\gdef\@journalfull{Applied System Innovation}\gdef\@journalshort{Appl. Syst. Innov.}\gdef\@doiabbr{asi}\gdef\@ISSN{2571-5577}}
\DeclareOption{atmosphere}{\gdef\@journal{atmosphere}\gdef\@journalfull{Atmosphere}\gdef\@journalshort{Atmosphere}\gdef\@doiabbr{atmos}\gdef\@ISSN{2073-4433}}
\DeclareOption{atoms}{\gdef\@journal{atoms}\gdef\@journalfull{Atoms}\gdef\@journalshort{Atoms}\gdef\@doiabbr{atoms}\gdef\@ISSN{2218-2004}}
\DeclareOption{audiolres}{\gdef\@journal{audiolres}\gdef\@journalfull{Audiology Research}\gdef\@journalshort{Audiol. Res.}\gdef\@doiabbr{audiolres}\gdef\@ISSN{2039-4349}\gdef\@continuouspages{yes}}
\DeclareOption{automation}{\gdef\@journal{automation}\gdef\@journalfull{Automation}\gdef\@journalshort{Automation}\gdef\@doiabbr{automation}\gdef\@ISSN{2673-4052}\gdef\@continuouspages{yes}}
\DeclareOption{axioms}{\gdef\@journal{axioms}\gdef\@journalfull{Axioms}\gdef\@journalshort{Axioms}\gdef\@doiabbr{axioms}\gdef\@ISSN{2075-1680}}
\DeclareOption{batteries}{\gdef\@journal{batteries}\gdef\@journalfull{Batteries}\gdef\@journalshort{Batteries}\gdef\@doiabbr{batteries}\gdef\@ISSN{2313-0105}}
\DeclareOption{bdcc}{\gdef\@journal{bdcc}\gdef\@journalfull{Big Data and Cognitive Computing}\gdef\@journalshort{Big Data Cogn. Comput.}\gdef\@doiabbr{bdcc}\gdef\@ISSN{2504-2289}}
\DeclareOption{behavsci}{\gdef\@journal{behavsci}\gdef\@journalfull{Behavioral Sciences}\gdef\@journalshort{Behav. Sci.}\gdef\@doiabbr{bs}\gdef\@ISSN{2076-328X}}
\DeclareOption{beverages}{\gdef\@journal{beverages}\gdef\@journalfull{Beverages}\gdef\@journalshort{Beverages}\gdef\@doiabbr{beverages}\gdef\@ISSN{2306-5710}}
\DeclareOption{biochem}{\gdef\@journal{biochem}\gdef\@journalfull{BioChem}\gdef\@journalshort{BioChem}\gdef\@doiabbr{biochem}\gdef\@ISSN{2673-6411}\gdef\@continuouspages{yes}}
\DeclareOption{bioengineering}{\gdef\@journal{bioengineering}\gdef\@journalfull{Bioengineering}\gdef\@journalshort{Bioengineering}\gdef\@doiabbr{bioengineering}\gdef\@ISSN{2306-5354}}
\DeclareOption{biologics}{\gdef\@journal{biologics}\gdef\@journalfull{Biologics}\gdef\@journalshort{Biologics}\gdef\@doiabbr{biologics}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{biology}{\gdef\@journal{biology}\gdef\@journalfull{Biology}\gdef\@journalshort{Biology}\gdef\@doiabbr{biology}\gdef\@ISSN{2079-7737}}
\DeclareOption{biomechanics}{\gdef\@journal{biomechanics}\gdef\@journalfull{Biomechanics}\gdef\@journalshort{Biomechanics}\gdef\@doiabbr{biomechanics}\gdef\@ISSN{2673-7078}\gdef\@continuouspages{yes}}
\DeclareOption{biomed}{\gdef\@journal{biomed}\gdef\@journalfull{BioMed}\gdef\@journalshort{BioMed}\gdef\@doiabbr{biomed}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{biomedicines}{\gdef\@journal{biomedicines}\gdef\@journalfull{Biomedicines}\gdef\@journalshort{Biomedicines}\gdef\@doiabbr{biomedicines}\gdef\@ISSN{2227-9059}}
\DeclareOption{biomedinformatics}{\gdef\@journal{biomedinformatics}\gdef\@journalfull{Biomedinformatics}\gdef\@journalshort{Biomedinformatics}\gdef\@doiabbr{biomedinformatics}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{biomimetics}{\gdef\@journal{biomimetics}\gdef\@journalfull{Biomimetics}\gdef\@journalshort{Biomimetics}\gdef\@doiabbr{biomimetics}\gdef\@ISSN{2313-7673}}
\DeclareOption{biomolecules}{\gdef\@journal{biomolecules}\gdef\@journalfull{Biomolecules}\gdef\@journalshort{Biomolecules}\gdef\@doiabbr{biom}\gdef\@ISSN{2218-273X}}
\DeclareOption{biophysica}{\gdef\@journal{biophysica}\gdef\@journalfull{Biophysica}\gdef\@journalshort{Biophysica}\gdef\@doiabbr{biophysica}\gdef\@ISSN{2673-4125}}
\DeclareOption{biosensors}{\gdef\@journal{biosensors}\gdef\@journalfull{Biosensors}\gdef\@journalshort{Biosensors}\gdef\@doiabbr{bios}\gdef\@ISSN{2079-6374}}
\DeclareOption{biotech}{\gdef\@journal{biotech}\gdef\@journalfull{BioTech}\gdef\@journalshort{BioTech}\gdef\@doiabbr{biotech}\gdef\@ISSN{2673-6284}}
\DeclareOption{birds}{\gdef\@journal{birds}\gdef\@journalfull{Birds}\gdef\@journalshort{Birds}\gdef\@doiabbr{birds}\gdef\@ISSN{2673-6004}\gdef\@continuouspages{yes}}
\DeclareOption{bloods}{\gdef\@journal{bloods}\gdef\@journalfull{Bloods}\gdef\@journalshort{Bloods}\gdef\@doiabbr{bloods}\gdef\@ISSN{2673-415X}}
\DeclareOption{brainsci}{\gdef\@journal{brainsci}\gdef\@journalfull{Brain Sciences}\gdef\@journalshort{Brain Sci.}\gdef\@doiabbr{brainsci}\gdef\@ISSN{2076-3425}}
\DeclareOption{buildings}{\gdef\@journal{buildings}\gdef\@journalfull{Buildings}\gdef\@journalshort{Buildings}\gdef\@doiabbr{buildings}\gdef\@ISSN{2075-5309}}
\DeclareOption{businesses}{\gdef\@journal{businesses}\gdef\@journalfull{Businesses}\gdef\@journalshort{Businesses}\gdef\@doiabbr{bus}\gdef\@ISSN{2673-7116}\gdef\@continuouspages{yes}}
\DeclareOption{cancers}{\gdef\@journal{cancers}\gdef\@journalfull{Cancers}\gdef\@journalshort{Cancers}\gdef\@doiabbr{cancers}\gdef\@ISSN{2072-6694}}
\DeclareOption{carbon}{\gdef\@journal{carbon}\gdef\@journalfull{C}\gdef\@journalshort{C}\gdef\@doiabbr{c}\gdef\@ISSN{2311-5629}}
\DeclareOption{cardiogenetics}{\gdef\@journal{cardiogenetics}\gdef\@journalfull{Cardiogenetics}\gdef\@journalshort{Cardiogenetics}\gdef\@doiabbr{cardiogenetics}\gdef\@ISSN{2035-8148}\gdef\@continuouspages{yes}}
\DeclareOption{catalysts}{\gdef\@journal{catalysts}\gdef\@journalfull{Catalysts}\gdef\@journalshort{Catalysts}\gdef\@doiabbr{catal}\gdef\@ISSN{2073-4344}}
\DeclareOption{cells}{\gdef\@journal{cells}\gdef\@journalfull{Cells}\gdef\@journalshort{Cells}\gdef\@doiabbr{cells}\gdef\@ISSN{2073-4409}}
\DeclareOption{ceramics}{\gdef\@journal{ceramics}\gdef\@journalfull{Ceramics}\gdef\@journalshort{Ceramics}\gdef\@doiabbr{ceramics}\gdef\@ISSN{2571-6131}\gdef\@continuouspages{yes}}
\DeclareOption{challenges}{\gdef\@journal{challenges}\gdef\@journalfull{Challenges}\gdef\@journalshort{Challenges}\gdef\@doiabbr{challe}\gdef\@ISSN{2078-1547}}
\DeclareOption{chemengineering}{\gdef\@journal{chemengineering}\gdef\@journalfull{ChemEngineering}\gdef\@journalshort{ChemEngineering}\gdef\@doiabbr{chemengineering}\gdef\@ISSN{2305-7084}}
\DeclareOption{chemistry}{\gdef\@journal{chemistry}\gdef\@journalfull{Chemistry}\gdef\@journalshort{Chemistry}\gdef\@doiabbr{chemistry}\gdef\@ISSN{2624-8549}\gdef\@continuouspages{yes}}
\DeclareOption{chemosensors}{\gdef\@journal{chemosensors}\gdef\@journalfull{Chemosensors}\gdef\@journalshort{Chemosensors}\gdef\@doiabbr{chemosensors}\gdef\@ISSN{2227-9040}}
\DeclareOption{chemproc}{\gdef\@journal{chemproc}\gdef\@journalfull{Chemistry Proceedings}\gdef\@journalshort{Chem. Proc.}\gdef\@doiabbr{chemproc}\gdef\@ISSN{2673-4583}}
\DeclareOption{children}{\gdef\@journal{children}\gdef\@journalfull{Children}\gdef\@journalshort{Children}\gdef\@doiabbr{children}\gdef\@ISSN{2227-9067}}
\DeclareOption{civileng}{\gdef\@journal{civileng}\gdef\@journalfull{CivilEng}\gdef\@journalshort{CivilEng}\gdef\@doiabbr{civileng}\gdef\@ISSN{2673-4109}\gdef\@continuouspages{yes}}
\DeclareOption{cleantechnol}{\gdef\@journal{cleantechnol}\gdef\@journalfull{Clean Technologies}\gdef\@journalshort{Clean Technol.}\gdef\@doiabbr{cleantechnol}\gdef\@ISSN{2571-8797}\gdef\@continuouspages{yes}}
\DeclareOption{climate}{\gdef\@journal{climate}\gdef\@journalfull{Climate}\gdef\@journalshort{Climate}\gdef\@doiabbr{cli}\gdef\@ISSN{2225-1154}}
\DeclareOption{clinpract}{\gdef\@journal{clinpract}\gdef\@journalfull{Clinics and Practice}\gdef\@journalshort{Clin. Prac.}\gdef\@doiabbr{clinpract}\gdef\@ISSN{2039-7283}\gdef\@continuouspages{yes}}
\DeclareOption{clockssleep}{\gdef\@journal{clockssleep}\gdef\@journalfull{Clocks \& Sleep}\gdef\@journalshort{Clocks\&Sleep}\gdef\@doiabbr{clockssleep}\gdef\@ISSN{2624-5175}\gdef\@continuouspages{yes}}
\DeclareOption{cmd}{\gdef\@journal{cmd}\gdef\@journalfull{Corrosion and Materials Degradation}\gdef\@journalshort{Corros. Mater. Degrad.}\gdef\@doiabbr{cmd}\gdef\@ISSN{2624-5558}\gdef\@continuouspages{yes}}
\DeclareOption{coatings}{\gdef\@journal{coatings}\gdef\@journalfull{Coatings}\gdef\@journalshort{Coatings}\gdef\@doiabbr{coatings}\gdef\@ISSN{2079-6412}}
\DeclareOption{colloids}{\gdef\@journal{colloids}\gdef\@journalfull{Colloids Interfaces}\gdef\@journalshort{Colloids Interfaces}\gdef\@doiabbr{colloids}\gdef\@ISSN{2504-5377}}
\DeclareOption{compounds}{\gdef\@journal{compounds}\gdef\@journalfull{Compounds}\gdef\@journalshort{Compounds}\gdef\@doiabbr{compounds}\gdef\@ISSN{2673-6918}\gdef\@continuouspages{yes}}
\DeclareOption{computation}{\gdef\@journal{computation}\gdef\@journalfull{Computation}\gdef\@journalshort{Computation}\gdef\@doiabbr{computation}\gdef\@ISSN{2079-3197}}
\DeclareOption{computers}{\gdef\@journal{computers}\gdef\@journalfull{Computers}\gdef\@journalshort{Computers}\gdef\@doiabbr{computers}\gdef\@ISSN{2073-431X}}
\DeclareOption{condensedmatter}{\gdef\@journal{condensedmatter}\gdef\@journalfull{Condensed Matter}\gdef\@journalshort{Condens. Matter}\gdef\@doiabbr{condmat}\gdef\@ISSN{2410-3896}}
\DeclareOption{conservation}{\gdef\@journal{conservation}\gdef\@journalfull{Conservation}\gdef\@journalshort{Conservation}\gdef\@doiabbr{conservation}\gdef\@ISSN{2673-7159}\gdef\@continuouspages{yes}}
\DeclareOption{constrmater}{\gdef\@journal{constrmater}\gdef\@journalfull{Construction Materials}\gdef\@journalshort{Constr. Mater.}\gdef\@doiabbr{constrmater}\gdef\@ISSN{2673-7108}\gdef\@continuouspages{yes}}
\DeclareOption{cosmetics}{\gdef\@journal{cosmetics}\gdef\@journalfull{Cosmetics}\gdef\@journalshort{Cosmetics}\gdef\@doiabbr{cosmetics}\gdef\@ISSN{2079-9284}}
\DeclareOption{crops}{\gdef\@journal{crops}\gdef\@journalfull{Crops}\gdef\@journalshort{Crops}\gdef\@doiabbr{crops}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{cryptography}{\gdef\@journal{cryptography}\gdef\@journalfull{Cryptography}\gdef\@journalshort{Cryptography}\gdef\@doiabbr{cryptography}\gdef\@ISSN{2410-387X}}
\DeclareOption{crystals}{\gdef\@journal{crystals}\gdef\@journalfull{Crystals}\gdef\@journalshort{Crystals}\gdef\@doiabbr{cryst}\gdef\@ISSN{2073-4352}}
\DeclareOption{curroncol}{\gdef\@journal{curroncol}\gdef\@journalfull{Current Oncology}\gdef\@journalshort{Curr. Oncol.}\gdef\@doiabbr{curroncol}\gdef\@ISSN{1718-7729}\gdef\@continuouspages{yes}}
\DeclareOption{cyber}{\gdef\@journal{cyber}\gdef\@journalfull{Cyber}\gdef\@journalshort{Cyber}\gdef\@doiabbr{cyber}\gdef\@ISSN{2624-800X}}
\DeclareOption{dairy}{\gdef\@journal{dairy}\gdef\@journalfull{Dairy}\gdef\@journalshort{Dairy}\gdef\@doiabbr{dairy}\gdef\@ISSN{2624-862X}\gdef\@continuouspages{yes}}
\DeclareOption{data}{\gdef\@journal{data}\gdef\@journalfull{Data}\gdef\@journalshort{Data}\gdef\@doiabbr{data}\gdef\@ISSN{2306-5729}}
\DeclareOption{dentistry}{\gdef\@journal{dentistry}\gdef\@journalfull{Dentistry Journal}\gdef\@journalshort{Dent. J.}\gdef\@doiabbr{dj}\gdef\@ISSN{2304-6767}}
\DeclareOption{dermato}{\gdef\@journal{dermato}\gdef\@journalfull{Dermato}\gdef\@journalshort{Dermato}\gdef\@doiabbr{dermato}\gdef\@ISSN{2673-6179}\gdef\@continuouspages{yes}}
\DeclareOption{dermatopathology}{\gdef\@journal{dermatopathology}\gdef\@journalfull{Dermatopathology}\gdef\@journalshort{Dermatopathology}\gdef\@doiabbr{dermatopathology}\gdef\@ISSN{2296-3529}\gdef\@continuouspages{yes}}
\DeclareOption{designs}{\gdef\@journal{designs}\gdef\@journalfull{Designs}\gdef\@journalshort{Designs}\gdef\@doiabbr{designs}\gdef\@ISSN{2411-9660}}
\DeclareOption{diabetology}{\gdef\@journal{diabetology}\gdef\@journalfull{Diabetology}\gdef\@journalshort{Diabetology}\gdef\@doiabbr{diabetology}\gdef\@ISSN{2673-4540}\gdef\@continuouspages{yes}}
\DeclareOption{diagnostics}{\gdef\@journal{diagnostics}\gdef\@journalfull{Diagnostics}\gdef\@journalshort{Diagnostics}\gdef\@doiabbr{diagnostics}\gdef\@ISSN{2075-4418}}
\DeclareOption{digital}{\gdef\@journal{digital}\gdef\@journalfull{Digital}\gdef\@journalshort{Digital}\gdef\@doiabbr{digital}\gdef\@ISSN{2673-6470}\gdef\@continuouspages{yes}}
\DeclareOption{disabilities}{\gdef\@journal{disabilities}\gdef\@journalfull{Disabilities}\gdef\@journalshort{Disabilities}\gdef\@doiabbr{disabilities}\gdef\@ISSN{2673-7272}\gdef\@continuouspages{yes}}
\DeclareOption{diseases}{\gdef\@journal{diseases}\gdef\@journalfull{Diseases}\gdef\@journalshort{Diseases}\gdef\@doiabbr{diseases}\gdef\@ISSN{2079-9721}}
\DeclareOption{diversity}{\gdef\@journal{diversity}\gdef\@journalfull{Diversity}\gdef\@journalshort{Diversity}\gdef\@doiabbr{d}\gdef\@ISSN{1424-2818}}
\DeclareOption{dna}{\gdef\@journal{dna}\gdef\@journalfull{DNA}\gdef\@journalshort{DNA}\gdef\@doiabbr{dna}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{drones}{\gdef\@journal{drones}\gdef\@journalfull{Drones}\gdef\@journalshort{Drones}\gdef\@doiabbr{drones}\gdef\@ISSN{2504-446X}}
\DeclareOption{dynamics}{\gdef\@journal{dynamics}\gdef\@journalfull{Dynamics}\gdef\@journalshort{Dynamics}\gdef\@doiabbr{dynamics}\gdef\@ISSN{2409-555X}\gdef\@continuouspages{yes}}
\DeclareOption{earth}{\gdef\@journal{earth}\gdef\@journalfull{Earth}\gdef\@journalshort{Earth}\gdef\@doiabbr{earth}\gdef\@ISSN{2673-4834}\gdef\@continuouspages{yes}}
\DeclareOption{ebj}{\gdef\@journal{ebj}\gdef\@journalfull{European Burn Journal}\gdef\@journalshort{Eur. Burn J.}\gdef\@doiabbr{ebj}\gdef\@ISSN{2673-1991}\gdef\@continuouspages{yes}}
\DeclareOption{ecologies}{\gdef\@journal{ecologies}\gdef\@journalfull{Ecologies}\gdef\@journalshort{Ecologies}\gdef\@doiabbr{ecologies}\gdef\@ISSN{2673-4133}\gdef\@continuouspages{yes}}
\DeclareOption{econometrics}{\gdef\@journal{econometrics}\gdef\@journalfull{Econometrics}\gdef\@journalshort{Econometrics}\gdef\@doiabbr{econometrics}\gdef\@ISSN{2225-1146}}
\DeclareOption{economies}{\gdef\@journal{economies}\gdef\@journalfull{Economies}\gdef\@journalshort{Economies}\gdef\@doiabbr{economies}\gdef\@ISSN{2227-7099}}
\DeclareOption{education}{\gdef\@journal{education}\gdef\@journalfull{Education Sciences}\gdef\@journalshort{Educ. Sci.}\gdef\@doiabbr{educsci}\gdef\@ISSN{2227-7102}}
\DeclareOption{ejihpe}{\gdef\@journal{ejihpe}\gdef\@journalfull{European Journal of Investigation in Health Psychology and Education}\gdef\@journalshort{Eur. J. Investig. Health Psychol. Educ.}\gdef\@doiabbr{ejihpe}\gdef\@ISSN{2254-9625}\gdef\@continuouspages{yes}}
\DeclareOption{electricity}{\gdef\@journal{electricity}\gdef\@journalfull{Electricity}\gdef\@journalshort{Electricity}\gdef\@doiabbr{electricity}\gdef\@ISSN{2673-4826}\gdef\@continuouspages{yes}}
\DeclareOption{electrochem}{\gdef\@journal{electrochem}\gdef\@journalfull{Electrochem}\gdef\@journalshort{Electrochem}\gdef\@doiabbr{electrochem}\gdef\@ISSN{2673-3293}\gdef\@continuouspages{yes}}
\DeclareOption{electronicmat}{\gdef\@journal{electronicmat}\gdef\@journalfull{Electronic Materials}\gdef\@journalshort{Electron. Mater.}\gdef\@doiabbr{electronicmat}\gdef\@ISSN{2673-3978}\gdef\@continuouspages{yes}}
\DeclareOption{electronics}{\gdef\@journal{electronics}\gdef\@journalfull{Electronics}\gdef\@journalshort{Electronics}\gdef\@doiabbr{electronics}\gdef\@ISSN{2079-9292}}
\DeclareOption{encyclopedia}{\gdef\@journal{encyclopedia}\gdef\@journalfull{Encyclopedia}\gdef\@journalshort{Encyclopedia}\gdef\@doiabbr{encyclopedia}\gdef\@ISSN{2309-3366}\gdef\@continuouspages{yes}}
\DeclareOption{endocrines}{\gdef\@journal{endocrines}\gdef\@journalfull{Endocrines}\gdef\@journalshort{Endocrines}\gdef\@doiabbr{endocrines}\gdef\@ISSN{2673-396X}\gdef\@continuouspages{yes}}
\DeclareOption{energies}{\gdef\@journal{energies}\gdef\@journalfull{Energies}\gdef\@journalshort{Energies}\gdef\@doiabbr{en}\gdef\@ISSN{1996-1073}}
\DeclareOption{eng}{\gdef\@journal{eng}\gdef\@journalfull{Eng-Advances in Engineering}\gdef\@journalshort{Eng}\gdef\@doiabbr{eng}\gdef\@ISSN{2673-4117}\gdef\@continuouspages{yes}}
\DeclareOption{engproc}{\gdef\@journal{engproc}\gdef\@journalfull{Engineering Proceedings}\gdef\@journalshort{Eng. Proc.}\gdef\@doiabbr{engproc}\gdef\@ISSN{2673-4591}}
\DeclareOption{entropy}{\gdef\@journal{entropy}\gdef\@journalfull{Entropy}\gdef\@journalshort{Entropy}\gdef\@doiabbr{e}\gdef\@ISSN{1099-4300}}
\DeclareOption{environments}{\gdef\@journal{environments}\gdef\@journalfull{Environments}\gdef\@journalshort{Environments}\gdef\@doiabbr{environments}\gdef\@ISSN{2076-3298}}
\DeclareOption{environsciproc}{\gdef\@journal{environsciproc}\gdef\@journalfull{Environmental Sciences Proceedings}\gdef\@journalshort{Environ. Sci. Proc.}\gdef\@doiabbr{environsciproc}\gdef\@ISSN{2673-4931}}
\DeclareOption{epidemiologia}{\gdef\@journal{epidemiologia}\gdef\@journalfull{Epidemiologia}\gdef\@journalshort{Epidemiologia}\gdef\@doiabbr{epidemiologia}\gdef\@ISSN{2673-3986}\gdef\@continuouspages{yes}}
\DeclareOption{epigenomes}{\gdef\@journal{epigenomes}\gdef\@journalfull{Epigenomes}\gdef\@journalshort{Epigenomes}\gdef\@doiabbr{epigenomes}\gdef\@ISSN{2075-4655}}
\DeclareOption{fermentation}{\gdef\@journal{fermentation}\gdef\@journalfull{Fermentation}\gdef\@journalshort{Fermentation}\gdef\@doiabbr{fermentation}\gdef\@ISSN{2311-5637}}
\DeclareOption{fibers}{\gdef\@journal{fibers}\gdef\@journalfull{Fibers}\gdef\@journalshort{Fibers}\gdef\@doiabbr{fib}\gdef\@ISSN{2079-6439}}
\DeclareOption{fire}{\gdef\@journal{fire}\gdef\@journalfull{Fire}\gdef\@journalshort{Fire}\gdef\@doiabbr{fire}\gdef\@ISSN{2571-6255}}
\DeclareOption{fishes}{\gdef\@journal{fishes}\gdef\@journalfull{Fishes}\gdef\@journalshort{Fishes}\gdef\@doiabbr{fishes}\gdef\@ISSN{2410-3888}}
\DeclareOption{fluids}{\gdef\@journal{fluids}\gdef\@journalfull{Fluids}\gdef\@journalshort{Fluids}\gdef\@doiabbr{fluids}\gdef\@ISSN{2311-5521}}
\DeclareOption{foods}{\gdef\@journal{foods}\gdef\@journalfull{Foods}\gdef\@journalshort{Foods}\gdef\@doiabbr{foods}\gdef\@ISSN{2304-8158}}
\DeclareOption{forecasting}{\gdef\@journal{forecasting}\gdef\@journalfull{Forecasting}\gdef\@journalshort{Forecasting}\gdef\@doiabbr{forecast}\gdef\@ISSN{2571-9394}\gdef\@continuouspages{yes}}
\DeclareOption{forensicsci}{\gdef\@journal{forensicsci}\gdef\@journalfull{Forensic Sciences}\gdef\@journalshort{Forensic. Sci.}\gdef\@doiabbr{forensicsci}\gdef\@ISSN{2673-6756}\gdef\@continuouspages{yes}}
\DeclareOption{forests}{\gdef\@journal{forests}\gdef\@journalfull{Forests}\gdef\@journalshort{Forests}\gdef\@doiabbr{f}\gdef\@ISSN{1999-4907}}
\DeclareOption{fractalfract}{\gdef\@journal{fractalfract}\gdef\@journalfull{Fractal and Fractional}\gdef\@journalshort{Fractal Fract.}\gdef\@doiabbr{fractalfract}\gdef\@ISSN{2504-3110}}
\DeclareOption{fuels}{\gdef\@journal{fuels}\gdef\@journalfull{Fuels}\gdef\@journalshort{Fuels}\gdef\@doiabbr{fuels}\gdef\@ISSN{2673-3994}\gdef\@continuouspages{yes}}
\DeclareOption{futureinternet}{\gdef\@journal{futureinternet}\gdef\@journalfull{Future Internet}\gdef\@journalshort{Future Internet}\gdef\@doiabbr{fi}\gdef\@ISSN{1999-5903}}
\DeclareOption{futuretransp}{\gdef\@journal{futuretransp}\gdef\@journalfull{Future Transportation}\gdef\@journalshort{Future Transp.}\gdef\@doiabbr{futuretransp}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
%\DeclareOption{futurepharmacol}{\gdef\@journal{futurepharmacol}\gdef\@journalfull{}\gdef\@journalshort{}\gdef\@doiabbr{}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{futurephys}{\gdef\@journal{futurephys}\gdef\@journalfull{Future Physics}\gdef\@journalshort{Future Phys.}\gdef\@doiabbr{futurephys}\gdef\@ISSN{2624-6503}}
\DeclareOption{galaxies}{\gdef\@journal{galaxies}\gdef\@journalfull{Galaxies}\gdef\@journalshort{Galaxies}\gdef\@doiabbr{galaxies}\gdef\@ISSN{2075-4434}}
\DeclareOption{games}{\gdef\@journal{games}\gdef\@journalfull{Games}\gdef\@journalshort{Games}\gdef\@doiabbr{g}\gdef\@ISSN{2073-4336}}
\DeclareOption{gases}{\gdef\@journal{gases}\gdef\@journalfull{Gases}\gdef\@journalshort{Gases}\gdef\@doiabbr{gases}\gdef\@ISSN{2673-5628}\gdef\@continuouspages{yes}}
\DeclareOption{gastroent}{\gdef\@journal{gastroent}\gdef\@journalfull{Gastroenterology Insights}\gdef\@journalshort{Gastroenterol. Insights}\gdef\@doiabbr{gastroent}\gdef\@ISSN{2036-7422}\gdef\@continuouspages{yes}}
\DeclareOption{gastrointestdisord}{\gdef\@journal{gastrointestdisord}\gdef\@journalfull{Gastrointestinal Disorders}\gdef\@journalshort{Gastrointest. Disord.}\gdef\@doiabbr{gidisord}\gdef\@ISSN{2624-5647}\gdef\@continuouspages{yes}}
\DeclareOption{gels}{\gdef\@journal{gels}\gdef\@journalfull{Gels}\gdef\@journalshort{Gels}\gdef\@doiabbr{gels}\gdef\@ISSN{2310-2861}}
\DeclareOption{genealogy}{\gdef\@journal{genealogy}\gdef\@journalfull{Genealogy}\gdef\@journalshort{Genealogy}\gdef\@doiabbr{genealogy}\gdef\@ISSN{2313-5778}}
\DeclareOption{genes}{\gdef\@journal{genes}\gdef\@journalfull{Genes}\gdef\@journalshort{Genes}\gdef\@doiabbr{genes}\gdef\@ISSN{2073-4425}}
\DeclareOption{geographies}{\gdef\@journal{geographies}\gdef\@journalfull{Geographies}\gdef\@journalshort{Geographies}\gdef\@doiabbr{geographies}\gdef\@ISSN{2673-7086}\gdef\@continuouspages{yes}}
\DeclareOption{geohazards}{\gdef\@journal{geohazards}\gdef\@journalfull{GeoHazards}\gdef\@journalshort{GeoHazards}\gdef\@doiabbr{geohazards}\gdef\@ISSN{2624-795X}\gdef\@continuouspages{yes}}
\DeclareOption{geomatics}{\gdef\@journal{geomatics}\gdef\@journalfull{Geomatics}\gdef\@journalshort{Geomatics}\gdef\@doiabbr{geomatics}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{geosciences}{\gdef\@journal{geosciences}\gdef\@journalfull{Geosciences}\gdef\@journalshort{Geosciences}\gdef\@doiabbr{geosciences}\gdef\@ISSN{2076-3263}}
\DeclareOption{geotechnics}{\gdef\@journal{geotechnics}\gdef\@journalfull{Geotechnics}\gdef\@journalshort{Geotechnics}\gdef\@doiabbr{geotechnics}\gdef\@ISSN{2673-7094}\gdef\@continuouspages{yes}}
\DeclareOption{geriatrics}{\gdef\@journal{geriatrics}\gdef\@journalfull{Geriatrics}\gdef\@journalshort{Geriatrics}\gdef\@doiabbr{geriatrics}\gdef\@ISSN{2308-3417}}
%\DeclareOption{hazardousmatters}{\gdef\@journal{hazardousmatters}\gdef\@journalfull{Hazardous Matters}\gdef\@journalshort{Hazard. Matters}\gdef\@doiabbr{}\gdef\@ISSN{0014-0014}}
\DeclareOption{healthcare}{\gdef\@journal{healthcare}\gdef\@journalfull{Healthcare}\gdef\@journalshort{Healthcare}\gdef\@doiabbr{healthcare}\gdef\@ISSN{2227-9032}}
\DeclareOption{hearts}{\gdef\@journal{hearts}\gdef\@journalfull{Hearts}\gdef\@journalshort{Hearts}\gdef\@doiabbr{hearts}\gdef\@ISSN{2673-3846}\gdef\@continuouspages{yes}}
\DeclareOption{hemato}{\gdef\@journal{hemato}\gdef\@journalfull{Hemato}\gdef\@journalshort{Hemato}\gdef\@doiabbr{hemato}\gdef\@ISSN{2673-6357}\gdef\@continuouspages{yes}}
\DeclareOption{heritage}{\gdef\@journal{heritage}\gdef\@journalfull{Heritage}\gdef\@journalshort{Heritage}\gdef\@doiabbr{heritage}\gdef\@ISSN{2571-9408}\gdef\@continuouspages{yes}}
\DeclareOption{highthroughput}{\gdef\@journal{highthroughput}\gdef\@journalfull{High-Throughput}\gdef\@journalshort{High-Throughput}\gdef\@doiabbr{ht}\gdef\@ISSN{2571-5135}}
\DeclareOption{histories}{\gdef\@journal{histories}\gdef\@journalfull{Histories}\gdef\@journalshort{Histories}\gdef\@doiabbr{histories}\gdef\@ISSN{2409-9252}\gdef\@continuouspages{yes}}
\DeclareOption{horticulturae}{\gdef\@journal{horticulturae}\gdef\@journalfull{Horticulturae}\gdef\@journalshort{Horticulturae}\gdef\@doiabbr{horticulturae}\gdef\@ISSN{2311-7524}}
\DeclareOption{humanities}{\gdef\@journal{humanities}\gdef\@journalfull{Humanities}\gdef\@journalshort{Humanities}\gdef\@doiabbr{h}\gdef\@ISSN{2076-0787}}
\DeclareOption{humans}{\gdef\@journal{humans}\gdef\@journalfull{Humans}\gdef\@journalshort{Humans}\gdef\@doiabbr{humans}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{hydrogen}{\gdef\@journal{hydrogen}\gdef\@journalfull{Hydrogen}\gdef\@journalshort{Hydrogen}\gdef\@doiabbr{hydrogen}\gdef\@ISSN{2673-4141}\gdef\@continuouspages{yes}}
\DeclareOption{hydrology}{\gdef\@journal{hydrology}\gdef\@journalfull{Hydrology}\gdef\@journalshort{Hydrology}\gdef\@doiabbr{hydrology}\gdef\@ISSN{2306-5338}}
\DeclareOption{hygiene}{\gdef\@journal{hygiene}\gdef\@journalfull{Hygiene}\gdef\@journalshort{Hygiene}\gdef\@doiabbr{hygiene}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{idr}{\gdef\@journal{idr}\gdef\@journalfull{Infectious Disease Reports}\gdef\@journalshort{Infect. Dis. Rep.}\gdef\@doiabbr{idr}\gdef\@ISSN{2036-7449}\gdef\@continuouspages{yes}}
\DeclareOption{ijerph}{\gdef\@journal{ijerph}\gdef\@journalfull{International Journal of Environmental Research and Public Health}\gdef\@journalshort{Int. J. Environ. Res. Public Health}\gdef\@doiabbr{ijerph}\gdef\@ISSN{1660-4601}}
\DeclareOption{ijfs}{\gdef\@journal{ijfs}\gdef\@journalfull{International Journal of Financial Studies}\gdef\@journalshort{Int. J. Financial Stud.}\gdef\@doiabbr{ijfs}\gdef\@ISSN{2227-7072}}
\DeclareOption{ijgi}{\gdef\@journal{ijgi}\gdef\@journalfull{ISPRS International Journal of Geo-Information}\gdef\@journalshort{ISPRS Int. J. Geo-Inf.}\gdef\@doiabbr{ijgi}\gdef\@ISSN{2220-9964}}
\DeclareOption{ijms}{\gdef\@journal{ijms}\gdef\@journalfull{International Journal of Molecular Sciences}\gdef\@journalshort{Int. J. Mol. Sci.}\gdef\@doiabbr{ijms}\gdef\@ISSN{1422-0067}}
\DeclareOption{ijns}{\gdef\@journal{ijns}\gdef\@journalfull{International Journal of Neonatal Screening}\gdef\@journalshort{Int. J. Neonatal Screen.}\gdef\@doiabbr{ijns}\gdef\@ISSN{2409-515X}}
\DeclareOption{ijtm}{\gdef\@journal{ijtm}\gdef\@journalfull{International Journal of Translational Medicine}\gdef\@journalshort{Int. J. Transl. Med.}\gdef\@doiabbr{ijtm}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{ijtpp}{\gdef\@journal{ijtpp}\gdef\@journalfull{International Journal of Turbomachinery Propulsion and Power}\gdef\@journalshort{Int. J. Turbomach. Propuls. Power}\gdef\@doiabbr{ijtpp}\gdef\@ISSN{2504-186X}}
\DeclareOption{immuno}{\gdef\@journal{immuno}\gdef\@journalfull{Immuno}\gdef\@journalshort{Immuno}\gdef\@doiabbr{immuno}\gdef\@ISSN{2673-5601}\gdef\@continuouspages{yes}}
\DeclareOption{informatics}{\gdef\@journal{informatics}\gdef\@journalfull{Informatics}\gdef\@journalshort{Informatics}\gdef\@doiabbr{informatics}\gdef\@ISSN{2227-9709}}
\DeclareOption{information}{\gdef\@journal{information}\gdef\@journalfull{Information}\gdef\@journalshort{Information}\gdef\@doiabbr{info}\gdef\@ISSN{2078-2489}}
\DeclareOption{infrastructures}{\gdef\@journal{infrastructures}\gdef\@journalfull{Infrastructures}\gdef\@journalshort{Infrastructures}\gdef\@doiabbr{infrastructures}\gdef\@ISSN{2412-3811}}
\DeclareOption{inorganics}{\gdef\@journal{inorganics}\gdef\@journalfull{Inorganics}\gdef\@journalshort{Inorganics}\gdef\@doiabbr{inorganics}\gdef\@ISSN{2304-6740}}
\DeclareOption{insects}{\gdef\@journal{insects}\gdef\@journalfull{Insects}\gdef\@journalshort{Insects}\gdef\@doiabbr{insects}\gdef\@ISSN{2075-4450}}
\DeclareOption{instruments}{\gdef\@journal{instruments}\gdef\@journalfull{Instruments}\gdef\@journalshort{Instruments}\gdef\@doiabbr{instruments}\gdef\@ISSN{2410-390X}}
\DeclareOption{inventions}{\gdef\@journal{inventions}\gdef\@journalfull{Inventions}\gdef\@journalshort{Inventions}\gdef\@doiabbr{inventions}\gdef\@ISSN{2411-5134}}
\DeclareOption{iot}{\gdef\@journal{iot}\gdef\@journalfull{IoT}\gdef\@journalshort{IoT}\gdef\@doiabbr{iot}\gdef\@ISSN{2624-831X}\gdef\@continuouspages{yes}}
\DeclareOption{j}{\gdef\@journal{j}\gdef\@journalfull{J}\gdef\@journalshort{J}\gdef\@doiabbr{j}\gdef\@ISSN{2571-8800}\gdef\@continuouspages{yes}}
\DeclareOption{jcdd}{\gdef\@journal{jcdd}\gdef\@journalfull{Journal of Cardiovascular Development and Disease}\gdef\@journalshort{J. Cardiovasc. Dev. Dis.}\gdef\@doiabbr{jcdd}\gdef\@ISSN{2308-3425}}
\DeclareOption{jcm}{\gdef\@journal{jcm}\gdef\@journalfull{Journal of Clinical Medicine}\gdef\@journalshort{J. Clin. Med.}\gdef\@doiabbr{jcm}\gdef\@ISSN{2077-0383}}
\DeclareOption{jcp}{\gdef\@journal{jcp}\gdef\@journalfull{Journal of Cybersecurity and Privacy}\gdef\@journalshort{J. Cybersecur. Priv.}\gdef\@doiabbr{jcp}\gdef\@ISSN{2624-800X}}
\DeclareOption{jcs}{\gdef\@journal{jcs}\gdef\@journalfull{Journal of Composites Science}\gdef\@journalshort{J. Compos. Sci.}\gdef\@doiabbr{jcs}\gdef\@ISSN{2504-477X}}
\DeclareOption{jdb}{\gdef\@journal{jdb}\gdef\@journalfull{Journal of Developmental Biology}\gdef\@journalshort{J. Dev. Biol.}\gdef\@doiabbr{jdb}\gdef\@ISSN{2221-3759}}
\DeclareOption{jfb}{\gdef\@journal{jfb}\gdef\@journalfull{Journal of Functional Biomaterials}\gdef\@journalshort{J. Funct. Biomater.}\gdef\@doiabbr{jfb}\gdef\@ISSN{2079-4983}}
\DeclareOption{jfmk}{\gdef\@journal{jfmk}\gdef\@journalfull{Journal of Functional Morphology and Kinesiology}\gdef\@journalshort{J. Funct. Morphol. Kinesiol.}\gdef\@doiabbr{jfmk}\gdef\@ISSN{2411-5142}}
\DeclareOption{jimaging}{\gdef\@journal{jimaging}\gdef\@journalfull{Journal of Imaging}\gdef\@journalshort{J. Imaging}\gdef\@doiabbr{jimaging}\gdef\@ISSN{2313-433X}}
\DeclareOption{jintelligence}{\gdef\@journal{jintelligence}\gdef\@journalfull{Journal of Intelligence}\gdef\@journalshort{J. Intell.}\gdef\@doiabbr{jintelligence}\gdef\@ISSN{2079-3200}}
\DeclareOption{jlpea}{\gdef\@journal{jlpea}\gdef\@journalfull{Journal of Low Power Electronics and Applications}\gdef\@journalshort{J. Low Power Electron. Appl.}\gdef\@doiabbr{jlpea}\gdef\@ISSN{2079-9268}}
\DeclareOption{jmmp}{\gdef\@journal{jmmp}\gdef\@journalfull{Journal of Manufacturing and Materials Processing}\gdef\@journalshort{J. Manuf. Mater. Process.}\gdef\@doiabbr{jmmp}\gdef\@ISSN{2504-4494}}
\DeclareOption{jmp}{\gdef\@journal{jmp}\gdef\@journalfull{Journal of Molecular Pathology}\gdef\@journalshort{J. Mol. Pathol.}\gdef\@doiabbr{jmp}\gdef\@ISSN{2673-5261}\gdef\@continuouspages{yes}}
\DeclareOption{jmse}{\gdef\@journal{jmse}\gdef\@journalfull{Journal of Marine Science and Engineering}\gdef\@journalshort{J. Mar. Sci. Eng.}\gdef\@doiabbr{jmse}\gdef\@ISSN{2077-1312}}
\DeclareOption{jne}{\gdef\@journal{jne}\gdef\@journalfull{Journal of Nuclear Engineering}\gdef\@journalshort{J. Nucl. Eng.}\gdef\@doiabbr{jne}\gdef\@ISSN{2673-4362}\gdef\@continuouspages{yes}}
\DeclareOption{jnt}{\gdef\@journal{jnt}\gdef\@journalfull{Journal of Nanotheranostics}\gdef\@journalshort{J. Nanotheranostics}\gdef\@doiabbr{jnt}\gdef\@ISSN{2624-845X}\gdef\@continuouspages{yes}}
\DeclareOption{jof}{\gdef\@journal{jof}\gdef\@journalfull{Journal of Fungi}\gdef\@journalshort{J. Fungi}\gdef\@doiabbr{jof}\gdef\@ISSN{2309-608X}}
\DeclareOption{joitmc}{\gdef\@journal{joitmc}\gdef\@journalfull{Journal of Open Innovation: Technology Market and Complexity}\gdef\@journalshort{J. Open Innov. Technol. Mark. Complex.}\gdef\@doiabbr{joitmc}\gdef\@ISSN{2199-8531}}
\DeclareOption{jor}{\gdef\@journal{jor}\gdef\@journalfull{Journal of Respiration}\gdef\@journalshort{J. Respir.}\gdef\@doiabbr{jor}\gdef\@ISSN{2673-527X}\gdef\@continuouspages{yes}}
\DeclareOption{journalmedia}{\gdef\@journal{journalmedia}\gdef\@journalfull{Journalism and Media}\gdef\@journalshort{Journal. Media}\gdef\@doiabbr{journalmedia}\gdef\@ISSN{2673-5172}\gdef\@continuouspages{yes}}
\DeclareOption{jox}{\gdef\@journal{jox}\gdef\@journalfull{Journal of Xenobiotics}\gdef\@journalshort{J. Xenobiot.}\gdef\@doiabbr{jox}\gdef\@ISSN{2039-4713}\gdef\@continuouspages{yes}}
\DeclareOption{jpm}{\gdef\@journal{jpm}\gdef\@journalfull{Journal of Personalized Medicine}\gdef\@journalshort{J. Pers. Med.}\gdef\@doiabbr{jpm}\gdef\@ISSN{2075-4426}}
\DeclareOption{jrfm}{\gdef\@journal{jrfm}\gdef\@journalfull{Journal of Risk and Financial Management}\gdef\@journalshort{J. Risk Financial Manag.}\gdef\@doiabbr{jrfm}\gdef\@ISSN{1911-8074}}
\DeclareOption{jsan}{\gdef\@journal{jsan}\gdef\@journalfull{Journal of Sensor and Actuator Networks}\gdef\@journalshort{J. Sens. Actuator Netw.}\gdef\@doiabbr{jsan}\gdef\@ISSN{2224-2708}}
\DeclareOption{jtaer}{\gdef\@journal{jtaer}\gdef\@journalfull{Journal of Theoretical and Applied Electronic Commerce Research}\gdef\@journalshort{J. Theor. Appl. Electron. Commer. Res.}\gdef\@doiabbr{jtaer}\gdef\@ISSN{0718-1876}\gdef\@continuouspages{yes}}
\DeclareOption{jzbg}{\gdef\@journal{jzbg}\gdef\@journalfull{Journal of Zoological and Botanical Gardens}\gdef\@journalshort{J. Zool. Bot. Gard.}\gdef\@doiabbr{jzbg}\gdef\@ISSN{2673-5636}\gdef\@continuouspages{yes}}
%\DeclareOption{kidney}{\gdef\@journal{kidney}\gdef\@journalfull{}\gdef\@journalshort{}\gdef\@doiabbr{}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{land}{\gdef\@journal{land}\gdef\@journalfull{Land}\gdef\@journalshort{Land}\gdef\@doiabbr{land}\gdef\@ISSN{2073-445X}}
\DeclareOption{languages}{\gdef\@journal{languages}\gdef\@journalfull{Languages}\gdef\@journalshort{Languages}\gdef\@doiabbr{languages}\gdef\@ISSN{2226-471X}}
\DeclareOption{laws}{\gdef\@journal{laws}\gdef\@journalfull{Laws}\gdef\@journalshort{Laws}\gdef\@doiabbr{laws}\gdef\@ISSN{2075-471X}}
\DeclareOption{life}{\gdef\@journal{life}\gdef\@journalfull{Life}\gdef\@journalshort{Life}\gdef\@doiabbr{life}\gdef\@ISSN{2075-1729}}
\DeclareOption{liquids}{\gdef\@journal{liquids}\gdef\@journalfull{Liquids}\gdef\@journalshort{Liquids}\gdef\@doiabbr{liquids}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{literature}{\gdef\@journal{literature}\gdef\@journalfull{Literature}\gdef\@journalshort{Literature}\gdef\@doiabbr{literature}\gdef\@ISSN{2410-9789}}
\DeclareOption{livers}{\gdef\@journal{livers}\gdef\@journalfull{Livers}\gdef\@journalshort{Livers}\gdef\@doiabbr{livers}\gdef\@ISSN{2673-4389}\gdef\@continuouspages{yes}}
\DeclareOption{logistics}{\gdef\@journal{logistics}\gdef\@journalfull{Logistics}\gdef\@journalshort{Logistics}\gdef\@doiabbr{logistics}\gdef\@ISSN{2305-6290}}
\DeclareOption{lubricants}{\gdef\@journal{lubricants}\gdef\@journalfull{Lubricants}\gdef\@journalshort{Lubricants}\gdef\@doiabbr{lubricants}\gdef\@ISSN{2075-4442}}
\DeclareOption{machines}{\gdef\@journal{machines}\gdef\@journalfull{Machines}\gdef\@journalshort{Machines}\gdef\@doiabbr{machines}\gdef\@ISSN{2075-1702}}
\DeclareOption{macromol}{\gdef\@journal{macromol}\gdef\@journalfull{Macromol}\gdef\@journalshort{Macromol}\gdef\@doiabbr{macromol}\gdef\@ISSN{2673-6209}\gdef\@continuouspages{yes}}
\DeclareOption{magnetism}{\gdef\@journal{magnetism}\gdef\@journalfull{Magnetism}\gdef\@journalshort{Magnetism}\gdef\@doiabbr{magnetism}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{magnetochemistry}{\gdef\@journal{magnetochemistry}\gdef\@journalfull{Magnetochemistry}\gdef\@journalshort{Magnetochemistry}\gdef\@doiabbr{magnetochemistry}\gdef\@ISSN{2312-7481}}
\DeclareOption{make}{\gdef\@journal{make}\gdef\@journalfull{Machine Learning and Knowledge Extraction}\gdef\@journalshort{Mach. Learn. Knowl. Extr.}\gdef\@doiabbr{make}\gdef\@ISSN{2504-4990}\gdef\@continuouspages{yes}}
\DeclareOption{marinedrugs}{\gdef\@journal{marinedrugs}\gdef\@journalfull{Marine Drugs}\gdef\@journalshort{Mar. Drugs}\gdef\@doiabbr{md}\gdef\@ISSN{1660-3397}}
\DeclareOption{materials}{\gdef\@journal{materials}\gdef\@journalfull{Materials}\gdef\@journalshort{Materials}\gdef\@doiabbr{ma}\gdef\@ISSN{1996-1944}}
\DeclareOption{materproc}{\gdef\@journal{materproc}\gdef\@journalfull{Materials Proceedings}\gdef\@journalshort{Mater. Proc.}\gdef\@doiabbr{materproc}\gdef\@ISSN{2673-4605}}
\DeclareOption{mathematics}{\gdef\@journal{mathematics}\gdef\@journalfull{Mathematics}\gdef\@journalshort{Mathematics}\gdef\@doiabbr{math}\gdef\@ISSN{2227-7390}}
\DeclareOption{mca}{\gdef\@journal{mca}\gdef\@journalfull{Mathematical and Computational Applications}\gdef\@journalshort{Math. Comput. Appl.}\gdef\@doiabbr{mca}\gdef\@ISSN{2297-8747}}
%\DeclareOption{measurements}{\gdef\@journal{measurements}\gdef\@journalfull{}\gdef\@journalshort{}\gdef\@doiabbr{}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{medicina}{\gdef\@journal{medicina}\gdef\@journalfull{Medicina}\gdef\@journalshort{Medicina}\gdef\@doiabbr{medicina}\gdef\@ISSN{1010-660X}}
\DeclareOption{medicines}{\gdef\@journal{medicines}\gdef\@journalfull{Medicines}\gdef\@journalshort{Medicines}\gdef\@doiabbr{medicines}\gdef\@ISSN{2305-6320}}
\DeclareOption{medsci}{\gdef\@journal{medsci}\gdef\@journalfull{Medical Sciences}\gdef\@journalshort{Med. Sci.}\gdef\@doiabbr{medsci}\gdef\@ISSN{2076-3271}}
\DeclareOption{membranes}{\gdef\@journal{membranes}\gdef\@journalfull{Membranes}\gdef\@journalshort{Membranes}\gdef\@doiabbr{membranes}\gdef\@ISSN{2077-0375}}
\DeclareOption{metabolites}{\gdef\@journal{metabolites}\gdef\@journalfull{Metabolites}\gdef\@journalshort{Metabolites}\gdef\@doiabbr{metabo}\gdef\@ISSN{2218-1989}}
\DeclareOption{metals}{\gdef\@journal{metals}\gdef\@journalfull{Metals}\gdef\@journalshort{Metals}\gdef\@doiabbr{met}\gdef\@ISSN{2075-4701}}
\DeclareOption{metrology}{\gdef\@journal{metrology}\gdef\@journalfull{Metrology}\gdef\@journalshort{Metrology}\gdef\@doiabbr{metrology}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{micro}{\gdef\@journal{micro}\gdef\@journalfull{Micro}\gdef\@journalshort{Micro}\gdef\@doiabbr{micro}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{microarrays}{\gdef\@journal{microarrays}\gdef\@journalfull{Microarrays}\gdef\@journalshort{Microarrays}\gdef\@doiabbr{microarrays}\gdef\@ISSN{2076-3905}}
\DeclareOption{microbiolres}{\gdef\@journal{microbiolres}\gdef\@journalfull{Microbiology Research}\gdef\@journalshort{Microbiol. Res.}\gdef\@doiabbr{microbiolres}\gdef\@ISSN{2036-7481}\gdef\@continuouspages{yes}}
\DeclareOption{micromachines}{\gdef\@journal{micromachines}\gdef\@journalfull{Micromachines}\gdef\@journalshort{Micromachines}\gdef\@doiabbr{mi}\gdef\@ISSN{2072-666X}}
\DeclareOption{microorganisms}{\gdef\@journal{microorganisms}\gdef\@journalfull{Microorganisms}\gdef\@journalshort{Microorganisms}\gdef\@doiabbr{microorganisms}\gdef\@ISSN{2076-2607}}
\DeclareOption{minerals}{\gdef\@journal{minerals}\gdef\@journalfull{Minerals}\gdef\@journalshort{Minerals}\gdef\@doiabbr{min}\gdef\@ISSN{2075-163X}}
\DeclareOption{mining}{\gdef\@journal{mining}\gdef\@journalfull{Mining}\gdef\@journalshort{Mining}\gdef\@doiabbr{mining}\gdef\@ISSN{2673-6489}\gdef\@continuouspages{yes}}
\DeclareOption{modelling}{\gdef\@journal{modelling}\gdef\@journalfull{Modelling}\gdef\@journalshort{Modelling}\gdef\@doiabbr{modelling}\gdef\@ISSN{2673-3951}\gdef\@continuouspages{yes}}
\DeclareOption{molbank}{\gdef\@journal{molbank}\gdef\@journalfull{Molbank}\gdef\@journalshort{Molbank}\gdef\@doiabbr{M}\gdef\@ISSN{1422-8599}}
\DeclareOption{molecules}{\gdef\@journal{molecules}\gdef\@journalfull{Molecules}\gdef\@journalshort{Molecules}\gdef\@doiabbr{molecules}\gdef\@ISSN{1420-3049}}
\DeclareOption{mps}{\gdef\@journal{mps}\gdef\@journalfull{Methods and Protocols}\gdef\@journalshort{Methods Protoc.}\gdef\@doiabbr{mps}\gdef\@ISSN{2409-9279}}
\DeclareOption{mti}{\gdef\@journal{mti}\gdef\@journalfull{Multimodal Technologies and Interaction}\gdef\@journalshort{Multimodal Technol. Interact.}\gdef\@doiabbr{mti}\gdef\@ISSN{2414-4088}}
\DeclareOption{nanoenergyadv}{\gdef\@journal{nanoenergyadv}\gdef\@journalfull{Nanoenergy Advances}\gdef\@journalshort{Nanoenergy Adv.}\gdef\@doiabbr{nanoenergyadv}\gdef\@ISSN{2673-706X}\gdef\@continuouspages{yes}}
\DeclareOption{nanomanufacturing}{\gdef\@journal{nanomanufacturing}\gdef\@journalfull{Nanomanufacturing}\gdef\@journalshort{Nanomanufacturing}\gdef\@doiabbr{nanomanufacturing}\gdef\@ISSN{2673-687X}\gdef\@continuouspages{yes}}
\DeclareOption{nanomaterials}{\gdef\@journal{nanomaterials}\gdef\@journalfull{Nanomaterials}\gdef\@journalshort{Nanomaterials}\gdef\@doiabbr{nano}\gdef\@ISSN{2079-4991}}
\DeclareOption{ncrna}{\gdef\@journal{ncrna}\gdef\@journalfull{Non-coding RNA}\gdef\@journalshort{Non-coding RNA}\gdef\@doiabbr{ncrna}\gdef\@ISSN{2311-553X}}
\DeclareOption{network}{\gdef\@journal{network}\gdef\@journalfull{Network}\gdef\@journalshort{Network}\gdef\@doiabbr{network}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{neuroglia}{\gdef\@journal{neuroglia}\gdef\@journalfull{Neuroglia}\gdef\@journalshort{Neuroglia}\gdef\@doiabbr{neuroglia}\gdef\@ISSN{2571-6980}\gdef\@continuouspages{yes}}
\DeclareOption{neurolint}{\gdef\@journal{neurolint}\gdef\@journalfull{Neurology International}\gdef\@journalshort{Neurol. Int.}\gdef\@doiabbr{neurolint}\gdef\@ISSN{2035-8377}\gdef\@continuouspages{yes}}
\DeclareOption{neurosci}{\gdef\@journal{neurosci}\gdef\@journalfull{NeuroSci}\gdef\@journalshort{NeuroSci}\gdef\@doiabbr{neurosci}\gdef\@ISSN{2673-4087}\gdef\@continuouspages{yes}}
\DeclareOption{nitrogen}{\gdef\@journal{nitrogen}\gdef\@journalfull{Nitrogen}\gdef\@journalshort{Nitrogen}\gdef\@doiabbr{nitrogen}\gdef\@ISSN{2504-3129}\gdef\@continuouspages{yes}}
\DeclareOption{notspecified}{\gdef\@journal{notspecified}\gdef\@journalfull{Journal Not Specified}\gdef\@journalshort{Journal Not Specified}\gdef\@doiabbr{}\gdef\@ISSN{}}
\DeclareOption{nri}{\gdef\@journal{nri}\gdef\@journalfull{Natural Resources Informatics}\gdef\@journalshort{Nat. Resour. Inform.}\gdef\@doiabbr{nri}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{nursrep}{\gdef\@journal{nursrep}\gdef\@journalfull{Nursing Reports}\gdef\@journalshort{Nurs. Rep.}\gdef\@doiabbr{nursrep}\gdef\@ISSN{2039-4403}\gdef\@continuouspages{yes}}
\DeclareOption{nutraceuticals}{\gdef\@journal{nutraceuticals}\gdef\@journalfull{Nutraceuticals}\gdef\@journalshort{Nutraceuticals}\gdef\@doiabbr{nutraceuticals}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{nutrients}{\gdef\@journal{nutrients}\gdef\@journalfull{Nutrients}\gdef\@journalshort{Nutrients}\gdef\@doiabbr{nu}\gdef\@ISSN{2072-6643}}
\DeclareOption{obesities}{\gdef\@journal{obesities}\gdef\@journalfull{Obesities}\gdef\@journalshort{Obesities}\gdef\@doiabbr{obesities}\gdef\@ISSN{2673-4168}\gdef\@continuouspages{yes}}
\DeclareOption{oceans}{\gdef\@journal{oceans}\gdef\@journalfull{Oceans}\gdef\@journalshort{Oceans}\gdef\@doiabbr{oceans}\gdef\@ISSN{2673-1924}\gdef\@continuouspages{yes}}
\DeclareOption{ohbm}{\gdef\@journal{ohbm}\gdef\@journalfull{Journal of Otorhinolaryngology Hearing and Balance Medicine}\gdef\@journalshort{J. Otorhinolaryngol. Hear. Balance Med.}\gdef\@doiabbr{ohbm}\gdef\@ISSN{2504-463X}}
\DeclareOption{onco}{\gdef\@journal{onco}\gdef\@journalfull{Onco}\gdef\@journalshort{Onco}\gdef\@doiabbr{onco}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
%\DeclareOption{oncopathology}{\gdef\@journal{oncopathology}\gdef\@journalfull{}\gdef\@journalshort{}\gdef\@doiabbr{}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{optics}{\gdef\@journal{optics}\gdef\@journalfull{Optics}\gdef\@journalshort{Optics}\gdef\@doiabbr{opt}\gdef\@ISSN{2673-3269}\gdef\@continuouspages{yes}}
\DeclareOption{oral}{\gdef\@journal{oral}\gdef\@journalfull{Oral}\gdef\@journalshort{Oral}\gdef\@doiabbr{oral}\gdef\@ISSN{2673-6373}\gdef\@continuouspages{yes}}
\DeclareOption{organics}{\gdef\@journal{organics}\gdef\@journalfull{Organics}\gdef\@journalshort{Organics}\gdef\@doiabbr{org}\gdef\@ISSN{2673-401X}\gdef\@continuouspages{yes}}
\DeclareOption{osteology}{\gdef\@journal{osteology}\gdef\@journalfull{Osteology}\gdef\@journalshort{Osteology}\gdef\@doiabbr{osteology}\gdef\@ISSN{2673-4036}\gdef\@continuouspages{yes}}
\DeclareOption{oxygen}{\gdef\@journal{oxygen}\gdef\@journalfull{Oxygen}\gdef\@journalshort{Oxygen}\gdef\@doiabbr{oxygen}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{parasites}{\gdef\@journal{parasites}\gdef\@journalfull{Parasites}\gdef\@journalshort{Parasites}\gdef\@doiabbr{parasites}\gdef\@ISSN{2673-5946}}
\DeclareOption{parasitologia}{\gdef\@journal{parasitologia}\gdef\@journalfull{Parasitologia}\gdef\@journalshort{Parasitologia}\gdef\@doiabbr{parasitologia}\gdef\@ISSN{2673-6772}\gdef\@continuouspages{yes}}
\DeclareOption{particles}{\gdef\@journal{particles}\gdef\@journalfull{Particles}\gdef\@journalshort{Particles}\gdef\@doiabbr{particles}\gdef\@ISSN{2571-712X}\gdef\@continuouspages{yes}}
\DeclareOption{pathogens}{\gdef\@journal{pathogens}\gdef\@journalfull{Pathogens}\gdef\@journalshort{Pathogens}\gdef\@doiabbr{pathogens}\gdef\@ISSN{2076-0817}}
\DeclareOption{pathophysiology}{\gdef\@journal{pathophysiology}\gdef\@journalfull{Pathophysiology}\gdef\@journalshort{Pathophysiology}\gdef\@doiabbr{pathophysiology}\gdef\@ISSN{0928-4680}\gdef\@continuouspages{yes}}
\DeclareOption{pediatrrep}{\gdef\@journal{pediatrrep}\gdef\@journalfull{Pediatric Reports}\gdef\@journalshort{Pediatr. Rep.}\gdef\@doiabbr{pediatric}\gdef\@ISSN{2036-7503}\gdef\@continuouspages{yes}}
\DeclareOption{pharmaceuticals}{\gdef\@journal{pharmaceuticals}\gdef\@journalfull{Pharmaceuticals}\gdef\@journalshort{Pharmaceuticals}\gdef\@doiabbr{ph}\gdef\@ISSN{1424-8247}}
\DeclareOption{pharmaceutics}{\gdef\@journal{pharmaceutics}\gdef\@journalfull{Pharmaceutics}\gdef\@journalshort{Pharmaceutics}\gdef\@doiabbr{pharmaceutics}\gdef\@ISSN{1999-4923}}
\DeclareOption{pharmacy}{\gdef\@journal{pharmacy}\gdef\@journalfull{Pharmacy}\gdef\@journalshort{Pharmacy}\gdef\@doiabbr{pharmacy}\gdef\@ISSN{2226-4787}}
\DeclareOption{philosophies}{\gdef\@journal{philosophies}\gdef\@journalfull{Philosophies}\gdef\@journalshort{Philosophies}\gdef\@doiabbr{philosophies}\gdef\@ISSN{2409-9287}}
\DeclareOption{photochem}{\gdef\@journal{photochem}\gdef\@journalfull{Photochem}\gdef\@journalshort{Photochem}\gdef\@doiabbr{photochem}\gdef\@ISSN{2673-7256}\gdef\@continuouspages{yes}}
\DeclareOption{photonics}{\gdef\@journal{photonics}\gdef\@journalfull{Photonics}\gdef\@journalshort{Photonics}\gdef\@doiabbr{photonics}\gdef\@ISSN{2304-6732}}
%\DeclareOption{physchem}{\gdef\@journal{}\gdef\@journalfull{}\gdef\@journalshort{}\gdef\@doiabbr{}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{physics}{\gdef\@journal{physics}\gdef\@journalfull{Physics}\gdef\@journalshort{Physics}\gdef\@doiabbr{physics}\gdef\@ISSN{2624-8174}\gdef\@continuouspages{yes}}
\DeclareOption{physiolsci}{\gdef\@journal{physiolsci}\gdef\@journalfull{Physiological Sciences}\gdef\@journalshort{Physiol. Sci.}\gdef\@doiabbr{physiolsci}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{plants}{\gdef\@journal{plants}\gdef\@journalfull{Plants}\gdef\@journalshort{Plants}\gdef\@doiabbr{plants}\gdef\@ISSN{2223-7747}}
\DeclareOption{plasma}{\gdef\@journal{plasma}\gdef\@journalfull{Plasma}\gdef\@journalshort{Plasma}\gdef\@doiabbr{plasma}\gdef\@ISSN{2571-6182}\gdef\@continuouspages{yes}}
\DeclareOption{pollutants}{\gdef\@journal{pollutants}\gdef\@journalfull{Pollutants}\gdef\@journalshort{Pollutants}\gdef\@doiabbr{pollutants}\gdef\@ISSN{2673-4672}\gdef\@continuouspages{yes}}
\DeclareOption{polymers}{\gdef\@journal{polymers}\gdef\@journalfull{Polymers}\gdef\@journalshort{Polymers}\gdef\@doiabbr{polym}\gdef\@ISSN{2073-4360}}
\DeclareOption{polysaccharides}{\gdef\@journal{polysaccharides}\gdef\@journalfull{Polysaccharides}\gdef\@journalshort{Polysaccharides}\gdef\@doiabbr{polysaccharides}\gdef\@ISSN{2673-4176}\gdef\@continuouspages{yes}}
\DeclareOption{preprints}{\gdef\@journal{preprints}\gdef\@journalfull{Preprints}\gdef\@journalshort{Preprints}\gdef\@doiabbr{}\gdef\@ISSN{}}
\DeclareOption{proceedings}{\gdef\@journal{proceedings}\gdef\@journalfull{Proceedings}\gdef\@journalshort{Proceedings}\gdef\@doiabbr{proceedings}\gdef\@ISSN{2504-3900}}
\DeclareOption{processes}{\gdef\@journal{processes}\gdef\@journalfull{Processes}\gdef\@journalshort{Processes}\gdef\@doiabbr{pr}\gdef\@ISSN{2227-9717}}
\DeclareOption{prosthesis}{\gdef\@journal{prosthesis}\gdef\@journalfull{Prosthesis}\gdef\@journalshort{Prosthesis}\gdef\@doiabbr{prosthesis}\gdef\@ISSN{2673-1592}\gdef\@continuouspages{yes}}
\DeclareOption{proteomes}{\gdef\@journal{proteomes}\gdef\@journalfull{Proteomes}\gdef\@journalshort{Proteomes}\gdef\@doiabbr{proteomes}\gdef\@ISSN{2227-7382}}
\DeclareOption{psych}{\gdef\@journal{psych}\gdef\@journalfull{Psych}\gdef\@journalshort{Psych}\gdef\@doiabbr{psych}\gdef\@ISSN{2624-8611}\gdef\@continuouspages{yes}}
\DeclareOption{psychiatryint}{\gdef\@journal{psychiatryint}\gdef\@journalfull{Psychiatry International}\gdef\@journalshort{Psychiatry Int.}\gdef\@doiabbr{psychiatryint}\gdef\@ISSN{2673-5318}\gdef\@continuouspages{yes}}
\DeclareOption{publications}{\gdef\@journal{publications}\gdef\@journalfull{Publications}\gdef\@journalshort{Publications}\gdef\@doiabbr{publications}\gdef\@ISSN{2304-6775}}
\DeclareOption{quantumrep}{\gdef\@journal{quantumrep}\gdef\@journalfull{Quantum Reports}\gdef\@journalshort{Quantum Rep.}\gdef\@doiabbr{quantum}\gdef\@ISSN{2624-960X}\gdef\@continuouspages{yes}}
\DeclareOption{quaternary}{\gdef\@journal{quaternary}\gdef\@journalfull{Quaternary}\gdef\@journalshort{Quaternary}\gdef\@doiabbr{quat}\gdef\@ISSN{2571-550X}}
\DeclareOption{qubs}{\gdef\@journal{qubs}\gdef\@journalfull{Quantum Beam Science}\gdef\@journalshort{Quantum Beam Sci.}\gdef\@doiabbr{qubs}\gdef\@ISSN{2412-382X}}
\DeclareOption{radiation}{\gdef\@journal{radiation}\gdef\@journalfull{Radiation}\gdef\@journalshort{Radiation}\gdef\@doiabbr{radiation}\gdef\@ISSN{2673-592X}\gdef\@continuouspages{yes}}
\DeclareOption{reactions}{\gdef\@journal{reactions}\gdef\@journalfull{Reactions}\gdef\@journalshort{Reactions}\gdef\@doiabbr{reactions}\gdef\@ISSN{2624-781X}\gdef\@continuouspages{yes}}
\DeclareOption{recycling}{\gdef\@journal{recycling}\gdef\@journalfull{Recycling}\gdef\@journalshort{Recycling}\gdef\@doiabbr{recycling}\gdef\@ISSN{2313-4321}}
%\DeclareOption{regeneration}{\gdef\@journal{regeneration}\gdef\@journalfull{}\gdef\@journalshort{}\gdef\@doiabbr{}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{religions}{\gdef\@journal{religions}\gdef\@journalfull{Religions}\gdef\@journalshort{Religions}\gdef\@doiabbr{rel}\gdef\@ISSN{2077-1444}}
\DeclareOption{remotesensing}{\gdef\@journal{remotesensing}\gdef\@journalfull{Remote Sensing}\gdef\@journalshort{Remote Sens.}\gdef\@doiabbr{rs}\gdef\@ISSN{2072-4292}}
\DeclareOption{reports}{\gdef\@journal{reports}\gdef\@journalfull{Reports}\gdef\@journalshort{Reports}\gdef\@doiabbr{reports}\gdef\@ISSN{2571-841X}}
\DeclareOption{reprodmed}{\gdef\@journal{reprodmed}\gdef\@journalfull{Reproductive Medicine}\gdef\@journalshort{Reprod. Med.}\gdef\@doiabbr{reprodmed}\gdef\@ISSN{2673-3897}\gdef\@continuouspages{yes}}
\DeclareOption{resources}{\gdef\@journal{resources}\gdef\@journalfull{Resources}\gdef\@journalshort{Resources}\gdef\@doiabbr{resources}\gdef\@ISSN{2079-9276}}
\DeclareOption{risks}{\gdef\@journal{risks}\gdef\@journalfull{Risks}\gdef\@journalshort{Risks}\gdef\@doiabbr{risks}\gdef\@ISSN{2227-9091}}
\DeclareOption{robotics}{\gdef\@journal{robotics}\gdef\@journalfull{Robotics}\gdef\@journalshort{Robotics}\gdef\@doiabbr{robotics}\gdef\@ISSN{2218-6581}}
\DeclareOption{safety}{\gdef\@journal{safety}\gdef\@journalfull{Safety}\gdef\@journalshort{Safety}\gdef\@doiabbr{safety}\gdef\@ISSN{2313-576X}}
\DeclareOption{sci}{\gdef\@journal{sci}\gdef\@journalfull{Sci}\gdef\@journalshort{Sci}\gdef\@doiabbr{sci}\gdef\@ISSN{2413-4155}}
\DeclareOption{scipharm}{\gdef\@journal{scipharm}\gdef\@journalfull{Scientia Pharmaceutica}\gdef\@journalshort{Sci. Pharm.}\gdef\@doiabbr{scipharm}\gdef\@ISSN{2218-0532}}
\DeclareOption{sensors}{\gdef\@journal{sensors}\gdef\@journalfull{Sensors}\gdef\@journalshort{Sensors}\gdef\@doiabbr{s}\gdef\@ISSN{1424-8220}}
\DeclareOption{separations}{\gdef\@journal{separations}\gdef\@journalfull{Separations}\gdef\@journalshort{Separations}\gdef\@doiabbr{separations}\gdef\@ISSN{2297-8739}}
\DeclareOption{sexes}{\gdef\@journal{sexes}\gdef\@journalfull{Sexes}\gdef\@journalshort{Sexes}\gdef\@doiabbr{sexes}\gdef\@ISSN{2411-5118}\gdef\@continuouspages{yes}}
\DeclareOption{signals}{\gdef\@journal{signals}\gdef\@journalfull{Signals}\gdef\@journalshort{Signals}\gdef\@doiabbr{signals}\gdef\@ISSN{2624-6120}\gdef\@continuouspages{yes}}
\DeclareOption{sinusitis}{\gdef\@journal{sinusitis}\gdef\@journalfull{Sinusitis}\gdef\@journalshort{Sinusitis}\gdef\@doiabbr{sinusitis}\gdef\@ISSN{2309-107X}\gdef\@continuouspages{yes}}
\DeclareOption{smartcities}{\gdef\@journal{smartcities}\gdef\@journalfull{Smart Cities}\gdef\@journalshort{Smart Cities}\gdef\@doiabbr{smartcities}\gdef\@ISSN{2624-6511}\gdef\@continuouspages{yes}}
\DeclareOption{sna}{\gdef\@journal{sna}\gdef\@journalfull{Sinusitis and Asthma}\gdef\@journalshort{Sinusitis Asthma}\gdef\@doiabbr{sna}\gdef\@ISSN{2624-7003}}
\DeclareOption{societies}{\gdef\@journal{societies}\gdef\@journalfull{Societies}\gdef\@journalshort{Societies}\gdef\@doiabbr{soc}\gdef\@ISSN{2075-4698}}
\DeclareOption{socsci}{\gdef\@journal{socsci}\gdef\@journalfull{Social Sciences}\gdef\@journalshort{Soc. Sci.}\gdef\@doiabbr{socsci}\gdef\@ISSN{2076-0760}}
\DeclareOption{soilsystems}{\gdef\@journal{soilsystems}\gdef\@journalfull{Soil Systems}\gdef\@journalshort{Soil Syst.}\gdef\@doiabbr{soilsystems}\gdef\@ISSN{2571-8789}}
\DeclareOption{solids}{\gdef\@journal{solids}\gdef\@journalfull{Solids}\gdef\@journalshort{Solids}\gdef\@doiabbr{solids}\gdef\@ISSN{2673-6497}\gdef\@continuouspages{yes}}
\DeclareOption{sports}{\gdef\@journal{sports}\gdef\@journalfull{Sports}\gdef\@journalshort{Sports}\gdef\@doiabbr{sports}\gdef\@ISSN{2075-4663}}
%\DeclareOption{standards}{\gdef\@journal{standards}\gdef\@journalfull{Standards}\gdef\@journalshort{Standards}\gdef\@doiabbr{}\gdef\@ISSN{2305-6703}}
\DeclareOption{stats}{\gdef\@journal{stats}\gdef\@journalfull{Stats}\gdef\@journalshort{Stats}\gdef\@doiabbr{stats}\gdef\@ISSN{2571-905X}\gdef\@continuouspages{yes}}
\DeclareOption{stresses}{\gdef\@journal{stresses}\gdef\@journalfull{Stresses}\gdef\@journalshort{Stresses}\gdef\@doiabbr{stresses}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{surfaces}{\gdef\@journal{surfaces}\gdef\@journalfull{Surfaces}\gdef\@journalshort{Surfaces}\gdef\@doiabbr{surfaces}\gdef\@ISSN{2571-9637}\gdef\@continuouspages{yes}}
\DeclareOption{surgeries}{\gdef\@journal{surgeries}\gdef\@journalfull{Surgeries}\gdef\@journalshort{Surgeries}\gdef\@doiabbr{}\gdef\@ISSN{2017-2017}\gdef\@continuouspages{yes}}
\DeclareOption{suschem}{\gdef\@journal{suschem}\gdef\@journalfull{Sustainable Chemistry}\gdef\@journalshort{Sustain. Chem.}\gdef\@doiabbr{suschem}\gdef\@ISSN{2673-4079}\gdef\@continuouspages{yes}}
\DeclareOption{sustainability}{\gdef\@journal{sustainability}\gdef\@journalfull{Sustainability}\gdef\@journalshort{Sustainability}\gdef\@doiabbr{su}\gdef\@ISSN{2071-1050}}
\DeclareOption{symmetry}{\gdef\@journal{symmetry}\gdef\@journalfull{Symmetry}\gdef\@journalshort{Symmetry}\gdef\@doiabbr{sym}\gdef\@ISSN{2073-8994}}
\DeclareOption{systems}{\gdef\@journal{systems}\gdef\@journalfull{Systems}\gdef\@journalshort{Systems}\gdef\@doiabbr{systems}\gdef\@ISSN{2079-8954}}
\DeclareOption{taxonomy}{\gdef\@journal{taxonomy}\gdef\@journalfull{Taxonomy}\gdef\@journalshort{Taxonomy}\gdef\@doiabbr{taxonomy}\gdef\@ISSN{2673-6500}\gdef\@continuouspages{yes}}
\DeclareOption{technologies}{\gdef\@journal{technologies}\gdef\@journalfull{Technologies}\gdef\@journalshort{Technologies}\gdef\@doiabbr{technologies}\gdef\@ISSN{2227-7080}}
\DeclareOption{telecom}{\gdef\@journal{telecom}\gdef\@journalfull{Telecom}\gdef\@journalshort{Telecom}\gdef\@doiabbr{telecom}\gdef\@ISSN{2673-4001}\gdef\@continuouspages{yes}}
\DeclareOption{textiles}{\gdef\@journal{textiles}\gdef\@journalfull{Textiles}\gdef\@journalshort{Textiles}\gdef\@doiabbr{textiles}\gdef\@ISSN{2673-7248}\gdef\@continuouspages{yes}}
\DeclareOption{thermo}{\gdef\@journal{thermo}\gdef\@journalfull{Thermo}\gdef\@journalshort{Thermo}\gdef\@doiabbr{thermo}\gdef\@ISSN{2673-7264}\gdef\@continuouspages{yes}}
\DeclareOption{tourismhosp}{\gdef\@journal{tourismhosp}\gdef\@journalfull{Tourism and Hospitality}\gdef\@journalshort{Tour. Hosp.}\gdef\@doiabbr{tourhosp}\gdef\@ISSN{2673-5768}\gdef\@continuouspages{yes}}
\DeclareOption{toxics}{\gdef\@journal{toxics}\gdef\@journalfull{Toxics}\gdef\@journalshort{Toxics}\gdef\@doiabbr{toxics}\gdef\@ISSN{2305-6304}}
\DeclareOption{toxins}{\gdef\@journal{toxins}\gdef\@journalfull{Toxins}\gdef\@journalshort{Toxins}\gdef\@doiabbr{toxins}\gdef\@ISSN{2072-6651}}
\DeclareOption{transplantology}{\gdef\@journal{transplantology}\gdef\@journalfull{Transplantology}\gdef\@journalshort{Transplantology}\gdef\@doiabbr{transplantology}\gdef\@ISSN{2673-3943}\gdef\@continuouspages{yes}}
\DeclareOption{traumas}{\gdef\@journal{traumas}\gdef\@journalfull{Traumas}\gdef\@journalshort{Traumas}\gdef\@doiabbr{traumas}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{tropicalmed}{\gdef\@journal{tropicalmed}\gdef\@journalfull{Tropical Medicine and Infectious Disease}\gdef\@journalshort{Trop. Med. Infect. Dis.}\gdef\@doiabbr{tropicalmed}\gdef\@ISSN{2414-6366}}
\DeclareOption{universe}{\gdef\@journal{universe}\gdef\@journalfull{Universe}\gdef\@journalshort{Universe}\gdef\@doiabbr{universe}\gdef\@ISSN{2218-1997}}
\DeclareOption{urbansci}{\gdef\@journal{urbansci}\gdef\@journalfull{Urban Science}\gdef\@journalshort{Urban Sci.}\gdef\@doiabbr{urbansci}\gdef\@ISSN{2413-8851}}
\DeclareOption{uro}{\gdef\@journal{uro}\gdef\@journalfull{Uro}\gdef\@journalshort{Uro}\gdef\@doiabbr{uro}\gdef\@ISSN{2673-4397}\gdef\@continuouspages{yes}}
\DeclareOption{vaccines}{\gdef\@journal{vaccines}\gdef\@journalfull{Vaccines}\gdef\@journalshort{Vaccines}\gdef\@doiabbr{vaccines}\gdef\@ISSN{2076-393X}}
\DeclareOption{vehicles}{\gdef\@journal{vehicles}\gdef\@journalfull{Vehicles}\gdef\@journalshort{Vehicles}\gdef\@doiabbr{vehicles}\gdef\@ISSN{2624-8921}\gdef\@continuouspages{yes}}
\DeclareOption{vetsci}{\gdef\@journal{vetsci}\gdef\@journalfull{Veterinary Sciences}\gdef\@journalshort{Vet. Sci.}\gdef\@doiabbr{vetsci}\gdef\@ISSN{2306-7381}}
\DeclareOption{vibration}{\gdef\@journal{vibration}\gdef\@journalfull{Vibration}\gdef\@journalshort{Vibration}\gdef\@doiabbr{vibration}\gdef\@ISSN{2571-631X}\gdef\@continuouspages{yes}}
\DeclareOption{viruses}{\gdef\@journal{viruses}\gdef\@journalfull{Viruses}\gdef\@journalshort{Viruses}\gdef\@doiabbr{v}\gdef\@ISSN{1999-4915}}
\DeclareOption{vision}{\gdef\@journal{vision}\gdef\@journalfull{Vision}\gdef\@journalshort{Vision}\gdef\@doiabbr{vision}\gdef\@ISSN{2411-5150}}
\DeclareOption{water}{\gdef\@journal{water}\gdef\@journalfull{Water}\gdef\@journalshort{Water}\gdef\@doiabbr{w}\gdef\@ISSN{2073-4441}}
\DeclareOption{wevj}{\gdef\@journal{wevj}\gdef\@journalfull{World Electric Vehicle Journal}\gdef\@journalshort{World Electr. Veh. J.}\gdef\@doiabbr{wevj}\gdef\@ISSN{2032-6653}}
\DeclareOption{women}{\gdef\@journal{women}\gdef\@journalfull{Women}\gdef\@journalshort{Women}\gdef\@doiabbr{women}\gdef\@ISSN{2673-4184}\gdef\@continuouspages{yes}}
\DeclareOption{world}{\gdef\@journal{world}\gdef\@journalfull{World}\gdef\@journalshort{World}\gdef\@doiabbr{world}\gdef\@ISSN{2673-4060}\gdef\@continuouspages{yes}}

==> chapters/abstractbackup.tex <==
\chapter*{Abstract}
\thispagestyle{fancy}

The analysis of data sets plays significant role in every scientific study, which can be mathematically represented as finite metric spaces. In this thesis we focus on finding new effective algorithms in area of computational geometry that can be effectively used for the analysis and classification of scientific data sets. 


%This thesis consists of three topics related to computational geometry and classification of point clouds. 

% and one topic related to topological data analysis (TDA), which combines fields of computational geometry and algebraic topology for analyzing data. 

%The first topic provides a new precise and efficient method to skeletonize data using a 1-dimensional skeleton. 
%In this topic, data is given in the form of unorganized clouds of points. During the research, we discovered that any clustering algorithms applied to the data can fail if actual clusters have complicated topological shapes with several branches. Such shapes are much better approximated by embedded skeletons, for example by trees with vertices connected by straight-line edges in a Euclidean space. Starting from a density estimation on a big cloud of points, we build a dense tree with a small number of vertices. By minimizing the distance to the given cloud by vertex movements, the resulting Optimal Dense Tree outperforms all past skeletonization algorithms on a large dataset of synthetic clouds sampled with high noise around given graphs.
%The applications include a quick quality estimation of micelles formed by oil molecules in colloidal products. 

\medskip
\noindent 
The first major contribution of this thesis is a new algorithm, that resolves the classical problem of finding $k$ nearest neighbors to of query points $Q$ in a larger reference points $R$, where $Q$ and $R$ both belong to some metric space $X$ in a near-linear time.
This project was inspired by the work of Beygelzimer, Kakade, and Langford in ICML 2006, where it was attempted to show that such problem can be resolved for $k=1$ in a near-linear time complexity. 
However, in 2015 it was pointed out the proof of their time complexity might contain mistakes, which was confirmed in this thesis by showing that the proposed proof fails for a concrete counterexample.
An important application of KNN ($k$-nearest neighbors) algorithm is KNN graph of a finite metric space $R$, that can be formed by letting $R$ to be the vertex set of the graph and connecting every point $p \in R$ with its $k$-nearest neighbors. The KNN graph finds its application in areas of data-skeletonization, where KNN graph can be used as an initial skeleton of the data set and cluster analysis, where the connected components of KNN graph can be used as the clusters.

\medskip
\noindent
Another application of KNN algorithm is Minimum spanning tree MST, which is an efficient way to visualize any unstructured data given only by distances, for example by any metric graph connecting abstract data points. Though many efficient algorithms for metric MST were developed, there was only one past attempt to justify a near-linear time complexity in the size of a given metric space. In 2010 March, Ram, and Gray claimed that MST of any finite metric space can be constructed in a parametrized near-linear time. 
In this work we showed that the proposed proof was incorrect by showing that a step in the proof is failed for multiple counterexamples.
Inspired by the work of 2010, this thesis produces a new algorithm that is based on Boruvka algorithm, which is combined with the KNN method to resolve metric MST problem in a near-linear time complexity.

\medskip
\noindent
In the final chapter of the thesis the MST algorithm is applied in the computation of new isometry invariant mergegram of Topological Data Analysis (TDA). 
TDA quantifies topological shapes hidden in unorganized data such as clouds of unordered points.
In the 0-dimensional case, the distance-based persistence is determined by a single-linkage (SL) clustering of a finite set in a metric space.
Equivalently, the 0D persistence captures only edge lengths of a Minimum Spanning Tree (MST).
Both SL dendrogram and MST are unstable under perturbations of points.
In this thesis, we define the new stable-under-noise mergegram, which outperforms
previous isometry invariants on a classification of point clouds by PersLay.

\medskip
\noindent
In conclusion, the developed fast algorithms in this thesis can be applied to various tasks in data science. The newly proposed corrected time complexity analysis of KNN and MST not only exposes the past issues in their theoretical justifications but also gives a way to fix the issues in other similar methods in the literature. 

% The output of knn algorithm can be used to divide point clouds into clusters, by forming knn graph and separating connected components 


% The well-known work by Beygelzimer, Kakade, and Langford in ICML 2006 introduced cover trees and claimed to guarantee a near-linear time complexity in the number $n$ of reference points. Section~5.3 of Curtin's PhD (2015) pointed out that the proof of this result was wrong. 
% The key step of the original proof attempted to show that the number of iterations can be estimated by multiplying the length of the longest root-to-leaf path in a cover tree by a constant factor.
% However, this estimate can miss many potential nodes in several branches of a cover tree, that should be considered during the search.
% The same erroneous argument was unfortunately repeated in several subsequent papers.
% This chapter gives formal counterexamples to the time complexity estimates of the cover tree construction algorithm and the nearest neighbors search in the past work. 
% We prove correct analogs of the past claims with slightly better bounds for any number $k\geq 1$ of neighbors. 
% A new compressed cover tree guarantees a parameterized time complexity that is near-linear in the maximum size of both query and reference set.

\bigskip

% The second part is about the construction of a Minimum Spanning Tree (MST) on any finite metric space. This is an efficient way to visualize any unstructured data given only by distances, for example by any metric graph connecting abstract data points. 
% Though many efficient algorithms for MST were developed, there was only one past attempt to justify a near-linear time complexity in the size of a given metric space.
% In 2010 March, Ram, and Gray claimed that MST of any finite metric space can be constructed in a parametrized near-linear time. 
% However, in this work we have discovered a counterexample showing that the provided proof was incorrect.
% The past obstacles are now resolved by the new concepts of a compressed cover tree and a minimized expansion constant.
% The main contribution is the first MST algorithm that correctly justifies a parametrized a near-linear time complexity.

%The experiments on thousands of real data points show that the new MST algorithm outperforms past approaches for certain metrics.



==> chapters/chapter3.tex <==
\chapter{Data skeletonization} % Write in your own chapter title
\label{ch:chapter3}


The tree reconstruction problem for an unorganized cloud of points in Euclidean space has found unexpected applications in the discovery of new colloidal products with desired physical properties such as viscosity.
Computer simulations typically output clusters of molecules or clouds of points (one point per molecule) that might have a large variety of topological shapes.  Many clustering algorithms can fail if actual clusters have complicated topological shapes with several branches. Such shapes are much better approximated by embedded skeletons, for example by trees with vertices connected by straight-line edges in a Euclidean space.
In this chapter we introduce new techniques to tackle the problem of tree reconstruction of an unorganized cloud of points in a Euclidean space.

%Real data are often given in the form of unorganized clouds of points. In this chapter we
%
% Many clustering algorithms can fail if actual clusters have complicated topological shapes with several branches. Such shapes are much better approximated by embedded skeletons, for example by trees with vertices connected by straight line edges in a Euclidean space.

\section{Motivations and the reconstruction problem}
\label{sec:intro}

By a \emph{cloud} $C$ of points we mean any finite set of unordered points in a Euclidean space $\R^m$.
The first picture in Fig.~\ref{fig:clouds} shows a cloud, where each point represents a polymer molecule in a liquid colloid, e.g. gel or shampoo.
These molecules with hydrophilic heads and hydrophobic tails self-aggregate into complex groups in a liquid solution. 
Shapes of micelles including edge-lengths and degrees of branched vertices determine important physical properties such as viscosity. 
\medskip

Since there is a huge variety of potential molecules for better products, new molecules are first tested by simulations to check if these molecules form suitable micelles with a few branches, but not too complicated.
Molecular simulations are usually slow and often become stuck with undesirable micelles.
Hence a lot of time and resources can be saved by automatically analyzing shapes of micelles and filtering out too short/simple micelles or too long/branched micelles.
\medskip


A shape of a micelle will be modeled as a \emph{straight-line} tree $T\subset\R^m$ whose vertices are located at points in $\R^m$ and connected by straight-line edges. Clouds and straight-line graph can be linked together using Definition \ref{dfn:epsilonSampleOfGraph}. The micelles are thought of as $\epsilon$-samples of Definition 
\ref{dfn:epsilonSampleOfGraph} of some known graph $T$, where $\epsilon$ correspond to the width of molecules. 


\begin{figure}[H]

    \centering
    \begin{subfigure}{.49\textwidth}
  \centering
  % include first image
  \includegraphics[width=.9\linewidth]{images/micelles/cylindrical_cloud.png}  
  \caption{Cloud corresponding to worm-type micelle }
 % \label{fig:sub-cloudsReferenceA}
\end{subfigure}
\begin{subfigure}{.49\textwidth}
  \centering
  % include first image
  \includegraphics[width=.9\linewidth]{images/micelles/branched_cloud.png}  
  \caption{ Cloud corresponding to branched-type micelle. }
 % \label{fig:sub-cloudsReferenceB}
\end{subfigure}
\caption{Clouds corresponding to real micelles}
\label{fig:clouds} 
%    \includegraphics[width=0.49\linewidth]{images/micelles/cylindrical_cloud.png}
%    \includegraphics[width=0.49\linewidth]{images/micelles/branched_cloud.png}
%    \caption{Left: Cloud corresponding to worm-type micelle. Right: Cloud corresponding to branched-type micelle.}
\end{figure}


\begin{dfn}[$\epsilon$-sample of a graph]
\label{dfn:epsilonSampleOfGraph}
We say that a point cloud $C$ is an $\epsilon$-\emph{sample} of a straight-line graph $T \subseteq \R^m$ if for every $p \in C$ there exists a point $q \in T$ for which $d(p,q) \leq \epsilon$ i.e $C \subset T^{\epsilon}$, where $d$ is euclidean distance. 
\end{dfn}
\begin{dfn}[Directed hausdorff distance]
\label{dfn:MaxMin}
Let $T$ be a straight-line graph and let $C$ be a point cloud in $\R^m$ we define directed hausdorff distance as follows:
%$$d_{\overleftarrow{H}}(T,C) = \max_{p \in C}\min_{}$$
%$d_{\overleftarrow{H}}(T,C) = \inf\{\epsilon \mid C \text{ is } \epsilon \text{-sample of } T\} $
$d_{\overleftarrow{H}}(T,C) = \max_{p \in C}\min_{q \in T} d(p,q).$
\end{dfn}


%\begin{dfn}
%\label{dfn:graph}
%A {\em straight-line} graph $G\subset\R^m$ (briefly, a {\em graph}) consists of vertices at points $q_1,\dots,q_k\in\R^m$ and undirected straight-line edges connecting pairs $q_i,q_j$, $i\neq j$, in such a way that any edges meet only at their common vertex.
%Let $d$ be the Euclidean distance.
%For $\ep>0$, a cloud $C\subset\R^m$ is $\ep$-{\em approximated} by a graph $G$ if $C$ is within the $\ep$-{\em offset} that is the union of $\ep$-balls at all points of $G$, i.e.
%$G^{\ep}=\{p\in\R^m \;|\; d(p,q)\leq\ep \mbox{ for some } q\in G\}$.
%\end{dfn}

\begin{figure}[H]
\centering

  \begin{subfigure}{.49\textwidth}
  \centering
  % include first image
  \includegraphics[width=.9\linewidth]{figures/stars/star4_cloud_ODT.png}  
  \caption{Cloud sample around Star4 tree}
 % \label{fig:sub-cloudsReferenceA}
\end{subfigure}
\begin{subfigure}{.49\textwidth}
  \centering
  % include first image
  \includegraphics[width=.9\linewidth]{figures/stars/star5_cloud_ODT.png}  
  \caption{Cloud sample around Star5 tree }
 % \label{fig:sub-cloudsReferenceB}
\end{subfigure}

%\includegraphics[width=0.49\linewidth]{figures/stars/star4_cloud_ODT.png}
%\includegraphics[width=0.49\linewidth]{figures/stars/star5_cloud_ODT.png}
%\caption{Two graphs (\textbf{Left: } Star4, \textbf{Right: } Star5) and their $\epsilon$-samples pictured}

\end{figure}



%Using the definition of $\epsilon$-sample we can now state the main problem \ref{pro:reconstruction} of this Chapter: 
%
%A shape of a micelle will be modeled as a \emph{straight-line} trees $T\subset\R^m$ whose vertices are located at points in $\R^m$ and connected by straight-line edges.
%Notice that $T$ can have polygonal lines with degree~2 vertices.
%A \emph{homeomorphism} is a continuous bijection $T\to G$, whose inverse is also continuous.
%Let $d$ be the standard Euclidean distance.  
%An $\ep$-sample of a tree $T\subset\R^m$ is a finite set of points that are at a distance $d\leq\ep$ from $T$.



\begin{problem}[Tree reconstruction]
\label{pro:reconstruction}
For any point cloud $C\subset\R^m$ that is $\ep$-sampled from an unknown straight-line tree $T\subset\R^m$ find conditions on $T$ and $C$
such that there exists an algorithm to build a straight-line tree $G\subset\R^m$ satisfying the following properties:

% , in such a way that there exists algorithm that builds a straight-line tree $G\subset\R^m$ so that
%we could build a straight-line tree $G\subset\R^m$ so that 
\begin{itemize}

\item[(\ref{pro:reconstruction}a) ] $G$ is homeomorphic to the original straight-line tree $T$; 
\label{pro:labela}

%\item[(\ref{pro:reconstruction}b) ] $G$ has a small distance to $C$ i.e. the directed Hausdorff distance $d_{\overleftarrow{H}}$ from $C$ to $G$ %has an upper bound. 

\item[(\ref{pro:reconstruction}b) ] $G$ is $2\epsilon$-close to $C$ i.e. $C \subseteq G^{2\epsilon}$.
\label{pro:labelb}


\item [(\ref{pro:reconstruction}c)] Number of vertices of $G$ has upper bound in terms of $T$ and $C$. 
\label{pro:labelc}
% $G$ has a small number of vertices in terms of $T$ and cloud $C$. 

\end{itemize}
\end{problem}
%
%\noindent
%(\ref{pro:reconstruction}a) 
%$G$ is homeomorphic to the original tree $T$
%\smallskip
%
%
%\noindent
%(\ref{pro:reconstruction}b) 
%$G$ has a smallest distance to $C$, e.g. the Mean Square Error (MSE) or the Maximum Distance (MD) from $C$ to a closest straight-line edge of $G$;
%\smallskip
%
%\noindent
%(\ref{pro:reconstruction}c) 
%$G$ has a small number of vertices relative to $n$.  
%\end{problem}

In Figure \ref{fig:NecessityOfConditions} below we have illustrated why that all the conditions of the Problem \ref{pro:reconstruction} are necessary to get a desired reconstruction of a micelle from given point cloud.

\begin{figure}[H]
    \centering

\begin{subfigure}{.33\textwidth}
  \centering
  % include first image
  \includegraphics[width=.9\linewidth]{images/ExtraGraphs/GraphConditionAOut2.png}  
  \caption{Condition (\ref{pro:labela}a) is left out. }
  \label{fig:sub-NecessityConditionsA}
\end{subfigure}
\begin{subfigure}{.33\textwidth}
  \centering
  % include second image
  \includegraphics[width=.9\linewidth]{images/ExtraGraphs/GraphConditionBOut2.png}  
  \caption{Condition (\ref{pro:labela}b) is left out.}
  \label{fig:sub-NecessityConditionsB}
\end{subfigure}    
\begin{subfigure}{.33\textwidth}
  \centering
  % include second image
  \includegraphics[width=.9\linewidth]{images/ExtraGraphs/GraphConditionCOut.png}  
  \caption{Condition (\ref{pro:labela}c) is left out.}
  \label{fig:sub-NecessityConditionsC}
\end{subfigure}    
    
%    \includegraphics[width=0.33\linewidth]{images/ExtraGraphs/GraphConditionAOut.png}
%    \includegraphics[width=0.33\linewidth]{images/ExtraGraphs/GraphConditionBOut.png}
%    \includegraphics[width=0.33\linewidth]{images/ExtraGraphs/GraphConditionCOut.png}
% 
    \caption{Potential solution to Problem \ref{pro:reconstruction}, when we leave out one of the requirements.}
    \label{fig:NecessityOfConditions}
\end{figure}

Assume that only conditions (\ref{pro:reconstruction}b) and (\ref{pro:reconstruction}c) are required. Then the skeleton that solved the 
Problem \ref{pro:reconstruction} is allowed to have any shape, such as single polygonal path of  Figure \ref{fig:sub-NecessityConditionsA} that visit furthest points of the point cloud in some order. If only conditions  (\ref{pro:reconstruction}a) and (\ref{pro:reconstruction}c) are required, then any output graph $G$ that is homeomorphic to the original cloud $T$ and that has no degree 2-vertices would be an optimal graph, illustrated in Figure \ref{fig:sub-NecessityConditionsB}. If the only required conditions are (\ref{pro:reconstruction}a) and (\ref{pro:reconstruction}b) , then the skeleton could have lots of unnecessary zig-zags , as illustrated in Figure \ref{fig:sub-NecessityConditionsC}.

%\begin{exa}
%\label{exa:requirmentsProblem}
%Assume that only conditions (\ref{pro:reconstruction}a) and (\ref{pro:reconstruction}b) are required, then the problem could be solved by constructing tree similar to a \emph{Minimum Spanning Tree} $\MST(C)$, which would be homeomorphic to original graph and would satisfy (\ref{pro:reconstruction}b) condition. This would however lead generally to undesirable outputs as the final skeleton would contain contain large number of unnecessary zig-zags. On the other hand if we require only (\ref{pro:reconstruction}a) and (\ref{pro:reconstruction}c) then the problem would simply reduce to finding the homeomorphism type of the original graph, because homeomorphic graph having smallest number of vertices can be obtained from any homeomorphic graph simply by collapsing all degree 2 points. 
%
%
%% has the vertex set $C$ and a minimum total length of edges, hence satisfies~(\ref{pro:reconstruction}a) with distance 0.
%
%%Condition~(\ref{pro:reconstruction}b) is necessary to avoid $\MST(C)$ as a trivial solution.
%%Short branches of $\MST(C)$ can be pruned in various ways, e.g. see a subtree $\core(C)\subset\MST(C)$ in \cite[Definition~6]{elkin2019fast}, to satisfy both %conditions~(\ref{pro:reconstruction}a,b).
%%Final condition~(\ref{pro:reconstruction}c) is needed to guarantee that a final skeleton has much fewer vertices than the number $n$ of points in $C$. 
%\end{exa}



Problem \ref{pro:reconstruction} will be solved by using Algorithm \ref{alg:DenseTreeAlgorithm}. We are able to show, that under certain assumption the output of the algorithm satisfies the 3 conditions of Problem \ref{pro:reconstruction}. The homeomorphism guarantee, Condition (\ref{pro:labela}a) is proved in Theorem \ref{thmm:GHT}. Guarantees regarding distance, Condition (\ref{pro:labelb}b) is proved in Theorem \ref{thmm:vcg} and vertex count guarantee, Condition (\ref{pro:labelc}c) is proved in Theorem \ref{thmm:dg}. 



\section{Theoretical framework}
\label{sec:theoreticalFramework}


%\subsection{Overview of Densetree-algorithm

In this thesis, we will prove that under certain constrains imposed on kernel density estimation function and the underlying graph structure we are able to reconstruct the original graph using the dense-tree algorithm starting from unstructured noisy data. The success of the reconstruction will depend on the sparsity of the dense set $D$, as well as the original graph we are trying to reconstruct. In particular, the underlying graph structure should serve as a good link between input point cloud structure and the original graph shape we are trying to reconstruct i.e. we wish that there wouldn't be any connections between non-adjacent branches, relatively small maximal edge length and that the graph would approximate the Euclidean distance inside each of the edge-cloud. 



%\begin{dfn}
%Let $T$ be a striaghtline embedded tree, let $D$ be an $\epsilon$ sample of $T$ and let $G$ be a graph that approximates $D$. We say that $D$ is $\delta$-sparse sample if $D^{\epsilon}$ covers vertices of $T$ and if $\delta$  .  For any points $a \neq b \in D$ the distance $d_G(a,b)$ is always bigger than $ \delta$.
%\end{dfn}

In the following definition the distance between two line-segments $e,h$ is defined as the Hausdorff distance (Definition \ref{dfn:HausdorffDistance}):
 $d_H(e,h) = \max \{\sup_{x \in e}\inf_{y \in h}d(x,y), \sup_{y \in Y}\inf_{x \in X}d(x,y)\}. $
In the following Definition we are using graph-notation of Definition \ref{dfn:GraphConstraints}.


\begin{dfn}[$\gamma$-approximation]
\label{dfn:GammaApproximation}
Let $T$ be a straight-line tree in $\R^m$ and let $C$ be its $\epsilon$-sample. We say that a connected graph $G$ with a vertex set $C$ is a
\emph{$\gamma$-approximation} of $(T,C)$ if the following two conditions are satisfied: 
\begin{enumerate}
\item If points $a,b$ belong to the same \emph{edge-set} $e^\epsilon \cap C$ where $e \in \mathbb{E}(T)$ then $d_G(a,b) \leq \gamma \cdot d(a,b) $
\item The minimal distance $d_{\min}$ ( Definition \ref{dfn:minMetric} ) between any two non adjacent edges of $T$ is larger than $l_{\max}(G) + 2\epsilon$.
%\item Let $r$ be minimal distance between two non-adjacent edges of $T$ then: $l(G) < r - 2\epsilon $
\end{enumerate}

\end{dfn}
%Let $\delta,\gamma \in \R_{+}$ be parameters.

The main Theorem \ref{thmm:GHT} proves that under certain assumption the homeomorphism guarantee of Problem \ref{pro:labela}(a) can be obtained. The Theorem will be proved in Section \ref{sec:homeoGuarantee}.

\begin{restatable}[\textbf{homeomorphism guarantees for a minimum spanning tree}]{thmm}{MainThm}
\label{thmm:GHT}
Let $T$ be a straight-line tree graph in $\mathbb{R}^m$ and let $C$ be its $\epsilon$ sample. Let $D \subseteq C$ be a $\delta$-sparse subsample of $C$ in metric $d_G$ satisfying $\mathbb{V}(T) \subseteq D^{\epsilon}$. Let a connected graph $G$ be an arbitrary $\gamma$-approximation of $(T,C)$ for some $\gamma \geq 1$. If the inequality

\begin{equation}
\tag{\ref{thmm:GHT}}
\label{eqa:GHT}
\delta \geq  2\gamma(\epsilon +\dfrac{\epsilon}{\sin(\frac{\theta(T)}{2})} + \dfrac{l_{\max}(G)}{\sin(\min(\theta(T), \frac{\pi}{2}))})
\end{equation}
% $$\delta \geq  2\gamma(\epsilon +\dfrac{\epsilon}{\sin(\frac{\theta(T)}{2})} + \dfrac{l(G)}{\sin(\min(\theta(T), \frac{\pi}{2}))})$$
 is satisfied, then $\MST(D, d_G)$ is homeomorphic to the tree $T$. 

 %If the subsample $D$ is $\delta$ sparse: For all $a,b \in D$: $d_G(a,b) > \delta$,


\end{restatable}


In the Theorem \ref{thmm:dg} that graph $\MST(D, d_G)$ built on the $\delta$-sparse subset $D$ using underlying graph $G$ is $2\epsilon$-close to the original sampling $C$ of graph $T$. In Theorem \ref{thmm:vcg} we prove that vertex count in the graph $\MST(D, d_G)$ can be bounded, when we assume conditions of Theorem \ref{thmm:GHT}. Both results will be proved in Section \ref{sec:DistanceAndVertexCount}.

\begin{restatable}[\textbf{distance guarantee}]{thmm}{CorProbA}
\label{thmm:dg}
Assume the conditions of Theorem \ref{thmm:GHT}. Then the distance between reconstruction and the cloud has the following bound: 
$d_{\overleftarrow{H}}(\MST(D, d_G), C) < 2 \epsilon$, where $d_{\overleftarrow{H}}$ is the directed hausdorff distance of Definition \ref{dfn:MaxMin}.
\end{restatable}

\begin{restatable}[\textbf{vertex count guarantee}]{thmm}{CorProB}
\label{thmm:vcg}
Assume the conditions of Theorem \ref{thmm:GHT}. Then the number of vertices in the reconstruction $\MST(D, d_G)$ has the following bound:
\begin{equation}
\tag{\ref{thmm:vcg}}
\label{eqa:vcg}
|D| \leq \sum_{e \in \mathbb{E}(T)} \dfrac{|e| + 2 \epsilon}{2\sqrt{\frac{\delta^2}{\gamma^2}-4\epsilon^2}}.
\end{equation}

\end{restatable}

%Algorithm \ref{alg:DenseTreeAlgorithm} on dataset $C$ with expansion constant $c$ ( Definition \ref{dfn:ExpansionConstantOk} ),  linkage expansion constant $c_l$ 
%(Definition \ref{dfn:LinkageClusterConstant}) and clustering expansion constant $c_p$ (Definition \ref{dfn:ClusterExpansionConstant}) is 



In the following Example \ref{exa:VertexCountBoundAssumption} we show that the bound presented in Theorem \ref{thmm:vcg} is scalable. 
\begin{exa}[Scale invariance]
\label{exa:VertexCountBoundAssumption}
Assume that tree $T$, cloud $C$ and  $\delta$-sparse subset $D$ of $C$ satisfies the conditions of Theorem \ref{thmm:GHT}. 
% 2\gamma(\epsilon +\dfrac{\epsilon}{\sin(\frac{\theta(T)}{2})} + \dfrac{l(G)}{\sin(\min(\theta(T), \frac{\pi}{2}))})
Assume that graph $T'$ , cloud $C'$ and $r \delta$-sparse dense-set $D'$ can be obtained by performing affine scaling of $T$, cloud $C$ and $D$ by a factor $r$. We note that $C'$ is in $r \epsilon$-offset of graph $T'$ and that the underlying graph $G'$ is built by performing affine scaling on each vertex of the graph $G$, which is a $\gamma$-approximation of $(T,C)$. We will first prove that $G'$ is a $\gamma$-approximation of $(T',C') $. We will now prove that $(T',C') $ satisfies condition (1) of Definition \ref{dfn:GammaApproximation} let $a$,$b$ be arbitrary points belonging to a same edge-set and let $a',b'$ be their corresponding points in graph $G'$ then 
$$d_{G'}(a',b') = r d_G(a,b) \leq \gamma r d(a,b) = \gamma d(a,b).$$
Let $e,h$ be arbitrary non-adjacent edges of graph $T$ and let $e',h'$ be the edges that are scaled by factor $r$. Then the condition (2) follows from the following chain of inequalities:
$$d(e',h') = r d(e,h) \geq r (l(G) + 2\epsilon) \geq l(G') + 2 r \epsilon $$
By the definition $\delta$-sparseness set $D'$ is $r \delta$-sprase. We will now show that it satisfies inequality (\ref{eqa:GHT})
Assume that $\delta$ was chosen to be the minimal real number satisfying equation (\ref{eqa:GHT}). We can now obtain the following bound:
% $$r \delta \geq  2\gamma(r \epsilon +\dfrac{r \epsilon}{\sin(\frac{\theta(T')}{2})} + \dfrac{l(G')}{\sin(\min(\theta(T'), \frac{\pi}{2}))}) = 
% 2\gamma r( \epsilon +\dfrac{ \epsilon}{\sin(\frac{\theta(T)}{2})} + \dfrac{l(G)}{\sin(\min(\theta(T), \frac{\pi}{2}))}) = r\delta $$
  $$r \delta \geq  r 2\gamma( \epsilon +\dfrac{ \epsilon}{\sin(\frac{\theta(T)}{2})} + \dfrac{l(G)}{\sin(\min(\theta(T), \frac{\pi}{2}))}) \geq
  2\gamma(r \epsilon +\dfrac{r \epsilon}{\sin(\frac{\theta(T')}{2})} + \dfrac{l(G')}{\sin(\min(\theta(T'), \frac{\pi}{2}))})  $$
  which proves the claim. Finally we will show that $D'$ satisfies the inequality (\ref{eqa:vcg}). It follows from the following set of equalities: 
$$ \text{Bound}(|D'|) = \sum_{e \in \mathbb{E}(T')} \dfrac{|e| + 2 r \epsilon}{2\sqrt{(r\delta)^2-4 r^2 \epsilon^2}} = 
\sum_{e \in \mathbb{E}(T)} \dfrac{r|e| + 2 r \epsilon}{2\sqrt{r^2\delta^2-4 r^2 \epsilon^2}} =
 \sum_{e \in \mathbb{E}(T)} \dfrac{|e| + 2 \epsilon}{2\sqrt{\delta^2-4  \epsilon^2}} = \text{Bound}(|D|).  $$
where the rightmost equation is the upper-bound for $D$. Thus the given bound is invariant under scaling operation. 
 

%both graph $T$ and cloud $C$ are scaled by a factor $r$.  

\end{exa}

\section{Theoretical guarantees}

In this section we will provide proofs for the theorems introduced in Section \ref{sec:theoreticalFramework}. 
Theorem \ref{thmm:GHT} will be proved in Section \ref{sec:homeoGuarantee}. Theorem \ref{thmm:dg} and Theorem \ref{thmm:vcg} will be proved in 
Section \ref{sec:DistanceAndVertexCount}. 

%We will proceed by first showing that the minimum spanning tree using the underlying graph structure on the deep vertices located in the edge-clouds are indeed connected into a chain that is homeomorphic to a single edge-segment. The final result is proved by inductively reconstructing the trees: Starting from Graph having a single vertex, in each step we will add a vertex-edge pair and show that they are homeomorphic to the corresponding minimum spanning trees of the deep vertices. 


\subsection{Homeomorphism guarantee}
\label{sec:homeoGuarantee}

In this section we prove Theorem \ref{thmm:GHT} about homeomorphism guarantees. Since we are using two different metrics in this section, we will denote the Euclidean distance by $d$ and the path metric of a given spatial graph $G$ by $d_G$. 
%For every vertex $v \in \mathbb{V}(T)$ denote its nearest neighbor in the set $D$ by $p_v$. 
%We say that two edges are adjacent in the graph $G$ via vertex $V$, if they share vertex $v \in \mathbb{V}(G)$. 
\begin{lem}[Uniqueness of vertex neighbors]
\label{lem:vertex-point}
Assume the conditions of Theorem \ref{thmm:GHT}. 
Any vertex $v$ of $T$ has a unique point $p_v\in D$ in the $\ep$-ball $B(v,\epsilon)$ at $v$ in the space $(\R^m, d)$.
\end{lem}
\begin{proof}
Given a vertex $v \in \mathbb{V}(T)$ it follows from conditions of Theorem \ref{thmm:GHT} that the nearest neighbor $p_v$ is in the $\ep$-ball $B(v,\ep)$.
If there is another point $q\in C\cap B(v, \ep)$, then by using the fact that $G$ is $\gamma$ approximation $(T,C)$ we obtain the following inequalities:
$$d_G(p_v,q) \leq  d_G(p_v, v) + d_G(q,v) \leq \gamma (d(p_v , v ) + d( q , v )) \leq 2 \gamma \ep < \de, $$ 
which is a contradiction, because from the Equation \ref{eqa:GHT} it follows that $\de \geq 2\gamma\ep $. 

%$d_k(p,q) \leq c_{\max}t_{\epsilon}(p,q)\leq 2c_{\max}\ep<\de$, 
\end{proof}





%the euclidean distance in space $\R^m$ will be denoted by $d$ in this section. We use the following concepts: 

%  We define $d_G$ as its path-metric in the following way:




\begin{figure}[H]
\centering
\begin{tikzpicture}[node distance=3.0cm,
    every node/.style={fill=white}, align=center]
  % Specification of nodes (position, etc.)
  \node[rectangle, draw=red, thick, fill=red!20]  (start)                    {Theorem \ref{thmm:GHT} };
  \node[rectangle, draw=green, thick, fill=green!20] (vertexLemma)     [ below left of=start]          {Lemma \ref{lem:somstod}};
  \node[rectangle, draw=orange, thick, fill=orange!20] (edgeLemma)     [ below right of=start]          {Proposition \ref{lem:edge-offset}};
 \node[rectangle, draw=green, thick, fill=green!20] (isomorphismThm) [right of= edgeLemma] {Lemma \ref{lem:homeomorphismGluingLemma}};
  \node[rectangle, draw=orange, thick, fill=orange!20] (helpVertexLemma) [ below of = vertexLemma] {Proposition \ref{lem:nonadjacentedgesgraph}};
  \node[rectangle, draw=green, thick, fill=green!20] (unionSubdivisionLemma) [right of = helpVertexLemma] {Lemma \ref{lem:MultiMSTGlue}};
  
 % \node[rectangle, draw=green, thick, fill=green!20] (helpEdgeLemma) [right of =unionSubdivisionLemma] {Lemma \ref{lem:edge-offset}};
  
 % \node[rectangle, draw=blue, thick, fill=blue!20] (defFourOneThree) [right of = edgeLemma] {Definition \ref{dfn:subdivision}};
   \node[rectangle, draw=green, thick, fill=green!20]  (dfnEordering) [right of = unionSubdivisionLemma] {Lemma \ref{lem:eordering}};

 % \node[rectangle, draw=blue, thick, fill=blue!20]  (dfnSeparationProperty) [below of = dfnEordering] {Definition \ref{dfn:TreeCover}};
  \node[rectangle, draw=green, thick, fill=green!20]  (lemmafourtwoseven) [below of = dfnEordering] {Lemma \ref{lem:MSTDecomposesIntoTrees}};

  %\node[rectangle, draw=blue, thick, fill=blue!20]  (dfnSep2) [below of = dfnSeparationProperty] {  Definition \ref{dfn:SplitOverVertex}};
  
 % \node[rectangle, draw=blue, thick, fill=blue!20]  (dfnSep1) [below of = dfnSeparationProperty] {  Definition \ref{dfn:multiStarCover}};
  
  %\node[rectangle, draw=blue, thick, fill=blue!20]  (dfnSep0) [below of = dfnSep2] {Definition \ref{dfn:RestrictionOfGraph}    };
  

  
  
  
  \node[rectangle, draw=green, thick, fill=green!20] (adjacentEdgesLemma)[left = 1.5cm of lemmafourtwoseven]{Lemma \ref{lem:AdjacentEdgesLemma}};
    \node[rectangle, draw=green, thick, fill=green!20] (vertexPointLemma) [left = 1.5cm of adjacentEdgesLemma] {Lemma \ref{lem:vertex-point}};

  \node[rectangle, draw=green, thick, fill=green!20] (vertexLinkExistence)[below of = vertexPointLemma]{Lemma \ref{ExistenceOfVertexLink}};
  \node[rectangle, draw=green, thick, fill=green!20] (structureOfPaths)[below of = vertexLinkExistence]{Lemma \ref{lem:structureofpaths}};
  \node[rectangle, draw=green, thick, fill=green!20]  (ssP)[left of =structureOfPaths]{Lemma \ref{lem:ExistenceOfRoutePoint}};
  
  \node[rectangle, draw=green, thick, fill=green!20]  (lemmafourtwosix)[below of =lemmafourtwoseven]{Lemma \ref{lem:EdgeOfMSTIsContainedInCoverSet}};
  
  \node[rectangle, draw=blue, thick, fill=blue!20]  (dfnTreeCover)[below of = lemmafourtwosix]{Definition \ref{dfn:TreeCover}};
  
   \node[rectangle, draw=blue, thick, fill=blue!20]  (dfnGraphCover)[below of = dfnTreeCover]{Definition \ref{dfn:multiStarCover}};

%  \node[rectangle, draw=blue, thick, fill=blue!20]  (dfnGraphCover)[below = dfnTreeCover]{Definition \ref{dfn:GraphCover}};
  
  %\node[rectangle, draw=blue, thick, fill=blue!20]  (ssP)[right of =structureOfPaths]{Definition \ref{shortestPathConnecting}};
  
  
  
  % lem:StarCoverProperty
%  \node[rectangle, draw=green, thick, fill=green!20] (starCoverProperty) [below left of=helpVertexLemma] {Lemma \ref{lem:StarCoverProperty}};
  
 % \node {Definition413} [right of = vertexPointLemma] {Lemma 4.13}
 
%  \node (onStartBlock)      [ below of=onCreateBlock]   {onStart()};
%  \node (onResumeBlock)     [ below of=onStartBlock]   {onResume()};
%  \node (activityRuns)      [ below of=onResumeBlock]
%                                                      {Activity is running};
%  \node (onPauseBlock)      [ below of=activityRuns, yshift=-1cm]
%                                                                {onPause()};
%  \node (onStopBlock)       [ below of=onPauseBlock, yshift=-1cm]
%                                                                 {onStop()};
%  \node (onDestroyBlock)    [ below of=onStopBlock, yshift=-1cm] 
%                                                              {onDestroy()};
%  \node (onRestartBlock)    [ right of=onStartBlock, xshift=4cm]
%                                                              {onRestart()};
%  \node (ActivityEnds)      [ left of=activityRuns, xshift=-4cm]
%                                                        {Process is killed};
%  \node (ActivityDestroyed) [ below of=onDestroyBlock]
%                                                    {Activity is shut down};     
  % Specification of lines between nodes specified above
  % with aditional nodes for description 
  %\draw[->] 			(starCoverProperty) -- (helpVertexLemma);
  %\draw[->]				(dfnSeparationProperty) -| (starCoverProperty);
  \draw[->]				(isomorphismThm) -- (start);
 % \draw[->] 			(dfnSep2) -- (dfnSeparationProperty);
 % \draw[->] 			(dfnSep1) -- (dfnSeparationProperty);
 % \draw[->] 			(dfnSep0) -- (dfnSep2);
  \draw[->]				(dfnEordering) -- (edgeLemma);
  \draw[->]             (vertexLemma) -- (start) ;
  \draw[->]             (edgeLemma) -- (start) ;
  \draw[->]				(helpVertexLemma) -- (vertexLemma) ;
 % \draw[->]				(helpEdgeLemma) -- (edgeLemma);
  \draw[->]				(vertexPointLemma) -- (helpVertexLemma);
  %\draw[->]				(defFourOneThree) -- (edgeLemma);
  \draw[->]				(unionSubdivisionLemma) -- (vertexLemma);
  \draw[->]				(unionSubdivisionLemma) -- (edgeLemma);
 % \draw[->]				(dfnSeparationProperty) -- (unionSubdivisionLemma);
 % \draw[->]				(dfnSeparationProperty) -- (helpVertexLemma);
%  \draw[->]				(dfnSeparationProperty) -- (helpEdgeLemma);
 % \draw[->]				(dfnEordering) -- (helpEdgeLemma);
  \draw[->]				(adjacentEdgesLemma) -- (helpVertexLemma);
 % \draw[->]				(adjacentEdgesLemma) -- (helpEdgeLemma);
  \draw[->]				(vertexLinkExistence) -| (helpVertexLemma);
  %\draw[->]				(vertexLinkExistence) -| (helpEdgeLemma);
  \draw[->]				(structureOfPaths) -- (vertexLinkExistence);
  \draw[->]				(ssP) -- (vertexLinkExistence);
  \draw[->]				(lemmafourtwoseven) -- (unionSubdivisionLemma);
  \draw[->]				(lemmafourtwosix) -- (lemmafourtwoseven);
  \draw[->] 			(dfnTreeCover) -- (lemmafourtwosix);
  \draw[->] 			(dfnGraphCover) -- (dfnTreeCover);
  \draw[->]				(dfnTreeCover) -| (helpVertexLemma);
  \end{tikzpicture}

\caption{Proof structure of Theorem \ref{thmm:GHT}. The Theorem is proved by combining Lemma \ref{lem:somstod}, which proves that minimum spanning tree over edge-clouds is homeomorphic to a single edge-segment of the original Graph and Proposition \ref{lem:somstod}  which shows that minimum spanning tree of the whole deep set can be decomposed into minimum spanning tree's of edge clouds. }
\end{figure}
\begin{figure}[H]
\centering
\includegraphics[width=0.49\linewidth]{UnderlyingGraph/Star2Sep.png}
\includegraphics[width=0.49\linewidth]{UnderlyingGraph/Star5Sep.png}
\caption{Single cover-element $C \cap e^{\epsilon}$ of Theorem \ref{thmm:GHT} colored with red in Star2 (on the left) and Star5 (on the right) graphs.}

\end{figure}


%In the conditions of Theorem \ref{thmm:GHT} we assumed that for every vertex $v \in T$ there exists a point $q \in D$ in its $\epsilon$-neighborhood. In the %following Lemma \ref{lem:vertex-point} we prove that it is unique, i.e. $p_v = q$. 
% $v^{\ep}$
% [Each vertex of $T$ has exactly one point in its $\ep$-ball]



%\begin{dfn}[Star-cover of a metric space]
%\label{dfn:SeparationProperty}
%Let $\{A_i\}$ be a finite cover of a metric space $(X,d)$ and assume that there exists a point $v \in X$ for which $A_j \cap A_i = \{v\}$ for all $i \neq j$. We say that $(\{A_i\} ; v)$ is star-cover of $(X,d)$ if for all $a \in A_i, b \in A_j $ for $i \neq j$ the following two inequalities hold:  $$d(a,v) < d(a,b) \text{ and } d(b,v) < d(a,b).$$ 
%\end{dfn}




\begin{dfn}[Graph-cover and its nerve]
\label{dfn:multiStarCover}
Let $\mathcal{E}$ be a finite cover of a metric space $(X,d)$ and let $\mathcal{V}$ be a finite collection of points in $X$. We say that $(\mathcal{V}, \mathcal{E})$ is a \emph{graph-cover} of $(X,d)$ if the following two conditions are satisfied:
\begin{enumerate}[label={(\arabic*)}]
\item For any distinct sets $A$ and $B$ in $\mathcal{E}$ the intersection $A \cap B$ is either empty or it is a single point of $\mathcal{V}$.
%\item For any distinct $A,B \in \mathcal{E}$ the following holds: $A \cap B = \{u\}$, where $u \in \mathcal{V} \cup \{\emptyset\}$. 
\item  Every $A \in \mathcal{E}$ contains exactly two elements from the set $\mathcal{V}$ i.e. $|\mathcal{V} \cap A| = 2$. 
\end{enumerate}
 We define \emph{the nerve} $\mathcal{N}(\mathcal{V}, \mathcal{E})$ of the graph-cover as the abstract graph having $\mathcal{V}$ as its vertex-set. For any two points
$u,v \in \mathcal{V}$ the set of edges of $\mathcal{N}(\mathcal{V}, \mathcal{E})$ connecting $u$ to $v$ are in 1-1 correspondence with sets $A \in \mathcal{E}$, such that $\{u,v\}$ is contained in the set $A$. For every edge $e \in \mathbb{E}(\mathcal{N}(\mathcal{V}, \mathcal{E}))$ we will denote its corresponding set of $\mathcal{E}$ by $\mathcal{E}(e)$.
 
%  The edge-set of $\mathcal{N}(\mathcal{A}, \mathcal{V})$ consists of all the cover-sets $A \in \mathcal{E}$ which connect the unique points  $u,v \in A \cap \mathcal{V}$ of the condition (2).

% $$\mathbb{V}(\mathcal{N}(\mathcal{A}, \mathcal{V})) = \mathcal{V} \text{ and } \mathbb{E}(\mathcal{N}(\mathcal{A}, \mathcal{V})) = \{(u,v) \in \mathcal{V} \times \mathcal{V} \mid \text{ there exists } A \in \mathcal{A}, \text{ for which } \{u,v\} \subset A\} $$
%We associate every edge of $e \in \mathcal{N}(\mathcal{A}, \mathcal{V})$ with a set $\mathcal{A}(e) \in \mathcal{A}$. 


%\begin{enumerate}
%\item for all $i \neq j$ there either exists $k$ in such a way that $A_i \cap A_j = {v_k}$ or $A_i \cap A_j = \emptyset$ 
%\item for all $i,j,k$ and any $a \in A_i$, $b \in A_j$, where $i \neq j$ the following inequalities hold:
% $$\max(d(a, v_k), d(b, v_k) ) < d(a,b) $$
%\end{enumerate}

\end{dfn}

%\begin{dfn}[Nerve of a graph-cover]
%Let $(\mathcal{A}, \mathcal{V})$ be a star cover of $(X,d)$. Define Nerve of multi-star-cover $\mathcal{N}(\mathcal{A}, \mathcal{V})$ as an graph having:
% $$\mathbb{V}(\mathcal{N}(\mathcal{A}, \mathcal{V})) = \mathcal{V} \text{ and } \mathbb{E}(\mathcal{N}(\mathcal{A}, \mathcal{V})) = \{(v_i, v_j) \mid \text{ there exists } A_k \text{ for which } \{v_i,v_j\} \subset A_k\} $$
%\end{dfn}

%\begin{dfn}[Wedge sum at a vertex] 
%\label{dfn:SplitOverVertex}
%Let $T$ be a tree and let $v \in \mathbb{V}(T)$ be a fixed vertex. We define the equivalence relation $\backsim_v$ on $\mathbb{V}(T) \setminus \{v\}$ in such a way that for $a,b \in \mathbb{V}(T): $ $a \backsim_v b $ if there exists a path from $a$ to $b$ in $T \setminus \{v\}$. For any equivalence class $Q$ of the relation $\backsim_v$, let
%$T | (Q \cup \{v\})$ be the restriction of graph $T$ to the set $Q \cup \{v\}$ defined in Definition \ref{dfn:RestrictionOfGraph}. We define wedge-sum of $T$ at the vertex $v$ as
% $$\mathcal{F}(T,v) = \{T | (Q \cup \{v\}) \text{, where } Q \text{ is a equivalence class of }\backsim_v)\}$$
%%Note that $T | (Q \cup \{v\})$ is a restriction of graph $T$ to the set $Q \cup \{v\}$ as defined in Definition \ref{dfn:RestrictionOfGraph}. 
%%be a collection of all the partition of the equivalence relation $\backsim$. 
%
%\end{dfn}

%\begin{remark}
%
%We note that for any tree $T$ and any vertex $v$ belonging to $T$ the tree $T$ can be considered as a wedge-sum of all the $\mathcal{F}(T,v)$. Hence it follows that  $\mathbb{E}(T) = \cup_{R \in \mathcal{F}(T,v)} \mathbb{E}(R)$.

% We note that for any vertex $v$ tree $T$ is wedge-sum of all the subgraphs in $\mathcal{F}(T,v)$ over a vertex $v$. From this observation is follows that $\mathbb{E}(T) = \cup_{R \in \mathcal{F}(T,v)} \mathbb{E}(R)$.
 %\end{remark}

%For every $Q \in \mathcal{C}(T,v) $ define graph $T(Q,v)$ to be the graph $T | (Q \cup v)$. 


\begin{dfn}[tree-cover]
\label{dfn:TreeCover}
Let $(\mathcal{V}, \mathcal{E})$ be a graph cover of a metric space $(X,d)$. We say that $(\mathcal{V}, \mathcal{E})$ is tree-cover if the following two conditions are satisfied:
\begin{enumerate}[label={(\arabic*)}]

\item The nerve $\mathcal{N}(\mathcal{V}, \mathcal{E})$ is a tree (is acyclic and connected).
\item For every distinct $u,v \in X$, if there does not exist a set $A \in \mathcal{E} $ satisfying $\{u,v\} \subseteq A $, then there exists a point $t \in X$ for which $\max(d(u, t), d(v, t) ) < d(u,v) $

%\item For every $a,b$ distinct points of $X$ satisfying $a \in A \in \mathcal{E}$, $b \in B \in \mathcal{E}$ and $A \neq B$. 
%There exists a point $v \in \mathcal{V}$ that satisfies $\max(d(a, v), d(b, v) ) < d(a,b) $.
%\item For every $v \in \mathcal{V}$ let $\mathcal{F}(\mathcal{N}(\mathcal{V}, \mathcal{E}),v)$ be wedge-sum of $T$ at the vertex $v$ defined in Definition \ref{dfn:SplitOverVertex}. Then for any two points $a,b \in X$ having $a \in \mathcal{E}(e)$ and $b \in \mathcal{E}(h)$ for edges $e,h$ that belong to distinct graphs of $\mathcal{F}(\mathcal{N}(\mathcal{V}, \mathcal{E}),v)$ the following inequality hold:
%$$\max(d(a, v), d(b, v) ) < d(a,b) $$

%   $\mathcal{C}(\mathcal{N}(\mathcal{A}, \mathcal{V}),v)$. Then for any $a \in \mathcal{A}(e)$ and $b \in \mathcal{A}(h)$ the following inequality hold:
%
%
%Removing $v \in \mathcal{V}$ splits $\mathcal{N}(\mathcal{A}, \mathcal{V}) \setminus \{v\}$ (treated as topological space) into two components $C_1, C_2$, in such a way that for all $i,j$ and any $a \in A_i$, $b \in A_j$, where $i \neq j$ the following inequality hold: $\max(d(a, v), d(b, v) ) < d(a,b) $
 
\end{enumerate}
\end{dfn}

%\begin{lem}
%Let $(\mathcal{A}, \mathcal{V})$ be a star cover of $(X,d)$, in such a way that its nerve $\mathcal{N}(\mathcal{A}, \mathcal{V})$ is a tree
%
%\end{lem}
%

%
%\begin{lem}
%\label{lem:StarCoverProperty}
%Let $\{A_i\}$ and $\{B_j\}$ be finite covers of a metric space $(X,d)$ satisfying the following condition: For every $A_i$ there exists $B_j$ having $A_i \subseteq B_j$. Assume that $\{A_i\}$ is a star-cover of $(X,d)$, then $\{B_i\}$ is a star-cover as well.
%\end{lem}
%\begin{proof}
%
%Let $B_j$ and $B_k$ be distinct cover elements of  $\{B_j\}$. Following from the imposed condition and the facts that both $\{A_i\}$ and $\{B_j\}$ are covers, we are able to decompose $B_j$ and $B_k$ as the following unions:
%$$B_j = \bigcup_{i_x}A_{i_x} \text{ and } B_k  = \bigcup_{i_y}A_{i_y} $$
%We can now compute their intersection by using "Intersection distributes over union"-property
%$$B_j \cap B_k = \bigcup_{i_x}A_{i_x} \cap \bigcup_{i_y}A_{i_y} = \bigcup_{(i_x,i_y)}A_{i_x} \cap A_{i_y} = \{v\}$$
%Thus it follows that $\{B_j\}$ is a star cover of the metric space $(X,d)$.
%
%\end{proof}

\begin{exa}
\label{exa:StarCover}
Let us pick an arbitrary star5-graph $T$, similar to one illustrated in the Figure \ref{fig:StarCover}. In this example we will show that we can build a tree-cover in two different ways: Firstly we can build tree-cover on $T$ in a combinatorial way, by defining $\mathcal{V} = \mathbb{V}(T)$ and $\mathcal{E} = \{\{u,v\} \mid (u,v) \in \mathbb{E}(T)\} $. We will show that $(\mathcal{V}, \mathcal{E})$ is a tree-cover of
 $(X, d_T )$, where $X = \mathcal{V}$ and $d_T$ is the path-metric of the graph $T$. By the definition of graph $T$ any two edges intersect at exactly one point, which we call a centroid point $o$. Also every edge $e$ contains exactly two points from the set of vertices $\mathcal{V}$. Thus  $(\mathcal{V}, \mathcal{E})$ is a graph-cover of $(\mathbb{V}(T), d_T )$. We note that the nerve $\mathcal{N}(\mathcal{V}, \mathcal{E})$ is isomorphic to graph $T$ and thus $\mathcal{N}(\mathcal{V}, \mathcal{E})$ is a tree. We are left to prove that the condition (2) of the Definition \ref{dfn:TreeCover} is satisfied. We note that any two $u,v \in X$ are not contained in the same set of $\mathcal{E}$, iff both $u,v$ are not the centroid point $o$. In this case we can select $o$ as the intermediate point that satisfies inequality $\max\{d_T(u,o), d_T(v,o)\} < d_T(u,v) $

Secondly in the continuous case a tree-cover can be built on $T$ treated as an infinite metric space, by setting $\mathcal{V} = \mathbb{V}(T)$ and 
$\mathcal{E} = \{e \mid e \in \mathbb{E}(T)\}$, where every edge $e$ is treated as infinite metric space which is isometric to an interval $[0,1]$. We can prove that $(\mathcal{V}, \mathcal{E})$ is a tree cover of $(T,d_T)$ similarly, as we did in the previous case. 
%
%We can build tree-cover on $T$ by treating as an infinite metric space and we can build tree-cover in a combinatorial by considering only vertices $\mathbb{V}(T)$. Denote $\mathcal{V} = \mathbb{V}(T) $ and let us use notation $\mathcal{E}$ for both, the collections of infinite metric space $\{e \mid e \in \mathbb{E}(T)\}$ and the collection of their end points 
%$\{\{u,v\} \mid (u,v) \in \mathbb{E}(T)\} $. We will show that  $(\mathcal{V}, \mathcal{E})$ is a tree-cover of a path metric space $(T,d_T)$, in both of the cases, when $T$ is treated as an infinite metric space and when $T$ is just a finite set of vertices. Let us show first that $(\mathcal{V}, \mathcal{E})$ is a graph-cover. By the definition of graph $T$ any two edges intersect at exactly one point, that we call a centroid point $o$. Also every edge $e$ contains exactly two points from the set of vertices $\mathcal{V}$. Thus  $(\mathcal{V}, \mathcal{E})$ is a graph-cover. 
%
%We note that the nerve $\mathcal{N}(\mathcal{V}, \mathcal{E})$ is isomorphic to graph $T$. This follows by considering the map $f$ which maps every point $p \in \mathcal{V}$ into a corresponding vertex of $\mathcal{N}(\mathcal{V}, \mathcal{E})$. We note that every edge in graph $T$ is mapped to a corresponding edge of $\mathcal{N}(\mathcal{V}, \mathcal{E})$. Because $f$ is an isomorphism it follows that $T$ is isomorphic to $\mathcal{N}(\mathcal{V}, \mathcal{E})$ and thus the nerve $\mathcal{N}(\mathcal{V}, \mathcal{E})$ has to be tree. The distance condition of tree-cover is satisfied because $o$ is the only point which belongs to $\mathcal{V}$ and removal of which splits graph $T$ into multiple components. We note that any path connecting arbitrary points $p,q$ belonging to distinct edges of $T$ has to go thought the centroid point $o$. Thus inequalities $d(p,o) \leq d(p,q)$ and $d(q,o) \leq d(p,q)$ are trivially satisfied. It follows that $(\mathcal{V}, \mathcal{E})$ is a tree-cover of a path metric space $(T,d_T)$.
%
%


%Let $\mathcal{E} = \mathbb{E}(T)$ and $\mathcal{V} = \mathbb{V}(T)$. Then $(\mathcal{V}, \mathcal{E})$ is tree-cover of $T$ treated as a metric space. Intersection between any two edges is the centroid point $o$. We will now show that $(\mathcal{V}, \mathcal{E})$ is a graph-cover. 
%We note that every edge contains exactly two points vertices and intersection of any two edges is indeed a single point or empty set. 
%Thus $(\mathcal{V},\mathcal{E})$ is a graph-cover. To prove that $(\mathcal{V},\mathcal{E})$ is a tree-cover, we note that $T$ is homeomorphic to
%the nerve $\mathcal{N}(\mathcal{V}, \mathcal{E})$. Finally the distance condition of tree-cover is satisfied, because any path between points $p, q$ belonging to different edges $e,h$ goes through point $o$ and thus $d(p,o) \leq d(p,q)$ and $d(q,o) \leq d(p,q)$. 

%
%% $\mathcal{V} = \{\}$
%
%
%In this example we prove that $(\mathbb{E}(T),o)$ forms tree-cover of $(T, d_T)$. The intersection condition is trivially satisfied by noting that $e_i \cap e_j = \{o\}$ for all  $e_i,e_j \in \mathbb{E}(T)$.
%
% The distance condition is satisfied, because any path between points $p, q$ belonging to different edges $e_i, e_j$ goes through point $o$ and thus $d(p,o) \leq d(p,q)$ and $d(q,o) \leq d(p,q)$. 
\end{exa}

\begin{figure}
\centering
\begin{tikzpicture}

\def \n {5}
\def \radius {3}
\def \margin {8} % margin in angles, depends on the radius

\node at (0,0) (o) {};
\filldraw[black] (0,0) circle (4pt);

% {360/\n * (\s - 1)}:\radius
\draw[fill=yellow, fill opacity=0.5] (1.5,0) ellipse (1.5 and 0.5);  
\draw[rotate around={360/5 * (2-1):({360/5 * (2 - 1)}:1.5)}, fill=red, fill opacity=0.5] ({360/5 * (2 - 1)}:1.5) ellipse (1.5 and 0.5);
\draw[rotate around={360/5 * (3-1):({360/5 * (3 - 1)}:1.5)}, fill=green, fill opacity=0.5] ({360/5 * (3 - 1)}:1.5) ellipse (1.5 and 0.5);  
\draw[rotate around={360/5 * (4-1):({360/5 * (4 - 1)}:1.5)}, fill=blue, fill opacity=0.5] ({360/5 * (4 - 1)}:1.5) ellipse (1.5 and 0.5);  
\draw[rotate around={360/5 * (5-1):({360/5 * (5 - 1)}:1.5)}, fill=orange, fill opacity=0.5] ({360/5 * (5 - 1)}:1.5) ellipse (1.5 and 0.5);  
  


\foreach \s in {1,...,\n}
{
  \node at ({360/\n * (\s - 1)}:\radius) (\s){};
  \filldraw[black] ({360/\n * (\s - 1)}:\radius) circle (4pt);
  \draw [thick,-] (o) -- (\s);

  %\draw[->, >=latex] ({360/\n * (\s - 1)+\margin}:\radius) 
  %  arc ({360/\n * (\s - 1)+\margin}:{360/\n * (\s)-\margin}:\radius);
}
\end{tikzpicture}

\caption{Tree-cover of a Star5 graph, as described in Example \ref{exa:StarCover}. The corresponding tree-cover sets have been marked using different colors.}
\label{fig:StarCover}
\end{figure}
%there exists $\MST(A \cup B)$ on set $A \cup B$ which is union

%We note that a given graph $G$ built on a set $X$ is $\MST$ if it is connected, acyclic and satisfies the cycle property: if we add any edge to graph $G$ then it will be the largest in the cycle that it creates. 

%\begin{lem}[Minimum spanning tree gluing lemma]
%\label{lem:MSTGlue} 
%Assume that $(\{A,B\} ; v)$ is a Star-cover of a finite metric space $(X,d)$. Then for any minimum spanning tree $W \in \MST(A \cup B, d) $ there exists minimum spanning trees $U \in \MST(A,d)$ and $V \in \MST(B,d)$ for which the following equality holds: $W = U \cup V$. If $U$ and $V$ are unique then $W$ is unique as well and we denote $$\MST(A \cup B, d) = \MST(A,d) \cup \MST(B,d).$$ 
%
%% $\MST(A,d) \cup \MST(B,d)$ is a minimum spanning tree on the set $A \cup B$. 
%% and $\MST(B)$ for which $\MST(A \cup B) = \MST(A) \cup \MST(B)$.
%\end{lem}
%
%\begin{proof}
%Let $W$ be an arbitrary minimum spanning tree on set $A \cup B$. Let us define $U = W | A$ and $V = W | B$ as restrictions of graph $W$ on sets $A$ and $B$ respectively. We will prove that $U \cup V$ is a minimum spanning tree on the set $A \cup B$ using the following definition: a given graph $G$ built on a set $X$ is $\MST$ if it is connected, acyclic, and satisfies the cycle property: if we add an edge to graph $G$ then it will be the largest in the cycle that it creates. 
%
%%\emph{Graph $U \cup V$ spans $\mathbb{V}(W)$} . Let $a,b$ be arbitrary points. 
%
%\textbf{Connectedness of graph $U \cup V$: } First of all we note that the graphs $U$ and $V$ are both connected and they have a non-empty intersection following from the cover tree property $A \cap B = \{v\}$. Thus $U \cup V$ is connected as well. 
%
%\textbf{Acyclicness of $U \cup V$: } We will use Eucler characteristic which states that a connected graph $G$ is acyclic iff 
%$\mathbb{E}(G) = \mathbb{V}(G) - 1$. By assumptions the following equations hold:
%$$\mathbb{E}(U) = \mathbb{V}(U) - 1 \text{, } \mathbb{E}(V) = \mathbb{V}(V) - 1.$$ 
%Also from structures of $\MST(A,d)$, $\MST(B,d)$ and $\MST(A \cup B,d)$ we obtain
%$$\mathbb{V}(U \cup V)  = \mathbb{V}(U) + \mathbb{V}(V) -1 $$ 
%$$\mathbb{E}(U \cup V)  = \mathbb{E}(U) + \mathbb{E}(V)$$
%Combining the equalities we get a chain of equalities which proves the claim.
%$$\mathbb{V}(U \cup V) - 1 = \mathbb{E}(U) + \mathbb{E}(V) = \mathbb{E}(U \cup V)  $$
% 
%\textbf{Graph $U \cup V$ satisfies cycle property: } Let $e = (x,y)$ be an arbitrary edge that doesn't belong to $U \cup V$ and let $l$ be the path that connects $x$ with $y$ in $U \cup V$. If the edge $e$ is completely contained in $A$, then $e$ has to be the longest edge by cycle property of $U$ (symmetrically if $e$ is contained in $B$, then we can use cycle property of $V$). In case $x$ and $y$ belong to distinct sets, say $x \in A$ and $y \in B$ we note that the path $l$ has to go through $v$, because its the only point that belongs to both $A$ and $B$ and there are no other connections between the aforementioned sets. Thus we can split path $l$ into two parts $f,g$, where $f$ is the shortest path from $x$ to $v$ and $g$ is the shortest path from $v$ to $y$. Using the cycle property of $U$ we obtain that either path $f$ consists of a single edge $(x,v)$ or the length of $(x,v)$ is larger than any element of path $f$. Similarly $g$ either consists of a single edge $(y,v)$ or $(y,v)$ is the largest element of the path $g$. Because we assumed that $(\{A,B\};v)$ is a star-cover we can use the second condition Definition \ref{dfn:SeparationProperty} to deduct $$\max \{d(y,v),d(x,v)\} < d(x,y). $$
%It follows that $(x,y)$ has to be largest edge in the cycle $l \cup (x,y)$. 
%
%
%
%\textbf{If both $\MST(A,d)$ and $\MST(B,d)$ are unique then $\MST(A \cup B,d)$ is unique as well: } We assume that both $\MST(A,d)$ and $\MST(B,d)$ are unique. Make counter assumption that $\MST(A \cup B,d)$ is not unique. Then there exists two trees $W, W'$ for which $W \neq W'$ . However ,we have assumed that both $\MST(A,d)$ and $\MST(B,d)$ consists only of a single graphs that we denote by $U$ and $V$ respectively. From the previous claims $W = U \cup V = W'$ which is a contradiction. 
%
%
%
%%Let $e \in \mathbb{E}(W') \setminus \mathbb{E}(W)$. Assume that $U$ and $V$ are the minimum spanning trees satisfying the condition $U \cup V = W $. Then edge $e$ should belong to either $U$ or $V$
%% From the previous claim we obtain that any edge in $W$ should be completely 
%%contained in $U$ or $V$. The claim holds, because, both $U$ and $V$ satisfy the cycle property separately. 
%
% %We have previously proved that there exist no edges having one end point in $\mathbb{V}(V) \setminus \{v\}$ and other in $\mathbb{V}(U)
%% \setminus \{v\}$ in $U \cup V$. Thus edge $e$ should be contained entirely in either $U$ or $V$, which is a contradiction because we %have assumed that $W = U \cup V$ and $e \notin W$ . 
%\end{proof}


We recall that Corollary \ref{cor:MSTProperty} stated that a given graph $G$ built on a set $X$ is $\MST$ iff it is connected, acyclic, and satisfies the cycle property defined in Definition \ref{dfn:CyclePropertyGraph}.



%\begin{lem}
%
%Assume that $(\mathcal{V}, \mathcal{E} )$ is a tree-cover of a finite metric space $(X,d)$. 
%
%\end{lem}

\begin{lem}[Each edge of $\MST$ on tree-cover is contained in some cover-set $\mathcal{E}$]
\label{lem:EdgeOfMSTIsContainedInCoverSet}

Assume that $(\mathcal{V}, \mathcal{E} )$ is a tree-cover of a finite metric space $(X,d)$.
Let $W$ be a minimum spanning tree of $(X,d)$. Then for every edge $(u,v)$ of the tree $W$ there exists a unique set $A \in \mathcal{E}$ containing both 
end points $u$ and $v$. 

\end{lem}
%there does not exist a set in the collection $\mathcal{E}$ which contain both $u$ and $v$. Let $A,B \in \mathcal{E}$ be arbitrary sets satisfying $u \in A$ and $v \in B$
\begin{proof}

Assume by contradiction that there exists an edge $(u,v) \in \mathbb{E}(W)$ whose end points are not covered by a single set $A \in \mathcal{E}$.  Condition (2) of Definition \ref{dfn:TreeCover} implies that there exists a point $t$ that satisfies $\max(d(v, t), d(u, t) ) < d(u,v) $. We note that the triplet $(v,t), (t,u), (u,v) $ of pairs in the space $X$ forms a cycle. From the cycle property we obtain that $(u,v)$ can't be part of minimum spanning tree $W$, because it has the largest edge-length. Thus we have reached contradiction and the original claim holds. 

%$(u,v,t)$ is a cycle , where $(u,v)$ is edge having the largest weight. Thus it can't be included in $W$, which is a contradiction. 

We have now proved that for every edge $(u,v)$ there exists a set  $A \in \mathcal{E}$ that contains both of the end points $u,v$. Assume now that there exists another set $B$ that contains them. Then edges corresponding to $A,B$ in the nerve $\mathcal{N}(\mathcal{V}, \mathcal{E})$ would form a cycle consisting of two edges. This is a contradiction, because we have assumed that the nerve $\mathcal{N}(\mathcal{V}, \mathcal{E})$ is a tree.


%

%Make counter assumption that there exists such edge $h \in \mathbb{E}(W)$ having end points $a$ and $b$, such that there does not exist a set $A \in \mathcal{E} $ containing both $a$ and $b$. Assume that $a \in A$ and $b \in B$ for some distinct $A,B \in  \mathcal{E} $.  Let $u,v$ be the end points of the edge $A$ in the graph $\mathcal{N}$. Let us consider a special case first where $A \cap B = u$ or $A \cap B = v$. By symmetry assume that $A \cap B = v$. From the assumption $ a \neq v $ and $b \neq v$. Thus $a$ and $b$ belong to different subgraphs of $\mathcal{F}(T,v) $ and we can use the tree-cover assumption (2) to deduct $\max( d(a,v) , d(b,v) ) < d(a,b)$. Now $(a,v) \cup (v,b)$ provides a path, where all the links are smaller than the direct route $(a,b)$. Thus $(a,b)$ does not belong to the minimum spanning tree $W$, which is a contradiction.
%
%Let us consider the case $A \cap B = \emptyset$ now. If $a$ and $b$ belong to the same collection of both $\mathcal{F}(T,v) $ and $\mathcal{F}(T,u) $, then the graph $\mathcal{N}$ would have to be disconnected and thus would lead to a contradiction. In other words either $\mathcal{F}(T,v) $ or $\mathcal{F}(T,u) $ splits $a$ and $b$ into different graphs. By symmetry let us assume that $v$ is such point. Again by the tree-cover assumption we can deduct $\max( d(a,v) , d(b,v) ) < d(a,b) $ and thus edge $(a,b)$ does not belong $W$, which is a contradiction. 

\end{proof}

\begin{dfn}[Restriction of a graph]
\label{dfn:RestrictionOfGraph}
Let $G$ be a graph and let $A$ be a subset of its vertex-set i.e. $A \subseteq \mathbb{V}(G)$. We define $G | A$ as the graph having
$\mathbb{V}(G | A) = A $ and $\mathbb{E}(G | A) = \{(u,v) \in \mathbb{E}(G) \mid u,v \in A\}$. 
\end{dfn}

\begin{lem}
\label{lem:MSTDecomposesIntoTrees}
Assume that $(\mathcal{V}, \mathcal{E} )$ is a tree-cover of a finite metric space $(X,d)$. Let $W$ be an arbitrary minimum spanning of space $(X,d)$. 
Then for every $e \in \mathcal{N}(\mathcal{V}, \mathcal{E} )$ the graph $W | \mathcal{E}(e)$ is a tree. 
\end{lem}
\begin{proof}
%We can now define collection $\mathcal{P}$ of subgraphs of $W$ as restrictions of the minimum spanning tree $W$ to the sets of collection $\mathcal{E}$ i.e. $$ \mathcal{P} = \{ ( W | \mathcal{E}(e) )\mid e \in \mathbb{E}(\mathcal{N})\}.$$ For any edge $e \in \mathbb{E}(\mathcal{N})$ we denote the graph $(\mathcal{P}(\mathcal{E}(e)))$ simply by $\mathcal{P}(e)$. We will now prove that for any edge $e \in \mathbb{E}(\mathcal{N})$ graph $\mathcal{P}(e)$ is a minimum spanning tree of the space $(\mathcal{E}(e),d)$.

In this Lemma we use the following notations: $W(e) =  W | \mathcal{E}(e)$ and $\mathcal{N} =  \mathcal{N}(\mathcal{V}, \mathcal{E} )$. We note first that if $W(e)$ contains a cycle for some $e \in \mathbb{E}(\mathcal{N})$, then $W$ would contain cycle as well. It follows that graph $W(e)$ is acyclic. By using Euler characteristic we deduct: $W(e)$ is connected iff $|\mathbb{E}(W(e))| = |\mathbb{V}(W(e))| - 1$.  By using Euler characteristic on the aforementioned graphs we obtain Equations
(\ref{eqa:firstAcycliness}) - (\ref{eqa:thridAcycliness})

%
%Then 
%  Using properties of collection $\mathcal{P}$ and $\mathcal{N}$ we can deduct the following two equalities:

%|\mathbb{E}(W)| = |\mathbb{V}(W)| - 1 \\

Equation \ref{eqa:firstAcycliness} follows from the fact any vertex $v \in \mathbb{V}(W)$ either belongs to $\mathcal{V}$ or there exists a unique $e \in \mathbb{E}(W)$ for which $v \in W(e)$.  Equation \ref{eqa:secondAcycliness} follows from Lemma \ref{lem:EdgeOfMSTIsContainedInCoverSet} which states that every edge $h \in \mathbb{E}(W)$ is contained in exactly one graph $W(e)$. Equations \ref{eqa:thridAcycliness} follow from the observation, that both $\mathcal{N}$ and $\mathcal{W}$ are acyclic and connected.

\begin{align}
|\mathbb{V}(W)| &=  \sum_{e \in \mathbb{E}(\mathcal{N})} |\mathbb{V}(W(e)) \setminus \mathcal{V}| + |\mathbb{V}(\mathcal{N})| =
\sum_{e \in \mathbb{E}(\mathcal{N})} |\mathbb{V}(W(e))| - 2|\mathbb{E}(\mathcal{N})| + |\mathbb{V}(\mathcal{N})|\label{eqa:firstAcycliness} \\
|\mathbb{E}(W)| &=  \sum_{e \in \mathbb{E}(\mathcal{N})} |\mathbb{E}(W(e))|  \label{eqa:secondAcycliness}  \\
|\mathbb{E}(\mathcal{N})| &= |\mathbb{V}(\mathcal{N})| - 1 \text{ and } |\mathbb{E}(W)| = |\mathbb{V}(W)| - 1 \label{eqa:thridAcycliness}
\end{align}

%Following from the fact that $\mathcal{N}$ and $W$ are trees we have as well $|\mathbb{E}(\mathcal{N})| = |\mathbb{V}(\mathcal{N})| - 1$ and $|
%\mathbb{E}(W)| = |\mathbb{V}(W)| - 1$.
By combining all the equations above we obtain: 
$$\sum_{e \in \mathbb{E}(\mathcal{N})} |\mathbb{E}(W(e))| = |\mathbb{E}(W)| = |\mathbb{V}(W)| - 1 =   |\mathbb{V}(W)| + |\mathbb{E}(\mathcal{N})| - |\mathbb{V}(\mathcal{N})| = \sum_{e \in \mathbb{E}(\mathcal{N})} |\mathbb{V}(W(e))| - |\mathbb{E}(\mathcal{N})|   $$

If $W(h)$ which is not connected for some edge $h \in \mathbb{E}(\mathcal{N})$ , then
$|\mathbb{E}(W(h))| < |\mathbb{V}(W(h))| - 1$.  From the equation above it follows that there exists an edge $h' \in \mathbb{E}(\mathcal{N})$ for which $ |\mathbb{E}(W(h'))| > |\mathbb{V}(W(h'))| - 1$. However, this means that $W(h')$ would have to contain cycle, which is a contradiction.
 It follows that for all $e \in \mathbb{E}(\mathcal{N})$ graphs $W(e)$ are all trees.  
\end{proof}


\begin{lem}[Minimum spanning tree gluing lemma]
\label{lem:MultiMSTGlue}
%\label{cor:MSTGLUE}
Assume that $(\mathcal{V}, \mathcal{E} )$ is a tree-cover of a finite metric space $(X,d)$.
Let $W$ be an arbitrary minimum spanning tree of $(X,d) $. Then for every $A \in \mathcal{E}$ there exists a minimum spanning tree $\MST(A,d)$ for which
 $W = \cup_{A \in \mathcal{A}}\MST(A,d) $. If for any $A \in \mathcal{E}$ the minimum spanning-tree $\MST(A,d)$ is unique, then the minimum spanning tree $\MST(X,d)$ is unique as well.
\end{lem}
\begin{proof}
 Let $W$ be an arbitrary minimum spanning tree of the space $(X,d)$. In this Lemma we use notations: $W(e) =  W | \mathcal{E}(e)$ and $\mathcal{N} =  \mathcal{N}(\mathcal{V}, \mathcal{E} )$. We conclude from Lemma \ref{lem:EdgeOfMSTIsContainedInCoverSet} that each edge $e \in \mathbb{E}(W)$ is included in some set $A \in \mathcal{E}$. It follows that $W = \bigcup_{e \in \mathbb{E}(\mathcal{N})}W(e)$. It follows from Lemma \ref{lem:MSTDecomposesIntoTrees} that every graph $W(e)$ is a tree. We will now show  that $W(e)$ is a minimum spanning tree of space $\mathcal{E}(e)$. 

%We will denote the nerve $\mathcal{N}(\mathcal{V}, \mathcal{E})$ simply by $\mathcal{N}$ in this Lemma. Let $W$ be an arbitrary minimum spanning of $(X,d)$. Following from Lemma \ref{lem:EdgeOfMSTIsContainedInCoverSet}  for every edge $(u,v)$ of the tree $W$ there exists a unique set 
%$A \in \mathcal{E}$ for which $u \in A$ and $v \in A$.  We can now define collection $\mathcal{P}$ of subgraphs of $W$ as restrictions of the minimum spanning tree $W$ to the sets of collection $\mathcal{E}$ i.e. $$ \mathcal{P} = \{ ( W | \mathcal{E}(e) )\mid e \in \mathbb{E}(\mathcal{N})\}.$$ For any edge $e \in \mathbb{E}(\mathcal{N})$ we denote the graph $(\mathcal{P}(\mathcal{E}(e)))$ simply by $\mathcal{P}(e)$. We will now prove that for any edge $e \in \mathbb{E}(\mathcal{N})$ graph $\mathcal{P}(e)$ is a minimum spanning tree of the space $(\mathcal{E}(e),d)$.

% Because there are no edges having end-points 




% the following holds true: 
%Let $a$ and $b$ be the endpoints of edge $h$. Then there exists a set $A \in \mathcal{E} $ for which $a \in A$ and $b \in A$. 

%Assume that $a \in A \in \mathcal{E}$ and $b \in B \in \mathcal{E}$, then $A \cap B \neq \emptyset$.
%\textbf{Any edge $h$ is completely contained in some set $A \in \mathcal{A}$:} 



%Make counter assumption that there exist such $a \in A$ and $b \in B$ which satisfy $A \cap B = \emptyset$ for which $(a,b) \in %\mathbb{E}(W)$.


%
%Let us denote $\mathcal{V}(s)$ to be a path on elements $\mathcal{V}$ formed by connecting consecutive occurrences of elements 
%$\mathcal{V}$ in path $s$. Let $v \in \mathcal{V}(s)$ be arbitrary element. Then by the tree-cover property we obtain 
%$\max( d(a,v) , d(b,v) ) < d(a,b) $. Because $(a,b)$ is larger than both $(a,v)$ and $(b,v)$, it creates a cycle where it has the largest size. This is a contradiction. Thus $(a,b) \notin \mathbb{E}(W)$ and both end points of every edge is indeed contained in some element of $\mathcal{A}$.
%



%Let $u,v$ be the first and last element of $\mathcal{V}(s)$ respectively. We define path $s'$ by connecting $u$ to $x$ and $v$ to $y$ i.e. $s' = (x,v) \cup \mathcal{V}(s) \cup (u,y)$.  

%Let $\mathcal{V}(s)$ be the ordered sequence of all the points in $\mathcal{V}$ that the path $s$ visits. 


%Let $v$ be arbitrary vertex that $\mathcal{V}(s)$ visits . Using the tree-cover property we obtain $\max(d(x,v), d(y,v) ) < d(x,y) $. We can now spit path $s'$ into two parts $s'_0$ and $s'_1$ where $s'_0$ is a path from $x$ to $v$ and $s'_1$ is a path from $v$ to $y$ in such a way that $s' = s'_1 \circ s'_0 $.  By repeating this process on all $v \in \mathcal{V}(s)$
%we obtain that for all the consecutive elements $(u,v)$ of $s'$ the following inequality holds:
%$$\max_{(\alpha,\beta) \in \mathcal{V}(s)}d(\alpha,\beta) < d(x,y)$$
%%We note that both end points $(\alpha,\beta) \in \mathcal{V}(s)$ belong to the same set $\mathcal{A}((\alpha,\beta))$. We have now proved that for any pair of points $x,y$ there exists a path connecting $x$ to $y$, where every intermediate edge $e$ is contained in some set $\mathcal{A}(e)$ and where $|e| < |(x,y)|$. Thus $(x,y)$ cannot be contained in  


%
%If $u,v$ are consecutive elements in $\mathcal{V}(s)$ then $u,v \in \mathcal{N}(e)$ for some edge $e$. Because $ \mathcal{N}(e)$ is $\MST$ it satisfies the cycle property. Thus it follows $$\max_{(\alpha, \beta) \in s | \mathcal{N}(e)} d(\alpha,\beta) < d(u,v). $$ Now by combining the two inequalities we obtain
%$$\max_{(\alpha, \beta) \in s} d(\alpha,\beta) < \max_{(u,v) \in \mathcal{V}(s)}d(u,v) < d(x,y) $$
%Thus edge $(x,y)$ is the largest in the cycle $s \cup (x,y)$. In other words $h \notin W$, which is a contradiction.


%\emph{Graph $U \cup V$ spans $\mathbb{V}(W)$} . Let $a,b$ be arbitrary points. 
%
%\textbf{Connectedness of graph $P$: } We will first prove that for any $u,v \in \mathcal{V}$ there exists a path between them in $\cup_{P \in \mathcal{P}}P$. We have assumed that the nerve $\mathcal{N}$ is connected, thus there exists a path $s$ connecting $u$ to $v$ in $\mathcal{N}$. Let $e = (x,y)$ be arbitrary edge in $s$ and let $\mathcal{P}(e)$ corresponding restriction of graph $W$. By the definition $\mathcal{P}(e)$ is connected. Thus there exists path $s'(e)$ from $x$ to $y$ in  $P$. We note that for any adjacent edges $e,h \in s$ their intersection is $\{q\}$ for some $q \in \mathcal{V}$. It follows that $\mathcal{P}(e) \cap \mathcal{P}(h) = \{q\}$ as well. It follows that $s' = \circ_{e \in \mathbb{E}(s)}s'(e)$ is a path that connects $u$ to $v$ in $P$.
%
%We can now prove the general claim by simply fixing some $v \in \mathcal{V}$ and showing that for any $p \in X$ there exists a path connecting $p$ to $v$. We note that if $p \in X$, then $p \in A$ for some $A \in \mathcal{A}$. By the definition of $\mathcal{P}(A)$ there exists some point $u \in A \cap \mathcal{V}$. Because $\mathcal{P}(A)$ is connected, there exists a path $\alpha$ connecting $p$ to $u$. Previously we have proved that there exists a path between any two points of $\mathcal{V}$ in  $P$. Let $\beta$ be a path between $v$ and $u$ in $\cup_{P \in \mathcal{P}}P$. Let us define $\gamma = \beta \circ \alpha$. This is indeed a path that connects $p$ to $v$. Because $p$ was selected arbitrary, the graph  $P$ is connected.


%Now if for every $i$ there exists a path from $x_i$ to $x_{i+1}$ in $\mathcal{N}(\mathcal{A}, \mathcal{V})$ we can combine them 

%
%Let us first prove that there exists a path in $\cup_{i \in J}U_i$ between any two $a,b \in \mathcal{V} $. Let us select arbitrary 
%$p,q \in \mathcal{V} \cap A_i$ for some $A_i \in \mathcal{A}$. We note that because $U_i$ was connected, there exists a path between $p$ and $q$ in $U_i$. We note that the edge $[p,q]$ in the nerve $\mathcal{N}(\mathcal{A}, \mathcal{V})$ indeed corresponds $A_i$ that contains both points $p,q$. Because the nerve is connected we can construct path $a$ to $b$ in the nerve that goes through some sets
% $A_{t_0}, A_{t_1} ... A_{t_k}$ in such a way that intersection of the consecutive elements is non-empty. Because every $U_{t_i}$ is connected, the points $a$ and $b$ can indeed be connected in graph $\cup_{i \in J}U_i$.
% 
% 
%Let us prove a general claim by fixing some $v \in \mathcal{V}$ and showing that for any $p \in \cup_{i \in J}U_i$ we are able to construct path from $p$ to $v$ in $\mathcal{A}$. Let $p \in   \cup_{i \in J}U_i$ be arbitrary point. Then $p \in U_k$ for some $k$. Because $U_k$ is connected, we can construct a path from $p$ to some point of $\mathcal{V}$. We have previously proved that there exists a path between any points in $\mathcal{V}$. Thus by combining a path inside $U_i$ with a path between elements of  $\mathcal{V}$, we are able to construct a path from $p$ to $v$, which proves the claim. 

%
%First of all we recall that we have assumed that $\mathcal{N}(\mathcal{A}, \mathcal{V})$ is connected. Thus there exists a path between %$a$ and $b$ in the nerve. 
%
%
%Recall that every edge $[p,q]$ in the nerve consists of sets of$\mathcal{A}$ which contains both endpoints 
%$p$ and $q$. We 
%
%
% Let us fix arbitrary point $v \in \mathcal{V}$. We will show that for any $p \in \cup_{i \in J}U_i$ we can construct path that connects $p$ to $v$. Let $p \in U_i$ be arbitrary selected point for some $U_i$. First of all we note that all the graphs $U_i$ are connected. Thus from any point in $U_i$ we can reach any point $v \in \mathcal{V} \cap U_i$. Now because the nerve $\mathcal{N}(\mathcal{A}, \mathcal{V})$ is connected and all the sets $U_i$ are connected we are able to reach point $v$. Because $p$ was selected arbitrary it follows that $\cup_{i \in J}U_i$ is a connected graph.

%and they have a non-empty intersection following from the cover tree property $A_i \cap A_j = \{v\}$ for all $i \neq j$. It follows that %$\cup_{i \in J}U_i$ is a connected graph.

%  We will use Euler characteristic which states that a connected graph $G$ is acyclic iff $|\mathbb{E}(G)| = |\mathbb{V}(G)| - 1$. 

 Let us fix arbitrary $e \in \mathbb{E}(\mathcal{N})$. Let $a,b \in \mathcal{E}(e)$ be such that 
$(a,b) \notin \mathbb{E}(W(e))$. Then also $(a,b) \notin \mathbb{E}(W)$ . Let $s$ be a path that connects $a$ to $b$ in the graph $W(e)$. This path is included into $W$. Now because $W$ is $\MST$. We can use Lemma \ref{lem:CycleProperty} to deduct that $d(a,b) \geq d(u,v)$ for any $(u,v) \in s$. Because points $a,b \in \mathcal{E}(e)$ were chosen arbitrarily, it follows that $W(e)$ satisfies the cycle property. Hence, we can use Lemma \ref{lem:CyclePropertyToMST} to deduct that $W(e)$ is a minimum spanning tree of $ \mathcal{E}(e)$. 
 
 
  %Following from cycle property 
%
%and thus it is the largest edge in cycle it creates in $W$. Because $W(e)$ is connected there exists a path $s$ between $a$ and $b$, which by the definition coincides with the shortest path between $a$ and $b$ in $W$. 
%Because $(a,b)$ was the largest edge in the cycle it creates in $W$ , it also the largest edge in the collection $s \cup (a,b)$. Thus $(a,b)$ can't be part of minimum spanning tree $W(e)$. Because $a,b$ were chosen arbitrarily, it follows that $W(e)$ is a minimum spanning tree of space $\mathcal{E}(e)$ for all $e \in \mathbb{E}(\mathcal{N})$. 


%
%We also note that every $P \in \mathcal{P}$ inherits the cycle property from graph $W$: Let us fix $P \in \mathcal{P}$ and let $a,b \in \mathbb{V}(P)$ , such that $(a,b) \notin \mathcal{P}$ and let path $s$ be connecting $a$ to $b$ in $P$. Then $s \cup (a,b)$ is a cycle in $P$ and thus is a cycle in $W$ as well. By the cycle property of $W$ the edge $(a,b)$ is largest in the cycle $s \cup (a,b)$. Hence it is largest in $P$ as well. Because $(a,b)$ was chosen arbitrarily it follows that all $P \in \mathcal{P}$ satisfy the cycle property.


Because $W = \cup_{e \in \mathbb{E}(\mathcal{N})}\mathcal{E}(e) $ and $W$ was chosen arbitrary. We have found the desired minimum spanning trees that satisfy the condition $\MST(X,d) = \cup_{A \in \mathcal{E}}\MST(A,d)$. Now if every set $\MST(A,d)$ is unique, then we can deduct trivially the minimum spanning tree $\MST(X,d)$ has to be unique as well. 



%$|\mathbb{E}(P)| = |\mathbb{V}(P)| - 1 $:

%
%\textbf{Every edge $h \in W$ is contained into some $N \in \mathcal{N}$: } Let us make counter assumption that $h = (a,b)$ has end points, which belong to different sets $x \in \mathcal{P}(e)$ and $y \in \mathcal{P}(e')$ for some $e,e' \in \mathbb{E}(N)$. Let $s$ be the shortest path connecting $a$ to $b$ in $P$. Let $\mathcal{V}(s)$ be the ordered sequence of all the points in $\mathcal{V}$ that the path $s$ visits. 
%Let $v \in \mathcal{V}(s)$ be arbitrary vertex. Using the tree-cover property we obtain $\max(d(x,v), d(y,v) ) < d(x,y) $. We can now spit path $s$ into two parts $s'$ and $s''$ where $s'$ is a path from $x$ to $v$ and $s''$ is a path from $v$ to $y$ in such a way that $s = s'' \circ s' $. We will perform recursively similar splits $s'$ and $s''$. By repeating this process on all $v \in \mathcal{V}(s)$
%we obtain that for all the consecutive elements $(u,v)$ of $\mathcal{V}(s)$ the following inequality holds:
%$$\max_{(u,v) \in \mathcal{V}(s)}d(u,v) < d(x,y)$$
%We note that if $u,v$ are consecutive elements in $\mathcal{V}(s)$ then $u,v \in \mathcal{N}(e)$ for some edge $e$. We note that because $ \mathcal{N}(e)$ is $\MST$ it satisfies the cycle property. Thus it follows $$\max_{(\alpha, \beta) \in s | \mathcal{N}(e)} d(\alpha,\beta) < d(u,v). $$ Now by combining the two inequalities we obtain
%$$\max_{(\alpha, \beta) \in s} d(\alpha,\beta) < \max_{(u,v) \in \mathcal{V}(s)}d(u,v) < d(x,y) $$
%Thus edge $(x,y)$ is the largest in the cycle $s \cup (x,y)$. In other words $h \notin W$, which is a contradiction.
%
%%\textbf{Every edge $h \in \mathbb{E}()$ is contained }
% 
%\textbf{Graph $P$ satisfies cycle property: } Let $h = (a,b)$ be an arbitrary edge having $a,b \in X$ that doesn't belong to 
%$P$ and let $l$ be the path that connects $a$ with $b$ in $P$. By previous claim the $h$ is completely contained in $N$ for some $N \in \mathcal{N}$. The edge $h$ has to be the longest edge by the cycle property of $\mathcal{N}(e)$.
%

%Assume now that $a,b$ belong to different subgraphs of $\mathcal{N}$. Let $s$ be the shortest path connecting $a$ to $b$ in $P$. Let $\mathcal{V}(s)$ be the ordered sequence of all the points in $\mathcal{V}$ that the path $s$ visits. 
%Let $v \in \mathcal{V}(s)$ be arbitrary vertex. Using the tree-cover property we obtain $\max(d(x,v), d(y,v) ) < d(x,y) $. We can now spit path $s$ into two parts $s'$ and $s''$ where $s'$ is a path from $x$ to $v$ and $s''$ is a path from $v$ to $y$ in such a way that $s = s'' \circ s' $. We will perform recursively similar splits $s'$ and $s''$. By repeating this process on all $v \in \mathcal{V}(s)$
%we obtain that for all the consecutive elements $(u,v)$ of $\mathcal{V}(s)$ the following inequality holds:
%$$\max_{(u,v) \in \mathcal{V}(s)}d(u,v) < d(x,y)$$
%We note that if $u,v$ are consecutive elements in $\mathcal{V}(s)$ then $u,v \in \mathcal{N}(e)$ for some edge $e$. We note that because %$ \mathcal{N}(e)$ is $\MST$ it satisfies the cycle property. Thus it follows $$\max_{(\alpha, \beta) \in s | \mathcal{N}(e)} d(\alpha,\beta) < d(u,v). $$ Now by combining the two inequalities we obtain
%$$\max_{(\alpha, \beta) \in s} d(\alpha,\beta) < \max_{(u,v) \in \mathcal{V}(s)}d(u,v) < d(x,y) $$
%Thus edge $(x,y)$ is the largest in the cycle $s \cup (x,y)$. Because path $x,y$ were arbitrary selected we have proved that graph $P$ %satisfies cycle property. 



%In the connectnedness part of the proof we have showed that there exists a path between $a$ and $b$ 


%In case $x$ and $y$ belong to distinct sets, say $x \in U_n$ and $y \in U_m$ we note that the path $l$ has to go through $v$, because its the only point that belongs to both $U_n$ and $U_m$ and there are no other connections between the aforementioned sets. Thus we can split path $l$ into two parts $f,g$, where $f$ is the shortest path from $x$ to $v$ and $g$ is the shortest path from $v$ to $y$. Using the cycle property of $U$ we obtain that either path $f$ consists of a single edge $(x,v)$ or the length of $(x,v)$ is larger than any element of path $f$. Similarly $g$ either consists of a single edge $(y,v)$ or $(y,v)$ is the largest element of the path $g$. Because we assumed that $(\mathcal{A};v)$ is a star-cover we can use the second condition Definition \ref{dfn:SeparationProperty} to deduct $$\max \{d(y,v),d(x,v)\} < d(x,y). $$
%It follows that $(x,y)$ has to be largest edge in the cycle $l \cup (x,y)$. 

%
%
%\textbf{If all the $\MST(A_i)$ are unique then $\MST(\cup_{i \in J}A_i,d)$ is unique as well: }We assume that all the $\MST(\cup_{i \in J}A_i,d)$ are unique. Make counter assumption that $\MST(\cup_{i \in J}A_i,d)$ is not unique. Then there exists two trees $W, W'$ for which $W \neq W'$ . However ,we have assumed that all the collections $\MST(A_i,d)$ consists only of a single graphs that we denote by $U_i$. From the previous claims $W = \cup_{i \in J}A_i = W'$ which is a contradiction. 


\end{proof}

%
%\begin{lem}[Minimum spanning tree gluing lemma]
%\label{lem:MSTGlue}
%%\label{cor:MSTGLUE}
%Assume that $(\mathcal{A} = \{A_i \mid i \in J\} ; v)$ is a Star-cover of a finite metric space $(X,d)$. Then for any minimum spanning tree $W \in \MST(\cup_{i \in J} A_i , d) $ for every  $i \in J $ there exists a minimum spanning trees $U_i \in \MST(A_i,d)$ for which
% $ W = \cup_{i \in J} U_i $. If for all $i \in J$ the minimum spanning trees $\MST(A_i,d)$ are unique i.e. each collection consists only of a single element, then $\MST(\cup_{i \in J} A_i , d)$ is unique as well. 
%\end{lem}
%\begin{proof}
%
%
%Let $W$ be an arbitrary minimum spanning tree on set $\cup_{i \in J} A_i$. Let us define $U_i = W | A_i$ as restrictions of graph $W$ on sets $A_i$. We will prove that $\cup_{i \in J}U_i$ is a minimum spanning tree on the set $\cup_{i \in J} A_i$ using the following definition: a given graph $G$ built on a set $X$ is $\MST$ if it is connected, acyclic, and satisfies the cycle property: if we add an edge to graph $G$ then it will be the largest in the cycle that it creates. 
%
%%\emph{Graph $U \cup V$ spans $\mathbb{V}(W)$} . Let $a,b$ be arbitrary points. 
%
%\textbf{Connectedness of graph $\cup_{i \in J}U_i$: } First of all we note that all the graphs $U_i$ are connected and they have a non-empty intersection following from the cover tree property $A_i \cap A_j = \{v\}$ for all $i \neq j$. It follows that $\cup_{i \in J}U_i$ is a connected graph.
%
%\textbf{Acyclicness of $U \cup V$: } We will use Eucler characteristic which states that a connected graph $G$ is acyclic iff 
%$\mathbb{E}(G) = \mathbb{V}(G) - 1$. Because each $U_i$ is acyclic and connected the following equation $\mathbb{E}(U_i) = \mathbb{V}(U_i) - 1 $ holds for all $i \in J$. From the definition of $\cup_{i \in J}U_i$ we obtain:
%$$\mathbb{V}(\cup_{i \in J} U_i )  = \sum_{i \in J} \mathbb{V}(U_i) -1 \text{ and }
%\mathbb{E}(\cup_{i \in J} U_i)  =  \sum_{i \in J} \mathbb{E}(U_i)  $$ 
%%$$$$
%Combining all the equalities we get a chain of equalities which proves the claim.
%$$\mathbb{V}(\cup_{i \in J} U_i) - 1 =  \sum_{i \in J} \mathbb{V}(U_i) -1 =  \sum_{i \in J} \mathbb{E}(U_i) = \mathbb{E}(\cup_{i \in J} U_i)  $$
% 
%\textbf{Graph $\cup_{i \in J} U_i$ satisfies cycle property: } Let $e = (x,y)$ be an arbitrary edge that doesn't belong to 
%$\cup_{i \in J} U_i$ and let $l$ be the path that connects $x$ with $y$ in $\cup_{i \in J} U_i$. If the edge $e$ is completely contained in $U_i$ for some $i \in J$,  then $e$ has to be the longest edge by cycle property of $U$. In case $x$ and $y$ belong to distinct sets, say $x \in U_n$ and $y \in U_m$ we note that the path $l$ has to go through $v$, because its the only point that belongs to both $U_n$ and $U_m$ and there are no other connections between the aforementioned sets. Thus we can split path $l$ into two parts $f,g$, where $f$ is the shortest path from $x$ to $v$ and $g$ is the shortest path from $v$ to $y$. Using the cycle property of $U$ we obtain that either path $f$ consists of a single edge $(x,v)$ or the length of $(x,v)$ is larger than any element of path $f$. Similarly $g$ either consists of a single edge $(y,v)$ or $(y,v)$ is the largest element of the path $g$. Because we assumed that $(\mathcal{A};v)$ is a star-cover we can use the second condition Definition \ref{dfn:SeparationProperty} to deduct $$\max \{d(y,v),d(x,v)\} < d(x,y). $$
%It follows that $(x,y)$ has to be largest edge in the cycle $l \cup (x,y)$. 
%
%
%
%\textbf{If all the $\MST(A_i)$ are unique then $\MST(\cup_{i \in J}A_i,d)$ is unique as well: }We assume that all the $\MST(\cup_{i \in J}A_i,d)$ are unique. Make counter assumption that $\MST(\cup_{i \in J}A_i,d)$ is not unique. Then there exists two trees $W, W'$ for which $W \neq W'$ . However ,we have assumed that all the collections $\MST(A_i,d)$ consists only of a single graphs that we denote by $U_i$. From the previous claims $W = \cup_{i \in J}A_i = W'$ which is a contradiction. 
%
%
%\end{proof}

%
%
%\begin{proof}


%This theorem can be proved by using an alternative definition of a minimum spanning tree, i.e a given graph $G$ built on a set $X$ is $\MST$ if it is connected, acyclic and satisfies the cycle property: if we add any edge to graph $G$ then it will be the largest in the cycle that it creates. We claim that $\MST(A,d) \cup \MST(B,d)$ is one of the possible minimum spanning trees of the set $A \cup B$.
%
%\emph{Connectedness:} First of all we note that the sets $\MST(A,d)$ and $\MST(B,d)$ are both connected and they have a non-empty intersection. It follows that $\MST(A,d) \cup \MST(B,d)$ is also connected.
%
%\emph{Acyclic:} We will use Eucler characteristic which states that a connected graph $G$ is acyclic iff 
%$\mathbb{E}(G) = \mathbb{V}(G) - 1$. By assumptions the following equations hold:
%$$\mathbb{E}(\MST(A,d)) = \mathbb{V}(\MST(A,d)) - 1 \text{, } \mathbb{E}(\MST(B,d)) = \mathbb{V}(\MST(B,d)) - 1.$$ 
%Also from structures of $\MST(A,d)$, $\MST(B,d)$ and $\MST(A \cup B,d)$ we obtain
%$$\mathbb{V}(\MST(A \cup B,d))  = \mathbb{V}(\MST(A,d)) + \mathbb{V}(\MST(B,d)) -1 $$ 
%$$\mathbb{E}(\MST(A \cup B,d))  = \mathbb{E}(\MST(A,d)) + \mathbb{E}(\MST(B,d))$$
%Combining the equalities we get a chain of equalities which proves the claim.
%$$\mathbb{V}(\MST(A \cup B,d)) - 1 = \mathbb{E}(\MST(A,d)) + \mathbb{E}(\MST(B,d)) = \mathbb{E}(\MST(A \cup B,d))  $$
% %and $$|\mathbb{E}(\MST(A) \cup \MST(B))| = |\mathbb{E}(\MST(A))| + |\mathbb{E}(\MST(B))|.$$
%\emph{Cycle property:} Let $e = (u,w)$ be an edge that doesn't belong to $\MST(A,d) \cup \MST(B,d)$ and let $l$ be a path that connects $u$ with $w$ in $\MST(A,d) \cup \MST(B,d)$. If both end points of the newly added edge $e$ belong to the same set $A$ or $B$ then it has to be the longest edge by definition of $\MST(A,d)$ (or definition of $\MST(B,d)$ respectively). In case $u$ and $w$ belong to distinct sets, say $u \in A$ and $w \in B$ we note that the path $l$ has to visit the point $v$ which belongs to both sets $A$ and $B$.  Using the cycle property of $\MST(A,d)$ we deduct $d(u,v) < d(u,w)$ and respectively from cycle property of $\MST(B,d)$ we obtain $d(v,w) < d(u,w)$. Using star-cover definition 
%
%%We will now apply 
%
%If $(u,v)$ belongs to $\MST(A,d)$ and $(u,w)$ belongs to $\MST(B,d)$ then path $l$ consists of exactly two elements which are both smaller than the newly added edge. Assume now that $(u,v)$ doesn't belong to $\MST(A,d)$. Then it is the largest edge among all the edges in restriction of the path $l$ to the set $A$. Similarly, if $d(u,w)$ doesn't belong to $\MST(B,d)$, by the cycle property all the other edges are larger. It follows that an edge $d(u,w)$ creates a cycle, where it is the largest edge. Because the points $u,w$ were selected arbitrarily, the original claim holds. 
%\end{proof}


%Assume that points of $\overline{D}_e$ are ordered according to their projection $\text{pr}$ on edge $e$. Let $\overline{D}_e[u,v]$ be set of all points of $\overline{D}_e$ which project onto interval $[u,v]$.






%\begin{dfn}[$e$-ordering]
%\label{dfn:eordering}
%Assume the conditions of Theorem \ref{thmm:GHT}. Let $e = [u,v]$ be a line segment and let $C$ be a finite point set in space $\mathbb{R}^m$. Let $\text{pr}_{e}:C \rightarrow e$ be a function that maps each point $a \in C$ to its nearest neighbor that we denote by $\text{pr}(a)$ (Each point of $C$ either maps orthogonally to $e$ or to one of the end point of the edge). We say that $C$ has $e$-ordering , if all points $a_i, a_j$ satisfying $ i \leq j $ have $d(\text{pr}(a_i), u) \leq d(\text{pr}(a_j), u) $. 
%\end{dfn}
%
%It should be noted that in the Definition \ref{dfn:starDecompose} we treat $T \setminus \{v\}$ as a graph having 
%$$\mathbb{V}(T \setminus \{v\}) = \mathbb{V}(T) \setminus \{v\} \text{ and } 
%\mathbb{E}(T \setminus \{v\}) = \{e \mid v \notin e \} \cup \{(u,\text{copy}(v)) \mid e = (v,u) \text{ for some } u\}.$$
%In other words every occurrence of $v$ in edges containing it in $T$ is copied into separate entity. 
%
%and replacing it with separate copies for every edge $e \in \mathbb{E}$ that contains it. In other words:
%$$\mathbb{V}(T \setminus \{v\}) = \mathbb{V}(T) \setminus \{v\} \text{ and } 
%\mathbb{E}(T \setminus \{v\}) = \{e \mid v \notin e \} \cup \{(u,\text{copy}(v)) \mid e = (v,u) \text{ for some } u\}.$$

%\begin{dfn}[Standard star cover over fixed vertex]
%\label{dfn:starDecompose}
%%Something will be written here. 
%
%Assume the conditions of Theorem \ref{thmm:GHT}. Let $v$ be an arbitrary vertex of a straight-line tree $T$. Let $T \setminus \{v\}$ be a graph obtained by removing vertex $v$ from spatial tree $T$. We define the \emph{standard star-cover} of $D$ over vertex $v$ in the following way:
%$$\mathcal{T}(v) = \{ D \cap (Q \cup \{v\})^{\epsilon} \mid Q \text{is a connected component of }T \setminus \{v\} \} $$
%
%\end{dfn}

Proposition \ref{lem:nonadjacentedgesgraph} and Proposition \ref{lem:edge-offset} will be proved in Section \ref{sec:TechnicalSection}.




%Let $k = |\text{degree}(v,T)| $ and let $\{e_i \mid i \in k\}$ be the set of edges having $v$ as one of their end points. Assume that the graph $T$ is split into graphs $\{T_i \mid i \in [k]\}$ in such a way that every $T_i$ contains $v$ and all the edges and vertices  which are closer to $e_i$ than any other edge $e_j$, where $j \in [k] \setminus {i}$.

%Let $T_i$ be set of trees 

%\begin{dfn}[Standard star-cover of a graph]
%\label{dfn:StandardStarCover}
%Assume that we are given tree $T$, graph $G$, cloud $C$ and a set $D$ that satisfy the conditions of Theorem \ref{thmm:GHT}.
%Let $T \setminus \{v\}$ be a graph obtained by removing vertex $v$ from spatial tree $T$. We define family of component trees over $v$ in the following way:
%
%$$\mathcal{Q}(T,v) = \{Q \cup \{v\} \mid Q \text{ is a connected component of }T \setminus \{v\}\}$$
%
%We define a standard star-cover over vertex $v$ as follows:
%
%$$\mathcal{S}(T,v) = \{ D \cap (Q)^{\epsilon} \mid Q \in \mathcal{Q} \}$$
%\end{dfn}
%
%\begin{dfn}[Standard star-cover of a graph]
%\label{dfn:StandardStarCover}
%Assume the conditions of Theorem \ref{thmm:GHT}. We define the multi-star cover of subset $D$ as $(\mathcal{A}, \mathcal{V})$, where 
%$\mathcal{A} = \{e^{\epsilon} \cap D \mid e \in \mathbb{E}(T)\}$ and $\mathcal{V} = \{p_v \mid v \in \mathbb{V}(T)\}$.  
%
%
%
%\end{dfn}


\begin{restatable}[Tree cover of vertices]{pro}{spov}
\label{lem:nonadjacentedgesgraph}


Assume the conditions of Theorem \ref{thmm:GHT}. Define collections $\mathcal{V} = \{p_v \mid v \in \mathbb{V}(T)\}$ and
$\mathcal{E} = \{e^{\epsilon} \cap D \mid e \in \mathbb{E}(T)\}$. Then $(\mathcal{V}, \mathcal{E})$ is tree-cover of $(D, d_G)$.

%Cover $(\mathcal{A}, \mathcal{V})$, whe
%$\mathcal{E} = \{e^{\epsilon} \cap D \mid e \in \mathbb{E}(T)\}$ and $\mathcal{V} = \{p_v \mid v \in \mathbb{V}(T)\}$ is tree-cover
%of $(D, d_G)$.


%Let $v$ be an arbitrary vertex of a straight-line tree $T$. The star-cover $(\mathcal{T}(T, v) ; p_v )$ defined in Definition \ref{dfn:StandardStarCover} is a star-cover of space $(D, d_G)$, where $p_v$ is the unique nearest neighbor of $v$ in $D$ as defined in Definition \ref{lem:vertex-point}.

%Let $v$ be an arbitrary vertex of the straight-line tree $T$. Let $k = |\text{degree}(v,T)| $ and let $\{e_i \mid i \in k\}$ be the set of edges having $v$ as one of their end points. Assume that the graph $T$ is split into graphs $\{T_i \mid i \in [k]\}$ in such a way that every $T_i$ contains $v$ and all the edges and vertices  which are closer to $e_i$ than any other edge $e_j$ having $j \neq i$. Let $T^{\epsilon}_i$ be the $\epsilon$-offset of set $T_i$. Then $(\{D \cap T^{\epsilon}_i \mid i \in [k]\}, p_v) $ is a star cover of space $(D, d_G)$. 

\end{restatable}


\begin{restatable}[a minimum spanning tree of the edge-set is a polygonal path]{pro}{spoe}
\label{lem:edge-offset}

Assume the conditions of Theorem \ref{thmm:GHT}. Then for every edge $e = (u,v) \in \mathbb{E}(T)$ the minimum spanning tree  $\MST(e^{\epsilon} \cap D, d_G)$ is a polygonal path connecting $p_u$ to $p_v$.




%$$(\mathcal{A} = \{\{r,q\} \mid r,q \text{ are consecutive elements in }e \text{ ordering }\}, \mathcal{V} = \{D \cap e^{\epsilon}\})$$ 
%is a tree-cover of $(D \cap e^\epsilon,d_G)$.
\end{restatable}

\begin{lem}[Structure of the minimum spanning tree on dense set]
\label{lem:somstod}
Assume the conditions of Theorem \ref{thmm:GHT}. Then $\MST(D, d_{G})$ is uniquely defined and 
$\MST(D, d_{G}) = \bigcup_{e \in \mathbb{E}(T)} \MST(e^{\epsilon} \cap D, d_G)$.
\end{lem}
\begin{proof}
By Proposition \ref{lem:nonadjacentedgesgraph} for $\mathcal{E} = \{e^{\epsilon} \cap D \mid e \in \mathbb{E}(T)\}$ and $\mathcal{V} = \{p_v \mid v \in \mathbb{V}(T)\}$ the pair $(\mathcal{V}, \mathcal{E})$ is a tree-cover of $(D,d_G)$. From 
Proposition \ref{lem:edge-offset} we obtain that $\MST(e^{\epsilon} \cap D, d_G)$ is uniquely defined. Now we can use Lemma 
\ref{lem:MultiMSTGlue} to deduct $\MST(D, d_{G}) = \bigcup_{e \in \mathbb{E}(T)} \MST(e^{\epsilon} \cap D, d_G)$.

\end{proof}

%\begin{restatable}[Star cover of vertices]{lem}{spov}
%\label{lem:nonadjacentedgesgraph}
%Assume that we are given tree $T$, graph $G$, cloud $C$ and a set $D$ that satisfy the conditions of Theorem \ref{thmm:GHT}.
%Let $v$ be an arbitrary vertex of a straight-line tree $T$. The star-cover $(\mathcal{T}(T, v) ; p_v )$ defined in Definition \ref{dfn:StandardStarCover} is a star-cover of space $(D, d_G)$, where $p_v$ is the unique nearest neighbor of $v$ in $D$ as defined in Definition \ref{lem:vertex-point}.
%
%%Let $v$ be an arbitrary vertex of the straight-line tree $T$. Let $k = |\text{degree}(v,T)| $ and let $\{e_i \mid i \in k\}$ be the set of edges having $v$ as one of their end points. Assume that the graph $T$ is split into graphs $\{T_i \mid i \in [k]\}$ in such a way that every $T_i$ contains $v$ and all the edges and vertices  which are closer to $e_i$ than any other edge $e_j$ having $j \neq i$. Let $T^{\epsilon}_i$ be the $\epsilon$-offset of set $T_i$. Then $(\{D \cap T^{\epsilon}_i \mid i \in [k]\}, p_v) $ is a star cover of space $(D, d_G)$. 
%
%\end{restatable}

% Assume that we are given tree $T$, Graph $G$, Cloud $C$ that satisfy the conditions of Theorem \ref{thmm:GHT}
% Let $D_i = \bigcup_{e \in \mathbb{E}(T_i)} e^\epsilon \cap D$.
%
%\begin{restatable}[Star cover of edges]{lem}{spoe}
%\label{lem:edge-offset}
%%Assume that $D \cap e^\epsilon^\epsilon^\epsilon$ is $e$-ordered
%%Let $\overline{D}_e[u,v]$ be set of all points of $D \cap e^\epsilon^\epsilon^\epsilon$ which project onto interval $[u,v]$.
%Assume the conditions of Theorem \ref{thmm:GHT}. Let $e = (u,v)$ be any edge of a straight-line tree $T\subset\R^m$.  For any $r,q \in D \cap e^\epsilon$ in $ p_u < r < q < p_v$ in $e$-ordering the pair $$(\{D \cap [u,\text{pr}_e(r)]^\epsilon, D \cap [\text{pr}_e(r),\text{pr}_e(q)]^{\epsilon}\}, q)$$ is a star-cover of $(D \cap [u,\text{pr}_e(q)]^\epsilon,d_G)$.\end{restatable}

%\begin{lem}[Assumption of Theorem \ref{thmm:GHT} are inherited in component-trees of Definition \ref{dfn:StandardStarCover}]
%\label{lem:Rtsg}
%
%Assume that we are given tree $T$, graph $G$, cloud $C$ and a set $D$ that satisfy the conditions of Theorem \ref{thmm:GHT}. Let $v$ be an arbitrary vertex and let $\mathcal{Q}(T,v)$ be as in Definition \ref{dfn:StandardStarCover}. Then for any $Q \in \mathcal{Q}(T,v)$ the combination involving: graph $Q$, graph $G \cap Q^{\epsilon}$, cloud $C \cap Q^{\epsilon}$ and set $D \cap Q^{\epsilon}$ satisfy the assumption of Theorem \ref{thmm:GHT}. 
%
%\end{lem}
%\begin{proof}
%
%We note that, because $D$ is $\delta$-sparse, then $D \cap Q^{\epsilon}$ is $\delta$-sparse as well. 
%
%
%\end{proof}
%
%

%\begin{dfn}[Subdivision]
%\label{dfn:subdivision}
%Let $G$, $H$ be abstract graphs. We say that the graph $H$ is a subdivision of the graph $G$ if for every edge $e = (u,w) \in \mathbb{E}(G)$ we can find a chain of vertices $v_0, ..., v_k   \in \mathbb{V}(H)$ for which $u = v_0$, $w = v_k$ and 
%$(v_i, v_{i+1}) \in \mathbb{E}(H)$ for all $i \in [k-1]$. 
%
%\end{dfn}
% on the points located in its $\epsilon$-offset 
%\begin{pro}
%\label{lem:eht}
%%Let a tree $T$ be as in assumption of Theorem 
%Assume the conditions of Theorem \ref{thmm:GHT}. Then for every edge $e = (u,v) \in \mathbb{E}(T)$ the minimum spanning tree  $\MST(e^{\epsilon} \cap D, d_G)$ is a polygonal path connecting $p_u$ to $p_v$.
%
%
%%in such a way that there exists a subdivision $e'$ of $e$ and an isomorphism $f_e:e' \rightarrow \MST(e^{\epsilon} \cap D, d_G)$ which maps $u$ to %$p_u$ and $v$ to $p_v$, where $p_u,p_v$ are the nearest neighbors of $u$ and $v$ respectively.
%%there exists a subdivision of $e'$ and isomorphism $f_e:e' \rightarrow \MST(e^{\epsilon} \cap D, d_G)$ for which $f(u) = p_u$ and $f(v) = p_v$. 
%\end{pro}
%\begin{proof}
%
%Let $a_0,..., a_k$ be the points of $e^{\epsilon} \cap D$ ordered by $e$-ordering. For every integer $i \geq 0$ we denote $S_i$ to be a set consisting of first $i+1$-elements of $D$. This claim will be proved by using induction on the index $i$ to show that $\MST(S_i)$ is a path that connects $a_0$ to $a_{i}$, in such a way that the path is formed by edges $[a_j,a_{j+1}]$ where $0 \leq j \leq i$.
%
%In the base case of induction $i = 1$ the set $S_i$ consists of two elements $a_0, a_1$. Because $\MST(S_1)$ is indeed a polygonal path connecting $a_0$ to $a_1$ the claim holds trivially. Let us now prove the induction step. We assume that the claim holds for $S_j$ for some $j$ and will prove that it holds for $S_{j+1}$ as well. Following from Lemma \ref{lem:edge-offset} we obtain that 
%$ (\{S_j, (a_j,a_{j+1}) \} ; a_j ) $ is a star-cover of $S_j$. Because both $\MST(S_i)$ and $\MST(\{a_j,a_{j+1}\})$ are unique we can use Lemma \ref{lem:MSTGlue} to deduct that $\MST(S_{i+1})$ is unique and $\MST(S_{i+1}) = \MST(S_i) \cup \MST(\{a_j,a_{j+1}\})$ , which is a combination of two paths: $\MST(S_i)$ connects $a_0$ to $a_{i}$ via $[a_j,a_{j+1}]$ where $0 \leq j \leq i$ and $ \MST(\{a_j,a_{j+1}\})$ is simply a straight-line path from $a_j$ to $a_{j+1}$. Thus we have proved the induction step.
%
%The final claim that $\MST(e^{\epsilon} \cap D, d_G)$ is the polygonal path connecting $p_u$ to $p_v$ follows from the fact that 
%$\MST(e^{\epsilon} \cap D, d_G) = \MST(S_k \cap D, d_G) $ , where $a_0 = p_u$ and $a_k = p_v$.
%
%
%
%
% \end{proof}
%It should be noted that following from Proposition \ref{lem:eht} are uniquely defined. Thus we can use $\MST(e^{\epsilon} \cap D, d_G)$ to denote the specific minimum spanning tree, rather than treating it as a collection.  
%\begin{pro}[Structure of the minimum spanning tree on dense set]
%\label{lem:somstod}
%Assume the conditions of Theorem \ref{thmm:GHT}. Then $\MST(D, d_{G})$ is uniquely defined and 
%$\MST(D, d_{G}) = \bigcup_{e \in \mathbb{E}(T)} \MST(e^{\epsilon} \cap D, d_G)$.
%
%
%%Assume that each set $e \cap D$ has $e$-ordering then graph $\MST(D, d_{G})$ has the following form:  For every edge $e$ in the set $a_i \in e \cap D$ all the adjacent vertices $a_i, a_{i+1}$ generate an edge in graph $\MST(D, d_{G}) $. 
% %Each edge $e \in \text{Edges}(\MST(D, d_{G}))$ consists 
%
%%Graph $\MST(D, d_{G})$ has the following form: The vertex set consists of all the points in set $D$. 
%
%%Every edge $e = (u,v)$ has one of the following form: 
%%\begin{enumerate}
%%\item one
%%\item two
%%\end{enumerate}
%%  By using Lemma \ref{lem:StarCoverProperty} we can simply modify the cover to consists of two parts, an edge $[u,y]$ and graph $R_{j}$
%\end{pro}
%%where $R_{i+1}$ is obtained from $R_i$ by adding a vertex outside of $R_i$ and connected it by an edge.
%\begin{proof}
%% $p \in R^{\epsilon}_i $ if $ d(p, R_i) \leq \epsilon$. 
%% introduces a new vertex and an edge from graph $T$ which are not contained in the previous element $R_{i}$. We denote $R^{\epsilon}_i$ to be the $\epsilon$-offset of $R_i$ i.e
%
%For every integer $i \geq 1$ we denote by $R \in \mathcal{R}_i$ to be the class of subtrees of $T$ having $i$ vertices. This proposition will be proved by using induction step on $i$ to show that has the decomposition property $ \cup_{e \in \mathbb{E}(R)} \MST(D \cap e^{\epsilon},d_G) = \MST(D \cap R^{\epsilon}, d_G)$ for all $R \in \mathcal{R}_i$ when $1 \leq j \leq i$. It should be noted that for index $k = |\mathbb{V}(T)|$ the set $\mathcal{R}_k$ consists of only a single element $\{T\}$ and $D \cap T^{\epsilon} = D$. Thus the claim will follow from the more general claim that every $R \in \mathcal{R}_i$ has the decomposition property for all $i$. 
%
%
%%of $T$, in such a way that $|\mathbb{V}(R_i)| = i$.
%
%%Let us first define a filtration $\{v_0\} = R_0 \subseteq R_1 \subseteq R_{2} \subseteq R_{3} \subseteq ... \subseteq R_{t} = T $, where 
%%$\mathbb{V}(R_{i+1}) = \mathbb{V}(R_{i}) \cup \{v_{i}\} \text{ and } \mathbb{E}(R_{i+1}) \cup \{e_i\} $ satisfying $v_i \in e_i$ , and $v_i$ and $e_i$ are ordered in such a way that Degree$(v_i ,R_i) = 1$ for all $i \geq 1$. This proposition will be proved using induction on $i$, by showing that 
%%$\MST(D \cap R_i^{\epsilon}, d_G) = \cup_{e \in \mathbb{E}(R_i)} \MST(D \cap e^{\epsilon},d_G).$ for all $i$. It should be noted that $D \cap R^{\epsilon}_{t} = D \cap T^{\epsilon} = D$. Thus the claim will follow from the fact that $R_i$ has the decomposition property for all $i$. 
%
%
%In the base case of induction we note that any $R \in \mathcal{R}_1$ consists of two vertices connected by an edge $e$. The decomposition claim for $R$ follows trivially, because it contains only a single edge. Assume now that $\MST(D \cap R^{\epsilon}) = \cup_{e \in \mathbb{E}(R)} \MST(D \cap e^{\epsilon},d_G)$  for any $R \in \mathcal{R}_i$, where $1 \leq i \leq j$ for some $j$. Let $R \in \mathcal{R}_{j+1}$ be an arbitrary tree in the collection. Let us choose an arbitrary vertex $v \in \mathbb{V}(R)$ which has at least degree $2$ in graph $R$. This is possible in every tree having at least $3$ vertices i.e. for any set $\mathcal{R}_i$, where $i \geq 2$.  Let  $(\mathcal{T}(R,v) ;  p_v)$ be the star-cover defined in Lemma \ref{lem:nonadjacentedgesgraph}. We note first that every $A_t \in \mathcal{T}(R,v)$ is exactly set $D \cap R^{\epsilon}_{t}$ for some $R_{t}\in \mathcal{R}_{q(t)}$. We will now prove that $q(t) \leq j$ for all $t$. We note first that $\mathcal{T}(R,v)$ has at least 2 elements , because $v$ have degree at least 2. From the definition of $\mathcal{T}(R,v)$ we obtain that
% $$\mathbb{E}(R) = \cup_{t \in |\mathcal{T}(R,v)|}\mathbb{E}(R_t) $$
% Lets assume that $|\mathbb{E}(A_r) | \geq j+1$ for some $r$. Then because $|\mathcal{T}(R,v)| \geq 2$ it follows that $|\mathbb{E}(R)| \geq j+2$. which is a contradiction. Thus  $|\mathbb{E}(A_r)| \leq j$ for all $A_r \in \mathcal{T}(R,v)$. By using induction assumption on every $A_r$ together with Lemma  \ref{lem:MSTGlue} we deduct:
% $$\bigcup_{e \in \mathbb{E}(R)} \MST(e^{\epsilon} \cap D, d_G) = \bigcup_{A_r \in \mathcal{T}(R,v)}\MST(D \cap A^{\epsilon}_r, d_G) = \MST(D \cap R^{\epsilon}, d_G) $$
% which concludes the induction step. 
%% $$  \MST(D \cap e^{\epsilon},d_G) $$
%
%%We will prove that the claim holds for $j+1$. Assume that $e_{j+1} = (v_{j+1}, w)$ for some $w$. 
%
%%Following from Lemma \ref{lem:nonadjacentedgesgraph} we can decompose $D \cap R_j^{\epsilon}$ space into parts, each of which corresponds to an $\epsilon$-offset of a connected component when point $u$ is removed from $R_{j+1}$. It thus follows that  $(\{R_j, [u,y]\},p_u) $ is a star-cover of $R_{j+1}$. Using Lemma \ref{lem:MSTGlue} we obtain that $\MST(R^{\epsilon}_k \cap D,d_G) \cup \MST(w^{\epsilon} \cap D,d_G) $ is minimum spanning tree of $R_{j+1}$. Using induction assumption on $j$ we obtain
%
% %we obtain that $\cup_{e \in }\MST(D \cap R^{\epsilon}_j  ) \cup \MST(e^\epsilon \cap D)$ is a minimum spanning tree on set 
%%$R_{j+1}$. The claim follows from this , as we know that
% %$$\MST(R^{\epsilon}_j,d_G) \cup \MST(w^\epsilon \cap D,d_G) = \bigcup_{e \in \mathbb{E}(R_{j+1})}\MST(e^{\epsilon} \cap D,d_G).$$
%
%%Thus $R_{k+1}$ is spanned by all the edges having adjacent indices in sets $D_q$, where $q$ is edge added in $R_i$ for some index $i \leq k+1$ . Thus we have proved that the Lemma holds for whole graph.
%
%%Thus claim holds for all values $t$ of the filtration, especially $R_{t}$ , which proves the claim. 
%
%
%
%\end{proof}

%\begin{lem}[Combining graph homeomorphisms]
%\label{lem:GraphHomeomorphism}
%Let $G$ and $H$ be graphs and let $G_i$ and $H_i$ be their finite graph-covers that i.e. $\cup_{i}G_i = G$ and $\cup_iH_i = H$ . Assume that every $G_i$ is homeomorphic to $H_i$ i.e. for every $i$ there exists a subdivision $G'_i$ of $G_i$ and $H'_i$ of $H_i$, for which there exists an isomorphism $f_i:G_i' \rightarrow H_i'$. Assume that for all $i \neq j$ and all $x \in \mathbb{V}(G')_i \cap \mathbb{V}(H')_i$ it follows that $f_i(x) = f_j(x)$. Then $G$ is homeomorphic to $H$.
%\end{lem}
%\begin{proof}


%\end{proof}

%\begin{cor}[Intersection of edge-sets contains at most a single point]
%\label{cor:IntersectionEdgesets}
%Assume the conditions of Theorem \ref{thmm:GHT}. Let $e,h$ be arbitrary edges, then: 
%
%\[ \begin{cases} 
%      (e^{\epsilon} \cap D) \cap (h^{\epsilon} \cap D) = \emptyset & \text{if edges } e \text{ and } h \text{are non-adjacent in }T \\
%      (e^{\epsilon} \cap D) \cap (h^{\epsilon} \cap D) = \{v\} & \text{if edges } e \text{ and } h \text{are adjacent in }T \\
%  
%   \end{cases}
%\]
%
%%$(e^{\epsilon} \cap D) \cap (h^{\epsilon} \cap D) = \emptyset$
%\end{cor}
%\begin{proof}
%Assume first that $e$ and $h$ are non adjacent. Make counter assumptions that there exists
% $ p \in (D \cap e^{\epsilon}) \cap (D \cap h^{\epsilon})$. Then $d(e,h) \leq d(e,p) + d(p,h) \leq 2\epsilon$, which is a contradiction, because $G$ was $\gamma$ approximation of $(T,C)$ (Definition \ref{dfn:GammaApproximation})
%
%Assume then that $e$ and $h$ are adjacent over some vertex $v$ in graph $T$. Then $(D \cap h^{\epsilon})$ and $(D \cap e^{\epsilon})$ are completely contained in different cover elements of $\mathcal{T}( T , v )$. 
%%Then for any $p \in e^{\epsilon} \cap D  \in h^{\epsilon} \cap D$
%
%\end{proof}

%construct a map from some subdivision of $T$ into $\MST(D, d_G)$. 
%Proving Theorem \ref{thmm:GHT} is now easy. We simply need to subdivide the graph $T$ into some graph $T'$ and construct an isomorphism $f: T' \rightarrow \MST(D, d_G) $. The Theorem \ref{thmm:GHT} was first presented in Section \ref{sec:intro}. For convenience we restate it below:


%\begin{proof}[\textbf{Proof of theorem \ref{thmm:GHT}:}]
%From Proposition \ref{lem:somstod} we obtain $\MST(D, d_{G}) = \bigcup_{e \in \mathbb{E}(T)} \MST(e^{\epsilon} \cap D, d_G)$. From proposition \ref{lem:eht} states that every $e \in \mathbb{E}(T)$ is homeomorphic to $ \MST(e^{\epsilon}  \cap D, d_G)$, in such a way that there exists a subdivision $e'$ of $e = (u,v)$ and a map $f_e: e' \rightarrow \MST(e^{\epsilon})$ for which  $f_e(u) = p_u$ and $f_e(v) = p_v$. Let us define tree $T'$ as the union of subdivided edges 
%$ \bigcup_{e \in \mathbb{E}(T)} e'$ and the homeomorphism $f:T' \rightarrow \MST(D, d_G)$ satisfying $f | e = f_e$ for all $e \in \mathbb{E}(T)$.
%%as $f = \bigcup_{e \in \mathbb{E}(T)}f_e$. 
%
%The map $f$ is well-defined: Let $e, w$ be distinct edges of $\mathbb{E}(T)$. They intersect at most at one vertex $v$. In this case both of the maps $f_e$ and $f_w$ map $v$ into $p_v$.
%
%Every edge in $\mathbb{E}(T')$ is mapped under $f$ into $\mathbb{E}(\MST(e^{\epsilon}))$ : This follows directly from the fact that every edge $e \in \mathbb{E}(T')$ is completely contained in one of the sets $\mathbb{E}(e')$. Thus the claim follows directly from a property of the map $f_e$. 
%
%Because every map in the union is an isomorphism it follows that the map $f$ is an isomorphism.  Thus we have found a map  $f: T' \rightarrow \MST(D, d_G) $ which is a graph isomorphism. Hence the graph $T$ is homeomorphic to $\MST(D, d_G)$. 
%
%
%\end{proof}


\begin{lem}
\label{lem:homeomorphismGluingLemma}
Let $(X,d_X)$ and $(Y,d_Y)$ be metric spaces. Let $\{U_i \mid i \in J\}$ and $\{V_i \mid i \in J\}$ be closed sets and finite covers of the spaces $(X,d_X)$ and $(Y,d_Y)$ respectively. Assume that there exists homeomorphisms $f_i: U_i \rightarrow V_i $ that agree on the all pairwise intersections.
 Assume that that the inverse maps $f^{-1}_i: V_i \rightarrow U_i$ also agree on the all pairwise intersections. Then $f:X \rightarrow Y$ defined by $f | U_i = f_i$ is homeomorphism between spaces $X$ and $Y$. 
\end{lem}
\begin{proof}
%
%Thus we can build topological homeomorphisms $f_e: e \rightarrow \MST(e^{\epsilon} \cap D, d_G)$ for which $f_e(u) = p_u$ and $f_e(v) = p_v$ and 
%$g_e:  \MST(e^{\epsilon} \cap D, d_G) \rightarrow e$ for which $g_e(p_u) = u$ and $g_e(p_v) = u$, for which $f \circ g = \text{id}$ and 
%$g \circ f = \text{id} $. Let us define maps $f: T \rightarrow \MST(D, d_G)$ and $g: \MST(D, d_G) \rightarrow T$ as maps satisfying $f | e = f_e$ and $g | e = g_e$. 


\textbf{Maps $f, f^{-1}$ are well-defined:} Follows directly from the fact that both $f, f^{-1}$ on all the pairwise intersection of $f_i$ and $f_i^{-1}$.

\textbf{Both maps $f, f_{-1}$ are bijections:} If $x \in X$. Then $x \in U_i$ for some $i \in J$. It follows that
$f^{-1} \circ f(x) = f_i^{-1} \circ f_i(x) = x $ . Similarly if $y \in Y$. Then $y \in V_i $ for some $i \in J$. It follows that
 $ \circ f^{-1}(y) = f_i \circ f^{-1}_i(y) = y $.

\textbf{Both maps $f, f_{-1}$ are continious:} Because all the sets $U_i$ and $V_i$ are closed it follows from the pasting lemma that both $f$ and $f^{-1}$ are continuous. 
%
%Because maps $f$ and $g$ are continuous and inverse-function of each other, it follows that $\MST(D,d_G)$
% is homeomoprhic to the tree $T$.
\end{proof}

\MainThm*
\begin{proof}[\textbf{Proof of theorem \ref{thmm:GHT}:}]

 We will apply Lemma \ref{lem:homeomorphismGluingLemma} by setting $X = T$ , $Y = \MST(D, d_G)$, 
$U_e = e$ and $V_e = \MST(e_i^{\epsilon} \cap D, d_G)$ where $e$ goes through all the edges $\mathbb{E}(T)$. 
Proposition states that for every edge $e = (u,v)$ graph $ \MST(e^{\epsilon} \cap D, d_G)$ is a polygonal path from $p_u$ to $p_v$. It follows that for all $e \in \mathbb{E}(T)$ is homeomorphic to $ \MST(e^{\epsilon} \cap D, d_G)$, in such a way that there exists a family of maps 
$f_e: e \rightarrow \MST(e^{\epsilon} \cap D, d_G)$ mapping $f_e(u) = p_u$ and $f_e(v) = p_v$. For any two edges $e,h \in \mathbb{E}(T) $, if $e \cap h \neq \emptyset$, then $e$ and $h$  are adjacent via some vertex $v$, by the definition of maps $f_e, f_h$ we obtain $f_e(v) = p_v = f_h(v)$.
Similarly for map $f^{-1}$ we inherit from Proposition \ref{lem:nonadjacentedgesgraph} the intersection of $e^{\epsilon} \cap D$ and 
$h^{\epsilon} \cap D$ for any two $e,h \in \mathbb{E}(T)$ is non-empty if $e$ and $h$ are adjacent via some vertex $v$ and in this case
$e^{\epsilon} \cap h^{\epsilon} \cap D = \{p_v\}$. It follows that $f^{-1}_e(p_v) = v = f^{-1}_h(p_v)$. We note that line-segments $e$ are compact sets for all $e \in \mathbb{E}(T)$. It follows that $\MST(e^{\epsilon} \cap D, d_G)$ are compact as well. Thus they are both closed in spaces $T$ and $\MST(D, d_G)$ respectively. Now all the conditions of Lemma \ref{lem:homeomorphismGluingLemma} are satisfied and it follows that
$T$ is homeomorphic to $\MST(D,d_G)$.


%
%From Proposition \ref{lem:somstod} we obtain $\MST(D, d_{G}) = \bigcup_{e \in \mathbb{E}(T)} \MST(e^{\epsilon} \cap D, d_G)$. Proposition states that for every edge $e = (u,v)$ graph $ \MST(e^{\epsilon} \cap D, d_G)$ is a polygonal path from $p_u$ to $p_v$. It follows that for all $e \in \mathbb{E}(T)$ is homeomorphic to $ \MST(e^{\epsilon} \cap D, d_G)$, in such a way that there exists a family of maps 
%$f_e: e \rightarrow \MST(e^{\epsilon} \cap D, d_G)$ mapping $f_e(u) = p_u$ and $f_e(v) = p_v$.


% Because all the line-segments $e$ are compact, then $\MST(e^{\epsilon} \cap D, d_G)$ are closed sets in $\MST(D,d_G)$. We note that the collection $\mathbb{E}(T)$ treated as collection of line-segments in $\R^m$ does indeed cover $T$. We can apply Lemma \ref{lem:homeomorphismGluingLemma} by setting $X = T$ , $Y = \MST(D, d_G)$, 
%$U_i = e_i$ and $V_i = \MST(e_i^{\epsilon} \cap D, d_G)$ where $i \in J$ goes through all the edges $\mathbb{E}(T)$. Because all the condition of Lemma \ref{lem:homeomorphismGluingLemma} are satisfied we obtain that $T$ is homeomorphic to $\MST(D,d_G)$.  

\end{proof}



\subsection{Star-cover of vertices and edges }
\label{sec:TechnicalSection}

The main purpose of this section is to provide necessary results to prove  Proposition \ref{lem:nonadjacentedgesgraph} and Lemma \ref{lem:edge-offset}, that will be done in the of this section. 
%In this section we handle the technical side of the main theoretical result. 
% which have angle $\theta$ between them and a common vertex $v$. 


\begin{lem}
\label{lem:AdjacentEdgesLemma}
Assume the conditions of Theorem \ref{thmm:GHT}.
Let $e$ and $h$ be adjacent edges of the graph $T$ via vertex $v$. Denote by $\theta$ be the angle between the edges $e$ and $h$ and let $r \in \R_{+}$ be a positive real number. Let us fix real number $r \in \mathbb{R}$ and let $q \in e^{\epsilon}$ be an arbitrary point for which there exists $t \in h^{\epsilon}$ having $d(q,t) < r$. Then the following inequality is satisfied:
$$d(q, v) \leq  \dfrac{\epsilon}{\sin(\frac{\theta}{2})} +  \dfrac{r}{\sin(\min(\theta, \frac{\pi}{2}))} $$ 




%$$\mathcal{A}(e,h,r) = \{q \in e^{\epsilon} \mid \text{ there exists } t \in h^{\epsilon} \text{ for which } d(q, t) < r\}. $$
% Then for any point $q \in \mathcal{A}(e,h,r)$ the following inequality is satisfied:

%\begin{align*}
%\centering
%    d(q, v) \leq \begin{cases}
%              \frac{\epsilon}{\sin(\frac{\theta}{2})} +  \frac{r}{\sin(\theta)}  & \text{if } \theta < \frac{\pi}{2},\\
%             \frac{\epsilon}{\sin(\frac{\theta}{2})} +  r & \text{if } \theta \geq \frac{\pi}{2}
%          \end{cases}
%\end{align*}

\end{lem}
\begin{proof}

\begin{figure}
    \centering
    \begin{tikzpicture}
  \draw
    (8,-3) coordinate (a) node[right] {}
    -- (0,0) coordinate (v) node[left] {v}
    -- (8,3) coordinate (c) node[above right] {}
    pic["$\theta$", draw=orange, <->, angle eccentricity=1.2, angle radius=1cm]
    {angle=a--v--c};
    \draw[dashed]
    (8,-1.5) coordinate (a2) node[right] {}
    -- (4,0) coordinate (v2) node[above] {w}
    -- (8,1.5) coordinate (c2) node[above right] {}
    pic["$\theta$", draw=orange, <->, angle eccentricity=1.2, angle radius=1cm]
    {angle=a2--v2--c2};
    \draw[loosely dashed] (v) -- node[below] {} node[above] {} ++ (v2);
    \filldraw[black] (4,0) circle (2pt);
    \filldraw[black] (0,0) circle (2pt);

    \filldraw[black] (3.5,-1.3) circle (2pt) coordinate (cc) node[anchor = north ]{c};
    \draw[loosely dashed] (v2) -- (cc);
    \draw(3.5,-0.6) coordinate (uv) node{$\epsilon$}; 
   % \tkzMarkRightAngle[size=.2](v,cc,v2);
    \filldraw[black] (8,-1.5) circle (2pt) coordinate (q) node[anchor = west]{q};
    \filldraw[black] (6.8,1.05) circle (2pt) coordinate (t) node[anchor = west]{t};
    \draw[loosely dashed] (q) -- (t);
   % \tkzMarkRightAngle[size=.2](q,t,v2);
    
    \draw(2.5, -1.25) coordinate (ne) node{$e$};
    \draw(2.5, 1.25) coordinate (nh) node{$h$};

    
    
\end{tikzpicture}
    \caption{Proof of Lemma \ref{lem:AdjacentEdgesLemma}. In this picture we have illustrated the special case when $q$ is on the boundary of the set $e^\epsilon$}
    \label{fig:Lemma12}
\end{figure}

We will first consider the case where $\theta \leq \frac{\pi}{2}$. Let $l$ be a line that goes through the point $q$ and is parallel to $e$. Let $w$ be the closest point to $q$ of the intersection $l \cap h^{\epsilon}$. Let $t \in h^{\epsilon}$ be a point which is closest to $q$. As illustrated in Figure \ref{fig:Lemma12} $\triangle wtq$ is a right triangle. By using the definition of sine $$d(w,q) = \dfrac{d(q,t)}{\sin(\theta)} \leq \dfrac{r}{\sin(\theta)}. $$ Let $c \in e$ be the point that is closest to $w$. We note now that $\triangle vcw$ is also a right-angled  triangle. Again using the sine theorem and the facts that $\angle wvc \leq \frac{\theta}{2}$ and $d(w,c) \leq  \epsilon$ we obtain 
$$d(v,w) = \frac{d(w,c)}{\sin(\angle wvc)} \leq   \frac{\epsilon}{\sin(\frac{\theta}{2})}. $$
Combining the previous two inequalities with the triangle inequality we obtain
$$d(v,q) \leq d(v,w) + d(w,q) \leq \frac{\epsilon}{\sin(\frac{\theta}{2})} +  \frac{r}{\sin(\theta)}. $$
In the case angle $\theta \geq \frac{\pi}{2}$ the intersection point $t$ is located on the other side of $w$ in line which is parallel to $h$. Thus $\triangle wqt$ forms a right-angled triangle again, where $qt$ is the longest side. Thus we can simply estimate $d(q,w) \leq d(q,t) \leq r$ and obtain the inequality $$ d(q, v) \leq \dfrac{\epsilon}{\sin(\frac{\theta}{2})} +  r  $$
which proves this lemma. 



\end{proof}

%It should be noted that if in Lemma \ref{AdjacentEdgesLemma} $r  = \delta$ then we can state 
%$$\dfrac{\epsilon}{\sin(\frac{\theta}{2})} +  \dfrac{r}{\sin(\min(\theta, \frac{\pi}{2}))} = \frac{\delta}{2\gamma} - \epsilon$$ 
%\begin{remark}
%$ \frac{\delta}{2\gamma} - \epsilon $
%\end{remark}


\begin{lem}
\label{lem:structureofpaths}
Assume the conditions of Theorem \ref{thmm:GHT}. Let $(a,b)$ be arbitrary edge in graph $G$. Let edges $e,h \in \mathbb{E}(T)$ be such that  $a \in  e^\epsilon$ and $b \in h^\epsilon $. Then either $e = h $ or $e$ and $h$ are adjacent in the tree $T$ .
%Assume that $a \in D \cap e^\epsilon$ and $b \in D \cap h^\epsilon $. Then either $e = h$, or $e$ and $h$ share a common vertex in the tree $T$. 
\end{lem}
\begin{proof}
Make the counter assumption that $e$ and $h$ are distinct, non-adjacent edges. By assumption of Theorem \ref{thmm:GHT} graph $G$ is $\gamma$-approximation (Defined in Definition \ref{dfn:GammaApproximation} of $(T,C)$. Thus the following inequality is satisfied: $l_{\max}(G) < r - 2\epsilon $ , where $r$ is the minimal length of non-adjacent edges. Using the triangle inequality we obtain:
 $$d(a,b) \geq d(e,h) - d(a,e) - d(b,h) \geq r - 2 \epsilon>  l_{\max}(G).$$
Which is a contradiction (Recall that $d(a,b) \leq e_{\max}(G)$ for all $a,b \in \mathbb{V}(G)$). It follows that either $e = h$ or $e$ and $h$ are adjacent edges.  
\end{proof}



%\begin{dfn}
%\label{shortestPathConnecting}
%Let $s$ be the shortest path connecting points $a,b$ in the graph $G$. Assume that $a \in D \cap e^\epsilon$ and $b \in D \cap h^{\epsilon}$ for $e \neq h$. We define the path $L(s)$ in the graph $T$ as the shortest path connecting the edges $e$ and $h$.  
%\end{dfn}

% dfn:starDecompose


%\begin{lem}[Existence of vertex-link]
%\label{ExistenceOfVertexLink}
%Let $s$ be the shortest path connecting points $a,b$ in the graph $G$. Assume that $a \in D \cap e^\epsilon$ and $b \in D \cap h^{\epsilon}$ for $e \neq h$ and let $v$ be an arbitrary vertex in $L(s)$. Then there exists an index $i$ and edges $e',h'$ that have a common vertex $v$ and which satisfy $s(i) \in C \cap e^\epsilon$ and $s(i+1) \in C \cap h'$.
%%for which there exists edges $e'$ and $h'$ which have a common vertex $v$ and for which $s(i) \in \overline{D}_{e'}$ and  $s(i+1) \in \overline{D}_{h'}$. 
%\end{lem}

\begin{lem}
\label{lem:ExistenceOfRoutePoint}
Assume the conditions of Theorem \ref{thmm:GHT}. Let $e \in \mathbb{E}(T)$  be an arbitrary edge. Assume that the graph $T \setminus \{e\}$ (We remove edge $e$ from the tree $T$)  consists of two connected components $C_1, C_2$. Then for any points $a,b \in C$ satisfying
$a \in C^{\epsilon}_1$ and $b \in C^{\epsilon}_2$ and a shortest path $s$ connecting them, there exists and a point $p \in C$, for which 
$p \in s \cap e^{\epsilon} $.
%
%
%Let $a,b$ be arbitrary points in $C$ and let $e$ be an edge of the tree $T$ and let $s$ be a s shortest path connecting $a$ to $b$ in the graph $G$. If the graph $T \setminus \{e\}$ (We remove edge $e$ from the tree $T$)  consists of two connected components $C_1, C_2$ in such a way that $ a \in C^{\epsilon}_1$ and 
%$b \in C^{\epsilon}_2$, then there exists a point $p$ in path $s$ for which $p \in e^{\epsilon}$. 

\end{lem}
\begin{proof}
Let path $s = (s_i)$ be a shortest path between $a$ and $b$, where $s_0 = a$ and $s_k = b$. 
Make counter assumption that there does not exist a point $p$ of path $s$ for which $p \in e^{\epsilon}$. We will first prove that any consecutive points $s_i,s_{i+1}$ of the path $s$ belong both to either $C^{\epsilon}_1$ or $C^{\epsilon}_2$. Make counter assumption, that  $s_i \in C^{\epsilon}_1$ and $s_{i+1} \in C^{\epsilon}_2$. Using Lemma \ref{lem:structureofpaths} we obtain that that points $s_i,s_{i+1}$ has to belong to edge-sets $s_i \in D \cap \alpha^{\epsilon}$ and $s_{i+1 }\in D \cap \beta^{\epsilon}$, where $\alpha$ and $\beta$ are adjacent edges. However, this is a contradiction, because graph components $C_1, C_2$ do not have common vertices. Thus every edge $(s_i, s_{i+1}) \in s$ belongs to either $C^{\epsilon}_1$ or $C^{\epsilon}_2$. We will now prove that for all $i$ all the points $s_i$ belong to the same component $C^{\epsilon}_1$ or $C^{\epsilon}_2$. By symmetry assume that $s_0 \in C^{\epsilon}_1 $. Let $j$ be the smallest index for which $s_j \in C^{\epsilon}_2$. Now $s_{j-1} \in C^{\epsilon}_1$ for some $j-1 \geq 0$. It follows that points
$s_{j-1},s_j$ belong to distinct component sets $C^{\epsilon}_1$ and $C^{\epsilon}_2$, which is a contradiction. Without loss of generality we assume that $s_i \in C^{\epsilon}_1$ for all $i \in \{0,...,k\}$. However, this is a contradiction, because we have assumed that $s_k = b \in C_2$. It follows that there exists a point $p \in C$ satisfying $p \in s \cap e^{\epsilon} $.


% By symmetry we can assume that $s$ is contained in $C^{\epsilon}_1$. However, this is a contradiction, because end points $a, b$ belong to distinct sets 
%$ C^{\epsilon}_1$ and $ C^{\epsilon}_2$. It follows that there exists point $p$ in path $s$ satisfying $ p \in e^{\epsilon}$.

%Using Lemma \ref{structureofpaths} we obtain that any edge $(x,y) \in s$
%
% for all It follows that the path $s$ has to be contained in $C^{\epsilon}_r$, which is a contradiction because points $a$ and $b$ belong to distinct connected components. Thus it follows that there exists an index $j$ for which $s(j) \in e$. 
\end{proof}

%\begin{lem}[Existence of vertex-link]
%\label{ExistenceOfVertexLink}
%Assume the conditions of Theorem \ref{thmm:GHT}. Let $a,b$ be arbitrary points of $C$ belonging to offsets of distinct edges
%$a \in e^{\epsilon} \cap D $ and $ b \in h^{\epsilon} \cap D$. Let $v$ be an arbitrary vertex in $T$, which can be found in the shortest path connecting edges $e$ to $h$ in tree $T$. Let $s$ be the shortest path connecting $a$ to $b$ in graph $G$. Then there exists two distinct edges $f,g \in \mathbb{E}(T)$ having $f \cap g = \{v\}$ and an edge $(x,y) \in s$, in such a way that $x \in f^{\epsilon}$ and $y \in g^{\epsilon}$.
%
%\end{lem}



\begin{lem}[Every path in the graph $G$ stays close to corresponding vertices in the tree $T$]
\label{ExistenceOfVertexLink}
Assume the conditions of Theorem \ref{thmm:GHT}. Let $v \in \mathbb{V}(T)$ be an arbitrary vertex in $T$. Let $a,b$ be arbitrary points for which 
there does not exist $e \in \mathbb{E}(T)$ for which $\{a,b\} \subseteq e^{\epsilon} \cap D $. Let $s$ be a shortest path between $a$ and $b$ in the graph $G$. Then there exists a vertex $v \in \mathbb{V}(T)$ and a point $q \in s$ for which $d_G(q,p_v) \leq \frac{\delta}{2}$
 
% Let $a,b$ be arbitrary points of $C$ belonging to offsets of distinct edges
%$a \in e^{\epsilon} \cap D $ and $ b \in h^{\epsilon} \cap D$. Let $v$ be an arbitrary vertex in $T$, which can be found in the shortest path connecting edges $e$ to $h$ in tree $T$. Let $s$ be the shortest path connecting $a$ to $b$ in graph $G$. Then there exists two distinct edges $f,g \in \mathbb{E}(T)$ having $f \cap g = \{v\}$ and an edge $(x,y) \in s$, in such a way that $x \in f^{\epsilon}$ and $y \in g^{\epsilon}$.

\end{lem}


%Let $v$ be an arbitrary vertex of graph $T$. Let $a,b$ be arbitrary points belonging to different elements $ $ of the tree-cover defined in Lemma \ref{lem:nonadjacentedgesgraph}. Let $s$ be the shortest path between $a$ and $b$ in graph $G$. Then there exists two edges $e,h$ having $v$ as one of their end points and an index $i \in \Z$ for which $s(i) \in D \cap e^{\epsilon} $ and 
%$s(i+1) \in D \cap h^{\epsilon}$. 
%\end{lem}

\begin{proof}

Let $(u,v)$ be arbitrary edge satisfying $a \in (u,v)^{\epsilon} \cap D$ . Let $C$ be a component of $T \setminus \{(u,v)\}$ containing point $b$. We note that either $u$ or $v$ belong to the component $C$. Without loss of generality we assume that $v \in C$. Let $s = (s_i)$ be a shortest path connecting $a$ to $b$ in graph $G$, in such a way that $s_0 = a$ and $s_k = b$.  We will now show that there exists a point $q \in s$ which satisfies $d(q, p_v) \leq \frac{\delta}{2}$



%
%Assume that $a \in A \in \mathcal{Q}$
%and $b \in B \in \mathcal{Q}$. Let edge $e \in \mathbb{E}(T)$ be the edge satisfying $e^{\epsilon} \cap A \neq \emptyset$ and $e = (u,v)$ for some vertex $u \in \mathbb{V}(T)$.
%We will now prove that there exists index $j$ for which $s_j \in e^{\epsilon}$. We note that $T \cap e$ splits the tree into two components $C_1,C_2$ in such a way that 
%$a \in C^{\epsilon}_1$ and $b \in C^{\epsilon}_2$. Thus we can apply Lemma \ref{lem:ExistenceOfRoutePoint} to show that there exists a point $x \in s$ for which $x \in e^{\epsilon}$. Thus there indeed exists an index $j$ satisfying $s_j \in e^{\epsilon}$.

Let $t$ be the maximal index for which $s_t \in e^{\epsilon}$. From Lemma \ref{lem:structureofpaths} it follows that $s_{t+1} \in h^{\epsilon}$ for some edge $h \in \mathbb{E}(T)$ for which $v \in h$ or $u \in h$. We note that $e \neq h$, because $k$ was the largest index for which $s_t \in e^{\epsilon}$. Let us assume first that $u \in h$. Then we note that  $T \setminus \{e\}$ splits the graph $T$ into two components $C_1, C_2$, in such a way that $s_{t+1} \in C^{\epsilon}_1$ and $b \in C^{\epsilon}_2$. By using Lemma \ref{lem:ExistenceOfRoutePoint} we can deduct again that the restriction of path $s$ to the subpath connecting $s_{t+1}$ to $b$ has to contain some point $q' \in e^{\epsilon}$. This is a contradiction, because $q' = s_{y}$ for some $y > j+1$. Which is a contradiction. Thus it follows that $v \in h$. We note that $e,h$ are adjacent edges of the graph $T$ via vertex $v$. We note that $d(s_{t}, s_{t+1}) < l_{\max}(T)$. Thus using Lemma \ref{lem:AdjacentEdgesLemma} we can deduct that 
$$d(s_t, v) \leq  \dfrac{\epsilon}{\sin(\frac{\theta}{2})} +  \dfrac{l_{\max}(G)}{\sin(\min(\theta, \frac{\pi}{2}))} $$ 
We recall that Equation \ref{eqa:GHT} states the following: 
$$\delta \geq  2\gamma(\epsilon +\dfrac{\epsilon}{\sin(\frac{\theta(T)}{2})} + \dfrac{l_{\max}(G)}{\sin(\min(\theta(T), \frac{\pi}{2}))}) $$ 
By combining the two inequalities above we obtain:
$$d(s_t, v) \leq  \frac{\delta}{2\gamma} - \epsilon $$
Now the claim follows for $q = s_k$ from the following triangle-inequality 
$$d_G(p_v, s_t) \leq d_G(v,s_t) + d_G(p_v,v) \leq  \gamma(d(v,s_t) + d(p_v,v)) \leq \gamma( \frac{\delta}{2\gamma} - \epsilon + \epsilon) \leq  \frac{\delta}{2} $$


\end{proof}

%\begin{proof}
%
%Let $s'$ be the shortest path connecting edge $e$ to $h$ in tree $T$. Let us denote the first edge of $s$ having $v$ as one of their end points by $f$. If $e = f$ then $x \in s \cap f^{\epsilon}$ . In case $e \neq f$ , then we can use Lemma \ref{lem:ExistenceOfRoutePoint}
%to deduct $s \cap f^{\epsilon} \neq \emptyset$. Let us denote the last point of the path $s$, which belongs to $f^{\epsilon}$ by $p$. Let $q$ be the next point after $p$ in the path $s$.
%
%Let $w$ be the second end point of $f$ (i.e. $f = (v,w)$). Following from Lemma \ref{lem:structureofpaths} $q \in z^{\epsilon} \cap D$ for some edge $z \in \mathbb{E}(T)$ for which $v \in z$ or $w \in z$. Because $q$ was chosen to be the next point after $p$, which was the last point of $s$ contained in $f^{\epsilon}$ it follows that $z \neq f$. Assume now that $w \in z$. Then graph $T \setminus \{f\}$ consists of two components, where points $q$ and $b$ belong to different components. By using Lemma \ref{lem:ExistenceOfRoutePoint} we can deduct again that the shortest path connecting $q$ to $b$ has to contain some point $q' \in f^{\epsilon}$. This is a contradiction, because $q'$ occurs after $p$ in path $s$ and $p$ was chosen to be the last point that belongs to $f^{\epsilon}$.
%
%It follows that $v \in z$. Now $f, z$ are edges that have a common vertex $v$ that contain edge $(p,q)$ in such a way that 
%$p \in f^{\epsilon}$ and $q \in z^{\epsilon}$, which proves the claim.
%
%\end{proof}
%


%Let $ p \in D$ be the last point of path $s$ 

%Let $e$ be an edge belonging to the cover element $A$, for which $v$ is one of their end point. We note first, because $a,b$ belong to different components of 
%$T \setminus \{e\} $ we can use Lemma \ref{lem:ExistenceOfRoutePoint} to find index $j$ for which $s(j) \in e$.

%Make the counter assumption that there doesn't exist such index $i$. Let $x,y$ be the two edges which are present in the path $l$ connecting the edges $e$ and $h$ in the straight-line tree $T$ having $v$ as their common vertex. We will first prove that there exist indices $j,k$ for which 
%$s(j) \in C \cap x$ and $s(k) \in C \cap y$. We will prove this claim only for $x$. The proof for the edge $y$ is symmetric. 

%First of all we note that graph $T \setminus \{e\}$ consists of two connected components $C_1$ and $C_2$ i.e. every pair of edges belonging to $C_1 \times C_2$ is non-adjacent. 

 
%
%we obtain that path $s$ stays in edge-sets $C_f$ having either $f \in C_1$ or $f \in C_2$ for all $f \in \mathbb{E}(T)$. However this is a contradiction, because $a,b$ belong to edge-sets of different components. 
%
%Without loss of generality we can assume that $j \leq k$. If $j + 1 = k$ we are done with the proof. Assume that $j + 1 \neq k$. 
%Let $j'$ be the largest index satisfying $s(j') \in D \cap e^{\epsilon}$.  Assume that $e = (v,u)$ for some vertex $u$ of $T$. Following from Lemma \ref{structureofpaths} and the maximality of $j'$ we deduct that $s(j'+1)$ belongs to some $ D \cap h^{\epsilon}$, where $h$ has either $v$ or $u$ as one of its end points. In case $h$ has $v$ one of its end points we are done with the proof. 
% 
%  Using Lemma  \ref{structureofpaths} we know that $s(j'+1)$ should belong to either the edge-set of the edge having common vertex $v$ with $x$ or an edge-set of the other vertex $u$ of the edge $x$. If it belongs to another edge-set of the vertex $v$, then the proof is complete, as we can select indices $j',j'+1$ which satisfy the assumption.
%
%Assume now that $h$ has $u$ as one of its end points. We note that $s(j'+1)$ and $s(k)$ belong to different components of $T \setminus \{h\}$. Thus from 
%Lemma \ref{lem:ExistenceOfRoutePoint} we can find index $t > j'+1$ for which $s(t) \in h^{\epsilon} \cap D$. This is contradiction, because $t > j'$ and $j'$ was chosen to be maximal element satisfying $s(j') \in h$.

% Assume first that for every index $i$ the following holds true: $s(i) \notin \overline{D}_e $ for all the edges $e$ having $v$ as one of their vertex. By removing $v$ 



\spov*


\begin{proof}

We will first show that $(\mathcal{V}, \mathcal{E})$ is a graph-cover of $(D,d_G)$. Let $e^\epsilon \cap D$ and $h^{\epsilon} \cap D$ be distinct cover elements of tree-cover for some $e,h \in \mathbb{E}(T)$.  If $e^{\epsilon} \cap h^{\epsilon} \neq \emptyset$ then $e$ and $h$ are adjacent edges in the tree $T$. Let $v$ be the common vertex of edges $e$ and $h$, then $p_v \in e^{\epsilon} \cap h^{\epsilon} \cap D$. We will now show that there are no other points in this intersection. Let $q \in e^{\epsilon} \cap h^{\epsilon} \cap D $ be a point for which $q \neq p_v$. We can apply Lemma \ref{lem:AdjacentEdgesLemma} using $r = 0$ to obtain $d(q, v) \leq \frac{\epsilon}{\sin(\frac{\theta(T)}{2} )} $.
We can now use triangle inequality to deduct:
$$\delta < d(q,p_v) \leq d(q,v) + d(v,p_v) \leq \epsilon + \frac{\epsilon}{\sin(\frac{\theta(T)}{2})} $$
However this is a contradiction, because $\delta$ defined in Equation \ref{eqa:GHT} is clearly larger than the right-most expression. We have now proved that $e^{\epsilon} \cap h^{\epsilon} = \{p_v\}$, where $v$ is the common vertex of $e$ and $h$. Let us now prove the second condition of graph-cover definition \ref{dfn:multiStarCover}.

Let $e \in T$ be an arbitrary edge having end points $u$ and $v$. Clearly $p_u \in e^{\epsilon} \cap D$  and $p_v \in e^{\epsilon} \cap D$. Let $q \in \mathbb{V}(T)$ be some vertex for which $q \neq v$ and $q \neq u$. Now $p_u$ is part of some non-adjacent edge $h$. Again from the fact that $G$ is $\gamma$-approximation of $(T,C)$ we obtain that $d(p_u, e) > \epsilon$. Thus $p_u$ can't be included into $D \cap e^{\epsilon}$. It follows that $D \cap e^{\epsilon} \cap \mathcal{V} = \{p_u, p_v\}$. We have to prove now that $\mathcal{N}(\mathcal{V}, \mathcal{E})$ is a tree. This will be done by proving that $\mathcal{N}(\mathcal{V}, \mathcal{E})$ is isomorphic to $T$. 

Let us define the map $f: T \rightarrow \mathcal{N}(\mathcal{V},\mathcal{E})$ which satisfies $f(v) = p_v$. This map is clearly an isomorphism. We have to prove now that if 
$(u,v)$ is an edge in graph $T$, then $(p_u, p_v)$ is an edge in the graph $\mathcal{N}(\mathcal{V},\mathcal{E})$. We note that for edge $(u,v)$ its corresponding edge-set $(u,v)^{\epsilon} \cap D$ contains points $p_u, p_v$. Thus $(p_u,p_v)$ is an edge in graph $\mathcal{N}(\mathcal{V}, \mathcal{E})$. It follows that $T$ is isomorphic to $\mathcal{N}(\mathcal{V},\mathcal{E})$. Because $T$ is a tree, then $\mathcal{N}(\mathcal{V},\mathcal{E})$ is tree as well.

%We are left to prove the last claim. Let $v$ be an arbitrary vertex of $T$. Assume that arbitrary points $a,b \in D$ belong to distinct 


We are left to prove the last claim. Let $a,b$ be arbitrary points for which 
there does not exist $e \in \mathbb{E}(T)$ for which $\{a,b\} \subseteq e^{\epsilon} \cap D $. Let $s$ be a shortest path connecting $a$ to $b$ in graph $T$. Using Lemma \ref{ExistenceOfVertexLink} we can find a point $q \in s$ for which $d_G(q,p_v) < \frac{\delta}{2}$. We note that from $\delta$-sparseness assumption it follows that 
$d_G(a,p_v) \geq \delta $ and $d_G(b,p_v) \geq \delta $. From triangle inequalities we can deduct 
\begin{align}
d_G(a,p_v) \geq& d_G(a,q) - d_G(q,p_v) > \delta - \frac{\delta}{2}  \geq \frac{\delta}{2}  \\
d_G(b,p_v) \geq& d_G(b,q) - d_G(q,p_v) > \delta - \frac{\delta}{2}  \geq \frac{\delta}{2}
\end{align}
We will prove that $d(a,p_v) < d(a,b)$. Proof for the fact that $d(b,p_v) < d(a,b)$ can be done similarly. 
We note that because $q$ was intermediate point of a shortest path $s$ connecting points $a$ and $b$ we have $d_G(a,b) = d_G(b,q) + d_G(a,q)$. By combining all the aforementioned facts we obtain: 
$$ d_G(a,p_v) \leq d_G(a,q) + d_G(p_v,q) = d_G(a,b) - d_G(b,q) + d_G(p_v,b) < d_G(a,b).$$


%d_G(a,b) = d_G(a,q) + d_G(q,b) \geq  $$
%
%Now because path $s$ was a shortest path between $a$ and $b$ and point $q$ was included into it we can deduct
%$$d_G(a,b) = d_G(a,q) + d_G(q,b) > \frac{\delta}{2} + \frac{\delta}{2} >  \delta$$




%Let $v$ be an arbitrary vertex of $T$. Let $e^\epsilon \cap D$ and $h^{\epsilon} \cap D$ be distinct cover elements of tree-cover for some $e,h \in \mathbb{E}(T)$. Let $a,b \in D$ be arbitrary points satisfying 
%$a \in e^\epsilon \cap D $ and $b \in h^{\epsilon} \cap D$. Let $s$ be a shortest path between $a$ and $b$. Using Lemma \ref{ExistenceOfVertexLink} we can find 

\end{proof}
%
%\begin{proof}
%
%%Let $e$ and $h$ be arbitrary edges having $v$ as one of their end points and let $a,b$ be arbitrary points satisfying $a \in D \cap e^{\epsilon}$ and 
%%$b \in D \cap h^{\epsilon}$. 
%
%
%
%Let $e^\epsilon \cap D$ and $h^{\epsilon} \cap D$ be distinct cover elements of tree-cover for some $e,h \in \mathbb{E}(T)$. We note first that following from Lemma \ref{lem:structureofpaths} edges $e,h$ have to be adjacent. Let vertex $v$ be in the intersection of $e$ and $h$ i.e. $e \cap h = \{v\}$. We note that the vertex point $p_v$ defined in Lemma \ref{lem:vertex-point} is contained in the intersection $e^{\epsilon} \cap h^{\epsilon} \cap D $. Let $q \in e^{\epsilon} \cap h^{\epsilon} \cap D $ be a point having $q \neq p_v$. 
%We can apply Lemma \ref{AdjacentEdgesLemma} with $r = 0$ to obtain $d(q, v) \leq \frac{\epsilon}{\sin(\frac{\theta(T)}{2} )} $.
%We can now use triangle inequality to deduct:
%$$\delta < d(q,p_v) \leq \gamma(d(q,v) + d(v,p_v)) \leq \epsilon + \frac{\epsilon}{\sin(\frac{\theta(T)}{2})} $$
%However this is a contradiction, because $\delta$ defined in Equation \ref{eqa:GHT} is clearly larger than the right-most expression.
%
% 
%We will now prove that for all $a \in e^\epsilon \cap D  $ and $b \in h^{\epsilon} \cap D $ the following two inequalities are satisfied: $d_G(p_v,a) \leq d_G(a,b)$ and $d_G(p_v,b) \leq d_G(a,b)$. Let $s$ be the shortest path connecting $a$ to $b$ in graph $G$. Using Lemma \ref{lem:ExistenceOfVertexLink} we obtain edges $e,h$ having a common vertex $v$ which satisfy $x \in \overline{D}_{e}$ and $y \in \overline{D}_{h}$ for some $(x,y) \in s$. We note that $d(x,y ) \leq l_{\max}(G)$ . Thus we can use  Lemma \ref{lem:AdjacentEdgesLemma}  with a bound $l_{\max}(G)$ to deduct 
%$$d(x, v) \leq  \dfrac{\epsilon}{\sin(\frac{\theta}{2})} +  \dfrac{l_{\max}(G)}{\sin(\min(\theta, \frac{\pi}{2}))} $$ 
%We recall that Equation \ref{eqa:GHT} states the following: 
%$$\delta \geq  2\gamma(\epsilon +\dfrac{\epsilon}{\sin(\frac{\theta(T)}{2})} + \dfrac{l_{\max}(G)}{\sin(\min(\theta(T), \frac{\pi}{2}))}) $$ 
%By combining the two inequalities above we obtain:
%$$d(x, v) \leq  \frac{\delta}{2\gamma} - \epsilon $$
% Using triangle inequalities and the fact that  we obtain the following inequalities: 
%% \frac{\epsilon}{\sin(\frac{\theta}{2})} +  \frac{l_{\max}(G)}{\sin(\min(\theta,\frac{\pi}{2}))}
%%We can now use Lemma \ref{AdjacentEdgesLemma} with a bound $l_{\max}(G)$ we obtain  $d(s(i),p_v) \leq \frac{\delta}{2} $ , where $\theta$ is the smallest angle over all the adjacent edges.
%%$$d_k(p_v, s(\alpha)) \leq & d_k(p_v,v) + d_k(v,s(\alpha)) \leq  c_{\max}(t_{\epsilon}(p_v,v) + t_{\epsilon}(v,s(\alpha)) \leq c_{\max}(\epsilon+ \frac{\epsilon}{\sin(\frac{\theta}{2})}  +  %\frac{r}{\sin(\theta )}) $$
%%\gamma(\epsilon+ \frac{\epsilon}{\sin(\frac{\theta}{2})} + \frac{l_{\max}(G)}{\sin(\theta )})
%$$d_G(p_v, x) \leq d_G(p_v,v) + d_G(v,x) \leq  \gamma(d(p_v,v) + d(v,x)) \leq  \gamma(\frac{\delta}{2\gamma} - \epsilon) +  \gamma \epsilon \leq  \frac{\delta}{2} $$
%$$d_G(a, x) \geq d_G(a,p_v) - d_G(p_v,x) > \delta - \frac{\delta}{2} \geq \frac{\delta}{2} $$
%$$d_G(b, y) \geq d_G(b,p_v) - d_G(p_v,y) > \delta - \frac{\delta}{2} \geq \frac{\delta}{2} $$
%%\gamma(\epsilon+ \frac{\epsilon}{\sin(\frac{\theta}{2})} + \frac{l_{\max}(G)}{\sin(\theta )})
%We note that, because $d_G$ is a path-metric we are able to split it into parts. Together with the previous inequalities we obtain the following chain of inequalities: 
%$$  d_G(a,b) \geq  d_G(a,x) + d_G(y, b) > d_G(a,x)  + \frac{\delta}{2} \geq d_G(a,x)  + d_G(p_v,x))  \geq d_G(a,p_v)  $$
%% \begin{equation*}
%% \begin{aligned}
%% d_G(a,b) \geq & d_G(a,s(i)) + d_G(s(i+1), b)  \\
%%     >    &  d_G(a,s(i))  + \frac{\delta}{2} \\
%%     \geq &  d_G(a,s(i))  + d_G(p_v,s(i)))\\
%%      \geq & d_G(a,p_v) 
%% \end{aligned}
%% \end{equation*}
%Using a similar inequality we obtain that $ d_G(a,b) > d_G(b,p_v) $. Thus the claim holds. 
%
%\end{proof}



\begin{lem}[$e$-ordering is well-defined]
\label{lem:eordering}
Assume the conditions of Theorem \ref{thmm:GHT}. Let $e = [u,v]$ be an arbitrary line segment of $T$. Let us define $\text{pr}_{e}:D \cap e^{\epsilon} \rightarrow e$ as a function mapping every $p \in D$ to its nearest neighbor in the line segment e, that will be denoted by $\text{pr}_{e}(p)$. Then $e$-ordering defined for all $p,q \in D \cap e^{\epsilon}$ as $p \leq q$ iff $d(u,\text{pr}(p)) \leq d(u,\text{pr}(q))$ is an ordering satisfying antisymmetry:
$$ \text{if } p \leq q \text{ and } q \leq p \text{ then } p = q. $$
\end{lem}

\begin{proof}

%Define $\mathcal[E} = \{(p_i, p_{i+1}) \}$ $\mathcal{V} = $  . We will now show that $(\mathcal[E}, \mathcal{V})$


%is a tree-cover of $D \cap e^{\epsilon}$. 

Let $p,q$ be arbitrary points of $D$ as in assumption. Assume now that $p \leq q $ and $q \leq p$. It follows that $d(u,\text{pr}(p)) = d(u,\text{pr}(q))$, because $u$ is an endpoint of a line segment there exists a unique point $s$ satisfying $d(u,s) = r$ for any $r \in \R$ in particular $\text{pr}(p) = \text{pr}(q)$. It thus follows that $d(p,q) \leq 2\epsilon$. We note that if $p \neq q$ then 
$d(p,q) \geq \delta > 2 \epsilon $, which is a contradiction. It follows that $p = q$. 
\end{proof}


\spoe*


\begin{proof}



Let $(p_i)$ be the points of $D \cap e^{\epsilon}$ ordered in $e$-ordering, where $i \in \{0,...,t\}$. 
Define $\mathcal{E} = \{(p_i, p_{i+1}) \mid 0 \leq i \leq k-1 \}$ and $\mathcal{V} = D \cap e^{\epsilon}$. We will now show that $(\mathcal{V}, \mathcal{E})$ is a 
tree-cover of $D \cap e^{\epsilon}$. The intersection of $\{p_i, p_{i+1}\} \cap \{p_j, p_{j+1}\}$  where $i \neq j$ is clearly either empty or is exactly single point of $\mathcal{V}$. We also note that each of the sets $\{p_i, p_{i+1}\}$ consists of exactly two elements, both of which belong to the set $\mathcal{V}$. Thus  $(\mathcal{V}, \mathcal{E})$ is a graph-cover.

To prove that $(\mathcal{V}, \mathcal{E})$ is a tree-cover we will now need to show that the nerve $\mathcal{N}(\mathcal{V}, \mathcal{E})$ is a tree graph and that for any $i < j < k$ the following inequalities are satisfied: $d_G(p_i, p_j) < d_G(p_i, p_k)$ and $d_G(p_j,p_k) < d_G(p_i,p_k)$. To prove that $\mathcal{N}(\mathcal{V}, \mathcal{E})$ is a tree, we note that for any index $i$ we have $\{p_i, p_{i+1}\} \cap \{p_{i+1}, p_{i+2}\} = \{p_{i+1}\}$  and for any integers $i + 1 < j$
$\{p_i, p_{i+1}\} \cap \{p_{j}, p_{j+1}\} = \emptyset$. Thus elements of $\mathcal{E}$ form a chain, that is connected and acyclic. 

To prove that the given cover is a tree-cover it is enough to prove that for any triplet of indices $i < j < k$ the inequality $d_G(p_i, p_j) < d_G(p_i, p_k)$ is satisfied. Let $s$ be the shortest path connecting $p_i$ to $p_k$. Let $P$ be the plane that contains point $p_j$ and is orthogonal to $e$. Because $p$ and $q$ are on the different sides of the plane $P$ path $s$ has to contain edge $(x,y)$ , in such a way that $x$ and $y$ are on different sides of the space divided by plane $P$. Because $d(x,y) \leq l_{\max}(G)$ it follows that $d(x,P) \leq l_{\max}(G)$. Let $q \in P$ be the point minimizing the distance $d(x,P)$ i.e. $d(x,q) = d(x,P)$. Then by using triangle the inequality 
$$d_G(p_i,x) \leq \gamma d(p_i,x) \leq \gamma d(x,q) + \gamma d(q,p_i) \leq  \gamma (l_{\max}(G) + \epsilon) < \frac{\delta}{2}. $$
The rest of the claim is proved similarly as in Proposition \ref{lem:nonadjacentedgesgraph}.
Using the triangle inequality we obtain:
\begin{align}
d_G(p_i, x) \geq&  d_G(p_i , p_j ) - d_G(p_j,x) > \frac{\delta}{2} \\
d_G(p_k, x) \geq&  d_G(p_j, p_k ) - d_G(p_k,x) > \frac{\delta}{2}
\end{align}
Because $x$ is intermediate point in a short path between $p_i$ and $p_k$ we have $d(p_i, p_k) = d(p_i, x) + d(x,p_k)$. The claim follows now form the following triangle inequality:
$$ d_G(p_i, p_j) \leq d_G(p_i,q) + d_G(q,p_j) = d_G(p_i, p_k) - d_G(p_k,x) + d_G(x,p_j) < d_G(p_i,p_k).$$
Inequality $d_G(p_j, p_k) < d_G(p_i, p_k)$ is proved similarly. It follows that $(\mathcal{V}, \mathcal{E})$ is a tree-cover of $D \cap e^{\epsilon}$. 
From Lemma \ref{lem:MultiMSTGlue} we obtain now that $$\MST(D \cap e^{\epsilon}, d_G) = \bigcup_{i \in [t]} \MST(\{p_i, p_{i+1}\}, d_G)$$
which is a polygonal path connecting $p_u$ to $p_v$.

%$$d_G(p_i, q) \geq  d_G(p_i , p_j ) - d_G(p_j,q) > \frac{\delta}{2}$$


% 
% 
% we can use triangle inequality to obtain $d(x,v) \leq 2 \epsilon + l_{\max}(G) $ and $d(y,v) \leq 2 \epsilon + l_{\max}(G) $. Similarly as in Lemma \ref{lem:nonadjacentedgesgraph} we obtain the following inequalities: 


%Point $\text{pr}_e(q)$ splits the edge $e$ into two parts. Let $e'$ be a subdivision of $e$ obtained by combining the two parts. Let us define 
%$T' = e$, $D' = e^{\epsilon} \cap D$ , $C' = C \cap e^{\epsilon}$ and $G' = G \cap e^{\epsilon}$.  We note that $T',D'$, $C'$ and $G'$ satisfy the conditions of Theorem \ref{thmm:GHT} and the standard star-cover $\mathcal{T}(v)$ consists of two elements corresponding to $D \cap [u,\text{pr}_e(q)]^{\epsilon}$ and
%$D \cap [\text{pr}_e(q),v]^{\epsilon}$. Result follows now by using Lemma \ref{lem:nonadjacentedgesgraph} on graph $T'$. 
%Let $p'$, $q'$ and $r'$ be the orthogonal projections of points $p,q$ and $r$ respectively. 
 
 %We can use exactly the same proof strategy as in Lemma \ref{lem:nonadjacentedgesgraph} by noting that we can subdivide edge $e$ by adding vertex $q'$, which satisfies $d(q,q') < \epsilon$.
 
  %for which $d(q,q') < \epsilon$. 
% 
% We can subdivide graph $T$ by defining $p',q',r'$ to be the new vertices. Each of the distances $d(p',p)$, $d(q,q')$, $d(r,r')$ is under $\epsilon$. Thus $
%[p',q']$ and $[q',r']$ can be treated as neighboring edges and  we can apply Lemma \ref{lem:vertexSeparation} to get the result $d(p,q) < d(q,r)$ and $d(q,r) %< d(p,r)$.
\end{proof}



\subsection{Distance and vertex count guarantee}
\label{sec:DistanceAndVertexCount}
%Before proving the distance theorem, we need the following technical Lemma:
%%
%%\begin{lem}
%%
%%\end{lem}
%%\begin{proof}
%%
%%\end{proof}

The main aim of this section is to prove the results regarding vertex count and distance guarantee for $\DT(C)$ as stated in Problem \ref{pro:reconstruction}.

\begin{lem}
Assume the conditions of Theorem \ref{thmm:GHT}. Then $d_{H}(\MST(D,d_G), T) \leq \epsilon$, where $d_H$ is the hausdorff-distance.
\end{lem}
\label{lem:HausdorffDistanceGHT}
\begin{proof}
To prove $d_{H}(\MST(D,d_G), T)$ we need to show that 
$$\sup_{p \in \MST(D,d_G)}\inf_{q \in T}d(p,q) \leq \epsilon \hspace{0.25cm} \text{ and } \hspace{0.25cm} \sup_{p \in T}\inf_{q \in \MST(D,d_G)}d(p,q) \leq \epsilon.$$ 
The proves of both of the claims are nearly identical and thus we will prove only the first one. Let $ p \in \MST(D,d_G) $ be arbitrary point. From Lemma \ref{lem:somstod}  we are able to decompose $\MST(D, d_{G})$ into $ \bigcup_{e \in \mathbb{E}(T)} \MST(e^{\epsilon} \cap D, d_G)$. Let $e$ be such that
$p \in \MST(e^{\epsilon} \cap D, d_G)$ . From Proposition \ref{lem:edge-offset} we obtain that $\MST(e^{\epsilon} \cap D, d_G)$ is a polygonal line
$(a_0, ..., a_k)$, where $a_i \in D$ for all $i$. It follows that for every index $i$ there exists $b_i \in e$ (in geometrical representation of $e \subseteq \R^m$) for which $d(a_i,b_i) \leq \epsilon$. Let index $j$ be such that $p$ is contained in segment $[a_j, a_{j+1}]$.
We note that the end points of $[a_j,a_{j+1}]$ and $[b_j, b_{j+1}]$ are at most $\epsilon$-distance away from each other, it follows that there exists an intermediate point $q \in [b_i, b_{i+1}]$ for which $d(p, q) \leq \epsilon$. Because $p$ was chosen arbitrarily and $q \in T$, it follows that 
$$\sup_{p \in \MST(D,d_G)}\inf_{q \in T}d(p,q) \leq \epsilon.$$


%We note first that using Proposition \ref{lem:somstod}


%and $d(a_i,T) \leq \epsilon$. Because $d_{M}(e, C) \leq \epsilon$, we can use triangle inequality to deduct:
%$$d_H(a_i,C) \leq d_H(a_i,e) + d_H(e,C) \leq 2\epsilon $$
%Because point cloud $C$ is $2\epsilon$-close to every $a_i$ it follows that a segment $[a_i, a_{i+1}]$ is $2\epsilon$-close to $C$ as well i.e.
%$d([a_i,a_{i+1}], C) \leq 2\epsilon$. By combining all the edges we obtain the final claim:
%$$d_H(\MST(D,d_G), C) \leq 2\epsilon $$

\end{proof}
\CorProbA*
\begin{proof}
Let $p \in C$ be arbitrary point. By conditions of Theorem \ref{thmm:GHT} there exists point $q \in e$ satisfying $d(p,q) \leq \epsilon$. By Lemma  \ref{lem:HausdorffDistanceGHT} there exists $w \in \MST(D,d_G)$ for which $d(q,w) \leq \epsilon$. Using triangle inequality:
$$d_{\overleftarrow{H}}(p,w) \leq d(p,q) + d_{\overleftarrow{H}}(q,w) \leq 2\epsilon.$$
Because $p$ was chosen arbitrarily it follows $d_{\overleftarrow{H}}(\MST(D,d_G),C) \leq 2\epsilon$.


%This can be extended to $d_{H}(\MST(e^{\epsilon} \cap D, d_G), C) < \epsilon$ and finally by combining all the polygonal paths of the form $\MST(e^{\epsilon} \cap D, d_G))$ we obtain the final claim:
%$$d_H(\MST(D,d_G), C) \leq 2\epsilon $$


%$$d(p,\MST(D, d_{G})) \leq d(p,q) + d(q,\MST(D, d_{G})) \leq 2 \epsilon $$
%we obtain the desired bound.
\end{proof}

\begin{lem}[Antipodal points maximize distance]
\label{lem:antipodalPoints}
Let $S$ be a hypersphere in $\R^m$ having $c$ as its central point. Let $t$ be arbitrary point and let $q$ be a point having $d(c,q) = r$ for fixed $r \in \R$. Let $l$ be a line that goes though points $t$ and $q$. We say that $q$ is in antipodal position if $q \in l$ and $d(q,t) > d(q,c)$. If point $q$ is in the antipodal position, then for any other point $w$ the inequality $d(q,t) > d(q,w)$ is satisfied.
\end{lem}

\begin{proof}
This Theorem will be proved using cosinus theorem. As illustrated Figure \ref{fig:antipodalProof} consider the triangle $\hat{twc}$. Using cosinus Theorem we 
obtain: $$d(w,t) = \sqrt{d(t,c)^2 + d(c,w)^2 - 2d(t,c)d(c,w)\cos(\angle tcw)}$$
This expression reaches maximum when $\cos(\angle tcw) = -1$. This is satisfied for $\angle tcw = \pi$, which happens exactly when $w = q$. Thus inequality $d(q,t) > d(q,w)$ holds. 
\end{proof}


\begin{figure}
\centering
\begin{tikzpicture}
\draw[thick, dashed] (0,0) circle(3.0);
\draw[thick, dashed] (0,0) circle(2.25);
\filldraw[black] (0,0) coordinate(c) circle (2pt);
\filldraw[black] (0,3) coordinate(t) circle (2pt);
\filldraw[black] (0,-2.25) coordinate (q) circle (2pt);
\filldraw[black] (-1.0,-2.0) coordinate (w) circle (2pt); 
\draw (c) -- (t);
\draw (c) -- (q);
\draw (c) -- (w);
\draw (t) -- (w);
%\draw (q) -- (w);
\draw[red] (0.25,0) node {$c$};
\draw[red] (0.25,2.75) node {$t$};
\draw[red] (0.25,-2.0) node {$q$};
\draw[red] (-1.25,-1.75) node {$w$};

%  \filldraw[black] (0,0) coordinate(c) circle (2pt) ;
 %  \filldraw[black] (0,0) coordinate(c) circle (2pt);
\end{tikzpicture}
\caption{Setup of Lemma \ref{lem:antipodalPoints}. Let $c$ be a centroid point and point $t$ be arbitrary point in sphere, point $q$ is antipodal position of $t$. We prove that for arbitrary point $w$ satisfying $d(w,c) = d(q,c)$ the inequality $d(t,q) \geq d(t,w)$ is satisfied.}
\label{fig:antipodalProof}
\end{figure}

\begin{figure}
    \centering


\begin{tikzpicture}
	\draw[dashed,color=gray] (0,0) arc (-90:90:0.5 and 1.5);% right half of the left ellipse
	\draw[semithick] (0,0) -- (8,0);% bottom line
	\draw[semithick] (0,3) -- (8,3);% top line
	\draw[semithick] (0,0) arc (270:90:0.5 and 1.5);% left half of the left ellipse
	\draw[dashed,color=gray] (8,0) arc (-90:90:0.5 and 1.5);% right ellipse
    \draw[semithick] (8,0) arc (270:90:0.5 and 1.5);% left half of the left ellipse
        \draw[semithick] (6.25,0) arc (270:90:0.5 and 1.5);% left half of the left ellipse

    \draw[semithick] (0,1.5) -- (8,1.5);
    \draw[dashed,color=gray] (6.25,0) arc (-90:90:0.5 and 1.5);% right ellipse
    \draw[red] (1.25,2.75)  node {$p$};
    \filldraw[black] (6.25,0.0) coordinate(q) circle (2pt);
        \filldraw[black] (6.25,3.0) coordinate(t) circle (2pt);
    \draw[red] (6.45,2.85)  node {$t$};


    \draw[red] (6.5,0.25)  node {$q$};
    \filldraw[black] (1.25,3.0) coordinate(p) circle (2pt);
    
     \draw[dashed,color=gray] (1.25,0) arc (-90:90:0.5 and 1.5);% right ellipse
	   \draw[semithick] (1.25,0) arc (270:90:0.5 and 1.5);% left half of the left ellipse
	   
	   \filldraw[black] (5.85,0.75) coordinate (w) circle (2pt);
	    \draw[red] (6.1,0.85) node {$w$};
	   \draw[dotted, thick] (w) -- (p);
	   \draw[dotted, thick] (q) -- (p);
	   \draw[blue] (2.5,1.25) node {$h$};
	   \draw[blue] (2.5,2.75) node {$l$};
	     \draw[dotted, thick] (w) -- (t);
	   \draw[dotted, thick] (q) -- (t);

%	\draw (-1,1.5) node {$\varnothing d_1$};
%	\draw (3.3,1.5) node {$\varnothing d_2$};
%	\draw[|-,semithick] (0,-0.5) -- (4,-0.5);
%	\draw[|->,semithick] (4,-0.5) -- (4.5,-0.5);
%	\draw (0,-1) node {$x=0$};
%	\draw (4,-1) node {$x=l$};
\end{tikzpicture}

    \caption{Situation arising in Theorem \ref{thmm:vcg}. When given line segment $h$ , points $p,q \in D$ we denote $l$ to be parallel line of $h$ which goes through point $p$. Point $t$ is intersection of $l$ and the plane of $q$ which is orthogonal to $l$. Point $w$ is point chosen arbitrary in the same plane with $q$}
    \label{fig:LemAntipodal}
\end{figure}

In the following Theorem we bound $|D|$ by finding upper bound on how many points we can place in $T^{\epsilon}$ satisfying $\delta$-sparsness condition i.e. $d(a,b) > \delta$ for all $a,b \in D$.   

\CorProB*
\begin{proof}
To solve this problem we note that the collection $\{e^{\epsilon} \cap D \mid e \in \mathbb{E}(T)\}$ covers set $D$. Let us fix an arbitrary edge $e \in \mathbb{E}(T)$. We note that for any $a,b \in e^{\epsilon} \cap D$ we have $\delta \leq d_G(a,b) \leq \gamma d(a,b)$. Which is equivalent
$\frac{\delta}{\gamma} < d(a,b)$. Thus $e^{\epsilon} \cap D$ is $\frac{\delta}{\gamma}$-sparse in the standard euclidean metric. Let $(p_i)$ be $e$-ordering of $e^{\epsilon} \cap D$ as defined in Lemma \ref{lem:eordering} . Denote by $h$ the line segment obtained by stretching out $e$ at its end points in both directions by factor $\epsilon$. Let $\text{pr}_{h}:D \cap e^\epsilon \rightarrow h$ be a similar projection function as $\text{pr}_h$, which instead of mapping every point to its nearest neighbor maps every set $D \cap e^\epsilon$ into line segment $h$ according to their orthogonal projection. We will now show that $d(\text{pr}(p_i) , \text{pr}(p_{i+1})) \geq 2 \sqrt{(\frac{\delta^2}{\gamma^2} - 4 \epsilon^2)}$ for all $i$.

Let $p,q$ be arbitrary consecutive elements of the sequence $(p_i)$. Assume that $d(p,q) \geq 2 \sqrt{\frac{\delta^2}{\gamma^2} - 4 \epsilon^2}$.
As illustrated in Figure \ref{fig:LemAntipodal} let $l$ be the line which goes through point $p$ and is parallel to $e$. Let $R_q$ be the plane which is orthogonal to $e$ and contains point $q$. Let $t$ be a point in the intersection $l \cap R_q$. Using Lemma \ref{lem:antipodalPoints} the antipodal position of $q$ maximizes the distance $d(q,t)$ in other words $d(q,t) \leq d(t,\text{pr}_{h}(q)) + d(q,\text{pr}_{h}(q)) \leq 2\epsilon$. Because plane $R_q$ is orthogonal to $l$ we can use Pythagorean Theorem to deduct
$$d(p,q) = \sqrt{d(q,t)^2 + d(p,t)^2} \leq \sqrt{4\epsilon^2 + (\sqrt{\frac{\delta^2}{\gamma^2} - 4 \epsilon^2})^2 } \leq \frac{\delta}{\gamma}$$
which is a contradiction, because set $D$ is $\frac{\delta}{\gamma}$-sparse in euclidean metric. We can now estimate $|D \cap h^{\epsilon}|$ in the following way:
$$|h| \geq  |D \cap h^{\epsilon}| \cdot 2\sqrt{\frac{\delta^2}{\gamma^2}-4\epsilon^2}$$
Modifying the aforementioned inequality and summing over all edges $e \in \mathbb{E}(T)$ we obtain the final result:
$$|D| \leq \sum_{e \in \mathbb{E}(T)} \dfrac{|e| + 2 \epsilon}{2\sqrt{\frac{\delta^2}{\gamma^2}-4\epsilon^2}} $$

% \geq \sum_{p \in D \cap h^{\epsilon}}|s_p|


%% Denote by $h$ the line segment obtained by stretching out $e$ at its end points in both directions by factor $\epsilon$. Let $\text{pr}_{h}:D $
%\cap e^\epsilon \rightarrow h$ be a similar projection function, which maps every set $D \cap e^\epsilon$ into line segment $h$ according to their %orthogonal projection.

%
%From condition of Theorem \ref{thmm:GHT} we know that $\frac{\delta}{\gamma} \geq 2\epsilon$, meaning function $\text{pr}_h$ is injective i.e. inverse image $\text{pr}_{h}^{-1}(q)$ contains at most one point for any $q \in h$. Define segment $s_p$ to be the maximal line segment which satisfies $\text{pr}^{-1}_h(s_p) =  \{p\}$. We will first show that $|s_p| \geq 2 \sqrt{\delta^2 - 4\epsilon^2}$. 

 %Depending on the position of points $p \in D$ and the parameter $\delta$ we can find a sub linesegment $s_p \subseteq h$ which satisfies $\text{pr}_{h}^{-1}(s_p) = \{p\}$. 

%To prove the claim we will show that for any other point $q \in D \cap e^\epsilon$ the distance $$d(\text{pr}_h(q), \text{pr}_h(p)) \geq \sqrt{\delta^2 - %4\epsilon^2}$$ 



%Assume the conditions of Theorem \ref{thmm:GHT}. Then the number of vertices in the reconstruction $\MST(D, d_G)$ has the following bound:
%$$|D| \leq \sum_{e \in \mathbb{E}(T)} \dfrac{|e| + 2 \epsilon}{2\sqrt{\delta^2-4\epsilon^2}} $$

 %$$d(\text{pr}_h(q), \text{pr}_h(p))  = d(p,t) = \sqrt{d(p,q)^2 - d(q,t)^2} \leq \sqrt{\delta^2 - 4\epsilon^2} .$$

%Because   $|s_p| \geq 2\sqrt{\delta^2 - 4\epsilon^2}$

%This will be proved analytically. For simplicity assume that the line segment $h$ have both of its end points on $X$-axis. Let $(p_1,...,p_m)$ be a vector-representation of point $p$ and define vector representation similarly for all the aforementioned points. Using spherical coordinates we are able to represent point $p$ using angles $\phi_1, ..., \phi_{n-1}$ in the following way:
%\begin{align*}
%&p_1 =  \text{pr}_{h}(p_1)  \\
%&p_2 =  d(p,\text{pr}_h(p))\cos(\phi_1) \\
%&p_3 =  d(p,\text{pr}_h(p))\sin(\phi_1)\cos(\phi_2) \\
%&p_4 =  d(p,\text{pr}_h(p))\sin(\phi_1)\sin(\phi_2)\cos(\phi_3)\\
%&p_n =  d(p,\text{pr}_h(p))\sin(\phi_1) \cdot \cdot \cdot \sin(\phi_{n-3})\cos(\phi_{n-2})
%\end{align*}
%
%Similarly using angles $\psi_1, ... , \psi_n$ we are able to represent vector $q$ in the following way:
%
%\begin{align*}
%&q_1 =  \text{pr}_{h}(p_1)  \\
%&q_2 =  d(p,\text{pr}_h(p))\cos(\psi_1) \\
%&q_3 =  d(p,\text{pr}_h(p))\sin(\psi_1)\cos(\psi_2) \\
%&q_4 =  d(p,\text{pr}_h(p))\sin(\psi_1)\sin(\psi_2)\cos(\psi_3)\\
%&q_n =  d(p,\text{pr}_h(p))\sin(\psi_1) \cdot \cdot \cdot \sin(\psi_{n-3})\cos(\psi_{n-2})
%\end{align*}

\end{proof}

%
%The $k$-nearest neighbor graph $\NN_k$ in Definition~\ref{dfn:MSG_k} is well-known, while we couldn't find any reference for a $k$-th minimum spanning graph $\MSG_k$, which extends a classical Minimum Spanning Tree $\MST=\MSG_1$.


\section{Algorithmic solution to the tree reconstruction problem}

% Explicitly this will be solved by providing an algorithm that selects $\delta$-sparse subset consisting of dense points $D$ using kernel density estimate and builds a connected underlying graph $\MSG_k$ based on $k$-nearest neighborhood search. 

By combining Theorems \ref{thmm:GHT}, \ref{thmm:dg} and \ref{thmm:vcg} we are able to solve Problem~\ref{pro:reconstruction}. In this section we will build an algorithm which aims to select sparse subset $D$ and the underlying graph $G$ in such a way that they satisfy the condition of  Theorem \ref{thmm:GHT}. The $\delta$-sparse set $D$ will be built by using kernel density estimate as explained in Section \ref{sec:KDEExp}. As underlying graph we will use $\MSG_k$ based on $k$-nearest neighborhood search of Definition \ref{dfn:MSG_k}. The results of both, the procedure to find sparse set and the underlying graph heavily depend on the sampling on cloud $C$ and therefore we will only provide Experimental validation, Experiment \ref{expe:starExp} for sparse sets, and Experiment \ref{expe:UnderlyingGraph} for $\MSG_k$ to show that with correctly chosen parameters such methods will retrieve objects that satisfy the assumptions of Theorem \ref{thmm:GHT}.

%
% We should note that, because the point cloud is randomly generated it is non-trivial task to find necessary constrains on the sampling of the point cloud that  would generate a dense and an underlying graph which would satisfy the assumptions of Theorem \ref{thmm:GHT}. We will however prove experimentally that it can be done succesfully with relatively high probability. Experiments regarding kernel density estimation will be provided in Section \ref{sec:KDEExp} and regarding the $\MSG_k$ graph will be available in Section \ref{sec:UnderlyingGraphExp}.

%
%Using kernel density estimation on a big cloud of points, we build a dense tree with a small number of vertices.
%By minimizing the distance to the given cloud by vertex movements, the resulting Optimal Dense Tree outperforms all past skeletonization algorithms on a large dataset of synthetic clouds sampled with high noise around given graphs.
%The applications include a quick quality estimation of micelles formed by oil molecules in colloidal products. 

\begin{dfn}[$\NN_k(C)$ and $\MSG_k(C)$]
\label{dfn:MSG_k}
Let $C$ be any finite metric space.
For any integer $k\geq 1$, a \emph{$k$-nearest neighbor graph} $\NN_k(C)$ has the vertex set $C$ and every vertex $v\in C$ is joined by a single edge to its $k$ nearest neighbors in $C$.
(In case of equal distances, there might be a choice of neighbors.)
The \emph{$k$-th minimum spanning graph} $\MSG_k(C)$ is obtained from 
 $\NN_k(C) \subseteq \MSG_k(C)$ by adding those edges between vertices that make $\MSG_k(C)$ connected and keep its total length of edges minimal.
\bs
\end{dfn}

\begin{figure}[H]

\centering
\begin{subfigure}{.33\textwidth}
 
  % include first image
  \includegraphics[width=.95\linewidth]{images/MSGPictures/pic4fix.png}  
  \caption{Random graph colored red and a point cloud $C$ around it}
  \label{fig:subFig-first}
\end{subfigure}
\begin{subfigure}{.33\textwidth}
  \centering
  % include second image
  \includegraphics[width=.95\linewidth]{images/MSGPictures/pic5fix.png}  
  \caption{$\text{MSG}_k(C)$ graph of Definition \ref{dfn:MSG_k} computed on the point cloud for $k = 3$.}
  \label{fig:subFig-second}
\end{subfigure}
\begin{subfigure}{.33\textwidth}
  \centering
  % include second image
  \includegraphics[width=.95\linewidth]{images/MSGPictures/pic6fix.png}  
  \caption{$\text{MSG}_k(C)$ graph of Definition \ref{dfn:MSG_k} computed on the point cloud for $k = 6$.}
  \label{fig:subFig-second}

  
\end{subfigure}

  \caption{Random cloud around randomly generated graph and $\text{MSG}_k$ graphs around it}
  \label{fig:MSGGraphExample}

%\caption{ }

\end{figure}

The graph $\MSG_k(C)$ can be considered as a rough approximation to a topological shape of $C$, see Figure \ref{fig:MSGGraphExample}.

%the top right pictures with many short cycles in Fig.~\ref{fig:branched} and ~\ref{fig:cylindrical}.

%All further constructions will use only $\MSG_k(C)$, hence we need a path metric $d_k$ defined on $\MSG_k(C)$ below.

%\begin{proof}
%bala bala
%\end{proof}
% This is proceeded by computation of the minimum spanning tree on the selected points using the metric inherited from the underlying graph structure.



%
 
%Problem~\ref{pro:reconstruction} can be considered as a minimization of a distance in (\ref{pro:reconstruction}a) for a fixed number of vertices in (\ref{pro:reconstruction}c) subject to the homeomorphism $G\approx T$ in (\ref{pro:reconstruction}b).
%\smallskip

%\vspace*{0mm}
%For condition~(\ref{pro:reconstruction}b), 


%we approximate vertices of a straight-line tree $T$ as a sparse subset $\SD\subset C$ of densest points in Definition~\ref{dfn:sparse_dense}.

%The sparsity of $\SD$ is controlled by a distance threshold $\de$, which helps to reduce a final number of vertices for~(\ref{pro:reconstruction}c).  

%
%\begin{figure}
%\centering
%\includegraphics[width=0.45\linewidth]{images/ODT_pipeline.png}
%\caption{Building an Optimized Dense Tree $\ODT(C)$.}
%\label{fig:pipeline}
%\end{figure}


%By summing up the complexities we obtain:
%
%$$O(\max\{c^{16}, c^2_p c^2_l c^{10} , k \log(k) c^9 , \log_2(\zeta) c^{10} , |D|\} N \log(N) \alpha(N))$$


%\end{proof}






%
%
%\noindent
%\textbf{Input} : 
%any unorganized cloud of points $C\subset\R^m$.
%\smallskip
%
%\noindent
%\textbf{Parameters}: 
%a distance threshold $\de$, a number $k$ of nearest neighbors, a kernel density estimation $K_f$ on $C$, a learning rate and number of iterations for a gradient descent by Tensorflow \cite{TensorflowSGD}. 
%\smallskip
%
%\noindent
%\textbf{Stage 1}.
%Given a cloud $C\subset\R^m$, find a $k$-th nearest neighbor graph $\NN_k(C)$ from Definition~\ref{dfn:MSG_k}. 
%\smallskip
%
%\noindent
%\textbf{Stage 2}.
%Extend the $k$-th nearest neighbor graph $\NN_k(C)$ to a Minimum Spanning Graph $\MSG_k(C)$.
%%, see Theorem~\ref{thmm:MSG_k-complexity}.
%\smallskip
%
%\noindent
%\textbf{Stage 3}.
%Compute a Kernel Density Estimation $K_f$ from Definition~\ref{dfn:KDE} on points of the cloud $C$. 
%\smallskip
%
%\noindent
%\textbf{Stage 4}.
%Find a sparse subset $\SD\subset C$ of densest points separated by a distance threshold $\de$ by Algorithm~\ref{alg:sparse_dense}.
%\smallskip
%
%\noindent
%\textbf{Stage 5}.
%Build a dense tree $\text{DT}(C)\subset\R^m$ as a Minimum Spanning Tree on $\SD$ with straight line edges using the metric $d_{\MSG_k(C)}$ on $\MSG_k(C)$.
%%from %Definition~\ref{dfn:path_metric}.
%\smallskip
%
%\noindent
%\textbf{Stage 6}.
%Get an Optimized Dense Tree $\ODT(C)\subset\R^m$ by a stochastic gradient descent on vertices of $\text{DT}(C)\subset\R^m$, which minimizes the mean squared distance from points of $C$ to an optimized straight-line tree.



%\section{Necessary definitions for new dense trees}
%\subsection{Necessary definitions for new dense trees}
%\label{sec:definitions}
%
%All concepts below make sense in any metric space, though algorithms have better complexity in $\R^m$.
%A finite metric space is any finite set $C$ with a distance $d:C\times C\to[0,+\infty)$ satisfying the 3 metric axioms.
%\medskip


%
%\begin{dfn}[path metric $d_k$]
%\label{dfn:path_metric}
%Let $G$ be a connected graph  whose vertex $C$ is a finite metric space.
%For any vertices $a,b\in G$, let $d_G(a,b)$ be the length of a shortest path joining $a,b$ within $G$.
%For the graph $G=\MSG_k(C)$, the path metric is denoted by $d_k$.
%\bs
%\end{dfn}

\subsection{Kernel density estimation (KDE)}
\label{sec:KDEExp}
To substantially improve the shape of $\MSG_k(C)$ containing too many vertices, these vertices will be ranked by their density within a cloud $C$. Our main aim is to find points which are either close to medial axis of the given point cloud or centroids of the cloud points which represent the noise around original branching points. We use approximate kernel density estimation for this task, that was first presented in Section \ref{sec:KDETheorySec}. 

In our reconstruction experiments we are using bounded uniform noise. Thus the most logical choice for the kernel density estimation is a function such that resembles $\epsilon$-neighborhood search i.e. one that computes the number of reference points in $\epsilon$-neighborhood of a given point. It will be experimentally verified that when $\epsilon$ is larger than the generation error we are able to effectively find points which are close to the medial axis. In addition, when $\epsilon$ is at least $25\%$ larger than the generation error, we able to find centroids of the branching clouds. The best candidate for a function representing $\epsilon$-neighborhood search is a sigmoid function of Definition \ref{dfn:KDESigmoid} that has value $1$ for nearby points and switches in a rapid way to value $0$ after some threshold value. 

\begin{figure}[H]
\label{fig:KDENuclearsun}
\centering 
\includegraphics[width = 0.49\linewidth]{images/KDE/functions.png}
\includegraphics[width = 0.30\linewidth]{images/KDE/NuclearSun.png}
\caption{\textbf{Left:} Family of sigmoid functions, mimicking amount of the reference points found $\epsilon$-neighborhood for chosen query point used as the basis for the kernel density estimation.  \textbf{Right:} Kernel density estimation, where query points were generated on the plane that includes point 
$(\frac{1}{2},0,0)$ an is perpendicular to the line segment $[(0,0,0),(1,0,0)]$, and reference points  were randomly generated around the line segment with an uniform bound $\epsilon = 0.1$. Red points represent points with higher values and blue with lower values respectively.}
\end{figure}

\begin{dfn}[Sigmoid kernel density estimation function]

\label{dfn:KDESigmoid}
Define sigmoid kernel density estimate fuction $K_{r,t}: \R \rightarrow \R$ as a sigmoid function $$K_{r,t}(x) = \frac{1}{1+e^{px+q}}, $$ where coefficents $p$ and $q$ are chosen in such a way that $K_{r,t}(r + \frac{t}{2}) = 0.01$ and $K_{r,t}(r - \frac{t}{2}) = 0.99$. 

% $$f_{a,b}(x) = \dfrac{1}{1+e^{\frac{\log (\frac{1}{99}) - \log(99)}{ (b-a)}x + \log (\frac{1}{99}) -  b\frac{ \log (\frac{1}{99}) - \log(99)}{ (b-a)}}}$$, %where parameters $a,b$ will be selected so that $f_{a,b}$ satisfies $f_{a,b}(a) = 0.99 $ and $f_{a,b}(b) = 0.01 $ i.e. the function has values close to $1$ %when $x < a$ and $0$ when $x > b$. 
    %This function is illustrated in \ref{fig:f_a,b}. 
%\bs
\end{dfn}




% For convenience we will denote $\gamma = \frac{a + b}{2}$.
%For convenience we will denote $f_{a,b}$ using parameter pairs by setting $\alpha(r,t) \rightarrow f_{r - \frac{t}{2} , r + \frac{t}{2}}$. Value $r$ corresponds to roughly to the radius of the region, where points are considered centered at any query point $p$. On the other hand, parameter $t$ corresponds to the speed of decrease of the function $f_{r - \frac{t}{2} , r + \frac{t}{2}}$ from $1$ to $0$ at the boundary of the region.  

 
%It should roughly correspond to the radius, we would have used in the $\epsilon$-neighborhood search. 

%n the first experiment, we will show that functions $f_{a,b}$ are indeed giving higher values to points close to the medial axis. 

\begin{expe}[Tube experiments]
\label{expe:Tube}
 Given a segment $s = [(0,0,0),(1,0,0)]$ in $\mathbb{R}^3$ we generate reference set $R$ consisting of uniformly random generated points satisfying 
$d(s, R) \leq \epsilon$. Let $w = (\frac{1}{2},0,0)$ be the middle point of the segment and let $P(w)$ be the plane that goes thought point $w$ and that is perpendicular to $s$. We generate query set $Q$ consisting of 200 points inside the intersection $s^{\epsilon} \cap P(w)$ uniformly. Afterwards let $f_K$ be the kernel density estimate function computed on query set $Q$ , reference set $R$ and function $K_{r,t}$ for $6$ different set of parameters $(r,t)$, where we varied parameter $r$ and fixed $t = 0.05$. For every query point $q \in Q$ we measured its distance to the medial axis $d(q,s)$, as well as its value $f_K(q)$. Afterwards we formed $K'_f$ which consisted of normalized values of $f_K(q)$, obtained by lineary scaling its image-range to $[0,1]$. Finally the results were plotted in Figure \ref{fig:StarExperiments} (Left) we plotted the results by setting $X = d(q,s)$ and $Y = f_K(q)$.
 
 %as a $(d(q,s), K_f(q))$-graph in Figure \ref{fig:StarExperiments} (Left).
 
  %We note that steepest decrease was obtained with value $r = 0.1$.
 
%The average of the values of the function $f_{r,t}$ 
 
 % We computed kernel density estimation $K_f = \text{KDE}(Q,R,f_{a,b})$ for $6$ different set of parameters of a function $f_{a,b}$ and plotted the results in Figure \ref{fig:StarExperiments} (Left). The best results were obtained when parameters were close to the generation error $\epsilon = 0.1$.
\end{expe}

\begin{figure}[H]
\centering
\resizebox{0.49\columnwidth}{!}{
\begin{tikzpicture}
\begin{axis}[xlabel = Distance, ylabel = Normalized value of $f_K$,grid, legend style={font = \small, at={(0.28,0.25)},anchor=center}, every axis plot/.append style={ultra thick}]
% [black,mark = *]
\addplot[yellow] table [x=Distance, mark=none, y=Param0.025, col sep=comma] {tables/Density/resultsTube.csv};
\addlegendentry{$r = 0.05, t = 0.05$.}
\addplot[orange] table [x=Distance, y=Param0.05, col sep=comma, mark=none] {tables/Density/resultsTube.csv};
\addlegendentry{$r = 0.075, t = 0.05$.}
\addplot[black] table [x=Distance, y=Param0.075, col sep=comma, mark=none] {tables/Density/resultsTube.csv};
\addlegendentry{$r = 0.1, t = 0.05 $.}
\addplot[red] table [x=Distance, y=Param0.1, col sep=comma,mark=none] {tables/Density/resultsTube.csv};
\addlegendentry{$r = 0.125, t = 0.05$.}
\addplot[blue] table [x=Distance, y=Param0.125, col sep=comma,mark=none] {tables/Density/resultsTube.csv};
\addlegendentry{$r = 0.15, t = 0.05$.}
\addplot[green] table [x=Distance, y=Param0.15, col sep=comma,mark=none] {tables/Density/resultsTube.csv};
\addlegendentry{$r = 0.175, t = 0.05$.}


\end{axis}
\end{tikzpicture}
}\resizebox{0.49\columnwidth}{!}{
\begin{tikzpicture}
\begin{axis}[xlabel = Total number of points, ylabel = Distance from the origin,grid ,every axis plot/.append style={ultra thick}]
% [black,mark = *]
\addplot[yellow] table [x=NumPoints, mark=none, y=Param0.025, col sep=comma] {tables/Density/resultsStar.csv};
%\addlegendentry{$a = 0.075, b = 0.025$}
\addplot[orange] table [x=NumPoints, y=Param0.05, col sep=comma, mark=none] {tables/Density/resultsStar.csv};
%\addlegendentry{$a = 0.1, b = 0.05$}
\addplot[black] table [x=NumPoints, y=Param0.075, col sep=comma, mark=none] {tables/Density/resultsStar.csv};
%\addlegendentry{$a = 0.125, b = 0.075 $}
\addplot[red] table [x=NumPoints, y=Param0.1, col sep=comma,mark=none] {tables/Density/resultsStar.csv};
%\addlegendentry{$a = 0.15, b = 0.1$}
\addplot[blue] table [x=NumPoints, y=Param0.125, col sep=comma,mark=none] {tables/Density/resultsStar.csv};
%\addlegendentry{$a = 0.175, b = 0.125$}
\addplot[green] table [x=NumPoints, y=Param0.15, col sep=comma,mark=none] {tables/Density/resultsStar.csv};
%\addlegendentry{$a = 0.2, b = 0.15$}


\end{axis}
\end{tikzpicture}
}

\caption{\textbf{Left:} Results of tube Experiments \ref{expe:Tube} \textbf{Right: }Results of star-Experiments \ref{expe:starExp}}
\label{fig:StarExperiments}



\end{figure}

Recall that $\text{Star}(n,\theta)$ was a class of straight-line trees defined Example \ref{exa:StarGraphs} was a tree graph consisting of $n+1$ vertices, where all the vertices are connected to a chosen centroid point and the minimal angle between any pair of edges was $\theta$.
\begin{expe}[Star experiments]
\label{expe:starExp} 
We start by generating collection $\mathcal{L}$ consisting of different $\text{Star}(4, \frac{\pi}{4})$-trees. For each of the trees $T \in \mathcal{L}$ we generated 10-different point clouds in $\mathcal{M}$, in such a way that for each $i \in \{0,1,...,9\}$ point cloud $\mathcal{M}[i]$ was sampled uniformly in the $\epsilon$-offset of $T$ and $\mathcal{M}[i]$ consisted of $400 \cdot (i+1)$ points. Then we proceeded by computing kernel density estimate $f_K$ on $K_{r,t}$ using $\mathcal{M}[i]$ as both, query and reference set.  Let $o$ be the centroid point of a given $\text{Star}4$-graph and let $p$ be the point in $\mathcal{M}[i]$ which has the maximal $f_K(p)$ value. Our main goal is to show that the distance $d(o,p)$ is relatively low, as it will help the reconstruction for well-chosen parameter $r$. The average distance over 100 different graph was plotted in Figure \ref{fig:StarExperiments} (Right). We note that results don't significantly improve for $r \geq 0.15$.

% for each number of points $i \in M$ the test was repeated 100 times using different $\text{Star}(4, \frac{\pi}{4} )$-graphs

%By using larger $\theta$ values we decrease the average distance between origin and densest point. However, clouds having higher density don't seem to %benefit from higher parameter values, when $\theta > \frac{3\epsilon}{2}$. 


%and copied the exact data to query $Q$ and reference set $R$. Kernel density estimation $K_f = \text{KDE}(f_{a,b}, Q,R) $ was computed on the same set of %functions $f_{a,b}$ as in the Tube-experiments.
%For each number of points $i \in M$ the test was repeated 100 times using different Star(4)-graphs. 

\end{expe}

%\begin{expe}[Star experiments]
% We start by generating Star$(4)$ i.e. a graph consists of total $5$ vertices, in such a way that the central vertex is located in the origin $(0,0,0)$ and it is connected to 4 vertices distance $1$ away from it. The minimal angle between any two edges in the Graph was set to be $\frac{\pi}{4}$. Then we generated point clouds consisting of $M = \{400, 800 , ..., 4000\}$ points around the graph using uniform bound $\epsilon = 0.1$ and copied the exact data to query $Q$ and reference set $R$.  Kernel density estimation $K_f = \text{KDE}(Q,R,f_{a,b}) $ was computed on the same set of functions $f_{a,b}$ as in the Tube-experiments. For each number of points $a \in M$ the test was repeated 100 times using different Star$(4)$-graphs. Our main goal was to compute the distance between the point with the highest $K_f$ value and the origin. The average result over the experiments was plotted in Figure \ref{fig:StarExperiments}. By using larger $\theta$ values we decrease the average distance between origin and densest point. However, clouds having higher density don't seem to benefit from higher parameter values, when $\theta > \frac{3\epsilon}{2}$. 
%\end{expe}

\textbf{Conclusion: } 
From from the results of Experiment \ref{expe:Tube} we note that the value $r$ of $f_{r,t}$ should be close to the generation error $\epsilon$. In Experiment \ref{expe:starExp} we showed that the distance between centroid and deepest point is significantly reduced when $r \leq \frac{3\epsilon}{2}$. Thus we propose that $r= \frac{3\epsilon}{2}$ should be used for reconstruction.

%Given that higher $\theta$ parameters increase computational time and can potentially count additional noisy points we wish to minimize it. Experimentally it %was verified that increase in performance is significant when $\gamma \leq \frac{3\epsilon}{2}$. Thus, when the generation error $\epsilon$ is known we %suggest that $\theta = \frac{3\epsilon}{2}$ should be used. 




%we generate $M$ points around it using uniform bound $\epsilon = 0.1$. Our goal is to measure how the average distance of the deepest vertex from origin %depends on number of points $M$. \newline

%%The main purpose of the kernel density estimation in this project is to find points close to medial axis of the input point cloud. Because analytical proves %are hard, we resort to show experimentally that function $f_{a,b}$ are effective at finding such points. The following experiments were produced:
%
%\begin{itemize}
%
%\item \textbf{Tube experiment setup:} Given an edge $[(0,0,0),(1,0,0)]$ in $\mathbb{R}^3$ we generate $M = 500$ random points. We plot a graph how different functions $f_{a,b}$ behave in the circle boundary around point $(\frac{1}{2},0,0) $ for different radius $r \in (0,1)$. 
%\item \textbf{Star experiment setup:} Given a Star Graph Star$(4)$ i.e. a graph consists of one central vertex in origin $(0,0,0)$ connected to 4 vertices distance $1$ away from it, we generate unfiromly $M$ points around it using uniform bound $\epsilon = 0.1$. Our goal is to measure how the average distance of the deepest vertex from origin depends on number of points $M$. 
%
%\end{itemize}
%





%\begin{figure}
%
%
%
%\caption{In this figure we illustrate Star-experiments. Higher parameters correspond to smaller distance between origin and the point having the highest density.}
%\label{fig:StarExperiments}
%
%\end{figure}
%



%
%\subsection{a sparse subset $\SD_k$ of densest points}
%\label{sec:sparse_dense}

\subsection{a dense tree $\text{DT}(C)$ on a cloud $C$}
\label{sec:dense_tree}


The section explains the details of Stages~4 and 5 in Fig.~\ref{fig:pipeline}, which requires the new concept in Definition~\ref{dfn:sparse_dense}. We use Kernel Density Estimation $f_K$ to is used to select at Stage~4 a small $\delta$-sparse subset $D\subset C$ of densest points, which will be vertices of a dense tree $\text{DT}(C)$ at Stage~5.

\begin{dfn}[a sparse set of densest points]
\label{dfn:sparse_dense}
Let $f_K$ be a kernel density estimate from Definition~\ref{dfn:KDE} computed on some kernel $K$ using $C$, as both query and reference set.
Choose a point $p_1\in C$ with a maximum value of $f_K(p_1)$.
For a distance threshold $\de>0$, let $C_1$ be obtained from $C$ by removing all points $q$ at a distance $d_{\MSG_k}(p_1,q)<\de$.
For $i\geq 1$, until the subset $C_i\subset C$ isn't empty for $i\geq 1$, keep choosing a point $p_{i+1}\in C_i$ with a maximum value of $f_K(p_{i+1})$ and setting $C_{i+1}=C_i-\{q\in C_i \vl d_{\MSG_k}(p_i,q)<\de\}$.
Denote the resulting set $\{p_1,p_2,\dots\}\subset C$ by $\SD_k(C,f_K,\de)$. For any $p_i \in C$ define the Voronoi neighborhood as
$$V(p_i) = \{q \in C \mid d_{\MSG_k}(q,p_i) \leq d_{\MSG_k}(q,p_j) \text{ for any } j \neq i \}.$$
%\bs
\end{dfn}


\begin{figure}[H]
\centering
\includegraphics[scale=0.325]{images/ClusteringExample0.png}
\hspace{0.5cm}
\includegraphics[scale=0.65]{images/ClusteringExample2.png}

\caption{\textbf{Left:} Kernel density estimation computed on worm-type micelle.  \textbf{Right:} Voronoi cluster of Definition \ref{dfn:sparse_dense}.}
\label{fig:VoronoiClusterKDE}

\end{figure}


% =\{q\in \mathbb{V}(\MSG_k(C)) \vl d_k(q,p_i)\leq d_k(q,p_j) \text{ for any }j\neq i\}$$
Algorithm~\ref{alg:vertex_neighborhood} finds the $\de$-neighborhood of a vertex $p$ in a graph $G$, which will be applied for $G=\MSG_k(C)$.
Algorithm~\ref{alg:sparse_dense} will call Algorithm~\ref{alg:vertex_neighborhood} to update the function $\NDP$ that associates any point $q\in C$ with its nearest densest point $p_i\in\SD_k(C,f_K,\de)$.
So $\NDP$ helps split a cloud $C$ into Voronoi neighborhoods $V(p_i)$ of densest points as shown in Figure \ref{fig:VoronoiClusterKDE}.
%in the middle right pictures of Fig.~\ref{fig:branched} and~\ref{fig:cylindrical}.
 % in Definition~\ref{dfn:sparse_dense}.




\begin{lem}
\label{thmm:SD_time}
For a cloud $C\subset\R^m$ the computational complexity of Algorithm~\ref{alg:sparse_dense} to find the sparse subset $\SD_k(C,f_K,\delta)\subset C$ has the upper bound $O(k|C|\log |C||\SD_k(C,f_K,\delta)|)$.
\end{lem}
\begin{proof}
Algorithm~\ref{alg:vertex_neighborhood} handles each vertex $v\in\MSG_k(C)$ at most $|\SD_k(C,f_K,\delta)|$ times. 
Each of these vertices has $k$ neighbors.
During each iteration we add and remove a vertex from the heap $H$ at most once, which has the complexity $O(\log |C|)$.
Indeed, the balls with the radius $\de$ and centers at the points of $\SD_k(C,f_K,\delta)$ cover the whole graph $\MSG_k(C)$, so we handle $N$ points. 
%Now multiplying all of the given information we get the bound $O(D(K_f, \delta)_{\max}\cdot k \cdot|C| \log(|C|) $. 
All other steps of Algorithm~\ref{alg:sparse_dense} have smaller complexities than $O(k|C|\log |C||\SD_k(C,f_K,\delta)|)$. 
\end{proof}

\begin{algorithm}[H]
\caption{For a graph $G$~with~a~metric~$d$, find a~$\de$-neighborhood~of~$p$}
\label{alg:vertex_neighborhood}
\begin{algorithmic}[1]
\STATE \textbf{Input} : a graph $G$, a vertex $p$, a distance threshold $\delta>0$, arrays $\text{Dist}:\text{Vertices}(G) \rightarrow \mathbb{R}$ and Nearest  Dense Point $\NDP: \text{Vertices}(G)\to\text{Vertices}(G)$
\STATE \textbf{Output} : updated arrays $\text{Dist}$ and $\NDP$
\STATE Initialize the heap $H$ consisting of pairs in $\text{Vertices}(G) \times \mathbb{R}$ with the single pair $(p,0)$
\STATE Dist$(p) \leftarrow 0$, $\NDP(p) \leftarrow \emptyset$
\WHILE{the heap $H$ is not empty}
\STATE q $\leftarrow$ H.pop()
\FOR{\text{each vertex } $r$ \text{ adjacent to $q$ in the graph $G$}}
\STATE $t \leftarrow \text{Dist}(q) + d(r,q)  $
\IF{Dist$(r) > t$ and $t < \delta$}
\STATE Dist$(r) \leftarrow t$, $\NDP(r) \leftarrow q$
\STATE H.push$(r, t)$
\ENDIF
\ENDFOR 
\ENDWHILE
\end{algorithmic}
\end{algorithm}

\begin{dfn}[a dense tree $\text{DT}(C)$ on a cloud]
\label{dfn:dense_tree}
Let $\SD_k(C,f_K,\de)\subset C$ be a sparse subset of densest points from Definition~\ref{dfn:sparse_dense}.
Then a \emph{Dense Tree} $\text{DT}(C)\subset\R^m$ is a Minimum Spanning Tree on the vertex set $\SD_k(C,f_K,\de)$ with the distance measured by the path metric $d_{\MSG_k(C)}$ via $\MSG_k(C)$ in Definition~\ref{dfn:MSG_k}.
%The Optimized Dense Tree $\ODT(C)\subset\R^m$ is obtained from $\DT(C)$ by a gradient descent on the vertices of $\DT(C)$ to minimize the mean squared distance from all points of $C$.
\bs
\end{dfn}


%finds a sparse subset $\SD_k(C,K_f,\de)\subset C$ from Definition~\ref{dfn:sparse_dense}. 

\begin{algorithm}[H]
\caption{Find $\SD_k(C,f_K,\de)$ in Definition~\ref{dfn:sparse_dense}.}
\label{alg:sparse_dense}
\begin{algorithmic}[1]
\STATE \textbf{Input} : $\MSG_k(C)$, KDE $f_K$, $\delta>0$
\STATE \textbf{Output} : dense points $\{p_i\}=\SD_k(C,f_K,\de)$.
\STATE Initialize the arrays $\text{Dist}:C \rightarrow \mathbb{R}$, $\NDP:C \rightarrow C$.
\FOR {$p \in C$}
\STATE $\text{Dist}(p) \leftarrow +\infty$, $\NDP(p) \leftarrow p$.
\ENDFOR
\STATE Order $C$ in the descending order by the values of $f_K$.
\FOR{$p \in C$} 
\IF{Dist$(p) < +\infty$  }
\STATE Algorithm~\ref{alg:vertex_neighborhood} finds a $\de$-neighborhood of the vertex $p$ in $\MSG_k(C)$ and its neighbor $\NDP(p_i)$.
\ENDIF
\ENDFOR
\end{algorithmic}
\end{algorithm}

\begin{algorithm}[H]
\caption{Find $\DT(C)$ from Definition~\ref{dfn:dense_tree}.}
\label{alg:dense_tree}
\begin{algorithmic}[1]
\STATE \textbf{Input} : a cloud $C$, the graph $\MSG_k(C)$ from Definition~\ref{dfn:MSG_k}, $\SD_k(C,f_K, \delta)$ from Definition~\ref{dfn:sparse_dense}, the arrays $\text{Dist},\NDP$ from Algorithm~\ref{alg:sparse_dense}
\STATE \textbf{Output} : a Dense Tree $T=\DT(C)$
\STATE Let a graph $G$ consist of isolated vertices from $\SD_k(C,f_K, \delta)$
\FOR{edge $e = (u,v) \in \MSG_k(C)$}
\IF{$\NDP(u) \neq \NDP(v)$}
\IF{there is an edge $(\NDP(u), \NDP(v))\in T$}
\STATE Set $\text{Size}(e) = \min\{\text{Size}(e), \text{Dist}(u) + \text{Dist}(v) + \text{length}(e)\}$
\ELSE
\STATE Add to $T$ the new edge $(\NDP(u), \NDP(v))$ of the length $\text{Dist}(u) + \text{Dist}(v) + \text{length}(e)$
\ENDIF
\ENDIF
\ENDFOR
\STATE Compute a Minimum Spanning Tree of the graph $G$ by Boruvka's algorithm and output it as $\DT(C)$.
\end{algorithmic}
\end{algorithm}
%5================================

%The section explains the details of Stage~5 in Fig.~\ref{fig:pipeline} by introducing a Dense Tree $\text{DT}(C)$ in Definition~\ref{dfn:dense_tree}.



% \cite{pettie2002optimal}
%\begin{figure}[h]
%\centering
%\includegraphics[width=0.49\linewidth]{images/micelles/Christmas_cloud_DT.png}
%\includegraphics[width=0.49\linewidth]{images/micelles/Christmas_cloud_ODT.png}    
%\label{fig:Christmas}
%\caption{\textbf{Left}: Dense Tree $\DT(C)$ for a highly branched micelle represented by a cloud $C$.
%\textbf{Right}: Optimized Dense Tree $\ODT(C)$ over the same $C$.}
%\end{figure}

\begin{lem}
\label{thmm:dense_tree}
For a cloud $C$, the computational complexity of Algorithm~\ref{alg:dense_tree} is $O(k|C|\log |C|)$.
\end{lem}
\begin{proof}
The graph $\MSG_k(C)$ has $O(k|C|)$ edges.
To process each of these edges, we only make constant time operations. 
Thus the complexity is bounded by computing a Minimum Spanning Tree on a graph $G$ that has fewer edges and vertices than $\MSG_k(C)$.
So the total complexity is bounded by $O(k|C|\log |C|)$.
\end{proof}



\begin{figure}[H]
    \footnotesize
    \centering
    \begin{tikzpicture}[ >=stealth,
    node distance=3cm,
    auto
  ]
        \node [align = left, rectangle, 
    rounded corners, 
    % fill=black!10,
    draw=black, very thick] (start) {\textbf{Input: }a point \\ cloud $C$ in $\mathbb{R}^m$};
        %\node [below = 2.0cm of start] (startText) {(1) Original centaur};

     % above right

        \node [align = left,rectangle, 
    rounded corners, 
    % fill=black!10,
    draw=black, very thick, above right of= start] (A1) {\textbf{Stage 1: } \\ graph $\text{NN}_k(C)$ };
        %\node [below = 2.0cm of A1] (A1Text) {(2) Rotated centaur };
        
 
    %    \node [block, right = 0.5cm of BDL] (B1){One B1};
    	\node [align = left,rectangle, 
    rounded corners, 
    % fill=black!10,
    draw=black, very thick, below right of= start] (A3) {\textbf{Stage 3: } \\ KDE $f_K$ on $C$};
    
    	\node [align = left,rectangle, 
    rounded corners, 
    % fill=black!10,
    draw=black, very thick, right = 2.25cm of A1] (A2) {\textbf{Stage 2: } \\ graph $\MSG_k(C)$};
    
    	\node [align = left,rectangle, 
    rounded corners, 
    % fill=black!10,
    draw=black, very thick, right = 2.25cm of A3] (A4) {\textbf{Stage 4: } \\ subset $\text{D}\subset C$};
    
    \node [align = left,rectangle, 
    rounded corners, 
    % fill=black!10,
    draw=black, very thick, right = 6cm of start] (A5) {\textbf{Stage 5: } new \\ dense tree $\text{DT}(C)$};
    
     \node [align = left,rectangle, 
    rounded corners, 
    % fill=black!10,
    draw=black, very thick, right = 2.5cm of  A5] (A6) {\textbf{Stage 6: } optimized \\ dense tree $\text{ODT}(C)$};
    
    \path[draw, ->] (A1) -- node[midway, below, align = left] {\scriptsize adding edges \\ \scriptsize for connectivity}  (A2);
    \path[draw, ->] (start) -- node[midway, right = 0.25cm, align = left, font = \scriptsize] {$k$-neighbors \\ per point} (A1);
    \path[draw, ->] (start) -- node[midway, right = 0.25cm, align = left, font = \scriptsize] {parameter \\ function $f$}(A3);
    \path[draw, ->] (A2) -- node[midway, right = 0.25cm, align = left, font = \scriptsize] {use path metric \\ $d_k$ on $\text{SD} \subset \MSG_k(C)$} (A5);
    \path[draw, ->] (A4) -- node[midway, right = 0.25cm, align = left, font = \scriptsize] {minimally \\ span $\text{SD}$}(A5);
    \path[draw, ->] (A3) -- node[midway, below, align = left, font = \scriptsize] {distance \\ threshold $\delta$}  (A4);
    \path[draw, ->] (A5) -- node[midway, below, align = left, font = \scriptsize] {gradient \\ descent on \\ vertices of DT$(C)$}(A6);
    
    
    
    
        
%        \node [rectangle, 
%    rounded corners, 
%    % fill=black!10,
%    draw=black, very thick, above = 1.5cm of tmp ] (A3){DenseTree-algorithm};
%                %\node [below = 2.0cm of A3] (A3Text) {(3a) Affine transformation };
%
%        
%        \node [rectangle, 
%    rounded corners, 
%    % fill=black!10,
%    draw=black, very thick, below = 1.5cm of tmp] (end){AlphaReeb-algorithm};
%               % \node [below = 2.0cm of end] (endText) {(3b) Projective transformation };
%		
%		\node[rectangle, 
%    rounded corners, 
%    % fill=black!10,
%    draw=black, very thick, right of = tmp] (opt) {Optimization};
%		
%		\node[rectangle, 
%    rounded corners, 
%    % fill=black!10,
%    draw=black, very thick, right of = opt] (out) {Output};
%		
		

        
  %	    \path[draw, ->] (A1) -- A(2);
  %     \path[draw, ->] (start) -- (A1);
       % \path[->] (start) edge (A1);

%       % \path[draw, ->] (A1) -- (A2);
%        \path[draw, ->] (A1) -- (A3);
%        \path[draw, ->] (A1) -- (end);
   %     \path[draw, ->] (start) -- (A3);
        
%        \path[draw,->] (tmp) -- (opt);
%        \path[draw,->] (end) -- (opt);
%        \path[draw,->] (A3) -- (opt);
%        
%        \path[draw,->] (opt) -- (out);
        
        
                    
    \end{tikzpicture}
    \caption{Building an Optimized Dense Tree $\text{ODT}(C)$}
    \label{fig:pipeline}
    \end{figure}


Algorithm \ref{alg:DenseTreeAlgorithm} solves the problem \ref{pro:labela} in a near linear time.

\begin{restatable}[\textbf{Computational time guarantee}]{thmm}{CompTime}
\label{thmm:CompTime}
Assume that dense tree-algorithm is computed (Algorithm \ref{alg:DenseTreeAlgorithm}) on cloud $C$ having expansion constant $c$ ( Definition \ref{dfn:ExpansionConstantOk} ),  linkage expansion constant $c_l$ (Definition \ref{dfn:LinkageClusterConstant}) and clustering expansion constant $c_p$ (Definition \ref{dfn:ClusterExpansionConstant}). Let $k$ be the number of neighbor of the underlying $\MSG_k$ graph and let $\zeta$ be a constant releated to Kernel density estimation $f_K$ defined in Theorem \ref{thmm:KDE_time} . Assume that cloud $C$ consists of $N$ points. Then the computational complexity of the dense tree-algorithm has the following bound:
\begin{equation}
\label{eqa:CompTime}
\tag{\ref{thmm:CompTime}}
O(\max\{c^{16}, c^2_p c^2_l c^{10} , k \log(k) c^{12} , \log_2(\zeta) c^{10} , |D|\} N \log(N) \alpha(N)),
\end{equation}
where $|D|$ is the size of set $D$ in Stage (4) of the algorithm. If we assume condition of Theorem \ref{thmm:GHT}. Then $|D|$ has upper-bound as defined in Equation \ref{thmm:vcg}.
\end{restatable}

\begin{proof}
The complexity $(\ref{eqa:CompTime})$ is obtained by summing up complexities of the Algorithm \ref{alg:DenseTreeAlgorithm}:

\begin{table}[H]
\small
\begin{tabular}{|l|l|l|}
\hline
Stage                                             & Complexity & Theorem \\ \hline
Stage 1: Computation of $k$-nearest neighbors     & $O(c^{12} k \log(k) \log (N) $   &  Corollary \ref{cor:KNNComplexity}  \\
Stage 2: Computation of $\MST$ on clusters        & $O(\max\{c^6,c_p^2c^2_l) \}c^{10}n\log n\,\al(n))$    & Theorem \ref{thmm:MST_time}         \\
Stage 3: Computation of kernel density estimate & $ O(c^{10 + \log_2(\zeta)}\log(N) N) $          &  Corollary \ref{cor:KDE_timeQR}       \\
Stage 4: Finding sparse subset                    & $k |D| \log(N) N $           & Lemma \ref{thmm:SD_time}        \\
Stage 5: Building the dense-tree                  & $O(kN\log(N) $           &   Lemma \ref{thmm:dense_tree}      \\ \hline
\end{tabular}
\end{table}

\end{proof}

\begin{algorithm}[H]
\caption{Dense tree algorithm }
   \label{alg:DenseTreeAlgorithm}
\begin{algorithmic}
\small
    \STATE\textbf{Input} : any unorganized cloud of points $C\subset\R^m$.
    \STATE \textbf{Parameters}: a distance threshold $\de$, a number $k$ of nearest neighbors, a kernel density estimation $f_K$ on $C$, a learning rate and number of iterations for a gradient descent by Tensorflow \cite{TensorflowSGD}. 
    \STATE \textbf{Stage 1:} Given a cloud $C\subset\R^m$, find a $k$-th nearest neighbor graph $\NN_k(C)$ from Definition~\ref{dfn:MSG_k}. 
    \STATE \textbf{Stage 2:} Extend the $k$-th nearest neighbor graph $\NN_k(C)$ to a Minimum Spanning Graph $\MSG_k(C)$.
    \STATE \textbf{Stage 3:} Compute a Kernel Density Estimation $f_K$ from Definition~\ref{dfn:KDE} on points of the cloud $C$. 
    \STATE \textbf{Stage 4:} Find a sparse subset $D\subset C$ of densest points separated by a distance threshold $\de$ by Algorithm~\ref{alg:sparse_dense}.
    \STATE \textbf{Stage 5:} Build a dense tree $\text{DT}(C)\subset\R^m$ as a Minimum Spanning Tree on $D$ with straight line edges using the metric $d_{\MSG_k(C)}$ on $\MSG_k(C)$.
    \STATE \textbf{Stage 6:} Get an Optimized Dense Tree $\ODT(C)\subset\R^m$ by a stochastic gradient descent on vertices of $\text{DT}(C)\subset\R^m$, which minimizes the mean squared distance from points of $C$ to $\text{DT}(C)$.
\end{algorithmic}
\end{algorithm}


%
%The points of $D$ are afterwards connected by a minimum spanning tree on $D$ using the metric based on graph $\MSG_k$ to form a dense tree $\text{DT}(C)$ in Definition~\ref{dfn:dense_tree}.
%For (\ref{pro:reconstruction}a), a gradient descent on vertices of $\text{DT}(C)$ minimizes a mean squared distance from $C$ to get an Optimized Dense Tree $\ODT(C)$. 
%Fig.~\ref{fig:pipeline} shows the algorithm pipeline.
%%\smallskip


\begin{figure}[H]
    \centering

\begin{subfigure}{.33\textwidth}
  \centering
  % include first image
  \includegraphics[width=.9\linewidth]{images/micelles/cylindrical_cloud.png}  
  \caption{\scriptsize Input cloud $C$ from the dataset of micelles, where each point is a molecule. }
  \label{fig:sub-first}
\end{subfigure}
\begin{subfigure}{.33\textwidth}
  \centering
  % include second image
  \includegraphics[width=.9\linewidth]{images/micelles/cylindrical_MSG_k.png}  
  \caption{A connected graph $\MSG_k(C)$, see Definition~\ref{dfn:MSG_k}. }
  \label{fig:sub-second}
\end{subfigure}    
\begin{subfigure}{.33\textwidth}
  \centering
  % include second image
  \includegraphics[width=.9\linewidth]{images/micelles/cylindrical_cloud_density.png}  
  \caption{Density of points on a blue-red scale.  }
  \label{fig:sub-second}
\end{subfigure} 
\begin{subfigure}{.33\textwidth}
  \centering
  % include first image
  \includegraphics[width=.9\linewidth]{images/micelles/cylindrical_clusters.png}  
  \caption{Clusters around sparsified densest points. }
  \label{fig:sub-first}
\end{subfigure}
\begin{subfigure}{.33\textwidth}
  \centering
  % include second image
  \includegraphics[width=.9\linewidth]{images/micelles/cylindrical_cloud_DT.png}  
  \caption{A brown Dense Tree $\DT(C)$ on densest points. }
  \label{fig:sub-second}
\end{subfigure}    
\begin{subfigure}{.33\textwidth}
  \centering
  % include second image
  \includegraphics[width=.9\linewidth]{images/micelles/cylindrical_cloud_ODT.png}  
  \caption{Red Optimized Dense Tree $\ODT(C)$}
  \label{fig:sub-second}
\end{subfigure}   
    
% \textbf{Top left}: input cloud $C$ from the dataset of micelles, where each point is a molecule. 
%\textbf{Top middle}: a connected graph $\MSG_k(C)$, see Definition~\ref{dfn:MSG_k}. 
%\textbf{Top right}: density of points on a blue-red scale. 
%\textbf{Bottom left}: clusters around sparsified densest points. 
%\textbf{Bottom middle}: a brown Dense Tree $\DT(C)$ on densest points. 
%\textbf{Bottom right}: red Optimized Dense Tree $\ODT(C)$.     
    
%    \includegraphics[width=0.33\linewidth]{images/micelles/cylindrical_cloud.png}
%    \includegraphics[width=0.33\linewidth]{images/micelles/cylindrical_MSG_k.png}
%    \includegraphics[width=0.33\linewidth]{images/micelles/cylindrical_cloud_density.png}
%    \includegraphics[width=0.33\linewidth]{images/micelles/cylindrical_clusters.png}
%\includegraphics[width=0.33\linewidth]{images/micelles/cylindrical_cloud_DT.png}
%\includegraphics[width=0.33\linewidth]{images/micelles/cylindrical_cloud_ODT.png}

\end{figure}
\begin{figure}[H]
\centering

\begin{subfigure}{.33\textwidth}
  \centering
  % include first image
  \includegraphics[width=.9\linewidth]{images/micelles/branched_cloud.png}  
  \caption{\scriptsize Input cloud $C$ from the dataset of micelles, where each point is a molecule. }
  \label{fig:sub-first}
\end{subfigure}
\begin{subfigure}{.33\textwidth}
  \centering
  % include second image
  \includegraphics[width=.9\linewidth]{images/micelles/branched_MSG_kd.png}  
  \caption{A connected graph $\MSG_k(C)$, see Definition~\ref{dfn:MSG_k}. }
  \label{fig:sub-second}
\end{subfigure}    
\begin{subfigure}{.33\textwidth}
  \centering
  % include second image
  \includegraphics[width=.9\linewidth]{images/micelles/branched_cloud_densityy.png}  
  \caption{Density of points on a blue-red scale.  }
  \label{fig:sub-second}
\end{subfigure} 
\begin{subfigure}{.33\textwidth}
  \centering
  % include first image
  \includegraphics[width=.9\linewidth]{images/micelles/branched_clusters.png}  
  \caption{Clusters around sparsified densest points. }
  \label{fig:sub-first}
\end{subfigure}
\begin{subfigure}{.33\textwidth}
  \centering
  % include second image
  \includegraphics[width=.9\linewidth]{images/micelles/branched_cloud_DT.png}  
  \caption{A brown Dense Tree $\DT(C)$ on densest points. }
  \label{fig:sub-second}
\end{subfigure}    
\begin{subfigure}{.33\textwidth}
  \centering
  % include second image
  \includegraphics[width=.9\linewidth]{images/micelles/branched_cloud_ODT.png}  
  \caption{Red Optimized Dense Tree $\ODT(C)$}
  \label{fig:sub-second}
\end{subfigure}   

%
%\includegraphics[width=0.33\linewidth]{images/micelles/branched_cloud.png}
%\includegraphics[width=0.33\linewidth]{images/micelles/branched_MSG_kd.png}
%\includegraphics[width=0.33\linewidth]{images/micelles/branched_cloud_densityy.png}
%\includegraphics[width=0.33\linewidth]{images/micelles/branched_clusters.png}
%\includegraphics[width=0.33\linewidth]{images/micelles/branched_cloud_DT.png}
%\includegraphics[width=0.33\linewidth]{images/micelles/branched_cloud_ODT.png}    
%\caption{
%\textbf{Top left}: input cloud $C$ from the dataset of micelles, where each point is a molecule. 
%\textbf{Top middle}: a connected graph $\MSG_k(C)$, see Definition~\ref{dfn:MSG_k}. 
%\textbf{Top right}: density of points on a blue-red scale. 
%\textbf{Bottom right}: clusters around sparsified densest points. 
%\textbf{Bottom middle}: a brown Dense Tree $\DT(C)$ on densest points. 
%\textbf{Bottom left}: red Optimized Dense Tree $\ODT(C)$. 
%}
\caption{Stages of Algorithm \ref{alg:DenseTreeAlgorithm} on branched dataset}
\label{fig:branched}
\end{figure}

%We are now ready to prove the main theoretical result regarding the computational complexity of the Algorithm. Theorems~\ref{thmm:MST_time}, \ref{thmm:KDE_time}, \ref{thmm:SD_time}, \ref{thmm:dense_tree} imply this estimate. 
%
%\CompTime*


%\begin{cor}
%\label{cor:dense_tree}
%The complexity of a Dense Tree $\DT(C)$ is a sum of complexities of Stages~1-5, which is almost linear in the number $n$ of points of $C$. 
%\bs
%\end{cor}




%\section{Unallocated}
% % Add a label in case you want to refer to the chapter.
%Real data is often given in the form of unorganized clouds of points. Most skeletonization principles are based on the 3-step framework. In the first step, we compute the underlying graph structure of the point cloud. This could be for example Delaunay triangulation or $k$-nearest neighborhood graph built on a given point cloud. In the next step we use a shape-detection algorithm, which extracts the essential information from the underlying graph structure. For example, in the graph-recognition task, we wish that the shape-detection step retrieves us a graph of desired form e.g. a graph that is homeomorphic to the ideal graph built on the point cloud. In the final step we post-process obtained shape into optimized form e.g. given an initial graph the algorithm moves its vertices to the position that minimizes mean square error to the original point cloud. 
%%
%%
%%\begin{figure}
%%\centering
%%\begin{tikzpicture}
%%  [node distance=.8cm,
%%  start chain=going below,]
%%     \node[punktchain, join] (intro) {Point cloud};
%%     \node[punktchain, join] (probf)      {Underlying graph};
%%     \node[punktchain, join] (investeringer)      {Algorithm};
%%     \node[punktchain, join] (perfekt) {Post processing};
%%     \node[punktchain, join, ] (emperi) {Final output};
%%     
%%     
%%   %   \node (asym) [punktchain ]  {Asymmetrisk information};
%%   %   \begin{scope}[start branch=venstre,
%%        %We need to redefine the join-style to have the -> turn out right
%%   %     every join/.style={->, thick, shorten <=1pt}, ]
%%   %     \node[punktchain, on chain=going left, join=by {<-}]
%%  %          (risiko) {Risiko og gamble};
%%  %    \end{scope}
%%  %    \begin{scope}[start branch=hoejre,]
%%  %    \node (finans) [punktchain, on chain=going right] {Det finansielle system};
%%  %  \end{scope}
%%  %\node[punktchain, join,] (disk) {Det imperfekte finansielle marked};
%%  %\node[punktchain, join,] (makro) {InvesteringsmÃ¦ssige konsekvenser};
%%  %\node[punktchain, join] (konk) {Konklusion};
%%  % Now that we have finished the main figure let us add some "after-drawings"
%%  %% First, let us connect (finans) with (disk). We want it to have
%%  %% square corners.
%% % \draw[|-,-|,->, thick,] (finans.south) |-+(0,-1em)-| (disk.north);
%%  % Now, let us add some braches. 
%%  %% No. 1
%% % \draw[tuborg] let
%% %   \p1=(risiko.west), \p2=(finans.east) in
%% %   ($(\x1,\y1+2.5em)$) -- ($(\x2,\y2+2.5em)$) node[above, midway]  {Teori};
%%  %% No. 2
%% % \draw[tuborg, decoration={brace}] let \p1=(disk.north), \p2=(makro.south) in
%% %   ($(2, \y1)$) -- ($(2, \y2)$) node[tubnode] {Analyse};
%%  %% No. 3
%% % \draw[tuborg, decoration={brace}] let \p1=(perfekt.north), \p2=(emperi.south) in
%% %   ($(2, \y1)$) -- ($(2, \y2)$) node[tubnode] {Problemfelt};
%%  \end{tikzpicture}
%%  
%%  \caption{Data-skeletonization process steps illustrated}
%%
%%
%%\end{figure}






%\subsection{Underlying graph experiments}

%Experiments of $\text{MSG}_k$ are presented below:



%\subsection{Post-proccess optimization}



\section{an Optimized Dense Tree $\ODT(C)$}
\label{sec:ODT}

The section describes a stochastic gradient descent at Stage 6 in Fig.~\ref{fig:pipeline}, which converts a straight-line Dense Tree $\DT(C)\subset\R^m$ from Definition~\ref{dfn:dense_tree} into an Optimized Dense Tree $\ODT(C)\subset\R^m$. The idea is to apply stochastic gradient descent on the set of vertices of the given graph by moving vertices slowly towards positions that minimize the given error measure. The algorithm is ran by defining the first approximation graph
 $\omega_0$ to be the dense-tree $\DT(C)$. During every iteration we start by searching for a nearest line segment of every cloud point of $C$. This is used to compute the gradient of mean square error of Definition \ref{dfn:errors} that will be used to construct $\omega_n$ from $\omega_{n-1}$.
 
 When we are dealing with large graphs, it takes too much time and memory to find a nearest line segment for every single point cloud. 
We fix this problem by specifying relatively set of closest edges for every cloud point. If such collections are chosen wisely the end result should be a relatively good approximation of the optimized skeleton that was ran without this extra constrain. This allocation procedure is explained in Definition \ref{dfn:AllocationOptimization}.

\begin{dfn}
\label{dfn:AllocationOptimization}

Let $V(p_i)$ be Voronoi-regions obtained from Algorithm \ref{alg:vertex_neighborhood}, where $p_i\in\SD_k(C,f_K,\de)$. Let Star$(p_i, \text{DT}(C))$ be a set of all the edges belonging to $\text{DT}(C)$ which have point $p_i$ as one of their vertices. Define allocation $A:C \rightarrow \text{Set}(\mathbb{E}(\text{DT}(C)))$ as a function which maps every cloud point $q \in C$ to a set of edges which are close to it by defining
 $$A(q) = \text{Star}(p_i,  \text{DT}(C)) \mid \text{ where } q \in V(p_i)$$
 
 %for every cloud point $q \in C$.  

\end{dfn}



\begin{dfn}[geometric errors MSE and AMSE]
\label{dfn:errors}
For a tree $T\subset\R^m$ approximating a cloud $C\subset\R^m$ of $n$ points, let $d(p,T)$ be the Euclidean distance from $p\in C$ to its closest edge of $T$.
The \emph{Mean Square Error} is
$\MSE(C,T)=\dfrac{1}{n}\sum\limits_{p\in C} d(p,T)$. 
When given an allocation $A:C \rightarrow \text{Set}(\mathbb{E}(\text{DT}(C)))$ we define Allocated Mean Square Error as 
$\text{AMSE}(C,T,A) =\dfrac{1}{n}\sum\limits_{p\in C} d(p,A(p))$






%The \emph{Maximum Distance} error is defined as $\MD(C,T)=\max\limits_{p\in C} d(p,T)$.  
\bs


\end{dfn}
 

 
 % The process is illustrated in Figure \ref{fig:optimizationSteps}: 
%
%\begin{figure}[H]
%\begin{subfigure}{.5\textwidth}
%  \centering
%  % include first image
%  \includegraphics[width=.8\linewidth]{images/KDESequence/out0fix.png}  
%  \caption{First approximation of a point cloud}
%  \label{fig:sub-first}
%\end{subfigure}
%\begin{subfigure}{.5\textwidth}
%  \centering
%  % include second image
%  \includegraphics[width=.8\linewidth]{images/KDESequence/out20fix.png}  
%  \caption{Skeleton after 20 iterations of Algorithm \ref{alg:SGDOptSkeleton}}
%  \label{fig:sub-second}
%\end{subfigure}
%
%\begin{subfigure}{.5\textwidth}
%  \centering
%  % include first image
%  \includegraphics[width=.8\linewidth]{images/KDESequence/out40fix.png}  
%  \caption{Skeleton after 40 iterations of Algorithm \ref{alg:SGDOptSkeleton}}
%  \label{fig:sub-third}
%\end{subfigure}
%\begin{subfigure}{.5\textwidth}
%  \centering
%  % include second image
%  \includegraphics[width=.8\linewidth]{images/KDESequence/out60fix.png}  
%  \caption{The final output of Algorithm \ref{alg:SGDOptSkeleton}}
%  \label{fig:sub-fourth}
%\end{subfigure}
%
%\caption{Put your caption here}
%\label{fig:optimizationSteps}
%
%%\newline
%
%\end{figure}



%\begin{subfigure}{.48\textwidth}
%  \centering
%  % include second image
%  \includegraphics[width=.95\linewidth]{images/stars/star5_cloud_DT.png}  
%  \caption{Dense tree $\text{DT}(C)$ built on Star$(5)$-tree.}
%  \label{fig:subFig-second}
%\end{subfigure}
%\begin{subfigure}{.48\textwidth}
%  \centering
%  % include second image
%  \includegraphics[width=.95\linewidth]{images/stars/star5_cloud_ODT.png}  
%  \caption{Optimized Dense tree $\text{ODT}(C)$ built on Star$(5)$-tree.}
%  \label{fig:subFig-second}
%\end{subfigure}

%\includegraphics[width=0.49\linewidth]{images/stars/star4_cloud_DT.png}
%\includegraphics[width=0.49\linewidth]{images/stars/star4_cloud_ODT.png} 
   
%\label{fig:star4}
%\caption{Optimization process on real micelles in $\R^3$}
%\end{figure}

%\begin{figure}[H]
%\centering
%\includegraphics[width=0.49\linewidth]{images/stars/star5_cloud_DT.png}
%\includegraphics[width=0.49\linewidth]{images/stars/star5_cloud_ODT.png}    
%\label{fig:star5}
%\caption{Optimization process on real micelles in $\R^3$}
%\end{figure}
%%\medskip

%\textbf{Left}: Dense Tree $\DT(C)$ for a random cloud $C$ sampled around a 5-star graph in $\R^3$.
%\textbf{Right}: Optimized Dense Tree $\ODT(C)$ over the same cloud $C$.






%Algorithm~\ref{alg:SGD} outlines a stochastic gradient descent  by the Tensorflow \cite{TensorflowSGD}, which allowed us to use GPU. 
%\medskip

%The default parameters in Algorithm~\ref{alg:SGD} below will be used for all experiments in section~\ref{sec:experiments}.

\begin{algorithm}[H]
\caption{Skeleton optimization algorithm}
\label{alg:SGDOptSkeleton}
\begin{algorithmic}[1]
\STATE \textbf{Input} : Graph $T$, learning rate $\eta$, number of iterations $I$, allocation $A$
\STATE \textbf{Output: } Optimized graph
   \STATE Set $\omega_0 = T$
   \FOR{$i \in [1,I]$}
   \STATE $\omega_{n+1} = \omega_n - \eta \nabla \text{A}\MSE(C,\omega_n,A)$
   \ENDFOR
   \STATE \textbf{return } $\omega_{n+1}$
\end{algorithmic}
\end{algorithm}


\begin{figure}[H]

\centering
\begin{subfigure}{.24\textwidth}
 
  % include first image
  \includegraphics[width=.95\linewidth]{images/SequenceOptimization/out0fixed.png}  
  \caption{First approximation}
  \label{fig:subFig-first1}
\end{subfigure}
\begin{subfigure}{.24\textwidth}
  \centering
  % include second image
  \includegraphics[width=.95\linewidth]{images/SequenceOptimization/out20fixed.png}  
  \caption{Graph after 20 iterations}
  \label{fig:subFig-second2}
\end{subfigure}
\begin{subfigure}{.24\textwidth}
  \centering
  % include second image
  \includegraphics[width=.95\linewidth]{images/SequenceOptimization/out40fixed.png}  
  \caption{Graph after 40 iterations}
  \label{fig:subFig-second3}
\end{subfigure}
\begin{subfigure}{.24\textwidth}
  \centering
  % include second image
  \includegraphics[width=.95\linewidth]{images/SequenceOptimization/out60fixed.png}  
  \caption{Final optimized graph}
  \label{fig:subFig-second4}

  
\end{subfigure}

  \caption{Optimization process of Algorithm \ref{alg:SGDOptSkeleton} on randomly generated graph and randomly generated cloud}
  \label{fig:OptimizationProcess}

%\caption{ }

\end{figure}


%
%Fig.~\ref{fig:star4}
%show how Algorithm~\ref{alg:SGDOptSkeleton} substantially improves Dense Trees $\DT(C)$ to Optimized Dense Trees $\ODT(C)$, which `sit deeper inside' their clouds $C$.


%\begin{figure}[H]
%\centering
%\includegraphics[width=0.49\linewidth]{images/KDESequence/out0fix.png}
%\includegraphics[width=0.49\linewidth]{images/KDESequence/out20fix.png}
%\includegraphics[width=0.49\linewidth]{images/KDESequence/out40fix.png}
%\includegraphics[width=0.49\linewidth]{images/KDESequence/out60fix.png} 
%\caption{Optimization of randomly generated graph
%}
%\label{fig:branched}
%\end{figure}
%





%\begin{figure}[H] 
%        \centering
%        \begin{subfigure}{0.475\textwidth}  
%            \centering
%            \includegraphics[width=\linewidth]{images/KDESequence/out0fix.png}
%            \caption[]%
%            {{\small Network 1}}    
%            \label{fig:mean and std of net14}
%        \end{subfigure}
%        \hfill
%        \begin{subfigure}
%            \centering 
%            \includegraphics[width=\linewidth]{images/KDESequence/out20fix.png}
%            \caption[]%
%            {{\small Network 2}}    
%            \label{fig:mean and std of net24}
%        \end{subfigure}
%        \vskip\baselineskip
%        \begin{subfigure}
%            \centering 
%            \includegraphics[width=\linewidth]{images/KDESequence/out40fix.png}
%            \caption[]%
%            {{\small Network 3}}    
%            \label{fig:mean and std of net34}
%        \end{subfigure}
%        \hfill
%        \begin{subfigure}
%            \centering 
%            \includegraphics[width=\linewidth]{images/KDESequence/out60fix.png} 
%            \caption[]%
%            {{\small Network 4}}    
%            \label{fig:mean and std of net44}
%        \end{subfigure}
%        \caption[ The average and standard deviation of critical parameters ]
%        {\small The average and standard deviation of critical parameters: Region R4} 
%        \label{fig:mean and std of nets}
%\end{figure}






%The experiments linking learning rate to number of iterations were performed for complex randomized tree-graphs of Figure \ref{fig:biggraphs}.

%\begin{figure}[H]
%%\resizebox{0.49\columnwidth}{!}{
%%\begin{tikzpicture}
%%\begin{axis}[xlabel = Number of iterations, ylabel = Mean Square Error,grid, legend style={at={(0.5,0.5)},anchor=center}, every axis plot/.append style={ultra thick}]
%%% [black,mark = *]
%%\addplot[yellow] table [x=Iteration, mark=none, y=lr5, col sep=comma] {tables/Optimization/SmallGraphOpt.csv};
%%\addlegendentry{LearningRate = 5}
%%\addplot[orange] table [x=Iteration, mark=none, y=lr10, col sep=comma] {tables/Optimization/SmallGraphOpt.csv};
%%\addlegendentry{LearningRate = 10}
%%\addplot[black] table [x=Iteration, mark=none, y=lr15, col sep=comma] {tables/Optimization/SmallGraphOpt.csv};
%%\addlegendentry{LearningRate = 15}
%%\addplot[red] table [x=Iteration, mark=none, y=lr20, col sep=comma] {tables/Optimization/SmallGraphOpt.csv};
%%\addlegendentry{LearningRate = 20}
%%\addplot[blue] table [x=Iteration, mark=none, y=lr25, col sep=comma] {tables/Optimization/SmallGraphOpt.csv};
%%\addlegendentry{LearningRate = 25}
%%\addplot[green] table [x=Iteration, mark=none, y=lr30, col sep=comma] {tables/Optimization/SmallGraphOpt.csv};
%%\addlegendentry{LearningRate = 30}
%%
%%
%%\end{axis}
%%\end{tikzpicture}
%%}
%% legend style={at={(0.5,-0.1)},anchor=north}
%\centering
%\begin{tikzpicture}
%\begin{axis}[xlabel = Number of iterations, ylabel = Mean Square Error,grid, every axis plot/.append style={ultra thick}]
%% [black,mark = *]
%\addplot[yellow] table [x=Iteration, mark=none, y=lr5, col sep=comma] {tables/Optimization/BigGraphOpt.csv};
%%\addlegendentry{LearningRate(5)}
%\addplot[orange] table [x=Iteration, mark=none, y=lr10, col sep=comma] {tables/Optimization/BigGraphOpt.csv};
%%\addlegendentry{LearningRate(10)}
%\addplot[black] table [x=Iteration, mark=none, y=lr15, col sep=comma] {tables/Optimization/BigGraphOpt.csv};
%%\addlegendentry{LearningRate(15)}
%\addplot[red] table [x=Iteration, mark=none, y=lr20, col sep=comma] {tables/Optimization/BigGraphOpt.csv};
%%\addlegendentry{LearningRate(20)}
%\addplot[blue] table [x=Iteration, mark=none, y=lr25, col sep=comma] {tables/Optimization/BigGraphOpt.csv};
%%\addlegendentry{LearningRate(25)}
%\addplot[green] table [x=Iteration, mark=none, y=lr30, col sep=comma] {tables/Optimization/BigGraphOpt.csv};
%%\addlegendentry{LearningRate(30)}
%
%
%\end{axis}
%\end{tikzpicture}
%
%\caption{Optimization rates }
%\end{figure}




\section{Experiments}

%To generate the datasets we are first required to generate sample graphs $T$ that have properties described in Theorem \ref{thmm:GHT}, such as relatively big %minimal angle $\theta(T) > \frac{\pi}{4}$, adequate size of edges and sufficient minimal distance between non-adjacent edges. This will be done using %Algorithm \ref{alg:ExperimentalGraphGeneration} . 

To conduct experiments we need to generate data. We construct sensible tree $T \in \mathcal{G}(l_{\max}, l_{\min}, \theta, w)$ defined in Definition \ref{dfn:SensibleGraph}. The construction will be conducted in an inductive manner, by starting with a graph containing only a single vertex, that is placed in origin. Assume that we have constructed a tree $T_{n-1}$ consisting of $n-1$ vertices. Having this graph we simply generate a new random vertex close to $T_{n-1}$ and connect it to a nearby vertex of $T_{n-1}$. This is accepted as graph $T_n$ if the newly constructed graph doesn't invalidate the minimal constraints of $\mathcal{G}(l_{\max}, l_{\min}, \theta, w)$. In order to have graphs that contain higher degree vertices in the collection, we give areas located close to higher degree vertices of $T_{n-1}$ a priority when we generate new vertices. 


After generating graphs we proceed by creating a point cloud around it. The point cloud is generated using the Monte-Carlo method, in a way where we generate points $p$ in bounding rectangle of the graph $T$ and accept them only if their directed hausdorff distance $d_{\overleftarrow{H}}(p,T) \leq \epsilon$, where $\epsilon$ is the generation error bound.  


%\begin{figure}[H]
%\label{fig:biggraphs}
%\centering
%\includegraphics[scale=1.0]{images/BigGraph1.png}
%\includegraphics[scale=1.0]{images/Graph2.png}
%\includegraphics[scale=1.0]{images/pic7.png}
%
%
%\caption{Example graphs generated from Algorithm \ref{alg:GraphGeneration} in $\mathbb{R}^2$ marked with red-color and a random point cloud marked with blue color. }
%\end{figure}



\begin{algorithm}[H]
\caption{Graph generation algorithm}
\label{alg:GraphGeneration}
\begin{algorithmic}[1]
\STATE \textbf{Input} : Number of vertices $n$, constants: $\theta$, $l_{\max}$, $l_{\min}$ and $w$. 
\STATE \textbf{Output: } Graph generated
\STATE Define graph $G: \mathbb{V}(G) = \{0\}, \mathbb{E}(G) = \emptyset$ 
\WHILE {$\mathbb{V}(G) < n$}
\STATE Choose random vertex $v$ using distribution $\mathbb{D}(v) = \dfrac{\text{Degree}(v)}{\sum_{u \in G}\text{Degree}(u)}$
\STATE Choose uniform random point $p \in \bar{B}(v,l_{\max}) \setminus \bar{B}(v,l_{\min})$
\IF {$G \cup [p,v])$ doesn't invalidate constraints}
\STATE Set $\mathbb{V}(G) = \mathbb{V}(G) \cup \{p\}$ and $\mathbb{E}(G) = \mathbb{E}(G) \cup \{(p,v)\}$ 
%\STATE Set $\mathbb{E}(G) = \mathbb{E}(G) \cup \{(p,v)\}$ 
\ENDIF
\ENDWHILE
\STATE \textbf{return} G
%   \STATE Set $\omega_0 = T$
%   \FOR{$i \in [1,I]$}
%   \STATE $\omega_{n+1} = \omega_n - \eta \nabla \text{A}\MSE(C,\omega_n,A)$
%   \ENDFOR
%  \STATE \textbf{return } $\omega_{n+1}$
\end{algorithmic}
\end{algorithm}




%\subsection{Underlying graph experiments}
%\label{sec:UnderlyingGraphExp}
The goal of Experiment \ref{expe:UnderlyingGraph} is to show that there exists values $k \in \Z$ for which the underlying graph $\MSG_k$ is a good $\gamma$-approximation of $(T,C) $.

\begin{expe}
\label{expe:UnderlyingGraph}
We computed 100 random $\text{Star}(4,\frac{\pi}{4})$. For every graph we generated a point cloud $C$ consisting of $\{400, 800, 1200,1600, 2000, 2400\}$ points. For every point cloud we computed 16 different $\MSG_k$ graphs for every integer $k \in [1,15]$. In each obtained graph we measured the $\gamma$-constant, maximal edge length, number of edges and the computational time. The results of the experiments are illustrated in Figures \ref{fig:UnderlyingGraphExp1} and \ref{fig:UnderlyingGraphExp2}.
\end{expe}

After performing experiments we obtained the following results:

\begin{figure}[H]
\resizebox{0.49\columnwidth}{!}{
\begin{tikzpicture}
\begin{axis}[xlabel = $k$-value, ylabel = $\gamma$-constant of $\MSG_k$ graph, grid, legend style={font = \small, at={(0.75,0.60)},anchor=center}, every axis plot/.append style={ultra thick}]
% [black,mark = *]
\addplot[yellow] table [x=features, y=Gamma, col sep=comma] {tables/MSGK/Point100.csv};
\addlegendentry{400 Points}
\addplot[orange] table [x=features, y=Gamma, col sep=comma] {tables/MSGK/Point200.csv};
\addlegendentry{800 Points}
\addplot[black] table [x=features, y=Gamma, col sep=comma] {tables/MSGK/Point300.csv};
\addlegendentry{1200 Points}
\addplot[red] table [x=features, y=Gamma, col sep=comma] {tables/MSGK/Point400.csv};
\addlegendentry{1600 Points}
\addplot[blue] table [x=features, y=Gamma, col sep=comma] {tables/MSGK/Point500.csv};
\addlegendentry{2000 Points}
\addplot[green] table [x=features, y=Gamma, col sep=comma] {tables/MSGK/Point600.csv};
\addlegendentry{2400 Points}


\end{axis}
\end{tikzpicture}
}
\resizebox{0.49\columnwidth}{!}{
\begin{tikzpicture}
\begin{axis}[xlabel = $k$-value, ylabel = max length of edge in graph $\MSG_k$, grid, every axis plot/.append style={ultra thick}]
%\addplot[black,mark = *] table [x=features, y=maxLength, col sep=comma] {UnderlyingGraph/finalOutT2.csv};
\addplot[yellow] table [x=features, y=maxLength, col sep=comma] {tables/MSGK/Point100.csv};
\addplot[orange] table [x=features, y=maxLength, col sep=comma] {tables/MSGK/Point200.csv};
\addplot[black] table [x=features, y=maxLength, col sep=comma] {tables/MSGK/Point300.csv};
\addplot[red] table [x=features, y=maxLength, col sep=comma] {tables/MSGK/Point400.csv};
\addplot[blue] table [x=features, y=maxLength, col sep=comma] {tables/MSGK/Point500.csv};
\addplot[green] table [x=features, y=maxLength, col sep=comma] {tables/MSGK/Point600.csv};
\end{axis}
\end{tikzpicture}
}
\caption{Results of Experiments \ref{expe:UnderlyingGraph}: Tests performed on $\text{Star}4$ graphs with different densities. \textbf{Left:} dependence of $\gamma$ constant on parameter $k$ of $\MSG_k$ graph. \textbf{Right:} maximum edge length found in graph $\MSG_k$}
\label{fig:UnderlyingGraphExp1}
\end{figure}

\begin{figure}[H]
\resizebox{0.49\columnwidth}{!}{
\begin{tikzpicture}
\begin{axis}[xlabel = $k$-value, ylabel = number of edges of $\MSG_k$,grid, every axis plot/.append style={ultra thick}]
%\addplot[black,mark = *] table [x=features, y=NumEdges, col sep=comma] {UnderlyingGraph/finalOutT2.csv};
\addplot[yellow] table [x=features, y=NumVertices, col sep=comma] {tables/MSGK/Point100.csv};
\addplot[orange] table [x=features, y=NumVertices, col sep=comma] {tables/MSGK/Point200.csv};
\addplot[black] table [x=features, y=NumVertices, col sep=comma] {tables/MSGK/Point300.csv};
\addplot[red] table [x=features, y=NumVertices, col sep=comma] {tables/MSGK/Point400.csv};
\addplot[blue] table [x=features, y=NumVertices, col sep=comma] {tables/MSGK/Point500.csv};
\addplot[green] table [x=features, y=NumVertices, col sep=comma] {tables/MSGK/Point600.csv};
\end{axis}
\end{tikzpicture}}
\resizebox{0.49\columnwidth}{!}{\begin{tikzpicture} 
\begin{axis}[xlabel = $k$-value, ylabel = average building time of $\MSG_k$ (ms),grid, every axis plot/.append style={ultra thick}]
%\addplot[black,mark = *] table [x=features, y=Time, col sep=comma] {UnderlyingGraph/finalOutT2.csv};
\addplot[yellow] table [x=features, y=Time, col sep=comma] {tables/MSGK/Point100.csv};
\addplot[orange] table [x=features, y=Time, col sep=comma] {tables/MSGK/Point200.csv};
\addplot[black] table [x=features, y=Time, col sep=comma] {tables/MSGK/Point300.csv};
\addplot[red] table [x=features, y=Time, col sep=comma] {tables/MSGK/Point400.csv};
\addplot[blue] table [x=features, y=Time, col sep=comma] {tables/MSGK/Point500.csv};
\addplot[green] table [x=features, y=Time, col sep=comma] {tables/MSGK/Point600.csv};

\end{axis}
\end{tikzpicture}}

\caption{Results of Experiments \ref{expe:UnderlyingGraph}: Tests performed on $\text{Star}4$ graphs with different densities.\textbf{Left:} dependence of number of edges $\MSG_k$ depending on parameter $k$. \textbf{Right:} building time of graph $\MSG_k$.}
\label{fig:UnderlyingGraphExp2}
\end{figure}

% \subsection{Skeleton optimization experiments}


%


%\subsection{Success rate experiments}

We will now compare the Optimized dense tree algorithm with two other Graph-clustering-based skeletonization algorithms: AlphaReeb and Mapper. The main challenge of the task is to correctly identify degree $k > 3$ branch points. We define concept of degree list recognition rate in Definition \ref{dfn:recognitionSuccess}.

%To make the comparison fair we use the same underlying graph and perform the same post-process optimization on each of the algorithms. 

\begin{dfn}\label{dfn:recognitionSuccess}[Degree list recognition]
Given graphs $G$ and $H$, where $G$ is an attempted reconstruction of graph $H$. Let $k$ be maximum degree over all vertices of $G$. For all $i \in [k]$ denote by $q(i,G)$ number of vertices in graph $G$ having degree $i$. The Degree-list recognition success rate $R(G,H) \in \R$ is defined the following way:
 $$R(G,H) =  1 - \dfrac{\sum_{i \in [k]} |q(i,G)-q(i,H)|}{\mathbb{V}(G)}$$
\end{dfn}




\begin{expe}
\label{expe:RecognitionSuccess}

Given the data, we perform experiments on 3 different algorithms computed on the same underlying graph $\text{MSG}_k$. After obtaining the initial skeletons 
we used optimization technique of Algorithm \ref{alg:SGDOptSkeleton}. The process is  illustrated in Figure \ref{fig:FrameworkExperiments}. We performed experiments on two artificially generated datasets. Both of the data-sets consists of randomly generated sensible graphs $\mathcal{G}(l_{\max} = 1.5, l_{\min} = 0.5,  \theta = \frac{\pi}{4} , w = 0.3 )$ first introduced in Definition \ref{dfn:SensibleGraph}. In the first data-set we fixed number of vertices to be $N = 100$ and varied the number of generated points. In the second data-set we fixed the density of points per vertex to be $\frac{M}{N} = 200$, where $N$ is number of vertices and $M$ number of generated cloud points.  In all the experiment runs we measured the computational time of the pre-optimized graph, the optimization time, number of the  vertices in the final skeleton, the degree-list success rate, as well as the directed hausdorff distances between the cloud and initial approximation and between cloud and the final skeleton. 

\begin{figure}[H]
    \footnotesize
    \centering
    \begin{tikzpicture}[ >=stealth,
    node distance=3cm,
    auto
  ]
        \node [rectangle, 
    rounded corners, 
    % fill=black!10,
    draw=black, very thick] (start) {Input };
        %\node [below = 2.0cm of start] (startText) {(1) Original centaur};

     % above right

        \node [rectangle, 
    rounded corners, 
    % fill=black!10,
    draw=black, very thick, right of= start] (A1) {Compute $\MSG_k$};
        %\node [below = 2.0cm of A1] (A1Text) {(2) Rotated centaur };
        
 
    %    \node [block, right = 0.5cm of BDL] (B1){One B1};
    	\node [rectangle, 
    rounded corners, 
    % fill=black!10,
    draw=black, very thick, right of= A1] (tmp) {Mapper-algorithm};
        
        \node [rectangle, 
    rounded corners, 
    % fill=black!10,
    draw=black, very thick, above = 1.5cm of tmp ] (A3){DenseTree-algorithm};
                %\node [below = 2.0cm of A3] (A3Text) {(3a) Affine transformation };

        
        \node [rectangle, 
    rounded corners, 
    % fill=black!10,
    draw=black, very thick, below = 1.5cm of tmp] (end){AlphaReeb-algorithm};
               % \node [below = 2.0cm of end] (endText) {(3b) Projective transformation };
		
		\node[rectangle, 
    rounded corners, 
    % fill=black!10,
    draw=black, very thick, right of = tmp] (opt) {Optimization};
		
		
    \node[rectangle, 
    rounded corners, 
    % fill=black!10,
    draw=black, very thick, right of = opt] (out1) {Mapper Output};

\node[rectangle, 
    rounded corners, 
    % fill=black!10,
    draw=black, very thick, below = 1.5cm of out1] (out) {DenseTree Output};    
    
    \node[rectangle, 
    rounded corners, 
    % fill=black!10,
    draw=black, very thick, above = 1.5cm of out1] (out2) {AlphaReeb Output};
		
		

        
  
       \path[draw, ->] (start) -- (A1);
       % \path[->] (start) edge (A1);

       % \path[draw, ->] (A1) -- (A2);
        \path[draw, ->] (A1) -- (A3);
        \path[draw, ->] (A1) -- (end);
        \path[draw, ->] (A1) -- (tmp);
        
        \path[draw,->] (tmp) -- (opt);
        \path[draw,->] (end) -- (opt);
        \path[draw,->] (A3) -- (opt);
        
        \path[draw,->] (opt) -- (out);
         \path[draw,->] (opt) -- (out1);
          \path[draw,->] (opt) -- (out2);
        
        
                    
    \end{tikzpicture}
    \caption{Framework of the Experiment \ref{expe:RecognitionSuccess} comparison of 3 three algorithms: DenseTree, Mapper and AlphaReeb}
    \label{fig:FrameworkExperiments}
    \end{figure}



%Given set of sensible graphs $\mathcal{G}(l_{\max} = 1.5, l_{\min} = 0.5,  \theta = \frac{\pi}{4} , w = 0.3 )$ and generation error $\epsilon = 0.1$.

%\textbf{First experiment:} We fix number of vertices $N = 100$ in graph $G$ and varied number of generated points $M$. The obtained results are illustrated in Figure \ref{fig:DenseTimeExperiment} , Figure \ref{fig:MassiveTest2Success} and Figure \ref{fig:MassiveTest2MaxMin}
%
%\textbf{Second experiment:} We fix number of points per vertex rate at $M / N = 200$ and vary the number of vertices in Graph. This is illustrated in Figures \ref{fig:ComplexTimeExperiment}, \ref{fig:MassiveTestSuccess} and \ref{fig:MassiveTestMaxMin}.

\textbf{Hardware used:} The skeletonization tasks were performed using single thread of Amd Ryzen 9 3950x - CPU. The optimization of a skeleton using gradient descent technique was performed using Nvidia RTX-2080 GPU. 

\textbf{Algorithms properies: } In the experiments, we have used DenseTree, Mapper and AlphaReeb algorithms produced on the underlying graph $\MSG_{10}$ with the following properites:

\begin{itemize}
\itemsep0em 
\item \textbf{AlphaReeb:} $\alpha = 0.60 $
\item \textbf{DenseTree:} $\delta = 0.45$, $f_{r,t}$ for parameter values: $(r = 0.15, t = 0.025)$  
\item \textbf{Mapper:} Number of intervals = 15, Overlap ratio = 0.5
\end{itemize}

\end{expe}

\begin{figure}[H]

\centering
\begin{subfigure}{.33\textwidth}
 
  % include first image
  \includegraphics[width=.95\linewidth]{images/BigGraph1.png}  
 % \caption{First approximation}
\end{subfigure}
\begin{subfigure}{.33\textwidth}
  \centering
  % include second image
  \includegraphics[width=.95\linewidth]{images/Graph2.png}  
  %\caption{Graph after 20 iterations}
\end{subfigure}
\begin{subfigure}{.33\textwidth}
  \centering
  % include second image
  \includegraphics[width=.95\linewidth]{images/pic7.png}  
  %\caption{Graph after 40 iterations}
\end{subfigure}


  \caption{Example graphs generated from Algorithm \ref{alg:GraphGeneration} in $\mathbb{R}^2$ marked with red-color and a random point cloud marked with blue color.}
 % \label{fig:OptimizationProcess}

%\caption{ }

\end{figure}


\textbf{Conclusion: } When we fixed graph to contain $100$ vertices and varied the number of cloud points generated around it, all the algorithms have around the same computational time. When dealing with point clouds of higher densities DenseTree becomes slower, because computation of kernel density estimate have to deal with higher number of points. The optimization time was around the same for all the graphs. DenseTree algorithm performed significantly in the recognizing branch points, than both AlphaReeb and Mapper. Mapper and AlphaReeb were equally bad at recognizing branch points. Mapper produced threetimes less number of vertices than AlphaReeb, but the skeleton of AlphaReeb was significantly closer to the original point cloud than the skeleton of Mapper, both before and after the optimization. The initial approximation of the skeleton of DenseTree algorithm was a bit worse than the approximation of AlphaReeb-output. However, after the optimization DenseTree algorithm outperformed the AlphaReeb algorithm in all densities. 

When we fix the density to be $200$ points per generated vertex, all the algorithm have similar computational time. DenseTree algorithm is slightly better than AlphaReeb on all the other metrics. The output of Mapper has significantly less points than the other skeletons, but it performs significantly worse than the other two algorithms.

\section{Further research directions}

In this chapter, we have presented the optimized dense tree algorithm that takes a cloud sampled from a tree as input. This algorithm can extend to handle samples generated from general graphs by similarly using 1-dimensional persistence as it was done with homologically persistent skeleton (HoPeS) \cite{smith2021skeletonisation}, \cite{kurlin2015one}.  Let $G$ be a graph computed in Algorithm \ref{alg:dense_tree}. As in \cite{smith2021skeletonisation} we can find critical edges by computing a 1-dimensional persistence diagram of $G$, that will be combined with $\MST(G)$ to get skeleton $\text{DT}(C)$ that will possibly contain cycles. We have illustrated an example of such reconstruction in Figure \ref{fig:CycliGraph1}.




\begin{figure}[H]

\centering
\begin{subfigure}{.33\textwidth}
 
  % include first image
  \includegraphics[width=.95\linewidth]{images/CyclicGraphs/CyclicCloud70.png}  
  \caption{Random cloud $C$ generated around random cyclic graph}
  \label{fig:subFig-first}
\end{subfigure}
\begin{subfigure}{.33\textwidth}
  \centering
  % include second image
  \includegraphics[width=.95\linewidth]{images/CyclicGraphs/Dense70.png}  
  \caption{Dense tree $\text{DT}(C)$  }
  \label{fig:subFig-second}
\end{subfigure}
\begin{subfigure}{.33\textwidth}
  \centering
  % include second image
  \includegraphics[width=.95\linewidth]{images/CyclicGraphs/Optimized70.png}  
  \caption{Final skeleton $\ODT(C)$}
  \label{fig:subFig-second}

  
\end{subfigure}

  \caption{Reconstruction of cyclic graph}
  \label{fig:CycliGraph1}

%\caption{ }

\end{figure}


%\begin{figure}[H]
%
%\centering
%\begin{subfigure}{.33\textwidth}
% 
%  % include first image
%  \includegraphics[width=.95\linewidth]{images/CyclicGraphs/CyclicCloud40.png}  
%  \caption{Random cloud $C$ generated around random cyclic graph}
%  \label{fig:subFig-first}
%\end{subfigure}
%\begin{subfigure}{.33\textwidth}
%  \centering
%  % include second image
%  \includegraphics[width=.95\linewidth]{images/CyclicGraphs/Dense40.png}  
%  \caption{Dense tree $\text{DT}(C)$ built on cloud $C$ }
%  \label{fig:subFig-second}
%\end{subfigure}
%\begin{subfigure}{.33\textwidth}
%  \centering
%  % include second image
%  \includegraphics[width=.95\linewidth]{images/CyclicGraphs/Optimized40.png}  
%  \caption{Final skeleton $\ODT(C)$}
%  \label{fig:subFig-second}
%
%  
%\end{subfigure}
%
%  \caption{Reconstruction of cyclic graph}
%  \label{fig:CycliGraph1}
%
%%\caption{ }
%
%\end{figure}

%. However, presented dense tree algorithm,  can also be generalized using idea developed \cite{smith2021skeletonisation}
%and \cite{kurlin2015one}.
%smith2021skeletonisation
%and \cite{kurlin2015one}. 

% s of \cite{kurlin2015one}


\vspace{\fill}
\pagebreak[0]
\vspace{-\fill}

% With fixed density of 200 points per edge all the algorithms have around the same computational time. However when density is increased, the dense tree algorithm becomes slower, because of the kernel density estimation. The dense tree algorithm had better degree-list recognition success rate than other algorithms and it was slightly better than AlphaReeb in minimizing the final recognition error. 




%\textbf{Experiments properties: } All the graphs in the further experiments were generated using the following properties: 
%$$\{l_{\max}(T) = 1.5, l_{\min}(T) = 0.5, w(T) = 0.3, \theta(T) = \frac{\pi}{4}, \epsilon = 0.1  \} $$
%where $l_{\max}(T)$ is size of the minimal edge of the graph $T$  , $ l_{\min}(T)$ is size of the maximal edge of the graph $T$,  $w(T)$ is the minimal distance between any two non-adjacent edge of the graph $T$, $\theta(T)$ is the minimal angle between any two adjacent edges of the graph $T$ and $\epsilon$ is the uniform error-bound of the point cloud. 



%\begin{itemize}
%\item \textbf{Density:} In the first experiment we fix number of vertices $N = 100$ in graph $G$ and varied number of generated points $M$. The obtained results are illustrated in Figure \ref{fig:DenseTimeExperiment} , Figure \ref{fig:MassiveTest2Success} and Figure \ref{fig:MassiveTest2MaxMin}
%\item \textbf{Complexity: }In the second experiment we fix number of points per vertex rate at $M / N = 200$ and vary the number of vertices in Graph. This is illustrated in Figures \ref{fig:ComplexTimeExperiment}, \ref{fig:MassiveTestSuccess} and \ref{fig:MassiveTestMaxMin}.
%\end{itemize}


%% given an error measure $\epsilon$ we generate point cloud $C$ using monte-carlo method. 

%The experiments were conducted using smart randomized spacial tree-graphs in $\R^3$, generated recursively according to the technical Definition \ref{dfn:technicalGraph}, idea of which is to produce graphs that could be unequivocally reconstructed. This would not be possible if, for example, two non-adjacent edges would pass too close to each other making it impossible to determine which edge was the point sampled from. A general plan is to generate tree-graphs in an as intuitive way as possible, for example by trying to add new vertices and edges randomly and doing retries if the iterating graph fails to satisfy given constraints. To make the task more challenging for algorithms we prioritize graphs with higher degree vertices, as they are usually the most difficult part to reconstruct correctly. 

%\begin{dfn}\label{dfn:technicalGraph}
%\textbf{Setup:} Let $\theta \in [0,2\pi]$ be an angle and let $L \in \R$ be a constant corresponding to minimal distance between two non-ajacent edges and let $l_{\min}, l_{\max} \in \R$ be constants corresponding to maximal and minimal edge-lengths. 
%
%\textbf{Probability of adding specific edge: } Let $T$ be an arbitrary graph and let $v \in \mathbb{V}(T)$, we write $\mathcal{P}(T,v)$ to be the probability that $u$ picked randomly in $B(u,l_{\max} ) \setminus B(u,l_{\min} ) $ forms an edge $e = (u,v)$ satisfying the following two conditions 
%\begin{enumerate}
%\item Edge $e$ is at least $L$-distance away from all the other edges i.e. $d(e,w) > L$ for all $w \in \mathbb{E}(T)$.
%\item For any $w \in \mathbb{E}(T)$ having $v$ as one of its end points the angle $\angle(e,w) > \theta$. 
%\end{enumerate}
%\textbf{Definition of smart Graph distribution:} Define $\mathcal{G}(n,\theta,L)$ to be a distribution of randomized spacial graphs defined in the following way: 
%\begin{itemize}
%\item We define $\mathcal{G}(1,\theta,L)$ to be a distribution that retrieves Graph with a single vertex $v$ and no edges. 
%\item In general $\mathcal{G}(n,\theta,L)$ is a distribution of graphs obtained by taking uniformly random graph $T \in \mathcal{G}(n-1,\theta,L)$ and adding random feasible edge (together with new vertex $u$) to vertex $v \in \mathbb{V}(T)$ with distribution
% $$D:\mathbb{V} \rightarrow [0,1] \mid D(v) = \dfrac{ \text{Degree}(v,T) \cdot \mathcal{P}(T,v)}{\sum_{q \in \mathbb{V}(T) \text{Degree}(q,T) \cdot \mathcal{P}(T,q) }}  $$
% In other words the priority is given to vertices of higher degree. 
%\end{itemize}
%\end{dfn}
%Because in most cases the reconstruction fails to get correct homeomorphism type due to either not detecting separate branches (edges containing a vertex of degree 1) or incorrectly splits vertex of higher degree into multiple vertices having smaller degree, we propose the following quick way to estimate the recognition success rate of the algorithm.
%\begin{dfn}\label{dfn:recognitionSuccess}[Recognition success rate]
%Given graphs $G$ and $H$, where $G$ is an attempted reconstruction of graph $H$. Let $k$ be maximum degree over all vertices of $G$. For all $i \in [k]$ denote by $q(i,G)$ number of vertices in graph $G$ having degree $i$. We define recognition success rate $R(G,H) \in \R$ in the following way:
% $$R(G,H) =  1 - \dfrac{\sum_{i \in [k]} |q(i,G)-q(i,H)|}{\mathbb{V}(G)}$$
%\end{dfn}
%\textbf{Cloud generation properties: } Given a spacial graph $G$, the point clouds are generated using Monte-carlo methodology: Given a bound $\epsilon \in \R$ and number of points $M \in \Z$, we generate a random point in space $\R^3$, if the generation is succesful i.e. $d(p,G) \leq \epsilon$, then the point $p$ is accepted. We proceed with the iteration procedure until we have $M$-accepted points. 


%

%%\resizebox{0.49\columnwidth}{!}{
%%\begin{tikzpicture}
%%\begin{axis}[xlabel = Total number of points, ylabel = Distance from origin,grid, legend style={at={(0.5,-0.1)},anchor=north},every axis plot/.append style={ultra thick}]
%%% [black,mark = *]
%%\addplot table [x=NumPoints, y=Param0.025, col sep=comma] {tables/Density/resultsStar.csv};
%%\addlegendentry{Param$(0.075, 0.025)$}
%%\addplot table [x=NumPoints, y=Param0.05, col sep=comma] {tables/Density/resultsStar.csv};
%%\addlegendentry{Param$(0.1, 0.05)$}
%%\addplot table [x=NumPoints, y=Param0.075, col sep=comma] {tables/Density/resultsStar.csv};
%%\addlegendentry{Param$(0.125, 0.075)$}
%%\addplot table [x=NumPoints, y=Param0.1, col sep=comma] {tables/Density/resultsStar.csv};
%%\addlegendentry{Param$(0.15, 0.1)$}
%%\addplot table [x=NumPoints, y=Param0.125, col sep=comma] {tables/Density/resultsStar.csv};
%%\addlegendentry{Param$(0.175, 0.125)$}
%%\addplot table [x=NumPoints, y=Param0.15, col sep=comma] {tables/Density/resultsStar.csv};
%%\addlegendentry{Param$(0.2, 0.15)$}
%%
%%
%%\end{axis}
%%\end{tikzpicture}
%%}
%%\caption{\textbf{Left:} Tube experiments. \textbf{Right:} Star experiments}
%\caption{Optimization performance of the gradient descent algorithm on dense tree $\text{DT}(C)$ using different learning rates.
%\textbf{Left:} 10000 points generated on graph consisting of around 100 edges . \textbf{Right:} 100000 Points generated on graph consisting of around 1000 edges}
%\label{fig:OptimizationExperiments}
%\end{figure}



\begin{figure}[H]

\centering
\begin{subfigure}{.48\textwidth}
\begin{tikzpicture}[thick,scale=0.85, every node/.style={transform shape}]
\begin{axis}[xlabel =Points per edge, ylabel = Time (seconds) ,grid,legend style={at={(0.25,0.75)},anchor=center}]
\addplot table [x=Points, y=Dense, col sep=comma] {tables/MassiveTest2/resultsTime.csv};
\addlegendentry{DenseTree}
\addplot table [x=Points, y=Mapper, col sep=comma] {tables/MassiveTest2/resultsTime.csv};
\addlegendentry{Mapper}
\addplot table [x=Points, y=Alpha, col sep=comma] {tables/MassiveTest2/resultsTime.csv};
\addlegendentry{AlphaReeb}
\end{axis}
\end{tikzpicture}
\caption{Computation time of the initial approximation}
\end{subfigure}
\begin{subfigure}{.48\textwidth}
\begin{tikzpicture}[thick,scale=0.85, every node/.style={transform shape}]
\begin{axis}[xlabel =Points per edge,grid,legend style={at={(0.5,-0.1)},anchor=north}]
\addplot table [x=Points, y=Dense, col sep=comma] {tables/MassiveTest2/TimeOptimization.csv};
%\addlegendentry{merge-diagram}
\addplot table [x=Points, y=Mapper, col sep=comma] {tables/MassiveTest2/TimeOptimization.csv};
%\addlegendentry{PD diagram}
\addplot table [x=Points, y=Alpha, col sep=comma] {tables/MassiveTest2/TimeOptimization.csv};
%\addlegendentry{NN(4) diagram}
\end{axis}
\end{tikzpicture}
\caption{ Computation time of the optimization}
\end{subfigure}
\label{fig:DenseTimeExperiment}
%\begin{tikzpicture}[thick,scale=0.75, every node/.style={transform shape}]
%\begin{axis}[xlabel =Standard deviation of gaussian noise ,grid,legend style={at={(0.5,-0.1)},anchor=north}]
%\addplot table [x=e, y=m, col sep=comma] {Tables/ProjectiveGaussian.csv};
%%\addlegendentry{merge-diagram}
%\addplot table [x=e, y=p, col sep=comma] {Tables/ProjectiveGaussian.csv};
%%\addlegendentry{PD diagram}
%\addplot table [x=e, y=nn4, col sep=comma] {Tables/ProjectiveGaussian.csv};
%%\addlegendentry{NN(4) diagram}
%\addplot table [x=e, y=c, col sep=comma] {Tables/ProjectiveGaussian.csv};
%%\addlegendentry{cloud}
%\end{axis}
%\end{tikzpicture}



%Table1: (Scale,Uniform), Table2: (Scale, Gaussian),Table3: (Projection,Uniform), Table4: (Projection, Gaussian) }
%\label{fig:MassiveTest2Time}
\begin{subfigure}{.49\textwidth}
\begin{tikzpicture}[thick,scale=0.85, every node/.style={transform shape}]
\begin{axis}[xlabel =Points per edge, ylabel = Recognition success ,grid,legend style={at={(0.5,-0.1)},anchor=north}]
\addplot table [x=Points, y=Dense, col sep=comma] {tables/MassiveTest2/SuccessRateReal.csv};
%\addlegendentry{merge-diagram}
\addplot table [x=Points, y=Mapper, col sep=comma] {tables/MassiveTest2/SuccessRateReal.csv};
%\addlegendentry{PD diagram}
\addplot table [x=Points, y=Alpha, col sep=comma] {tables/MassiveTest2/SuccessRateReal.csv};
%\addlegendentry{NN(4) diagram}
\end{axis}
\end{tikzpicture}
\caption{ Recognition success rate }
\end{subfigure}
\begin{subfigure}{.49\textwidth}
\begin{tikzpicture}[thick,scale=0.85, every node/.style={transform shape}]
\begin{axis}[xlabel =Points per edge,grid, ylabel = Number of vertices,legend style={at={(0.5,-0.1)},anchor=north}]
\addplot table [x=Points, y=Dense, col sep=comma] {tables/MassiveTest2/VertexNumReal.csv};
%\addlegendentry{merge-diagram}
\addplot table [x=Points, y=Mapper, col sep=comma] {tables/MassiveTest2/VertexNumReal.csv};
%\addlegendentry{PD diagram}
\addplot table [x=Points, y=Alpha, col sep=comma] {tables/MassiveTest2/VertexNumReal.csv};
%\addlegendentry{NN(4) diagram}
\end{axis}
\end{tikzpicture}
\caption{Number of vertices in the final output}
\end{subfigure}
\label{fig:MassiveTest2Success}
%\begin{tikzpicture}[thick,scale=0.75, every node/.style={transform shape}]
%\begin{axis}[xlabel =Standard deviation of gaussian noise ,grid,legend style={at={(0.5,-0.1)},anchor=north}]
%\addplot table [x=e, y=m, col sep=comma] {Tables/ProjectiveGaussian.csv};
%%\addlegendentry{merge-diagram}
%\addplot table [x=e, y=p, col sep=comma] {Tables/ProjectiveGaussian.csv};
%%\addlegendentry{PD diagram}
%\addplot table [x=e, y=nn4, col sep=comma] {Tables/ProjectiveGaussian.csv};
%%\addlegendentry{NN(4) diagram}
%\addplot table [x=e, y=c, col sep=comma] {Tables/ProjectiveGaussian.csv};
%%\addlegendentry{cloud}
%\end{axis}
%\end{tikzpicture}


%Table1: (Scale,Uniform), Table2: (Scale, Gaussian),Table3: (Projection,Uniform), Table4: (Projection, Gaussian) }
%\label{fig:MassiveTest2Success}
%\end{figure}

%\begin{figure}
%\centering
\begin{subfigure}{.49\textwidth}
\begin{tikzpicture}[thick,scale=0.85, every node/.style={transform shape}]
\begin{axis}[xlabel =Points per edge, ylabel = Error ,grid,legend style={at={(0.5,-0.1)},anchor=north}]
\addplot table [x=Points, y=Dense, col sep=comma] {tables/MassiveTest2/MaxMinOriginal.csv};
%\addlegendentry{merge-diagram}
\addplot table [x=Points, y=Mapper, col sep=comma] {tables/MassiveTest2/MaxMinOriginal.csv};
%\addlegendentry{PD diagram}
\addplot table [x=Points, y=Alpha, col sep=comma] {tables/MassiveTest2/MaxMinOriginal.csv};
%\addlegendentry{NN(4) diagram}
\end{axis}
\end{tikzpicture}
\caption{Directed Hausdorff error before optimization}
\end{subfigure}
\begin{subfigure}{.49\textwidth}
\begin{tikzpicture}[thick,scale=0.85, every node/.style={transform shape}]
\begin{axis}[xlabel =Points per edge,grid,legend style={at={(0.5,-0.1)},anchor=north}]
\addplot table [x=Points, y=Dense, col sep=comma] {tables/MassiveTest2/MaxMinUpgraded.csv};
%\addlegendentry{merge-diagram}
\addplot table [x=Points, y=Mapper, col sep=comma] {tables/MassiveTest2/MaxMinUpgraded.csv};
%\addlegendentry{PD diagram}
\addplot table [x=Points, y=Alpha, col sep=comma] {tables/MassiveTest2/MaxMinUpgraded.csv};
%\addlegendentry{NN(4) diagram}
\end{axis}
\end{tikzpicture}
\caption{Directed Hausdorff error after optimization}
\end{subfigure}
%\begin{tikzpicture}[thick,scale=0.75, every node/.style={transform shape}]
%\begin{axis}[xlabel =Standard deviation of gaussian noise ,grid,legend style={at={(0.5,-0.1)},anchor=north}]
%\addplot table [x=e, y=m, col sep=comma] {Tables/ProjectiveGaussian.csv};
%%\addlegendentry{merge-diagram}
%\addplot table [x=e, y=p, col sep=comma] {Tables/ProjectiveGaussian.csv};
%%\addlegendentry{PD diagram}
%\addplot table [x=e, y=nn4, col sep=comma] {Tables/ProjectiveGaussian.csv};
%%\addlegendentry{NN(4) diagram}
%\addplot table [x=e, y=c, col sep=comma] {Tables/ProjectiveGaussian.csv};
%%\addlegendentry{cloud}
%\end{axis}
%\end{tikzpicture}
%\caption{ \textbf{Left: }MaxMin-error before optimization averaged over 100 point clouds \textbf{Right: } MaxMin-error after optimization averaged over 100 point clouds.
%}

%Table1: (Scale,Uniform), Table2: (Scale, Gaussian),Table3: (Projection,Uniform), Table4: (Projection, Gaussian) }
%\label{fig:MassiveTest2MaxMin}
\caption{Experiments, where we have varied density of a point cloud generated on dataset consisting of random trees having 100 vertices}

\end{figure}


\begin{figure}[H]

\centering

\begin{subfigure}{.48\textwidth}
\begin{tikzpicture}[thick,scale=0.85, every node/.style={transform shape}]
\begin{axis}[xlabel = Number of vertices, ylabel = Time (seconds) ,grid,legend style={at={(0.25,0.75)},anchor=center}]
\addplot table [x=Vertices, y=Dense, col sep=comma] {tables/MassiveTest/resultsTime.csv};
\addlegendentry{DenseTree}
\addplot table [x=Vertices, y=Mapper, col sep=comma] {tables/MassiveTest/resultsTime.csv};
\addlegendentry{Mapper}
\addplot table [x=Vertices, y=Alpha, col sep=comma] {tables/MassiveTest/resultsTime.csv};
\addlegendentry{AlphaReeb}
\end{axis}
\end{tikzpicture}
\caption{Computation time of the initial approximation}
\end{subfigure}
\begin{subfigure}{.48\textwidth}
\begin{tikzpicture}[thick,scale=0.85, every node/.style={transform shape}]
\begin{axis}[xlabel =Number of vertices,grid,legend style={at={(0.5,-0.1)},anchor=north}]
\addplot table [x=Vertices, y=Dense, col sep=comma] {tables/MassiveTest/TimeOptimization.csv};
%\addlegendentry{merge-diagram}
\addplot table [x=Vertices, y=Mapper, col sep=comma] {tables/MassiveTest/TimeOptimization.csv};
%\addlegendentry{PD diagram}
\addplot table [x=Vertices, y=Alpha, col sep=comma] {tables/MassiveTest/TimeOptimization.csv};
%\addlegendentry{NN(4) diagram}
\end{axis}
\end{tikzpicture}
\caption{ Computation time of the optimization}
\end{subfigure}
%\begin{tikzpicture}[thick,scale=0.75, every node/.style={transform shape}]
%\begin{axis}[xlabel =Standard deviation of gaussian noise ,grid,legend style={at={(0.5,-0.1)},anchor=north}]
%\addplot table [x=e, y=m, col sep=comma] {Tables/ProjectiveGaussian.csv};
%%\addlegendentry{merge-diagram}
%\addplot table [x=e, y=p, col sep=comma] {Tables/ProjectiveGaussian.csv};
%%\addlegendentry{PD diagram}
%\addplot table [x=e, y=nn4, col sep=comma] {Tables/ProjectiveGaussian.csv};
%%\addlegendentry{NN(4) diagram}
%\addplot table [x=e, y=c, col sep=comma] {Tables/ProjectiveGaussian.csv};
%%\addlegendentry{cloud}
%\end{axis}
%\end{tikzpicture}

%\label{fig:ComplexTimeExperiment}


%Table1: (Scale,Uniform), Table2: (Scale, Gaussian),Table3: (Projection,Uniform), Table4: (Projection, Gaussian) }
%\label{fig:MassiveTest2Time}

\begin{subfigure}{.49\textwidth}
\begin{tikzpicture}[thick,scale=0.85, every node/.style={transform shape}]
\begin{axis}[xlabel =Number of vertices, ylabel = Recognition success ,grid,legend style={at={(0.5,-0.1)},anchor=north}]
\addplot table [x=Vertices, y=Dense, col sep=comma] {tables/MassiveTest/SuccessRateReal.csv};
%\addlegendentry{merge-diagram}
\addplot table [x=Vertices, y=Mapper, col sep=comma] {tables/MassiveTest/SuccessRateReal.csv};
%\addlegendentry{PD diagram}
\addplot table [x=Vertices, y=Alpha, col sep=comma] {tables/MassiveTest/SuccessRateReal.csv};
%\addlegendentry{NN(4) diagram}
\end{axis}
\end{tikzpicture}
\caption{Recognition success rate }
\end{subfigure}
\begin{subfigure}{.49\textwidth}
\begin{tikzpicture}[thick,scale=0.85, every node/.style={transform shape}]
\begin{axis}[xlabel =Number of vertices,grid, ylabel = Number of vertices (output),legend style={at={(0.5,-0.1)},anchor=north}]
\addplot table [x=Vertices, y=Dense, col sep=comma] {tables/MassiveTest/VertexNumReal.csv};
%\addlegendentry{merge-diagram}
\addplot table [x=Vertices, y=Mapper, col sep=comma] {tables/MassiveTest/VertexNumReal.csv};
%\addlegendentry{PD diagram}
\addplot table [x=Vertices, y=Alpha, col sep=comma] {tables/MassiveTest/VertexNumReal.csv};
%\addlegendentry{NN(4) diagram}
\end{axis}
\end{tikzpicture}
\caption{Number of vertices in the final output}
\end{subfigure}
%\caption{Complexity experiments: \textbf{Left: }Average recognition success rate, as defined in Definition \ref{dfn:recognitionSuccess} . \textbf{Right: } Average %number of vertices in the final output.}
%\label{fig:MassiveTestSuccess}
%\begin{tikzpicture}[thick,scale=0.75, every node/.style={transform shape}]
%\begin{axis}[xlabel =Standard deviation of gaussian noise ,grid,legend style={at={(0.5,-0.1)},anchor=north}]
%\addplot table [x=e, y=m, col sep=comma] {Tables/ProjectiveGaussian.csv};
%%\addlegendentry{merge-diagram}
%\addplot table [x=e, y=p, col sep=comma] {Tables/ProjectiveGaussian.csv};
%%\addlegendentry{PD diagram}
%\addplot table [x=e, y=nn4, col sep=comma] {Tables/ProjectiveGaussian.csv};
%%\addlegendentry{NN(4) diagram}
%\addplot table [x=e, y=c, col sep=comma] {Tables/ProjectiveGaussian.csv};
%%\addlegendentry{cloud}
%\end{axis}
%\end{tikzpicture}


%Table1: (Scale,Uniform), Table2: (Scale, Gaussian),Table3: (Projection,Uniform), Table4: (Projection, Gaussian) }
%\label{fig:MassiveTest2Success}
%\end{figure}

%\begin{figure}
%\centering

\begin{subfigure}{.49\textwidth}
\begin{tikzpicture}[thick,scale=0.85, every node/.style={transform shape}]
\begin{axis}[xlabel =Number of vertices, ylabel = initial error ,grid,legend style={at={(0.5,-0.1)},anchor=north}]
\addplot table [x=Vertices, y=Dense, col sep=comma] {tables/MassiveTest/MaxMinOriginal.csv};
%\addlegendentry{merge-diagram}
\addplot table [x=Vertices, y=Mapper, col sep=comma] {tables/MassiveTest/MaxMinOriginal.csv};
%\addlegendentry{PD diagram}
\addplot table [x=Vertices, y=Alpha, col sep=comma] {tables/MassiveTest/MaxMinOriginal.csv};
%\addlegendentry{NN(4) diagram}
\end{axis}
\end{tikzpicture}
\caption{Directed Hausdorff error before optimization}
\end{subfigure}
\begin{subfigure}{.49\textwidth}
\begin{tikzpicture}[thick,scale=0.85, every node/.style={transform shape}]
\begin{axis}[xlabel =Number of vertices, ylabel = final error,grid,legend style={at={(0.5,-0.1)},anchor=north}]
\addplot table [x=Vertices, y=Dense, col sep=comma] {tables/MassiveTest/MaxMinUpgraded.csv};
%\addlegendentry{merge-diagram}
\addplot table [x=Vertices, y=Mapper, col sep=comma] {tables/MassiveTest/MaxMinUpgraded.csv};
%\addlegendentry{PD diagram}
\addplot table [x=Vertices, y=Alpha, col sep=comma] {tables/MassiveTest/MaxMinUpgraded.csv};
%\addlegendentry{NN(4) diagram}
\end{axis}
\end{tikzpicture}
\caption{Directed Hausdorff error after optimization}
\end{subfigure}
%\caption{ Complexity experiments: \textbf{Left: } MaxMin-error before optimization \textbf{Right: } MaxMin-error after optimization
%}

%\begin{tikzpicture}[thick,scale=0.75, every node/.style={transform shape}]
%\begin{axis}[xlabel =Standard deviation of gaussian noise ,grid,legend style={at={(0.5,-0.1)},anchor=north}]
%\addplot table [x=e, y=m, col sep=comma] {Tables/ProjectiveGaussian.csv};
%%\addlegendentry{merge-diagram}
%\addplot table [x=e, y=p, col sep=comma] {Tables/ProjectiveGaussian.csv};
%%\addlegendentry{PD diagram}
%\addplot table [x=e, y=nn4, col sep=comma] {Tables/ProjectiveGaussian.csv};
%%\addlegendentry{NN(4) diagram}
%\addplot table [x=e, y=c, col sep=comma] {Tables/ProjectiveGaussian.csv};
%%\addlegendentry{cloud}
%\end{axis}
%\end{tikzpicture}

%Table1: (Scale,Uniform), Table2: (Scale, Gaussian),Table3: (Projection,Uniform), Table4: (Projection, Gaussian) }
\label{fig:MassiveTestMaxMin}

\caption{Result of experiments, where we have fixed the density of generated point cloud generated varied the number of vertices of the randomly generated graphs.}

\end{figure}



==> chapters/chapter4.tex <==
\chapter{Data skeletonization} % Write in your own chapter title
\label{ch:chapter2} % Add a label in case you want to refer to the chapter.



\section{Theoretical guarantees}
We present a general theorem that can be used to prove that the point sample coming from a given tree-graph can be reconstructed in a creative way. In this section we denote the euclidean distance in space $\R^m$ by $d_E$. The following concepts will be used:

\begin{dfn}[$\epsilon$-sample of a graph]
We say that a point cloud $C$ is an $\epsilon$-\emph{sample} of a straight-line graph $T \subseteq \R^m$ if for every $p \in C$ there exists a point $q \in T$ for which $d_E(p,q) < \epsilon$ i.e $C \subset T^{\epsilon}$.
\end{dfn}
\begin{figure}
\centering
\includegraphics[width=0.49\linewidth]{figures/stars/star4_cloud_ODT.png}
\includegraphics[width=0.49\linewidth]{figures/stars/star5_cloud_ODT.png}
\caption{Two graphs and their $\epsilon$-samples pictured}

\end{figure}
%  We define $d_G$ as its path-metric in the following way:

 
\begin{dfn}[path metric on a graph $G$]
Let $C$ be a point cloud in euclidean space $\mathbb{R}^m$ and let $G$ be a straight-line graph for which $\mathbb{V}(G) = C$ . For $a,b \in \mathbb{V}(G)$  define the path metric $d_G(a,b)$ to be the length of the shortest path between $a$ and $b$ in the graph $G$. 

%and let $s$ be the shortest path between $a$ and $b$ in graph $G$. Define distance $d_G$ in the following way:
%$$d_G(a,b) = \sum_{(u,v) \in s}d_E(u,v)$$
\end{dfn}
We say that two edges are adjacent in the graph $G$, if they have a common vertex.
\begin{dfn}
Let $G$ be a straight-line graph in $\mathbb{R}^m$. Denote the \emph{maximal edge length} of $G$ by $l(G)$ and the minimal angle over all adjacent edges in the graph $G$ by $\theta(G)$.  
%Let $G$ be a spacial graph in $\mathbb{R}^m$, let $C$ and let $T$ be an approximation of $G^{\epsilon}$ 
\end{dfn}
%<--- Condition 1 

%\begin{dfn}
%Let $T$ be a striaghtline embedded tree, let $D$ be an $\epsilon$ sample of $T$ and let $G$ be a graph that approximates $D$. We say that $D$ is $\delta$-sparse sample if $D^{\epsilon}$ covers vertices of $T$ and if $\delta$  .  For any points $a \neq b \in D$ the distance $d_G(a,b)$ is always bigger than $ \delta$.
%\end{dfn}

In the following definition the distance between two line-segments $e,h$ is defined as the Hausdorff distance
 $d_H(e,h) = \max \{\sup_{x \in e}\inf_{y \in h}d_E(x,y), \sup_{y \in Y}\inf_{x \in X}d_E(x,y)\} $
\begin{dfn}
Let $a,b$ the two points in $\mathbb{R}^m $, we denote the line segment by $[a,b]$.  
\end{dfn}

\begin{dfn}[$\gamma$-approximation]
Let $T$ be a straight-line tree in $\R^m$ and let $C$ be its $\epsilon$-sample. Let $\mathcal{U}$ be an arbitrary covering of $C$.
 We say that a graph $G$ with a vertex set $C$ is a
\emph{$\gamma$-approximation} of $(T,C,\mathcal{U})$ if the following two conditions are satisfied: 
\begin{enumerate}
\item If for points $a,b$ belong to the same covering element of $\mathcal{U}$ then $d_G(a,b) \leq \gamma \cdot d_E(a,b) $
\item The minimal distance between two non adjacent edges of $T$ is larger than $l(G) + 2\epsilon$.
%\item Let $r$ be minimal distance between two non-adjacent edges of $T$ then: $l(G) < r - 2\epsilon $
\end{enumerate}

\end{dfn}
%Let $\delta,\gamma \in \R_{+}$ be parameters.



\begin{thm}[homeomorphism guarantees for a minimum spanning tree]
\label{thm:GHT}
Let $T$ be a straight-line tree graph in $\mathbb{R}^m$ and let $C$ be an $\epsilon$-sample of $\mathbb{R}^m$. Let $D \subseteq C$ be a subsample of $C$ which covers vertices of $T$, i.e $\mathbb{V}(T) \subseteq D^{\epsilon}$. Define covering of the cloud $\mathcal{U} = \{C \cap e \mid e \in \mathbb{E}(T)\} $. Let the graph $G$ be an arbitrary $(\gamma,C, \mathcal{U})$-approximation of $T$ for $\gamma \geq 1$ and let $d_G$ be its path metric.
Let $$\delta =  2\gamma(\epsilon +\dfrac{\epsilon}{\sin(\frac{\theta(T)}{2})} + \dfrac{l(G)}{\sin(\min(\theta(T), \frac{\pi}{2}))})$$
 If the subsample $D$ is $\delta$ sparse: For all $a,b \in D$: $d_G(a,b) > \delta$, then $\MST(D, d_G)$ is homeomorphic to the tree $T$. 

 


\end{thm}


\begin{figure}
\centering
\includegraphics[width=0.49\linewidth]{UnderlyingGraph/Star2Sep.png}
\includegraphics[width=0.49\linewidth]{UnderlyingGraph/Star5Sep.png}
\caption{Single cover-element $C \cap e$ of Theorem \ref{thm:GHT} colored with red in Star2 (on the left) and Star5 (on the right) graphs}

\end{figure}


\begin{figure}
\centering
\begin{tikzpicture}[node distance=3.0cm,
    every node/.style={fill=white}, align=center]
  % Specification of nodes (position, etc.)
  \node (start)                    {Theorem \ref{thm:GHT} };
  \node (vertexLemma)     [ below left of=start]          {Proposition \ref{lem:somstod}};
  \node (edgeLemma)     [ below right of=start]          {Proposition \ref{lem:eht}};
  \node (helpVertexLemma) [ below of = vertexLemma] {Lemma \ref{lem:nonadjacentedgesgraph}};
  \node (unionSubdivisionLemma) [right of = helpVertexLemma] {Lemma \ref{lem:MSTGlue}};
  \node (helpEdgeLemma) [right of =unionSubdivisionLemma] {Lemma \ref{lem:edge-offset}};
  \node (vertexPointLemma) [right of = helpEdgeLemma] {Lemma \ref{lem:vertex-point}};
  \node (defFourOneThree) [right of = edgeLemma] {Definition \ref{dfn:subdivision}};
  \node (dfnSeparationProperty) [below of = unionSubdivisionLemma] {Definition \ref{dfn:SeparationProperty}};
  \node (dfnEordering) [below of = vertexPointLemma] {Definition \ref{dfn:eordering}};
  \node (adjacentEdgesLemma)[below of = dfnSeparationProperty]{Lemma \ref{AdjacentEdgesLemma}};
  \node (vertexLinkExistence)[below of = adjacentEdgesLemma]{Lemma \ref{ExistenceOfVertexLink}};
  \node (structureOfPaths)[below of = vertexLinkExistence]{Lemma \ref{structureofpaths}};
  \node (ssP)[right of =structureOfPaths]{Definition \ref{shortestPathConnecting}};
  
 % \node {Definition413} [right of = vertexPointLemma] {Lemma 4.13}
 
%  \node (onStartBlock)      [ below of=onCreateBlock]   {onStart()};
%  \node (onResumeBlock)     [ below of=onStartBlock]   {onResume()};
%  \node (activityRuns)      [ below of=onResumeBlock]
%                                                      {Activity is running};
%  \node (onPauseBlock)      [ below of=activityRuns, yshift=-1cm]
%                                                                {onPause()};
%  \node (onStopBlock)       [ below of=onPauseBlock, yshift=-1cm]
%                                                                 {onStop()};
%  \node (onDestroyBlock)    [ below of=onStopBlock, yshift=-1cm] 
%                                                              {onDestroy()};
%  \node (onRestartBlock)    [ right of=onStartBlock, xshift=4cm]
%                                                              {onRestart()};
%  \node (ActivityEnds)      [ left of=activityRuns, xshift=-4cm]
%                                                        {Process is killed};
%  \node (ActivityDestroyed) [ below of=onDestroyBlock]
%                                                    {Activity is shut down};     
  % Specification of lines between nodes specified above
  % with aditional nodes for description 
  \draw[->]             (vertexLemma) -- (start) ;
  \draw[->]             (edgeLemma) -- (start) ;
  \draw[->]				(helpVertexLemma) -- (vertexLemma) ;
  \draw[->]				(helpEdgeLemma) -- (edgeLemma);
  \draw[->]				(vertexPointLemma) -- (edgeLemma);
  \draw[->]				(defFourOneThree) -- (edgeLemma);
  \draw[->]				(unionSubdivisionLemma) -- (vertexLemma);
  \draw[->]				(unionSubdivisionLemma) -- (edgeLemma);
  \draw[->]				(dfnSeparationProperty) -- (unionSubdivisionLemma);
  \draw[->]				(dfnSeparationProperty) -- (helpVertexLemma);
  \draw[->]				(dfnSeparationProperty) -- (helpEdgeLemma);
  \draw[->]				(dfnEordering) -- (helpEdgeLemma);
  \draw[->]				(adjacentEdgesLemma) -- (helpVertexLemma);
  \draw[->]				(adjacentEdgesLemma) -- (helpEdgeLemma);
  \draw[->]				(vertexLinkExistence) -| (helpVertexLemma);
  \draw[->]				(vertexLinkExistence) -| (helpEdgeLemma);
  \draw[->]				(structureOfPaths) -- (vertexLinkExistence);
  \draw[->]				(ssP) -- (vertexLinkExistence);





  \end{tikzpicture}

\caption{Proof structure of Theorem \ref{thm:GHT}}
\end{figure}

For every vertex $v \in \mathbb{V}(T)$ denote its nearest neighbor in the set $D$ by $p_v$. In the conditions of Theorem \ref{thm:GHT} we assumed that for every vertex $v \in T$ there exists a point $q \in D$ in its $\epsilon$-neighborhood. In the following Lemma \ref{lem:vertex-point} we prove that it is unique, i.e. $p_v = q$. 

\begin{lem}[Each vertex of $T$ has exactly one point in its $\ep$-ball]
\label{lem:vertex-point}
Any vertex $v$ of $T$ has a unique point $p_v\in D$ in the $\ep$-ball $v^{\ep}$ at $v$ in the space $(\R^m, d_E)$
\end{lem}
\begin{proof}
Given a vertex $v \in \mathbb{V}(T)$ it follows from conditions of Theorem \ref{thm:GHT} that the nearest neighbor $p_v$ is in the $\ep$-ball $v^{\ep}$.
If there is another point $q\in C\cap v^{\ep}$, then $d_E(p_v,q) \leq 2 \ep < \de $ which is a contradiction because of the condition $\de \geq 2\ep $. 

%$d_k(p,q) \leq c_{\max}t_{\epsilon}(p,q)\leq 2c_{\max}\ep<\de$, 
\end{proof}



\begin{dfn}[$e$-ordering]
\label{dfn:eordering}
Let $e = [u,v]$ be a line segment and let $C$ be a finite point set in space $\mathbb{R}^m$. Let $\text{pr}_{e}:C \rightarrow e$ be a function that maps each points $a \in C$ to its orthogonal projection $\text{pr}(a)$. We say that $C$ has $e$-ordering , if all points $a_i, a_j$ satisfying $ i \leq j $ have $d(\text{pr}(a_i), u) \leq d(\text{pr}(a_j), u) $. 
\end{dfn}

\begin{dfn}[Star-cover of a metric space]
\label{dfn:SeparationProperty}
Let $\{A_i\}$ be a finite cover of a metric space $(X,d)$ and assume that there exists a point $v \in X$ for which $A_j \cap A_i = \{v\}$ for all $i \neq j$. We say that $(\{A_i\},v)$ is star cover of $(X,d)$ if for all $a \in A_i, b \in A_j $ for $i \neq j$ the following two inequalities hold:  $d(a,v) \leq d(a,b)$ and $d(b,v) \leq d(a,b)$. 
\end{dfn}
%there exists $\MST(A \cup B)$ on set $A \cup B$ which is union
\begin{lem}[Minimum spanning tree gluing lemma]
\label{lem:MSTGlue} 
Assume that $(\{A,B\},v)$ is a star-cover of a finite metric space $(X,d)$. Then $\MST(A,d) \cup \MST(B,d)$ is minimum spanning tree on the set $A \cup B$. 
% and $\MST(B)$ for which $\MST(A \cup B) = \MST(A) \cup \MST(B)$.
\end{lem}
\begin{proof}
This theorem can be proved by using an alternative definition of a minimum spanning tree, i.e a given graph $G$ built on a set $X$ is $\MST$ if it is connected, acyclic and satisfies the cycle property: if we add any edge to graph $G$ then it will be the largest in the cycle that it creates. We claim that $\MST(A,d) \cup \MST(B,d)$ is one of the possible minimum spanning trees of the set $A \cup B$.

\emph{Connectedness:} First of all we note that the sets $\MST(A,d)$ and $\MST(B,d)$ are both connected and they have a non-empty intersection. It follows that $\MST(A,d) \cup \MST(B,d)$ is also connected.

\emph{Acyclic:} We will use Eucler characteristic which states that a connected graph $G$ is acyclic iff 
$\mathbb{E}(G) = \mathbb{V}(G) - 1$. By assumptions the following equations hold:
$$\mathbb{E}(\MST(A,d)) = \mathbb{V}(\MST(A,d)) - 1 \text{, } \mathbb{E}(\MST(B,d)) = \mathbb{V}(\MST(B,d)) - 1.$$ 
Also from structures of $\MST(A,d)$, $\MST(B,d)$ and $\MST(A \cup B,d)$ we obtain
$$\mathbb{V}(\MST(A \cup B,d))  = \mathbb{V}(\MST(A,d)) + \mathbb{V}(\MST(B,d)) -1\text{ and } \mathbb{E}(\MST(A \cup B,d))  = \mathbb{E}(\MST(A,d)) + \mathbb{E}(\MST(B,d))$$
Combining the equalities we get a chain of equalities which proves the claim.
$$\mathbb{V}(\MST(A \cup B,d)) - 1 = \mathbb{E}(\MST(A,d)) + \mathbb{E}(\MST(B,d)) = \mathbb{E}(\MST(A \cup B,d))  $$
 %and $$|\mathbb{E}(\MST(A) \cup \MST(B))| = |\mathbb{E}(\MST(A))| + |\mathbb{E}(\MST(B))|.$$
\emph{Cycle property:} Let $e = (u,w)$ be an edge that doesn't belong to $\MST(A,d) \cup \MST(B,d)$ and let $l$ be a path that connects $u$ with $w$ in $\MST(A,d) \cup \MST(B,d)$. If both end points of the newly added edge $e$ belong to the same set $A$ or $B$ then it has to be the longest edge by definition of $\MST(A,d)$ (or definition of $\MST(B,d)$ respectively). In case $u$ and $w$ belong to distinct sets, say $u \in A$ and $w \in B$ we note that the path $l$ has to visit the point $v$ which belongs to both sets $A$ and $B$.  Using the cycle property of $\MST(A,d)$ we deduct $d(u,v) < d(u,w)$ and respectively from cycle property of $\MST(B,d)$ we obtain $d(v,w) < d(u,w)$. 

%We will now apply 

If $(u,v)$ belongs to $\MST(A)$ and $(u,w)$ belongs to $\MST(B,d)$ then path $l$ consists of exactly two elements which are both smaller than the newly added edge. Assume now that $(u,v)$ doesn't belong to $\MST(A,d)$. Then it is the largest edge among all the edges in restriction of the path $l$ to the set $A$. Similarly, if   $d(u,w)$ doesn't belong to $\MST(B,d)$, by the cycle property all the other edges are larger. It follows that an edge $d(u,w)$ creates a cycle, where it is the largest edge. Because the points $u,w$ were selected arbitrarily, the original claim holds. 
\end{proof}


%Assume that points of $\overline{D}_e$ are ordered according to their projection $\text{pr}$ on edge $e$. Let $\overline{D}_e[u,v]$ be set of all points of $\overline{D}_e$ which project onto interval $[u,v]$.

The following two Lemmas \ref{lem:edge-offset} and \ref{lem:nonadjacentedgesgraph} will be proven in Section \ref{TechnicalSection}


\begin{restatable}[Star cover of edges]{lem}{spoe}
\label{lem:edge-offset}
%Assume that $D \cap e^\epsilon^\epsilon^\epsilon$ is $e$-ordered
%Let $\overline{D}_e[u,v]$ be set of all points of $D \cap e^\epsilon^\epsilon^\epsilon$ which project onto interval $[u,v]$.
Let $e = (u,v)$ be any edge of a straight-line tree $T\subset\R^m$. Let $\text{pr}_{e}:D \cap e^\epsilon \rightarrow e$ be a function which projects elements of $D$ in orthogonally into $e$ . For any $q \in D \cap e^\epsilon$ the pair $(\{D \cap [u,\text{pr}_e(q)]^\epsilon, D \cap [\text{pr}_e(q),v]^{\epsilon}\}, q)$ is a star cover of $(D \cap e^\epsilon,d_G)$.\end{restatable}




\begin{restatable}[Star cover of vertices]{lem}{spov}
\label{lem:nonadjacentedgesgraph}
Let $v$ be an arbitrary vertex of the straight-line graph $T$. Let $k = |\text{degree}(v)| $ and let $\{e_i \mid i \in k\}$ be the set of edges having $v$ as one of their end points. Assume that the graph $T$ is split into graphs $\{T_i \mid i \in [k]\}$ in such a way that every $T_i$ contains $v$ and all the edges and vertices  which are closer to $e_i$ than any other edge $e_j$, where $j \in [k] \setminus {i}$.  Let $D_i = \bigcup_{e \in \mathbb{E}(T_i)} e^\epsilon \cap D$. Then $(\{D_i \mid i \in [k]\}, p_v) $ is a star cover of space $(D, d_G)$. 

\end{restatable}

\begin{dfn}[Subdivision]
\label{dfn:subdivision}
Let $G$, $H$ be abstract graphs. We say that the graph $H$ is a subdivision of the graph $G$ if for every edge $e = (u,w) \in \mathbb{E}(G)$ we can find a chain of vertices $v_0, ..., v_k   \in \mathbb{V}(H)$ for which $u = v_0$, $w = v_k$ and 
$(v_i, v_{i+1}) \in \mathbb{E}(H)$ for all $i \in [k-1]$. 

\end{dfn}

\begin{pro}
\label{lem:eht}
%Let a tree $T$ be as in assumption of Theorem 
Assume the conditions of Theorem \ref{thm:GHT}. Then every edge $e = (u,v) \in \mathbb{E}(T)$ is homeomorphic to $\MST(e^{\epsilon} \cap D, d_G)$, in a way that preserves end points, i.e. given a subdivision $e'$ of $e$, the isomorphism $f_e:e' \rightarrow \MST(e^{\epsilon} \cap D, d_G)$ maps $u$ to $p_u$ and $v$ to $p_v$, where $p_u,p_v$ are the nearest neighbors of $u$ and $v$ respectively.
%there exists a subdivision of $e'$ and isomorphism $f_e:e' \rightarrow \MST(e^{\epsilon} \cap D, d_G)$ for which $f(u) = p_u$ and $f(v) = p_v$. 
\end{pro}
\begin{proof}
Let $a_0,..., a_k$ be the points of $D$ ordered by $e$-ordering. Using Lemma \ref{lem:vertex-point} we can deduct that $a_0 = p_u$ and $a_k = p_v $. Let $U_i = \{a_0,...,a_i\} $. Define the graph $G(U_i)$ as a graph having the following structure $$\mathbb{V}(G(U_i)) = \{a_0,...,a_i\} \text{\hspace{0.3cm} and \hspace{0.3cm}} 
\mathbb{E}(G(U_i)) = \{(a_0,a_1), (a_1, a_2) , ... , (a_{i-1},a_i)\}$$ 
%Let us start by noting that the set $U_0$ which consists of two elements $\{a_0, a_1\}$.
The graph $G(U_i)$ is naturally isomorphic to the edge $e$. We note that $G(U_0)$ consists of two vertices which are connected by an edge. This is isomorphic to the graph $\MST(U_0,d_G)$. 
 
Assume now that the claim holds for $U_j$. We will prove that it holds for $U_{j+1}$ as well. We should note that $U_{j+1}$ is obtained from $U_j$ by adding an extra point $a_{j+1}$. Following Lemma \ref{lem:edge-offset} the triplet $(U_j, \{a_{j}, a_{j+1}\}, a_{j})$ is a separation of $U_j$. Thus we can apply Lemma \ref{lem:MSTGlue} which states $\MST(U_{k+1},d_G) = \MST(U_{k},d_G) \cup \MST(\{a_{k},a_{k+1}\},d_G)$. Clearly $\MST(U_{k+1},d_G)$ has exactly the same structure as $G(U_{k+1})$. The induction claim holds and we can state that $\MST(U_{i},d_G) = G(U_{i})$ for all $i$, in particular for $i = k$. 

Define the graph $e'$ as a subdivision of the edge $e$ into $k-1$ parts i.e. $\mathbb{V}(e') = \{v_0, ..., v_k\}$ and 
$\mathbb{E}(e') = \{(v_0,v_1) , ... , (v_{k-1},v_k)\} $ . We can now easily construct a map $f:e' \rightarrow \MST(e^{\epsilon} \cap D,d_G)$ for which $f(v_i) = a_i$. 
%First of all we note that if $U \subseteq e \cap D$  consists of two points $a_0, a_1$, then $\MST(e \cap D)$ is . Assume now that claim holds for $e \cap D$ consisting of $k$ elements $U_{k} = \{a_0, ... , a_{k-1}\}$. We will show that $\MST(U_{k+1})$ is spanned by edges of the form $a_ia_{i+1}$.  By induction assumption this holds for  $U_k$ and 
% $\MST(\{a_{k-1},a_{k}\})$ . Because $a_{k-1}$ is separation for set $U$ which splits into two parts $\{a_{k-1},a_{k}\}$, $U_{k-1}$ we can use Lemma \ref{lem:MSTGlue} which states that $\MST(U_{k+1}) = \MST(U_{k}) \cup \MST(\{a_{k-1},a_{k}\})$ . This has the exact form we require. Thus the claim holds.
 \end{proof}

\begin{pro}[Structure of the minimum spanning tree on dense set]
\label{lem:somstod}
Assume the conditions of Theorem \ref{thm:GHT}. Then  
$\MST(D, d_{G})$ can be decomposed as union $ \bigcup_{e \in \mathbb{E}(T)} \MST(e^{\epsilon} \cap D, d_G)$.


%Assume that each set $e \cap D$ has $e$-ordering then graph $\MST(D, d_{G})$ has the following form:  For every edge $e$ in the set $a_i \in e \cap D$ all the adjacent vertices $a_i, a_{i+1}$ generate an edge in graph $\MST(D, d_{G}) $. 
 %Each edge $e \in \text{Edges}(\MST(D, d_{G}))$ consists 

%Graph $\MST(D, d_{G})$ has the following form: The vertex set consists of all the points in set $D$. 

%Every edge $e = (u,v)$ has one of the following form: 
%\begin{enumerate}
%\item one
%\item two
%\end{enumerate}

\end{pro}
%where $R_{i+1}$ is obtained from $R_i$ by adding a vertex outside of $R_i$ and connected it by an edge.
\begin{proof}

Let us define a filtration $\{v\} = R_0 \subseteq R_1 \subseteq R_{2} \subseteq R_{3} \subseteq ... \subseteq R_{t} = T $, where each $R_{i+1}$ introduces a new vertex and an edge from graph $T$ which are not contained in the previous element $R_{i}$. Assume that $\MST(R_{k})$ can be decomposed . Let a vertex $y$ and an edge $e = [u,y]$ be recently added ingredients to $R_{k+1}$. Following from Lemma \ref{lem:nonadjacentedgesgraph} we know that $(\{R_k,e^{\epsilon} \cap D\},u) $ is a star-cover of $R_{k+1}$. Using Lemma \ref{lem:MSTGlue} we obtain that $\MST(R_k) \cup \MST(e^\epsilon \cap D)$ is a minimum spanning tree on set $R_{k+1}$. The claim follows from this , as we know that
 $$\MST(R_k,d_G) \cup \MST(e^\epsilon \cap D,d_G) = \bigcup_{e \in \mathbb{E}(R_{k+1})}\MST(e^{\epsilon} \cap D,d_G).$$

%Thus $R_{k+1}$ is spanned by all the edges having adjacent indices in sets $D_q$, where $q$ is edge added in $R_i$ for some index $i \leq k+1$ . Thus we have proved that the Lemma holds for whole graph.



\end{proof}
%construct a map from some subdivision of $T$ into $\MST(D, d_G)$. 
Proving Theorem \ref{thm:GHT} is now easy. We simply need to subdivide the graph $T$ into some graph $T'$ and construct an isomorphism $f: T' \rightarrow \MST(D, d_G) $.


\begin{proof}[\textbf{Proof of theorem \ref{thm:GHT}:}]
From Proposition \ref{lem:somstod} we obtain $\MST(D, d_{G}) = \bigcup_{e \in \mathbb{E}(T)} \MST(e^{\epsilon} \cap D, d_G)$. Proposition \ref{lem:eht} states that every $e \in \mathbb{E}(T)$ is homeomorphic to $ \MST(e^{\epsilon}  \cap D, d_G)$, in such a way that there exists a subdivision $e'$ of $e = [u,v]$ and a map $f_e: e' \rightarrow \MST(e^{\epsilon})$ for which  $f_e(u) = p_u$ and $f_e(v) = p_v$. Let us define the graph $T'$ as the union of subdivided edges 
$ \bigcup_{e \in \mathbb{E}(T)} e'$ and the map $f:T' \rightarrow \MST(D, d_G)$ as $f = \bigcup_{e \in \mathbb{E}(T)}f_e$. 

The map $f$ is well-defined: Let $e, w$ be distinct edges of $\mathbb{E}(T)$. They intersect at most at one vertex $v$. In this case both of the maps $f_e$ and $f_w$ map $v$ into $p_v$.

The map $f$ is a graph-homomorphism: This follows directly from the fact that every edge $e \in \mathbb{E}(T')$ is completely contained in one of the sets $\mathbb{E}(e')$. Thus the claim follows directly from a property of the map $f_e$. 

The map $f$ is an isomorphism, because every map in the union is an isomorphism. 

Thus we have found a map  $f: T' \rightarrow \MST(D, d_G) $ which is a graph isomorphism. The claim holds. 


\end{proof}


\section{Technical results }
\label{TechnicalSection}

In this section we handle the technical side of the main theoretical result. 
% which have angle $\theta$ between them and a common vertex $v$. 


\begin{lem}
\label{AdjacentEdgesLemma}

Let $e$ and $h$ be adjacent edges of a graph $T$ via vertex $v$. Denote by $\theta$ be the angle between the edges $e$ and $h$ and let $r \in \R_{+}$ be a positive real number.  Let
$$\mathcal{A}(e,h,r) = \{q \in e^{\epsilon} \mid \text{ there exists } t \in h^{\epsilon} \text{ for which } d_E(q, t) < r\}. $$
 Then for any point $q \in \mathcal{A}(e,h,r)$ the following inequality is satisfied:

$$d_E(q, v) \leq  \dfrac{\epsilon}{\sin(\frac{\theta}{2})} +  \dfrac{r}{\sin(\min(\theta, \frac{\pi}{2}))} $$ 
%\begin{align*}
%\centering
%    d(q, v) \leq \begin{cases}
%              \frac{\epsilon}{\sin(\frac{\theta}{2})} +  \frac{r}{\sin(\theta)}  & \text{if } \theta < \frac{\pi}{2},\\
%             \frac{\epsilon}{\sin(\frac{\theta}{2})} +  r & \text{if } \theta \geq \frac{\pi}{2}
%          \end{cases}
%\end{align*}

\end{lem}
\begin{proof}

\begin{figure}
    \centering
    \begin{tikzpicture}
  \draw
    (8,-3) coordinate (a) node[right] {}
    -- (0,0) coordinate (v) node[left] {v}
    -- (8,3) coordinate (c) node[above right] {}
    pic["$\theta$", draw=orange, <->, angle eccentricity=1.2, angle radius=1cm]
    {angle=a--v--c};
    \draw[dashed]
    (8,-1.5) coordinate (a2) node[right] {}
    -- (4,0) coordinate (v2) node[above] {w}
    -- (8,1.5) coordinate (c2) node[above right] {}
    pic["$\theta$", draw=orange, <->, angle eccentricity=1.2, angle radius=1cm]
    {angle=a2--v2--c2};
    \draw[loosely dashed] (v) -- node[below] {} node[above] {} ++ (v2);
    \filldraw[black] (4,0) circle (2pt);
    \filldraw[black] (0,0) circle (2pt);

    \filldraw[black] (3.5,-1.3) circle (2pt) coordinate (cc) node[anchor = north ]{c};
    \draw[loosely dashed] (v2) -- (cc);
    \draw(3.5,-0.6) coordinate (uv) node{$\epsilon$}; 
   % \tkzMarkRightAngle[size=.2](v,cc,v2);
    \filldraw[black] (8,-1.5) circle (2pt) coordinate (q) node[anchor = west]{q};
    \filldraw[black] (6.8,1.05) circle (2pt) coordinate (t) node[anchor = west]{t};
    \draw[loosely dashed] (q) -- (t);
   % \tkzMarkRightAngle[size=.2](q,t,v2);
    
    \draw(2.5, -1.25) coordinate (ne) node{$e$};
    \draw(2.5, 1.25) coordinate (nh) node{$h$};

    
    
\end{tikzpicture}
    \caption{Proof of Lemma \ref{AdjacentEdgesLemma}. In this picture we have illustrated the special case when $q$ is on the boundary of the set $e^\epsilon$}
    \label{fig:Lemma12}
\end{figure}

Let us first consider the case where $\theta \leq \frac{\pi}{2}$. Let $q \in \mathcal{A}(e,h,r)$ be an arbitrary point and let $l$ be a line that goes through the point $q$ and is parallel to $e$. Let $w$ be the closest point to $q$ of the intersection $l \cap h^{\epsilon}$. Let $t \in h^{\epsilon}$ be a point which is closest to $q$. As illustrated in Figure \ref{fig:Lemma12} $\triangle wtq$ is a right triangle. Thus by using the sinus theorem we obtain: $$d_E(w,q) = \dfrac{d_E(q,t)}{\sin(\theta)} \leq \dfrac{r}{\sin(\theta)}. $$ Let $c \in e$ be the point that is closest to $w$. We note now that $\triangle vcw$ is also a right triangle. Again using the sinus theorem and the facts that $\angle wvc \leq \frac{\theta}{2}$ and $d_E(w,c) \leq  \epsilon$ we obtain 
$$d_E(v,w) = \frac{d_E(w,c)}{\sin(\angle wvc)} \leq   \frac{\epsilon}{\sin(\frac{\theta}{2})} $$
Combining the previous two inequalities with the triangle inequality we obtain
$$d_E(v,q) \leq d_E(v,w) + d_E(w,q) \leq \sin(\frac{\theta}{2})\epsilon +  \frac{r}{\sin(\theta)}. $$

In the case angle $\theta \geq \frac{\pi}{2}$ the intersection point $t$ is located on the other side of $w$ in line which is parallel to $h$. Thus $\triangle wqt$ forms a right triangle again, where $qt$ is the longest side. Thus we can simply estimate $d(q,w) \leq d(q,t) \leq r$ and obtain the inequality $$ d_E(q, v) \leq \dfrac{\epsilon}{\sin(\frac{\theta}{2})} +  r  $$
which proves this lemma. 



\end{proof}

It should be noted that if in Lemma \ref{AdjacentEdgesLemma} $r  = \delta$ then we can state 
$$\dfrac{\epsilon}{\sin(\frac{\theta}{2})} +  \dfrac{r}{\sin(\min(\theta, \frac{\pi}{2}))} = \frac{\delta}{2\gamma} - \epsilon$$ 
%\begin{remark}
%$ \frac{\delta}{2\gamma} - \epsilon $
%\end{remark}


\begin{lem}[Structure of a path $s$ between two points of the  graph $G$] 
\label{structureofpaths}
Let $s$ be a path connecting points $a,b$ in the graph $G$. Then for every index $i$ of the path $s$ the following holds true: 
Assume that $s(i) \in D \cap e^\epsilon $ and $s(i+1) \in D \cap h$. Then either $e = h$, or $e$ and $h$ share a common vertex in the graph $T$. 
\end{lem}
\begin{proof}
Make the counter assumption that $e$ and $h$ are non adjacent edges. By assumption of the graph $G$ the following inequality is satisfied: $l_{\max}(G) < r - 2\epsilon $ , where $r$ is the minimal length of non-adjacent edges. Using the triangle inequality
 $$d(a,b) \geq d(e,h) - d(a,e) - d(h,b) > e_{\max}(G)$$
which is a contradiction, as we have assumed that $d(a,b) \leq e_{\max}(G)$ for all $a,b \in G$. 
\end{proof}



\begin{dfn}
\label{shortestPathConnecting}
Let $s$ be the shortest path connecting points $a,b$ in the graph $G$. Assume that $a \in D \cap e^\epsilon$ and $b \in D \cap h$ for $e \neq h$. We define the path $L(s)$ in the graph $T$ as the shortest path connecting the edges $e$ and $h$.  
\end{dfn}

\begin{lem}[Existence of vertex-link]
\label{ExistenceOfVertexLink}
Let $s$ be the shortest path connecting points $a,b$ in the graph $G$. Assume that $a \in D \cap e^\epsilon$ and $b \in D \cap h$ for $e \neq h$ and let $v$ be an arbitrary vertex in $L(s)$. Then there exists an index $i$ and edges $e',h'$ that have a common vertex $v$ and which satisfy $s(i) \in C \cap e^\epsilon$ and $s(i+1) \in C \cap h'$.
%for which there exists edges $e'$ and $h'$ which have a common vertex $v$ and for which $s(i) \in \overline{D}_{e'}$ and  $s(i+1) \in \overline{D}_{h'}$. 
\end{lem}
\begin{proof}
Make the counter assumption that there doesn't exist such index $i$. Let $x,y$ be the two edges which are present in the path $l$ connecting the edges $e$ and $h$ in the straight-line tree $T$ having $v$ as their common vertex. We will first prove that there exist indices $j,k$ for which 
$s(j) \in C \cap x$ and $s(k) \in C \cap y$. We will prove this claim only for $x$. The proof for the edge $y$ is symmetric. 

First of all we note that removing the edge $x$ splits the graph $T$ into two connected components $C_1$ and $C_2$ i.e. every pair of edges belonging to $C_1 \times C_2$ is non-adjacent. From Lemma \ref{structureofpaths} we obtain that path $s$ stays in edge-sets $C_f$ having either $f \in C_1$ or $f \in C_2$ for all $f \in \mathbb{E}(T)$. However this is a contradiction, because $a,b$ belong to edge-sets of different components. 

In case $j + 1 = k$ we are done with the proof. Assume that $j + 1 \neq k$. Let $j'$ be the largest index satisfying $s(j') \in D \cap x$. Using Lemma  \ref{structureofpaths} we know that $s(j'+1)$ should belong to either the edge-set of the edge having common vertex $v$ with $x$ or an edge-set of the other vertex $u$ of the edge $x$. If it belongs to another edge-set of the vertex $v$, then the proof is complete, as we can select indices $j',j'+1$ which satisfy the assumption.

Assume that it belongs to another edge-set of vertex $u$. Again by using Lemma \ref{structureofpaths} we can deduct that the path $s$ have to eventually visit $D \cap x$ again. This will happen for some index $t > j'$, which is a contradiction. Thus we can deduct that the indices $j',j'+1$ satisfy the condition of this lemma and we are done with the proof. 

% Assume first that for every index $i$ the following holds true: $s(i) \notin \overline{D}_e $ for all the edges $e$ having $v$ as one of their vertex. By removing $v$ 
\end{proof}

\spov*

\begin{proof}



Let $s$ be the shortest path connecting the points $a \in \overline{D}_e $ and $b \in \overline{D}_h$ in the graph $G$. Let $v$ be an arbitrary vertex that belongs to the path $L(s)$ of $T$. Our goal is to prove that $d_G(p_v,a) \leq d_G(a,b)$ and $d_G(p_v,b) \leq d_G(a,b)$. Using Lemma \ref{ExistenceOfVertexLink} we obtain an index $i$ and edges $f,g$ having a common vertex $v$ which satisfy
  $s(i) \in \overline{D}_{f}$ and $ s(i+1) \in \overline{D}_{g}$. 
% \frac{\epsilon}{\sin(\frac{\theta}{2})} +  \frac{l_{\max}(G)}{\sin(\min(\theta,\frac{\pi}{2}))}
We can now use Lemma \ref{AdjacentEdgesLemma} with a bound $l_{\max}(G)$ we obtain  $d_E(s(i),p_v) \leq \frac{\delta}{2} $ , where $\theta$ is the smallest angle over all the adjacent edges. Using triangle inequalities we obtain the following chain: 
%$$d_k(p_v, s(\alpha)) \leq & d_k(p_v,v) + d_k(v,s(\alpha)) \leq  c_{\max}(t_{\epsilon}(p_v,v) + t_{\epsilon}(v,s(\alpha)) \leq c_{\max}(\epsilon+ \frac{\epsilon}{\sin(\frac{\theta}{2})}  +  %\frac{r}{\sin(\theta )}) $$
%\gamma(\epsilon+ \frac{\epsilon}{\sin(\frac{\theta}{2})} + \frac{l_{\max}(G)}{\sin(\theta )})

$$d_G(p_v, s(i)) \leq d_G(p_v,v) + d_G(v,s(i)) \leq  \gamma(d_E(p_v,v) + d_E(v,s(i)) \leq  \gamma(\frac{\delta}{2\gamma} - \epsilon) +  \gamma \epsilon \leq  \frac{\delta}{2} $$
Using triangle inequalities we also obtain $$d_k(a, s(i)) \geq d_G(a,p_v) - d_G(p_v,s(i)) > \delta - \frac{\delta}{2} > \frac{\delta}{2} $$
$$d_G(b, s(i+1)) \geq d_G(b,p_v) - d_G(p_v,s(i+1)) > \delta - \frac{\delta}{2} \geq \frac{\delta}{2} $$
%\gamma(\epsilon+ \frac{\epsilon}{\sin(\frac{\theta}{2})} + \frac{l_{\max}(G)}{\sin(\theta )})
We note that because $d_G$ is a path-metric we can split it into parts. Together with the previous inequalities we obtain the following chains: 
 \begin{equation*}
 \begin{aligned}
 d_G(a,b) \geq & d_G(a,s(i)) + d_G(s(i+1), b)  \\
     >    &  d_G(a,s(i))  + \frac{\delta}{2} \\
     \geq &  d_G(a,s(i))  + d_G(p_v,s(i)))\\
      \geq & d_G(a,p_v) 
 \end{aligned}
 \end{equation*}
Using a similar inequality we obtain that $ d_G(a,b) > d_G(b,p_v) $. Thus the claim holds. 

\end{proof}

\spoe*


\begin{proof}
 Let $p'$, $q'$ and $r'$ be the orthogonal projections of points $p,q$ and $r$ respectively. We can use exactly the same proof strategy as in \ref{lem:nonadjacentedgesgraph} by noting that we can subdivide edge $e$ by adding vertex $q'$ for which $d(q,q') < \epsilon$. 
% 
% We can subdivide graph $T$ by defining $p',q',r'$ to be the new vertices. Each of the distances $d(p',p)$, $d(q,q')$, $d(r,r')$ is under $\epsilon$. Thus $[p',q']$ and $[q',r']$ can be treated as neighboring edges and  we can apply Lemma \ref{lem:vertexSeparation} to get the result $d(p,q) < d(q,r)$ and $d(q,r) < d(p,r)$.
\end{proof}





==> chapters/chapterKNN.tex <==
\chapter{Spatial algorithms} % Write in your own chapter title


\section{Space partitioning data structures}
\label{sec:SpacePartDataStructure}
Space partitioning data structures are multidimensional analogues of binary search trees, often employed for storing spatial data. They were  developed to gain a near-logarithmic query time to nearest neighborhood problem, but were later utilized to assist in resolving more complex tasks as well. The most notable examples of the space partitioning data-structures are: Quadtree \cite{finkel1974quad}, Octatree  \cite{jackins1980oct} ,  $k$-d tree  \cite{bentley1975multidimensional} built on a finite data set of $\R^k$ and CoverTree \cite{beygelzimer2006cover} can be applied on a finite metric spaces. In the following example we show how a $k$-d tree is constructed starting from a dataset in $\R^k$. 

%For $k = 3$ For example, in a 3-dimensional tree, the root would have an x-aligned plane, the root's children would both have y-aligned planes, the root's grandchildren would all have z-aligned planes, the root's great-grandchildren would all have x-aligned planes, the root's great-great-grandchildren would all have y-aligned planes, and so on.). This process have been formalized in Algorithm \ref{alg:constructKDTree}.

    \begin{algorithm}[H]
\caption{k-dtree(pointSet, depth)}
\label{alg:constructKDTree}
\begin{algorithmic}[1]
\STATE \textbf{Input} : pointList, depth,
\STATE \textbf{Output} : Root
\STATE 				  we select \textbf{axis} indexed by depth mod k
\STATE                select median by \textbf{axis} from pointList
\STATE 			      Create new Root node
\STATE                Root.location $\gets$ median\;
\STATE                Root.left $\gets$ k-dtree(points {\bf in} pointSet {\bf before} median, depth + 1)
\STATE                Root.right $\gets$ k-dtree(points {\bf in} pointSet {\bf after} median, depth + 1)
\end{algorithmic}
\end{algorithm}

\begin{exa}[$k$-d tree example]
\label{exa:KDTree}

There are many different ways of constructing $k$-d tree. In this example we show one of them. 
Assume that we are given a dataset in an Euclidean space $\R^k$. During the iteration we will cycle through the $k$ axes. The tree is constructed by splitting the current dataset into two equal parts and then calling the $k$-d tree construction algorithm recursively on the two parts. Splitting the dataset will be done by selecting a plane orthogonal to one of the axes, which halves the dataset and allocating sets belonging to different sides of the plane to different nodes. As we go down the tree we cycle through the axes. Consider the following data set in $C$ in $\R^2$: $  A_0 = \{(1, 9), (2, 3), (4, 1), (3, 7), (5, 4),(6, 8), (7, 2), (8, 8), (7, 9), (9, 6)\} $
%        \begin{equation*}\begin{split}
%           A_0 = \{&(1, 9), (2, 3), (4, 1), (3, 7), (5, 4),(6, 8), (7, 2), (8, 8), (7, 9), (9, 6)\}
%        \end{split}\end{equation*}
  \begin{figure}[H]
    \centering

   \tikzset{
                        up/.style = {fill = orange!90!blue,
                            label = center:\textsf{\Large X}},
                        down/.style = {fill = blue!70!yellow, text = black,
                            label = center:\textsf{\Large Y}}
                    }
                    \begin{tikzpicture}[
                        scale = 0.8, transform shape, thick,
                        every node/.style = {draw, circle, minimum size = 10mm},
                        grow = down,  % alignment of characters
                        level 1/.style = {sibling distance=3cm},
                        level 2/.style = {sibling distance=6cm},
                        level 3/.style = {sibling distance=4cm},
                        level distance = 2cm
                    ]
                    \node[shape = rectangle, rounded corners, minimum width = 4cm] {The dataset}
                    child{
                        node[up](Start){}
                        child{
                            node [down] (A) {}
                            child{
                                node [shape = rectangle, rounded corners, text width = 10mm] (B) {
                                    (2, 3) (4, 1)
                                }
                            }
                            child{
                                node [shape = rectangle, rounded corners, text width = 10mm] (C) {
                                    (1, 9)
                                    (3, 7)
                                    (5, 4)
                                }
                            }
                        }
                        child{
                            node [down] (D) {}
                            child {
                                node [shape = rectangle, rounded corners, text width = 10mm] (E) {
                                    (7, 2)
                                    (9, 6)
                                }
                            }
                            child {
                                node [shape = rectangle, rounded corners, text width = 10mm] (F) {
                                    (6, 8)
                                    (7, 9)
                                    (8, 8)
                                }
                            }
                        }
                    };

                    % Labels
                    \begin{scope}[nodes = {draw = none}]
                        \path (Start) -- (A) node [near start, left]  {$<6$};
                        \path (A)     -- (B) node [near start, left]  {$<4$};
                        \path (A)     -- (C) node [near start, right] {$\geq4$};
                        \path (Start) -- (D) node [near start, right] {$\geq6$};
                        \path (D)     -- (E) node [near start, left]  {$<8$};
                        \path (D)     -- (F) node [near start, right] {$\geq8$};
                    \end{scope}
                \end{tikzpicture}    
    \small
\begin{tikzpicture}[scale = 0.7]
  % Axes.
  \coordinate (Origin) at (0.25, 0.25);
  \coordinate (XAxisMin) at (0.25, 0.25);
  \coordinate (XAxisMax) at (9.75, 0.25);
  \coordinate (YAxisMin) at (0.25, 0.25);
  \coordinate (YAxisMax) at (0.25, 9.75);
  \draw [thin, gray, -latex] (XAxisMin) -- (XAxisMax);
  \draw [thin, gray, -latex] (YAxisMin) -- (YAxisMax);
%
%  % S_r
 \filldraw[fill=gray] (0.25, 0.25) -- (0.25, 9.75) -- (9.75, 9.75) -- (9.75, 0.25) -- cycle;  
 \node [ ] at (6, 0.35) { $A_0$ };
 
  \filldraw[fill=lightgray] (0.5, 0.5) -- (0.5, 9.5) -- (5.25, 9.5) -- (5.25, 0.5) -- cycle;
  
   \filldraw[fill=lightgray] (5.75, 1.5) -- (5.75, 9.5) -- (9.5, 9.5) -- (9.5, 1.5) -- cycle;
    \node [ ] at (3.1, 1.0) { $A_1$ };
    \node [ ] at (8.1, 2.35) { $A_2$ };
%
%  % S_p
%  \filldraw[fill=lightgray] (1, 2) -- (1, 3) -- (2, 3) -- (2, 2) -- cycle;
%  \node [ ] at (2.3, 2.5) { $\mathcal{S}_p$ };
%
%  % Points x_1 to x_5.
%  \node [draw, circle, inner sep=1pt, fill] at (2, 2) { };
%  \node [ ] at (2.2, 1.8) { $x_1$ };
%
%  \node [draw, circle, inner sep=1pt, fill] at (1, 2.5) { };
%  \node [ ] at (1.2, 2.3) { $x_2$ };
%
%  \node [draw, circle, inner sep=1pt, fill] at (0.5, 0.5) { };
%  \node [ ] at (0.7, 0.3) { $x_3$ };
%
%  \node [draw, circle, inner sep=1pt, fill] at (1, 3) { };
%  \node [ ] at (1.2, 2.8) { $x_4$ };
%
%  \node [draw, circle, inner sep=1pt, fill] at (1.5, 2.5) { };
%  \node [ ] at (1.7, 2.3) { $x_5$ };
  
  
  \node [draw, circle, inner sep=1pt, fill] at (1, 9) { };
    \node [ ] at (1.2, 8.8) { $(1,9)$ };
  \node [draw, circle, inner sep=1pt, fill] at (2, 3) { };
   \node [ ] at (2.2,2.8) { $(2,3)$ };
  \node [draw, circle, inner sep=1pt, fill] at (4, 1) { };
     \node [ ] at (4.2,0.8) { $(4,1)$ };
  \node [draw, circle, inner sep=1pt, fill] at (3, 7) { };
     \node [ ] at (3.2,6.8) { $(3,7)$ };
  \node [draw, circle, inner sep=1pt, fill] at (5, 4) { };
    \node [ ] at (5.2,3.8) { $(5,4)$ };
  \node [draw, circle, inner sep=1pt, fill] at (6, 8) { };
     \node [ ] at (6.2,7.8) { $(6,8)$ };
  \node [draw, circle, inner sep=1pt, fill] at (7, 2) { };
     \node [ ] at (7.2,1.8) { $(7,2)$ };
  \node [draw, circle, inner sep=1pt, fill] at (8, 8) { };
     \node [ ] at (8.2,7.8) { $(8,8)$ };
  \node [draw, circle, inner sep=1pt, fill] at (7, 9) { };
     \node [ ] at (7.2,8.8) { $(7,9)$ };
  \node [draw, circle, inner sep=1pt, fill] at (9, 6) { };
     \node [ ] at (9.2,5.8) { $(9,6)$ };
  
  
  

\end{tikzpicture}    
\small
\begin{tikzpicture}[scale = 0.7]
  % Axes.
  \coordinate (Origin) at (0.25, 0.25);
  \coordinate (XAxisMin) at (0.25, 0.25);
  \coordinate (XAxisMax) at (9.75, 0.25);
  \coordinate (YAxisMin) at (0.25, 0.25);
  \coordinate (YAxisMax) at (0.25, 9.75);
  \draw [thin, gray, -latex] (XAxisMin) -- (XAxisMax);
  \draw [thin, gray, -latex] (YAxisMin) -- (YAxisMax);
  \definecolor{lgray}{gray}{0.85}
%
%  % S_r
 \filldraw[fill=gray] (0.25, 0.25) -- (0.25, 9.75) -- (9.75, 9.75) -- (9.75, 0.25) -- cycle;  
% \node [ ] at (6, 0.35) { $A_0$ };
 
  \filldraw[fill=lightgray] (0.5, 0.5) -- (0.5, 9.5) -- (5.25, 9.5) -- (5.25, 0.5) -- cycle;
  
   \filldraw[fill=lightgray] (5.75, 1.5) -- (5.75, 9.5) -- (9.5, 9.5) -- (9.5, 1.5) -- cycle;
   

  \filldraw[fill=lgray] (1.75, 0.75) -- (1.75, 3.25) -- (4.25, 3.25) -- (4.25, 0.75) -- cycle;
  
   \filldraw[fill=lgray] (0.75, 3.75) -- (0.75, 9.25) -- (5.125, 9.25) -- (5.125, 3.75) -- cycle;
   
    \filldraw[fill=lgray] (5.85, 7.75) -- (8.25, 7.75) -- (8.25, 9.25) -- (5.85, 9.25) -- cycle;
    
     \filldraw[fill=lgray] (6.75, 1.75) -- (9.25, 1.75) -- (9.25, 6.25) -- (6.75, 6.25) -- cycle;
  
  % \filldraw[fill=lightgray] (5.75, 1.5) -- (5.75, 9.5) -- (9.5, 9.5) -- (9.5, 1.5) -- cycle;   
   
  %  \node [ ] at (3.1, 1.0) { $A_1$ };
  %  \node [ ] at (8.1, 2.35) { $A_2$ };
%
%  % S_p
%  \filldraw[fill=lightgray] (1, 2) -- (1, 3) -- (2, 3) -- (2, 2) -- cycle;
%  \node [ ] at (2.3, 2.5) { $\mathcal{S}_p$ };
%
%  % Points x_1 to x_5.
%  \node [draw, circle, inner sep=1pt, fill] at (2, 2) { };
%  \node [ ] at (2.2, 1.8) { $x_1$ };
%
%  \node [draw, circle, inner sep=1pt, fill] at (1, 2.5) { };
%  \node [ ] at (1.2, 2.3) { $x_2$ };
%
%  \node [draw, circle, inner sep=1pt, fill] at (0.5, 0.5) { };
%  \node [ ] at (0.7, 0.3) { $x_3$ };
%
%  \node [draw, circle, inner sep=1pt, fill] at (1, 3) { };
%  \node [ ] at (1.2, 2.8) { $x_4$ };
%
%  \node [draw, circle, inner sep=1pt, fill] at (1.5, 2.5) { };
%  \node [ ] at (1.7, 2.3) { $x_5$ };
  
  
  \node [draw, circle, inner sep=1pt, fill] at (1, 9) { };
    \node [ ] at (1.2, 8.8) { $(1,9)$ };
  \node [draw, circle, inner sep=1pt, fill] at (2, 3) { };
   \node [ ] at (2.2,2.8) { $(2,3)$ };
  \node [draw, circle, inner sep=1pt, fill] at (4, 1) { };
     \node [ ] at (4.2,0.8) { $(4,1)$ };
  \node [draw, circle, inner sep=1pt, fill] at (3, 7) { };
     \node [ ] at (3.2,6.8) { $(3,7)$ };
  \node [draw, circle, inner sep=1pt, fill] at (5, 4) { };
    \node [ ] at (5.2,3.8) { $(5,4)$ };
  \node [draw, circle, inner sep=1pt, fill] at (6, 8) { };
     \node [ ] at (6.2,7.8) { $(6,8)$ };
  \node [draw, circle, inner sep=1pt, fill] at (7, 2) { };
     \node [ ] at (7.2,1.8) { $(7,2)$ };
  \node [draw, circle, inner sep=1pt, fill] at (8, 8) { };
     \node [ ] at (8.2,7.8) { $(8,8)$ };
  \node [draw, circle, inner sep=1pt, fill] at (7, 9) { };
     \node [ ] at (7.2,8.8) { $(7,9)$ };
  \node [draw, circle, inner sep=1pt, fill] at (9, 6) { };
     \node [ ] at (9.2,5.8) { $(9,6)$ };
  
  
  

\end{tikzpicture}    
    \caption{Building a $k$-d tree from training data.}
    \end{figure}
        
        
	 We first note that a line, which perpendicular to the $x$-axis and intersects the $x$-axis at point $(6,0)$, splits the dataset into two equal parts. This line will define two new nodes $A_1,A_2$ that will be connected to the original dataset $A_1$, that will serve as the root node. 
	 \begin{equation*}\begin{split}
            A_1 = \{&(2,3), (4,1), (1,9), (3,7), (5,4)\}\\
            A_2 = \{ &(7,2), (9,6), (6,8), (7,9) , (8,8)\}
        \end{split}\end{equation*}
       Next split $A_1$ into two nearly-equal parts: the first child will consist of the points for which $y$-coordinate satisfies
        $y < 4$ and the other child that satisfies $y \geq 4$. Similarly $A_2$ gets split on points for which $y$-coordinate satisfies $y < 8$ and points 
        for which $y \geq 8$. 
        
      %  We then similarly split the two obtained nodes by splitting 
        
      %   obtain the following figure:
       % The first will be split at point $y = 4$ and the second at $y = 8$, which will split the two aforementioned parts into similar-sized sets. 

\end{exa}

%
%\begin{figure}[H]
%\centering
%               
%                 
%            \caption{ }
%    \end{figure}
    
  

% we start with Definition \ref{dfn:SpacePartioningDatastructure}




\subsection{Cover trees}
\label{sec:CoverTrees}
The cover tree is a complex data structure that allows near-linear time worst-time complexity bounds for tasks such as nearest neighborhood search 
(Section \ref{sec:knn} ),  computation of minimum spanning tree on a point cloud (Section \ref{sec:MST}), and kernel density estimation (Section \ref{sec:KDETheorySec}).
This section presents the key definition and state important properties of the cover tree data structure.


%In this section we serve only elementary introduction to the definitions and basic properties of the cover-tree data structure. 
\begin{figure}[H]

\centering
\begin{tikzpicture}[align=center, node distance = 1.25cm, scale = 0.5]
    % Place nodes
    
%    \node [blockz] (init) {1};
%    \node [left of=init](scaleinf) {$C_{\infty}$};
%   % \node [cloud, left of=init] (expert) {expert};
%    \node [blockz, below of=init] (scale0) {1};
%    \node [left of=scale0](scale0text) {$C_{0}$};
%
%	\node [blockz, below left of =scale0] (scalem1a) {1};
%	\node [blockz, below right of =scale0] (scalem1b) {2};
%	\node [left of=scalem1a](scalem1text) {$C_{-1}$};
	
	\node (scaleminftext) {$C_{-\infty}$};
	\node [blockz, right of =scaleminftext] (scaleminf1) {1};
	\node [blockz, right of =scaleminf1] (scaleminf2) {2};
	\node [blockz, right of =scaleminf2] (scaleminf3) {3};
	\node [blockz, right of =scaleminf3] (scaleminf4) {4};
	\node [blockz, right of =scaleminf4] (scaleminf5) {5};

	\node [above of =scaleminftext](scalem1text) {$C_{-1}$};
	\node [blockz, above of =scaleminf1] (scalem11) {1};
	\node [blockz, above of =scaleminf2] (scalem12) {2};
	\node [blockz, above of =scaleminf3] (scalem13) {3};
	\node [blockz, above of =scaleminf4] (scalem14) {4};
	\node [blockz, above of =scaleminf5] (scalem15) {5};
	
	\node [above of =scalem1text](scale0text) {$C_{0}$};
	\node [blockz, above of =scalem11] (scale01) {1};
	\node [blockz, above of =scalem13] (scale03) {3};
	\node [blockz, above of =scalem15] (scale05) {5};	
	
	\node [above of =scale0text](scale1text) {$C_{1}$};
	\node [blockz, above of =scale01] (scale11) {1};
	\node [blockz, above of =scale05] (scale15) {5};
	
	\node [above of =scale1text](scale2text) {$C_{2}$};
	\node [blockz, above of =scale11] (scale21) {1};

	
	\node [above of =scale2text](scaleinftext) {$C_{\infty}$};
	\node [blockz, above of =scale21] (scaleinf1) {1};

	

  %  \node [block, below of=init] (identify) {identify candidate models};
  %  \node [block, below of=identify] (evaluate) {evaluate candidate models};
  %  \node [block, left of=evaluate, node distance=3cm] (update) {update model};
  %  \node [decision, below of=evaluate] (decide) {is best candidate better?};
  %  \node [block, below of=decide, node distance=3cm] (stop) {stop};
    % Draw edges
    
      \draw[dashed,->] (scalem11) -> (scaleminf1);
      \draw[dashed,->] (scalem12) -> (scaleminf2);
      \draw[dashed,->] (scalem13) -> (scaleminf3);
      \draw[dashed,->] (scalem14) -> (scaleminf4);
      \draw[dashed,->] (scalem15) -> (scaleminf5);
      

	  \draw[->] (scale01) -> (scalem11);
	  \draw[->] (scale03) -> (scalem13); 
	  \draw[->] (scale05) -> (scalem15);     
	  
	  \draw[->] (scale01) -> (scalem12);
	  \draw[->] (scale03) -> (scalem14);
	  
	  \draw[dashed,->] (scaleinf1) -> (scale21);
	  \draw[->] (scale21) -> (scale11);
	  \draw[->] (scale15) -> (scale05);
	  
	  \draw[->] (scale11) -> (scale01);
	  \draw[->] (scale11) -> (scale03);
	  \draw[->] (scale21) -> (scale15);
      
 %    \draw[->] (scale0) -> (scalem1a);
 %    \draw[->] (scale0) -> (scalem1b);
 %    \draw[dashed,->] (scalem1a) -> (scaleminfa);
 %    \draw[dashed,->] (scalem1b) -> (scaleminfb);
 
  %  \path [line] (init) -> (kde);
  %  \path [line] (kde) -> (clustering);
  %  \path [line] (clustering) -> (cmp);
  %  \path [line] (cmp) -> (mst);
    %\path [line] (identify) -- (evaluate);
    %\path [line] (evaluate) -- (decide);
    %\path [line] (decide) -| node [near start] {yes} (update);
    %\path [line] (update) |- (identify);
    %\path [line] (decide) -- node {no}(stop);
    %\path [line,dashed] (expert) -- (init);
    %\path [line,dashed] (system) -- (init);
    %\path [line,dashed] (system) |- (evaluate);
\end{tikzpicture}

\caption{Let $X = \{1,2,3,4,5\}$ and let $d(x,y) = |x-y|$. In this figure we have illustrated a cover tree (Definition \ref{covertreedefinition} ) built on  the space $X$. 
}
\label{fig:CoverTree}

%Implicit representation of the cover tree of Example \ref{CovertreeExample}. Explicit representation is obtained by collapsing all the infinite dashed chains into a single node}
%\label{fig:GraphicalRepresentationCoverTree}
\end{figure}

\begin{dfn}[Cover tree  {\cite[Section. ~ 2]{beygelzimer2006cover}}  ]
\label{covertreedefinition}

Let $(X,d)$ be a finite metric space. Consider subsets $C_s$ (that will be called level $s$) of $X$ satisfying the following conditions:



%A \emph{cover tree}  $\mathcal{T}$ on a finite metric space $(X,d)$ is a leveled tree, where balls centered at nodes at a certain level cover the levels beneath it. Every node $p_i \in \mathcal{T}$ is associated with a point in $X$ and is located at scale $s_i$ in the cover tree. Each point in $X$ may be associated with multiple nodes in the tree; however, every point can appear at most once in every level. The set of points located at scale $i$ will be denoted by $C_i$. The cover tree satisfies the following conditions for all $i$:
 
%of  a finite metric space $X$ rooted by an element $t \in X$ is a filtration of subsets $C_i \subseteq X$ indexed  $i \in \mathbb{Z}\cup\{\pm \infty\}$  %satisfying the following conditions:
% n$\{t\} = C_{\infty} \subseteq ... \subseteq C_i \subseteq ... \subseteq C_{-\infty} = X$
%This implies that once a point $p \in X$ appears in $C_{s_j}$ for some $j$, then every lower level in the tree contains a node associated with $p$.

\begin{enumerate}[label={(\arabic*)}]
\item The set $C_{+\infty}$ consists of a single point of $X$. The set $C_{-\infty}$ contains all the points from set $X$.
\item \emph{The nesting condition}: $C_i \subseteq C_{i-1}$. 
\item \emph{The covering tree condition}: For every point $p \in C_{i-1}$, there exists $q \in C_{i}$ satisfying $d(p,q) \leq 2^{i}$ and exactly one such $q$ is the parent of $p$.
\item \emph{The separation condition}: For all distinct $p, q \in C_{i}$, $d(p,q) > 2^{i}$.

\end{enumerate}

\emph{A cover tree} $\mathcal{T}$ built on set $X$ from filtration $( C_i )_{i \in [-\infty, \infty]}$ is an infinite tree (Figure \ref{fig:CoverTree}), which consists of a collection of nodes $(p,s) \in X \times \Z$, where $p \in C_s$. For every node $N \in\mathcal{T}$ denote $s(N)$ as the level of a node $N$. Every $(p,i)$ is connected to unique \emph{parent} $(q,i+1)$ as defined in condition (3). We say that $p$ is \emph{a child} of $q$, if $q$ is the parent of $p$.  We say that $p$ is \emph{ a descendant} of $q$, if there exists a sequence of nodes $(w_j)$ for $j \in [k]$ for which $w_0 = p$, $w_k = q$ and $w_{j+1}$ is the parent of $w_{j}$ for all $j \in [k]$.




%We define level $i$ to be a set $C_i = \{(p,j) \in \mathcal{T} \mid j = i \}$

\end{dfn}

In the actual algorithmic implementation of the cover tree we present it in compressed form, where all the infinite chains, that consists of nodes containing only a single self-child are collapsed into a single node. In Figure \ref{fig:CoverTree} the chain of 1s from $C_\infty$ to $C_1$ is collapsed into a single node. Similarly chains of $1$ and and chain of $3$ starting from $C_{-1}$ will be collapsed into a single node.

\begin{dfn}[maximal depth of a point in cover tree]
\label{dfn:maximalDepth}
Let $(X,d)$ be a finite metric space and let $\mathcal{T}$ be its cover tree. Define relation $\backsim$ on the nodes of $\mathcal{T}$, in such a way that 
$a \backsim b$ if there exists an infinite chain $(w_i)$, where $w_i$ is the only child of $w_{i+1}$ that contains both $a$ and $b$. Let us denote 
$\mathcal{T} / \backsim $ to be the \emph{explicit tree}, where all the infinite chains are collapsed. For every class $D$ of $\mathcal{T} / \backsim $ we define its depth to be the maximal level of each element contained in $D$. 
%and let $p \in X$ be arbitrary point. 

\end{dfn} 
% In the algorithmic representation of the cover we have collapsed 
%The cover tree of Definition \ref{}

%
%\begin{dfn}[Definition of child, parent and descendant] 
%\label{dfn:NotationCoverTree}
%Let $X$ be a finite metric space and let $\{C_i\}$ be its cover tree filtration. Let $p \in C_i$ and $q \in C_j$ be a cover tree nodes. We use the following terminology:
%\begin{enumerate}[label={(\arabic*)}]
%\item Assume that $j = i+1$ and that $q$ is the unique element satisfying the Cover tree condition for point $p$. Then we say that $q$ is a \emph{parent} of $p$ and $p$ is  a \emph{child} of $q$.
%\item Assume $j > i$ and assume that there exists a chain $p_j,...,p_{i}$ in such a way that $p_m$ is a child of $p_{m+1}$, for all $m \in [j-1,i]$. Then we say that $p_i$ is a  \emph{descendant} of $p_j$ and $p_j $ is an \emph{ancestor} of $p_i$.
%\end{enumerate}
%\end{dfn}

\begin{lem}
\label{lem:coverTreeBound}
Let $(X,d)$ be a finite metric space and let $\mathcal{T}$ be a cover tree of $X$. Let $q \in \mathcal{T} $ be arbitrary node located at level $s$ and let $p$ be arbitrary descendant of $q$.Then $d(p,q) \leq 2^{s+1}$
\end{lem}

\begin{proof}
Consequently from Definitions \ref{covertreedefinition} we note that, if $p$ is a descendant point of $q$ then $d(p, q) \leq 2^{i+1}$. This follows from the fact that there always exists a chain $(w_i)$ , for which $w_0 = p$, $w_k = q$ and $w_{j+1}$ is parent of $w_{j}$ for all $j \in [k]$. By applying triangle inequality and the covering tree condition repeatedly the following inequality is obtained:

$$d(p,q) \leq \sum^k_{i = 0}d(w_i, w_{i+1}) \leq \sum^k_{i = 0}2^{s(w_i)} \leq  \sum^{}_{t \leq s(w_k) }2^{t} \leq 2^{s(q)+1}$$

Therefore it follows that the descendant distance of node $q$ is bounded by $2^{s(q)+1}$. 

\end{proof}

%\begin{exa}
%\label{CovertreeExample}
%Let $X = \{1,2,3,4,5\}$ and let $d(x,y) = |x-y|$, then cover tree built on the metric space $(X,d)$ has the geometrical representation as in Figure \ref{fig:GraphicalRepresentationCoverTree}
%\end{exa}
%\begin{figure}

Recall that $|\bar{B}(x,r)|$ is the number of elements in the closed ball $\bar{B}(x,r) = \{p \in X \mid d(p,x) \leq r\}$.

\begin{dfn}[Expansion constant  {\cite[Section.~1]{beygelzimer2006cover}}]
\label{dfn:ExpansionConstantOk}
Let $(X,d)$ be a finite metric space. The expansion constant $c$ is defined to be the smallest real number $c \geq 2$ for which $$\forall x : |\bar{B}(x,2r)| \leq c|\bar{B}(x,r)|$$ 
\end{dfn}


%
%\begin{dfn}[Explicit and implicit representation of a cover tree]
%The following concepts will be used: 
%\begin{itemize}
%\item \emph{The implicit representation} of a cover tree is its geometrical representation consisting of all the nodes of the cover tree.
%Each of the nodes is connected to its children and to its parent node. This construction forms an infinite tree as illustrated in 
%Figure \ref{fig:GraphicalRepresentationCoverTree}
%%We simply connect every child to its parent node to obtain an infinite tree 
%\item \emph{The explicit representation} of a cover tree is a similar representation to the implicit one. With the exception that we collapse all the infinite chains, where each child of each node of the infinite chain is a self-child into a single node. 
%\end{itemize}
%\end{dfn}


% For any cover tree

%Both Lemmas \ref{lem:CoverTechnical1} and \ref{lem:CoverTechnical2} are proved in the original paper \cite{beygelzimer2006cover}:

\begin{lem}[Width bound of a cover tree  {\cite[Lemma.~4.1]{beygelzimer2006cover}}]
\label{lem:CoverTechnical1}
Let $X$ be a finite metric space and $\mathcal{T}$ be its cover tree. For any node $q$ in the cover tree $\mathcal{T}$ the number of its children is bounded by $c^4$, where $c$ is the expansion constant of $X$.
\end{lem}

% Explciit, implicit representation take this from the original cover tree paper. 

\begin{lem}[Depth bound of a cover tree  {\cite[Lemma.~4.2]{beygelzimer2006cover}}]
\label{lem:CoverTechnical2}
Let $X$ be a metric space and  $\mathcal{T}$ be its cover tree. For any node $p$ in the explicit tree $\mathcal{T}$ its maximum depth (Definition \ref{dfn:maximalDepth}) is  $O(c^2\log_{}|X|)$
\end{lem}

The following technically important Lemma \ref{lem:PackingBoundCoverLemma} serves in the following proofs theoretical guarantees in dual-tree algorithms using the cover trees. %The prove of the result is available in PhD dissertation of Ryan Curtin \cite{curtin2015improving}

\begin{lem}[Packing Lemma for the cover trees {\cite[Lemma.~1]{curtin2015plug}} ]
\label{lem:PackingBoundCoverLemma}
Let $(X,d)$ be a metric space having expansion constant $c$. Let $S$ be a $\delta$-sparse subset of $X$ i.e. $d(a,b) > \delta$ for all $a,b \in C$. Then, for any point $ p \in X$ and any radius $\mu \delta > 0:$
$$|\bar{B}(p, \mu \delta)  \cap S | \leq c^{2 + \lceil \log_2 \mu \rceil } $$
\end{lem}



% \cite{ram2009linear}

\subsection{Abstract space trees}
%In Section \ref{sec:CoverTrees} we defined a space partitioning data structure Cover tree, as well as we introduced a concept of $k$-d tree in Example \ref{exa:KDTree}

In this section we introduce a concept of abstract space tree, which generalizes concepts of $k$-d tree from Example \ref{exa:KDTree} and Cover tree introduced in Section \ref{sec:CoverTrees}. 

%The abstract space tree data structure will be defined in Definition \ref{dfn:SpacePartioningDatastructure} and the notation related to it will be presented in \mbox{Definition \ref{dfn:SpacePartionNotation}.}

\begin{dfn}[Space tree  {\cite[Definition.~1]{curtin2013tree}}] 
\label{dfn:SpacePartioningDatastructure}
A \emph{space tree} on a finite set of points $C$ in an euclidean space is an undirected, connected , acyclic, rooted graph with the following properties:
\begin{itemize}
\item Each node holds a number of points and is connected to one parent node and a number of child nodes
\item There is one node in every space tree with no parent. This is the root node of the tree
\item Each point in $C$ is contained in at least one node 
\item Each node corresponds to some subset of $\mathbb{R}^m$ that contains each point in that node and also the subsets that correspond to each child of the node.
\end{itemize}

\end{dfn}

%The following space-partitioning tree terminology will be used:

\begin{dfn}[Space tree notation \cite{curtin2013tree}]
\label{dfn:SpacePartionNotation}
Given a spatial tree node $\mathcal{N}_i$ we denote:
\begin{itemize}

\item The set of child nodes of a node $\mathcal{N}_i$ is denoted $\mathcal{C}(\mathcal{N}_i)$.
\item The set of points held in node $\mathcal{N}_i$ is denoted $\mathcal{P}(\mathcal{N}_i)$.
\item The set of descendant nodes of a node $\mathcal{N}_i$ is denoted by $\mathcal{D}(\mathcal{N}_i)$. 
\item The center of the region corresponding to $\mathcal{N}_i$ is denoted as $\mu(\mathcal{N}_i)$.
\item The furthest descendant distance for a node $\mathcal{N}_i$ will be denoted as $\lambda(\mathcal{N}_i)$.

\end{itemize}

\end{dfn}

\begin{dfn}[Max and min distance between nodes {\cite[Definition.~2]{curtin2013tree}}, {\cite[Definition.~3]{curtin2013tree}}]
\label{dfn:maxminmetriccover}
Let $(X,d)$ be a metric space and let $\mathcal{T}_q$ and $\mathcal{T}_r$ be cover trees built on some finite subsets of $X$. Let
$\mathcal{N}_i \in \mathcal{T}_q$ and $\mathcal{N}_j \in \mathcal{T}_r$ be arbitrary nodes of the corresponding space trees. The minimum distance between  $\mathcal{N}_i$ and $\mathcal{N}_j$ is defined as 
$$d_{\min}(\mathcal{N}_i,\mathcal{N}_j) = \min \{ d(p_i,p_j)  \forall p_i \in \mathcal{D}(\mathcal{N}_i), p_j \in \mathcal{D}(\mathcal{N}_j) \}.$$
On the other hand the maximum distance is defined as:
$$d_{\max}(\mathcal{N}_i,\mathcal{N}_j) =  \max \{ d(p_i, p_j) \forall p_i \in \mathcal{D}(\mathcal{N}_i), p_j \in \mathcal{D}(\mathcal{N}_j) \}.$$
\end{dfn}

\begin{table}[H]
\caption{Notation used in abstract spatial tree datastructures and its appliance to Cover and KD-trees}
\scriptsize
\begin{tabular}{|l|l|l|l|}
\hline
\textbf{Quantity} & \textbf{Description}        & \textbf{Value for $k-d$ trees}                 & \textbf{Value for Cover-trees}                   \\ \hline
$\mathcal{C}_i$   & children of $\mathcal{N}_i$ & $0$ for leaves, otherwise 2       &At most $c^4$ children      \\
$\mathcal{P}_i$   & points of $\mathcal{N}_i$    & only contains points if it s a leaf node    & Each node corresponds to specific point \\
$\mathcal{S}_i$   & region of $\mathcal{N}_i$   & bounding hyper-rectangle                    & On level $k$, ball of radius $2^{k+1}$  \\
$\mu_i$           & center of $\mathcal{N}_i$   & center of the hyper-rectangle               & Same as the point                       \\
$\lambda_i$       & furtest desc. distance      & half of the diagonal of the hyper-rectangle & On level $k$, radius is $2^{k+1}$       \\ \hline
\end{tabular}

\end{table}

%\begin{table}[]
%\begin{tabular}{|l|l|l|l|}
%\hline
%\textbf{Quantity} & \textbf{Description}        & \textbf{Value for kd-trees}                 & Value for Cover-trees                   \\ \hline
%$\mathcal{S}_i$   & children of $\mathcal{N}_i$ & $\emptyset$ for leaves, otherwise 2|        & Potentially any number of child         \\
%$\mathcal{P}_i$   & points of $\mathcal{N}_i$    & only contains points if it s a leaf node    & Each node corresponds to specific point \\
%$\mathcal{S}_i$   & region of $\mathcal{N}_i$   & bounding hyper-rectangle                    & On level $k$, ball of radius $2^{k+1}$  \\
%$\mu_i$           & center of $\mathcal{N}_i$   & center of the hyper-rectangle               & Same as the point                       \\
%$\lambda_i$       & furtest desc. distance      & half of the diagonal of the hyper-rectangle & On level $k$, radius is $2^{k+1}$       \\ \hline
%\end{tabular}
%\end{table}


%

%\begin{figure}
%\begin{table}[]
%\resizebox{\textwidth}{!}{
%\begin{tabular}{|l|l|l|l|}
%\hline
%\textbf{Quantity} & \textbf{Description}        & \textbf{Value for KD-trees}                 & \textbf{Value for Cover-trees}                   \\ \hline
%$\mathcal{S}_i$   & children of $\mathcal{N}_i$ & $\emptyset$ for leaves, otherwise 2       &At most $c^4$ child      \\
%$\mathcal{P}_i$   & points of $\mathcal{N}_i$    & only contains points if it s a leaf node    & Each node corresponds to specific point \\
%$\mathcal{S}_i$   & region of $\mathcal{N}_i$   & bounding hyper-rectangle                    & On level $k$, ball of radius $2^{k+1}$  \\
%$\mu_i$           & center of $\mathcal{N}_i$   & center of the hyper-rectangle               & Same as the point                       \\
%$\lambda_i$       & furtest desc. distance      & half of the diagonal of the hyper-rectangle & On level $k$, radius is $2^{k+1}$       \\ \hline
%\end{tabular}
%}
%\end{table}
%\caption{Notation used in abstract spatial tree datastructures and its appliance to Cover and KD-trees}
%\label{fig:NotationExamples}
%
%
%\end{figure}


\section{Tree independent dual-tree algorithms}

This section discusses dual-tree algorithms. That can reduce quadratic complexity in search problems to nearly linear time by applying space partitioning techniques of Section \ref{sec:SpacePartDataStructure}.
%
%In this section, we present a concept of dual-tree algorithms. This technique is usually applied to problems that have brute-force complexity of $O(N^2)$ to reduce their complexity to nearly-linear time by applying space partioning techniques of Section \ref{sec:SpacePartDataStructure}.



% However, using the space partitioning data structures we are usually able to get better complexities. 

%In this Section we show that the ideas used Algorithm \ref{alg:KDDualTree} to solve the nearest neighborhood problem can be generalized to a large variety of different problems, using any space partitioning structure satisfying certain properties. 

\subsection{Theory of the dual-tree algorithms }
 By observing commonalities of the dual-tree algorithms , we are able to decompose them as in \cite{curtin2013tree} into the following four logical parts:
\begin{itemize}
\item Query and reference space partitioning trees (Definition \ref{dfn:SpacePartioningDatastructure})
\item A pruning dual-tree traversal, which visits nodes in the two space trees, and is parameterized by a BaseCase() and a Score() functions.
\item A BaseCase() function that defines the action to take, when we are handling combination of leaf-nodes. 
\item A Score() function that determines if a given combination of subtrees should be visited during the traversal. 
\end{itemize}

Although we will prove worst-time complexity results only for cover tree, the algorithms in this thesis will be presented in a general form, that allow us to use any space partitioning technique satisfying conditions of Definition \ref{dfn:SpacePartioningDatastructure}. Recall that for every space tree node $\mathcal{N}$ we denote a set containing all the points inside it by $\mathcal{P}(\mathcal{N})$ and a set consisting of all the descendants by $\mathcal{D}(\mathcal{N})$. We define the dual-tree traversal in the following way:

\begin{dfn}[Pruning dual tree traversal {\cite[Definition.~9]{curtin2013tree}}]
\label{dfn:PrunningDualTreeTraversal}
A pruning dual-tree traversal is a family of algorithms satisfying the following conditions: When given two space trees $\mathcal{T}_q$ (the query tree, built on query set $S_q$) and $\mathcal{T}_r$ (the reference tree built on the reference set $S_r$), the algorithm will visit combinations of nodes $(\mathcal{N}_q, \mathcal{N}_r)$ such that $\mathcal{N}_q \in \mathcal{T}_q$ and $\mathcal{N}_r \in \mathcal{T}_r$ no more than once, and call a function Score$(\mathcal{N}_q, \mathcal{N}_r)$ to assign a score to that node. If the score is $\infty$, the combination is pruned and no combinations $\mathcal{N}_{qc},\mathcal{N}_{rc}$ such that $\mathcal{N}_{qc} \in \mathcal{D}(\mathcal{N}_q)$ and $\mathcal{N}_{rc} \in \mathcal{D}(\mathcal{N}_r)$ are visited. Otherwise , for every combination of points $(p_q, p_r)$ such that $p_q \in \mathcal{P}(\mathcal{N}_q)$ and $p_r \in \mathcal{P}(\mathcal{N}_r)$, a function BaseCase$(p_q,p_r)$ is called. If no node combinations are pruned during the traversal, BaseCase$(p_q, p_r)$ is called at least once on each combination of $p_q \in S_q$ and $p_r \in S_r$.
\end{dfn}

As a special case of general traversal we present standard Cover tree traversal in Algorithm \ref{alg:StandardCoverTreeTraversal} as defined in \cite[Algorithm.~1]{curtin2015plug}. To present the general run time bound result Theorem \ref{thmm:DualTreeGeneralRunTimeBound} for standard cover tree traversal we need the following concepts:


% \tag{\ref{thmm:GHT}}
% \label{eqa:GHT}



% we can define an abstract concept of a dual-tree algorithms.

%Using space partitioning data structures we can build quick algorithms to compute main geometrical invariants, such as $k$-nearest neighbors and minimum %spanning tree over the dataset.



\begin{dfn}[Cover tree imbalance, {\cite[Definition.~2]{curtin2015plug}}, {\cite[Definition.~3]{curtin2015plug}}]
\label{dfn:DfnNineOfDissertation}
The cover tree imbalance $I(\mathcal{N}_i)$ for a cover tree node $\mathcal{N}_i$ located on level $s_i$ in the cover tree $\mathcal{T}$ is the cumulative number of missing levels between the node and its parent $\mathcal{N}_p$ located on level $s_p$. If the node is a leaf child, then number of missing levels is defined as the difference between $s_p$ and $s_{\min}-1$. Where $s_{\min}$ is the lowest level of a non-leaf node in the explicit tree $\mathcal{T} / \backsim$ (Definition \ref{dfn:maximalDepth} ). Explicitly written,
%$$i_n(\mathcal{N}_i) $$
\[I(\mathcal{N}_i)  = \begin{cases} 
      s_p - s_i -1 & \text{if } \mathcal{N}_i \text{ is not a leaf and not the root node } \\
      \max(s_p - s_{\min} - 1, 0) & \text{if } \mathcal{N}_i \text{ is a leaf} \\
      0 & \text{if } \mathcal{N}_i \text{ is the root node.}  
   \end{cases}
\]

The cover tree imbalance $I(\mathcal{T})$ for a cover tree $\mathcal{T}$ is defined simply as the cumulative number of missing levels in the tree. This can be expressed as a sum:

$$I(\mathcal{T}) = \sum_{\mathcal{N}_i \in \mathcal{T}} I(\mathcal{N}_i)$$
\end{dfn}

\begin{algorithm}[H]
\caption{The standard pruning dual-tree traversal for cover trees {\cite[Algorithm.~1]{curtin2015plug}}}
\label{alg:StandardCoverTreeTraversal}
\begin{algorithmic}[1]
\STATE \textbf{Input} : query node $\mathcal{N}_q$, set of reference nodes $R$.
\STATE \textbf{Global input: } Score($\cdot, \cdot $) function on non-leaf nodes and BaseCase($\cdot, \cdot $) function on points.
\STATE $s^{\max}_r \leftarrow \max_{\mathcal{N}_r \in R} S_r$

\IF {$s_q < s^{\max}_r$}
\FOR{$\mathcal{N}_r \in R$}
\STATE BaseCase$(p_q,p_r)$
\ENDFOR
\STATE $R_r \leftarrow \{\mathcal{N}_r \in R \mid s_r = s^{\max}_r\}$
\STATE $R_{r-1} \leftarrow \{\mathcal{C}(\mathcal{N}_r) \mid \mathcal{N}_r \in R_r\} \cup (R \setminus R_r)$ 
\STATE $R'_{r-1} \leftarrow \{\mathcal{N}_r \in R_{r-1} \mid \text{Score}(\mathcal{N}_q, \mathcal{N}_r) \neq \infty \} $
\STATE recurse with $\mathcal{N}_q$ and $R'_{r-1}$
\ELSE
\FOR {$\mathcal{N}_{qc} \in \mathcal{C}(\mathcal{N}_q) $}
\STATE $R' \leftarrow \{\mathcal{N}_r \in R \mid \text{Score}(\mathcal{N}_q, \mathcal{N}_r) \neq \infty\}$
\STATE recurse with $\mathcal{N}_qc$ and $R'$
\ENDFOR
\ENDIF

\end{algorithmic}
\end{algorithm}

%Recall that we say that a finite metric space $(X,d)$ is $\delta$-sparse if 

\begin{lem}[Extra reference recursion bound, {\cite[Algorithm.~1]{curtin2015plug}} ]
\label{lem:FourOfDissertation}
Let $S_q, S_r$ be finite metric spaces and let $N = \max(|S_q| ,|S_r|)$. Let
$\mathcal{T}_q$ and $\mathcal{T}_r$ be cover trees built on spaces $S_q$ and $S_r$, respectively. For dual-tree algorithm using cover trees $\mathcal{T}_q$ as the query tree and $\mathcal{T}_r$ as the reference tree together with traversal given in Algorithm \ref{alg:StandardCoverTreeTraversal}, the number of extra reference recursion that happen after the last query recursion is bounded by
%$$\theta = \max\{ \min \{ O(N\log_2(\delta_q)) \} , 0 \}. $$
\begin{equation}
\tag{\ref{lem:FourOfDissertation}}
\label{eqa:FourOfDissertation}
\theta(S_q, S_r) = \max\{ \min \{ O(N\log_2(\frac{\delta_q}{\delta_r})),O(N^2) \} , 0 \}.
\end{equation}
where $\delta_q$ and $\delta_r$ are the smallest nonzero pairwise distances in $S_q$ and $S_r$ respectively. 
\end{lem}

\begin{thmm}[General dual tree runtime bound result,  {\cite[Theorem.~1]{curtin2015plug}}]
\label{thmm:DualTreeGeneralRunTimeBound}
Let $S_q, S_r$ be finite metric spaces and let $N = \max(|S_q| ,|S_r|)$. Let
$\mathcal{T}_q$ and $\mathcal{T}_r$ be cover trees built on spaces $S_q$ and $S_r$, respectively. 
Let $c_r$ be the expansion constant of $S_r$. Then a standard cover tree based dual-tree algorithm (Algorithm \ref{alg:StandardCoverTreeTraversal}) takes 
\begin{equation}
\label{eqa:DualTreeGeneralRunTimeBound}\tag{\ref{thmm:DualTreeGeneralRunTimeBound}}
O(c_r^4|R^{*}|\alpha \beta(N + I(\mathcal{T}_{q}) + \theta(S_q, S_r)) 
\end{equation}

time, where $ |R^{*}| $ is the maximum size of the reference set $R$ during the dual-tree recursion, $\alpha$ is the complexity of BaseCase() operation, $\beta$ is the complexity of Score() operation and $\theta(S_q,S_r)$ is defined in 
Lemma \ref{lem:FourOfDissertation}. 
\end{thmm}

%We note that the worst-case cover tree $\mathcal{T}$ which is entirely a chain-like structure with maximum scale $s_{\max}$ and minimum scale $s_{\min}$ will have imbalance $I(\mathcal{T}) = N(s_{\max} - s_{\min})$. Following from Lemma \ref{lem:CoverTechnical2} maximal depth of any point in explicit cover-tree is 
%bounded by $O(c^2\log(N))$, where $c$ is the expansion constant of the underlying space of the tree  $\mathcal{T}$  . Thus we can estimate that in the worst case scenario the cover-tree imbalance of arbitrary tree $\mathcal{T}$ is $I(\mathcal{T}) = O(c^2 N \log(N))$. Also, when query tree $\mathcal{T}_q$ and reference tree $\mathcal{T}_r$ are the same in Theorem \ref{thmm:DualTreeGeneralRunTimeBound}, then the term $\theta(\mathcal{T}_q, \mathcal{T}_r)$ vanishes. Thus we obtain the following result:

\begin{lem}
\label{lem:CoverTreeImbalanceUpperBound}
Let $(X,d)$ be a finite metric space consisting of $N$ points and having an expansion constant $c$. Let $\mathcal{T}$ be an arbitrary explicit cover-tree built on $S$. Then cover-tree imbalance has the following bound: $I(\mathcal{T}) \leq c^2 \log(N) $
%The cover-tree imbalance $I(\mathcal{T})$ has the upper-bound $c^2 \log(N)$
\end{lem}

\begin{proof}
We note that the worst-case the explicit cover tree $\mathcal{T} / \backsim$ , which is entirely a chain-like structure with maximum level $s_{\max}$ and minimum level $s_{\min}$ will have imbalance $I(\mathcal{T}) = N(s_{\max} - s_{\min})$. By Lemma \ref{lem:CoverTechnical2} maximal depth of any point in explicit cover-tree is 
bounded by $O(c^2\log(N))$
\end{proof}


We note that when query tree $\mathcal{T}_q$ and reference tree $\mathcal{T}_r$ are the same in Theorem \ref{thmm:DualTreeGeneralRunTimeBound}, then the term $\theta(\mathcal{T}_q, \mathcal{T}_r)$ vanishes. Combining this remark with Lemma \ref{lem:CoverTreeImbalanceUpperBound} we obtain the following result:

\begin{cor}
\label{cor:DualTreeGeneralRunTimeBoundQR}

%Assume the conditions of Theorem \ref{thmm:DualTreeGeneralRunTimeBound}. If $S_q = S_r$ then $\theta(S_q,S_R) = 0$
Let $(X,d)$ be a finite metric space consisting of $N$ points and having an expansion constant $c$. Then a standard cover tree based dual-tree algorithm (Algorithm \ref{alg:StandardCoverTreeTraversal}) applied by using $X$, as both, the query and reference set takes 
$$O(c^6 |R^{*}| \alpha \beta \log(N) N) $$
time, where $ |R^{*}| $ is the maximum size of the reference set $R$ during the dual-tree recursion, $\alpha$ is the complexity of BaseCase() operation, $\beta$ is the complexity of Score() operation.
\end{cor}

%%
%
%\medskip
%
%Also, when query tree $\mathcal{T}_q$ and reference tree $\mathcal{T}_r$ are the same in Theorem \ref{thmm:DualTreeGeneralRunTimeBound}, then the term $
%\theta(\mathcal{T}_q, \mathcal{T}_r)$ vanishes. Thus when $\mathcal{T}_r$ has size $N$ we can estimate the complexity to be
%$$O(c^6 |R^{*}| \alpha \beta \log(N) N) $$

\subsection{k-nearest neighborhood search}
\label{sec:knn}
In this section we present theory related to $k$-nearest neighborhood search. For simplicity the theory will be presented only for cover-trees. 


\begin{problem}[Problem statement of $k$-nearest neighborhood search]
\label{pro:KNN}
%  outputs a function $\text{argmin}_{p \in S_r}d(\cdot, p):S_q \rightarrow S_r $ i.e. a function
Let $(X,d)$ be a finite metric space and let $Q$ and $R$ be its subspaces. Design a near linear time algorithm in size of $R$ and $Q$ that find a point $r \in R$ for every $q \in Q$ satisfying $d(q, r) \leq d(q,R)$, where $d(q,R)$ is the minimal distance between $q$ and $R$. 

% finds a nearest neighbor in $S_r$ for every point of the set $S_q$ 



%, for each point $p_q \in S_q$ find a fast algorithm that computes the $k$ nearest neighbors in $S_r$ and their distances from $p_q$.
\end{problem}


When given query and reference sets $Q,R$ Problem \ref{pro:KNN} can be solved in quadratic time $O(|Q||R|)$ simply by using two loops. We will however present a faster technique that utilizes space partioning data structures to cut the computational time to near-linear. Let us denote a space tree built on the set $Q$ as $\mathcal{T}_q$. 

A near linear algorithm using dual-tree strategy to solve Problem \ref{pro:KNN} was first presented \cite{ram2009linear}. This algorithm was later extended to any space partioning data structures in \cite{curtin2015plug}. However, until this day the worst-case complexity result was formulated and proved only for the algorithm using cover trees.

\begin{dfn}
\label{dfn:lambdaFunction}
Let $(X,d)$ be a finite metric space and let $\mathcal{T}_r$ be a cover-tree built on $X$. Let $R = \{r_i\}$ be a finite set of cover-tree nodes and let $p \in X$ be an arbitrary point, for example a representative point of a query node. 
Let us denote $\mathcal{T}(r)$ to be restriction of tree $\mathcal{T}$ to point $r$ as its root and let $|\mathcal{T}(r)|$ be the number of different points contained in tree $\mathcal{T}(r)$. Assume that $R$ is ordered by their distance to $p$ i.e. $d(r_i, p) \leq d(r_j, p)$ for every $i \leq j$. For any $k \in \mathbb{N}$ we define $\lambda_k(p,R) \in R$ to be $r_i$ having largest index $i$ satisfying 
$$\sum_{j \in [0,i]}| \mathcal{T} (q_j) | \leq k$$
\end{dfn}


\begin{dfn}[Notation for KNN]
\label{dfn:KNNBound}


We denote the array consisting of the nearest neighbors for a point $q \in Q$ as $N_{q}$ and the array consisting distances to the nearest neighbors for $q$ as $D_{q}$. We note that in the end of the traversal the $k$-th nearest neighbor of a point $q$ is $N_{q}[k]$ and distance to it $D_{q}[k] = d(q, N_{q}[k])$. 

%Let $\mathcal{T}_q$ be a space tree built on $S_q$. For arbitrary query node $\mathcal{N}_q \in \mathcal{T}_q $ the bound function will be defined simply as 
%$$B(\mathcal{N}_q, ) = \max_{p \in \mathcal{D}(\mathcal{N})}D_p[k],$$
%where $\mathcal{D}(\mathcal{N})$ denote all the descendants of node $\mathcal{N}$ in the tree $\mathcal{T}_q$.

%\begin{align}
%d_{\min}(\mathcal{N}_q, \mathcal{N}_r) &\leq B(\mathcal{N}_q) \\
%d_{\min}(\mathcal{N}_q, \mathcal{N}_r) &\leq d(p_q, \hat{p}_r) + 2^{s_q + 1}   \\
%d(p_q, p_r) &\leq d(p_q, \hat{p}_r) + 2^{s_q + 1} + 2^{s_r + 1} + 2^{s_q+1} \\
%&\leq d(p_q, \hat{p}_r) + 2(2^{s^{\max}_r + 1}) 
%\end{align}


\end{dfn}

\begin{dfn}[Degree of bichromaticity {\cite[Definition ~3.1]{ram2009linear}}]
\label{dfn:degreeOfBichromaticity}
Let $S$ and $T$ be cover trees built on query set $Q$ and reference set $R$ respectively.
Consider a dual-tree algorithm with the property that the scales of $S$ and $T$ are kept as close as
possible – i.e. the tree with the larger scale is always descended. Then, the degree of bichromaticity
$\kappa$ of the query-reference pair $(Q,R)$ is the maximum number of descends in $S$ between any two
descends in $T$.
\end{dfn}

\begin{algorithm}[H]
\caption{FindAllNN()-algorithm}
\label{alg:KNNSearchAlgorithm}
\begin{algorithmic}[1]
\STATE \textbf{Input} : query node $q_j$, set of reference nodes $R_i$.
%\STATE \textbf{Global input: } Score($\cdot, \cdot $) function on non-leaf nodes and BaseCase($\cdot, \cdot $) function on points.
\IF {$ i = -\infty$}
\FOR {$r \in R$}
\IF{$t < D_{q_j}[k]$}
\STATE insert $t$ into max-binary heap $D_{q_j}$ and remove the maximal element of $D_{q_j}$
\STATE Update $N_{q_j}$ accordingly. 
\ENDIF
\ENDFOR
\ELSIF{$j < i $}
\STATE $ R = \{\text{Children}(r) \mid r \in R_i\}$
\STATE $ R_{i-1} = \{r \in R \mid d(q_j, r) \leq d(q_j, \lambda_k(q_j,R)) + 2^{i} + 2^{j+2}\}$
\STATE FindAllNN($q_j, R_{i-1} $)
\ELSE
\FOR{$q_{j-1} \in \text{Children}(q_j) $}
\STATE FindAllNN($q_{j-1},R_i $)
\ENDFOR
\ENDIF


\end{algorithmic}
\end{algorithm}

\begin{dfn}[{\cite[Section~5]{curtin2015plug}}]
\label{dfn:ExpConstantKNNNot}
Given a reference set $R$ and query set $Q$, we denote the expansion constant of $R$ by $c_r$ and the expansion constant of $Q$ by $c_q$. For notation convenience we define the $(R, Q)$-traversal expansion constant $c_{qr}$ as follows:
$$c_{qr} = \max\{c_r, \max_{q \in Q}c'_r\},$$
where $c'_r$ is the expansion constant of the set $R \cup \{q\}$.
\end{dfn}

The following result is a new result extending  \cite[Theorem ~3.1]{ram2009linear}, which solved Problem \ref{pro:KNN} in a near linear time for $k = 1$. 

\begin{thmm}
\label{thmm:knn}
Let $(X,d)$ be a metric space and let $Q,R$ be finite subsets of $X$ corresponding to query set and reference set respectively.
Let $\kappa$ be a degree of bichromaticity of the $(Q,R) $ pair defined in Definition \ref{dfn:degreeOfBichromaticity} . Let $N = \max(|Q|, |R|)$ , let $c_Q$ be the expansion constant of  $Q$ and let $C_R$ be the expansion constant of $R$  . Let $c_{qr}$ be the expansion constant of  pair $(Q,R)$ as defined in Definition \ref{dfn:ExpConstantKNNNot}. Then Algorithm \ref{alg:KNNSearchAlgorithm} computes the nearest neighbor in $R$ of each point in $Q$ in $O(k \log(k) c_{qr}^{6}c_R^{6}c^{4\kappa}_QN)$ time.
\end{thmm}

\begin{proof}

The computation at Lines 2-8 is done for each of the query nodes at most once. In each iteration we insert and remove element from max-binary heap that contains at most $k$ elements . Hence it takes $O(k \log(k)\max_i|R_i| N) $ computations. Similarly line 9 takes at most $O(\max_i|R_i| N) $

The traversal of a reference node is duplicated over the set of queries only if the query tree is
descended just before the reference tree descend. For every query descend, there would be at most
$ O(c_Q^4) $ duplications (width bound) for every reference node traversal. Since the number of query
descends between any two reference descends is upper bounded by $\kappa$ and the number of explicit
reference nodes is $O(N)$, the total number of reference node considered in Line 11  in the whole
algorithm is at most $O(c_Q^{4\kappa} N) $

Since at any level of recursion, the size of $R$ is bounded by $c_R^4\max_{i}|R_i|$(width bound), and the
maximum depth of any point in the explicit tree is $O(c_R^2 \log (N))$ (depth bound), the number of nodes
encountered in Line 12 is $O(c_R^{4 + 2}\max_{i}|R_i|\log(N) $. Since the traversal down the query tree causes
duplication, and the duplication of any reference node is upper bounded by $c^{4\kappa}_Q $, Line 6 takes at most
$c^{4\kappa}_Qc^6_R\max_i|R_i|\log(N) $ in the whole algorithm.

Line 9 is executed just once for each of the explicit nodes of the query tree and hence takes at most
$O(N)$ time. To complete the proof we need to find an upper bound for $|R_i|$. 

Consider any $R_{i-1} = \{r \in R : d(q_j, r) \leq d + 2^{i} + 2^{j+2}\}$ where $d = d(q_j,\lambda_k(q_j,R))$. Given that 
$C_{i-1}$ is the $(i-1)$-th level of the reference tree we obtain:
\begin{equation}
\label{eqa:QBound}
R_{i-1} = B(q_j, d+2^{i}+2^{j+2}) \cap R \subseteq B(q_j, d+2^{i} + 2^{j+2)}) \cap C_{i-1} \subseteq B(q_j, d+2^{i} + 2^{i+1}) \cap C_{i-1}
\end{equation}
Since $R \subseteq C_{i-1}$ and $j < i$ in this part of recursion. Let us assume now that $d > 2^{i+2}$. Let us order $R_{i-1} = \{r_s\}$  by their distances to $q_j$ as in Definition \ref{dfn:lambdaFunction}. Let $q_t = \lambda(q_j, R_{i-1})$. We note that $\sum_{w \in [0,t-1]} |\mathcal{T}(r_w)| < k$. By pigeonhole principle there exists index $t'$ for which $t' \geq t$ and $r_{t'}$ contains one of true $k$-nearest neighbors of point $p$ as its descendant. Let $\beta$ be a point among true $k$-nearest neighbors of $q_j$ that is a descendant of $r_{t'}$.   
$$d = d(q_j,r_t) \leq d(q_j, r_{t'}) \leq d(q_j,\beta) + d(r_{t'} ,\beta) \leq d(q_j,\beta) +2^{i}$$
It follows that $3\cdot2^{i} \leq d(q_j,\beta)$. Combining this with Equation \ref{eqa:QBound} we obtain: % 2^{i+2}
$$|R_{i-1}|  \leq |B(q_j,d(p,\beta) +  2^{i+2})| \leq |B(q_j,4d(p,\beta))| \leq c_{qr}^3|B(p,\frac{d(q_j,\beta)}{2})|$$
We note that $\beta$ is among $k$-nearest neighbors of $p$. Thus $|B(p,\frac{d(p,\beta)}{2})| \leq k$. It follows that $|Q_{i-1}| \leq c_{qr}^2k$. 
Assume now that $d \leq 2^{i+2}$. By using Equation \ref{eqa:QBound} we obtain:
$$R_{i-1} \subseteq  B(q_j,2^{i+2} + 2^{i+1} +2^{i}) \cap C_{i-1}  \subseteq  B(p,2^{i+3}) \cap C_{i-1}$$
From cover-tree condition we know that all the points in $C_{i-1}$ are separated by $2^{i-1}$. By using Lemma \ref{lem:PackingBoundCoverLemma} with $\mu = 16$ and $\delta = 2^{-1}$ we obtain $|Q_{i-1}| \leq |B(p,2^{i+2}) \cap C_{i-1}| \leq c_{qr}^6$.

Thus the algorithm takes $O(k\log(k)c^6_{qr}kN + c_Q^{4\kappa}N + c_{qr}^{6}c^6_{R}c_Q^{4\kappa}\log(N) +N ) $ which is $$ O(k\log(k)c_R^{12}c_Q^{4\kappa} N).$$

\end{proof}
When query set and reference sets are the same we can simplify the result as Corollary \ref{cor:KNNComplexity}.
\begin{cor}
\label{cor:KNNComplexity}
Let $X$ be a finite space with expansion constant $c$. Let $k \leq |X|$ be an integer. Then Algorithm \ref{alg:KNNSearchAlgorithm}  computes the nearest neighbor in $X$ of each point in $X$ in $O(c^{12}k\log(k)N) $ time. 
\end{cor}
\begin{proof}
The proof follows from Theorem \ref{thmm:knn} by noting that $\kappa = 1$ and $c_Q = c_R = c_{qr}$.
\end{proof}
%\subsection{k-nearest neighborhood search}
%\label{sec:knn}
%%Given a query set $S_q$ and reference set $S_r$
%In this section we present theory related to $k$-nearest neighborhood search.
%
% %all-$k$-nearest neighborhood search in a given dataset. 
%
%%In this section we present shortly the $k$-nearest neighborhood search as presented Ryan Curtins PhD thesis \cite{curtin2015improving} and as a new result we extend the worst case time complexity result of the $k$-nearest neighbor search for arbitrary integer $k \in \Z$. We state the original problem in Problem \ref{pro:KNN}. 
%\begin{problem}[Problem statement of $k$-nearest neighborhood search]
%\label{pro:KNN}
%%  outputs a function $\text{argmin}_{p \in S_r}d(\cdot, p):S_q \rightarrow S_r $ i.e. a function
%Let $(X,d)$ be a finite metric space and let $S_q$ and $S_r$ be its subspaces. Design a near linear time algorithm in size of $S_r$ and $S_q$ that find a point $p_r \in S_r$ for every $p_q \in S_q$ satisfying $d(p_q, p_r) \leq d(p_q,S_r)$, where $d(p_q,S_r)$ is the minimal distance between $p_q$ and $S_r$. 
%
%% finds a nearest neighbor in $S_r$ for every point of the set $S_q$ 
%
%
%
%%, for each point $p_q \in S_q$ find a fast algorithm that computes the $k$ nearest neighbors in $S_r$ and their distances from $p_q$.
%\end{problem}
%%
%When given query and reference sets $S_q,S_r$ Problem \ref{pro:KNN} can be solved in quadratic time $O(|S_q||S_r|)$ simply by using two loops. We will however present a faster technique that utilizes space partioning data structures to cut the computational time to near-linear. Let us denote a space tree built on 
%set $S_q$ as $\mathcal{T}_q$. Before proceeding to the algorithms, we need to define a bound function $B:\mathcal{T}_q \rightarrow \R$ that will help us to determine, if a combination should be pruned during traversal of space-tree Definition \ref{dfn:PrunningDualTreeTraversal}. Than tighter bound we use than less query node and reference node combination we go through resulting in better computation time. In this section subscripts $q$ and $r$ will refer to points in query set and reference set, respectively. 
%
%%\begin{dfn}[Notation of $k$-nearest neighbor and distance to it]
%%
%%\end{dfn}
%%
%
%
%
%\begin{dfn}
%\label{dfn:lambdaFunction}
%Let $(X,d)$ be a finite metric space and let $\mathcal{T}_r$ be a cover-tree built on $X$. Let $R = \{r_i\}$ be a finite set of cover-tree nodes and let $p \in X$ be an arbitrary point, for example a representative point of a query node. 
%Let us denote $\mathcal{T}(r)$ to be restriction of tree $\mathcal{T}$ to point $r$ as its root and let $|\mathcal{T}(r)|$ be the number of different points contained in tree $\mathcal{T}(r)$. Assume that $R$ is ordered by their distance to $p$ i.e. $d(r_i, p) \leq d(r_j, p)$ for every $i \leq j$. For any $k \in \mathbb{N}$ we define $\lambda_k(p,R) \in R$ to be $r_i$ having largest index $i$ satisfying 
%$$\sum_{j \in [0,i]}| \mathcal{T} (q_j) | \leq k$$
%\end{dfn}
%
%
%\begin{dfn}[Bound function for KNN {\cite[Section.~5]{curtin2015plug}}]
%\label{dfn:KNNBound}
%
%
%We denote the array consisting of the nearest neighbors for a point $p_q \in S_q$ as $N_{p_q}$ and the array consisting distances to the nearest neighbors for $p_q$ as $D_{p_q}$. We note that in the end of the traversal the $k$-th nearest neighbor of a point $p_q$ is $N_{p_q}[k]$ and distance to it $D_{p_q}[k] = d(p_q, N_{p_q}[k])$. 
%
%Let $\mathcal{T}_q$ be a space tree built on $S_q$. For arbitrary query node $\mathcal{N}_q \in \mathcal{T}_q $ the bound function will be defined simply as 
%$$B(\mathcal{N}_q, ) = \max_{p \in \mathcal{D}(\mathcal{N})}D_p[k],$$
%where $\mathcal{D}(\mathcal{N})$ denote all the descendants of node $\mathcal{N}$ in the tree $\mathcal{T}_q$.
%
%%\begin{align}
%%d_{\min}(\mathcal{N}_q, \mathcal{N}_r) &\leq B(\mathcal{N}_q) \\
%%d_{\min}(\mathcal{N}_q, \mathcal{N}_r) &\leq d(p_q, \hat{p}_r) + 2^{s_q + 1}   \\
%%d(p_q, p_r) &\leq d(p_q, \hat{p}_r) + 2^{s_q + 1} + 2^{s_r + 1} + 2^{s_q+1} \\
%%&\leq d(p_q, \hat{p}_r) + 2(2^{s^{\max}_r + 1}) 
%%\end{align}
%
%
%\end{dfn}
%
%%\begin{dfn}[Bound function for KNN {\cite[Section.~5]{curtin2015plug}}]
%%\label{dfn:KNNBound}
%%
%%Let $\mathcal{T}_q$ be a space tree built on $S_q$. For arbitrary node $\mathcal{N} \in \mathcal{T}_q $ the bound function will be defined simply as 
%%$$B(\mathcal{N}) = \max_{p \in \mathcal{D}(\mathcal{N})}D_p[k],$$
%%where $\mathcal{D}(\mathcal{N})$ denote all the descendants of node $\mathcal{N}$ in the tree $\mathcal{T}_q$.
%%
%%\end{dfn}
%
%
%
%It should be noted that the algorithm can be built in such a way that that it computes $B(\mathcal{N}_q)$ during the traversal as a byproduct and thus doesn't increase the computational complexity. For our purpose its enough to provide reasonable upper-bound in special case where both, the query and reference tree are cover trees. By using Lemma \ref{lem:coverTreeBound} we can state:
%
%$$B(\mathcal{N}_q) \leq D_{p_q}[k] + 2^{s(p_q) + 1}.$$
%
%
%Similarly to the other dual-tree algorithms we define BaseCase() and Score() methods in Algorithms \ref{alg:BaseCaseKNN} and \ref{alg:ScoreKNN} respectively. To make the proof and results clearer we use the following notation:
%
%\begin{dfn}[{\cite[Section~5]{curtin2015plug}}]
%\label{dfn:ExpConstantKNNNot}
%Given a reference set $S_r$ and query set $S_q$, we denote the expansion constant of $S_r$ by $c_r$ and the expansion constant of $S_q$ by $c_q$. For notation convenience we define the $(S_r, S_q)$-traversal expansion constant $c_{qr}$ as follows:
%$$c_{qr} = \max\{c_r, \max_{p_q \in S_q}c'_r\},$$
%where $c'_r$ is the expansion constant of the set $S_r \cup \{p_q\}$.
%\end{dfn}
%
%\begin{algorithm}[H]
%\caption{$k$-nearest neighbors BaseCase()}
%\label{alg:BaseCaseKNN}
%\begin{algorithmic}[1]
%\STATE \textbf{Input} : query point $p_q$, reference point $p_r$, list of $k$ nearest candidate points $N_{p_q}$ and $k$ candidate distances $D_{p_q}$ (both ordered by ascending distance)
%%\STATE \textbf{Output} : distance $d$ between $p_q$ and $p_r$.
%\STATE $ t \leftarrow d(p_q,p_r)$
%\IF {$t < D_{p_q}[k] $ \textbf{and} BaseCase$(p_q, p_r)$ not yet called}
%%\STATE $f_p(p_q) \leftarrow f_p(p_q) + f(d(p_q,p_r))$
%\STATE insert $t$ into max-binary heap $D_{p_q}$ and remove the maximal element of $D_{p_q}$
%\STATE Update $N_{p_q}$ accordingly. 
%\ENDIF
%\STATE \textbf{return} $t$
%%\STATE Initialize the heap $H$ consisting of pairs in $\text{Vertices}(G) \times \mathbb{R}$ with the single pair $(p,0)$
%%\STATE Dist$(p) \leftarrow 0$, $\NDP(p) \leftarrow \emptyset$
%%\WHILE{the heap $H$ is not empty}
%%\STATE q $\leftarrow$ H.pop()
%%\FOR{\text{each vertex } $r$ \text{ adjacent to $q$ in the graph $G$}}
%%\STATE $\leftarrow \text{Dist}(q) + d(r,q)  $
%%\IF{Dist$(r) > t$ and $t < \delta$}
%%\STATE Dist$(r) \leftarrow t$, $\NDP(r) \leftarrow q$
%%\STATE H.push$(r, t)$
%%\ENDIF
%%\ENDFOR 
%%\ENDWHILE
%\end{algorithmic}
%\end{algorithm}
%
%\begin{algorithm}[H]
%\caption{$k$-nearest neighbors Score()}
%\label{alg:ScoreKNN}
%\begin{algorithmic}[1]
%\STATE \textbf{Input} : query node $\mathcal{N}_q$, reference node $\mathcal{N}_r$
%\STATE \textbf{Output} : a score for the node combination $(\mathcal{N}_q, \mathcal{N}_r)$ or $\infty$ if the combination should be pruned
%\IF{$d_{\min}(\mathcal{N}_q, \mathcal{N}_r) < B(\mathcal{N}_q, \mathcal{N}_r) $ }
%\STATE \textbf{return} $d_{\min}(\mathcal{N}_q,\mathcal{N}_r)$
%\ENDIF
%\STATE \textbf{return} $\infty$
%
%%\STATE $f_p(p_q) \leftarrow f_p(p_q) + f(d(p_q,p_r))$
%%\STATE \textbf{return} $f(d(p_q,p_r))$
%%\STATE Initialize the heap $H$ consisting of pairs in $\text{Vertices}(G) \times \mathbb{R}$ with the single pair $(p,0)$
%%\STATE Dist$(p) \leftarrow 0$, $\NDP(p) \leftarrow \emptyset$
%%\WHILE{the heap $H$ is not empty}
%%\STATE q $\leftarrow$ H.pop()
%%\FOR{\text{each vertex } $r$ \text{ adjacent to $q$ in the graph $G$}}
%%\STATE $\leftarrow \text{Dist}(q) + d(r,q)  $
%%\IF{Dist$(r) > t$ and $t < \delta$}
%%\STATE Dist$(r) \leftarrow t$, $\NDP(r) \leftarrow q$
%%\STATE H.push$(r, t)$
%%\ENDIF
%%\ENDFOR 
%%\ENDWHILE
%\end{algorithmic}
%\end{algorithm}
%
%% for $k$-nearest neighbor when $k$ is fixed. 
%Before proceeding to the main result, we show that a distance array $D_{p_q}$ can be treated as a max-binary heap, which allows $O(\log(k))$ addition time and $O(1)$-lookup time. The original result that $k$-nearest neighborhood problem can be solved in a near linear time was proven by Ryan Curtin in \cite[Theorem~2]{curtin2015plug} for $k = 1$. We prove the generalized result for arbitrary value $k$ in Proposition \ref{pro:ComputationTimeKNN}. 
%
%\begin{lem}
%\label{lem:dualHeapLookUp}
%The BaseCase() function (Algorithm \ref{alg:BaseCaseKNN}) of the $k$-nearest neighborhood search have algorithimc complexity of $O(\log(k))$, when the distance array $D$ is implemented as Binary heap ( Definition \ref{dfn:BinaryHeap}).
%
%
%% and \ref{alg:ScoreKNN} can be implemented in such a way that Score() could be solved in $O(1)$ and BaseCase() in $(O(\log(k))$ time where $k$ is the size of %query tree. 
%\end{lem}
%\begin{proof}
%For every point $p_q$ in query set $S_q$ let us implement $D_{p_q}$ as max-heap having at most $k$-elements. Lemma \ref{lem:BinaryHeap} implies that retrieving the maximal element can be done in  a constant time. It follows that complexity of  $t < D_{p_q}[k]$ has $O(1)$ look-up complexity . The complexity of inserting and removing an element having the max-value from max-heap can be both done in $O(\log(k))$. By summing up all the complexities we archive the desired complexity $O(\log(k))$.
%\end{proof}
%
%
%
%% \cite[Theorem~4]{curtin2015improving}.
%
%%\cite{curtin2015improving}, Theorem .
%
% % Assume that $|S_r| = O(N)$ and $|S_q| = O(N)$ for some $N$.
%\begin{pro}[Extension of complexity of KNN search {\cite[Theorem~2]{curtin2015plug}}]
%% alg:StandardCoverTreeTraversal
%\label{pro:ComputationTimeKNN}
%Let $S_q$ and $S_r$ be finite subsets of metric space $(X,d)$. The Problem \ref{pro:KNN} imposed on query set $S_q$ and reference set $S_r$ can be solved by first building cover trees $\mathcal{T}_q$ and $\mathcal{T}_r$ on $S_q$ and $S_r$, respectively and then running the standard cover tree pruning dual-tree traversal (Algorithm \ref{alg:StandardCoverTreeTraversal}) on  $\mathcal{T}_q$, $\mathcal{T}_r$ parameterized by the $k$ nearest neighbor search functions BaseCase() and Score() as given in Algorithms \ref{alg:BaseCaseKNN} and \ref{alg:ScoreKNN}, respectively.
%Let $N = \max(|S_r|, |S_q|) $ and let $c_r$ be the expansion constant of $S_r$. Then running time of the algorithm is bounded by
%%$$ O(c^4_r c^3_{qr}(c^{2}_{qr}+k)\log(k)(N + I(\mathcal{T}_q) + \theta ) ) $$
%\begin{equation}
%\tag{\ref{pro:ComputationTimeKNN}}
%\label{eqa:ComputationTimeKNN}
% O(c^4_r c^3_{qr}(c^{2}_{qr}+k)\log(k)(N + I(\mathcal{T}_q) + \theta(S_q, S_r) ) )
%\end{equation}
%
%% \tag{\ref{pro:ComputationTimeKNN}}
%% \label{eqa:ComputationTimeKNN}
%% 
%% O(c^4_r c^3_{qr}(c^{2}_{qr}+k)\log(k)(N + I(\mathcal{T}_q) + \theta ) ) 
%% 
%% \end{equation}
%% 
%where $I(\mathcal{T}_q)$ is defined in Definition \ref{dfn:DfnNineOfDissertation} and $\theta(S_q, S_r)$ is defined in Lemma \ref{lem:FourOfDissertation}.
%
%\end{pro}
%\begin{proof}
%%The correctness of the proposed Algorithm was proved in\cite[Theorem.~3]{curtin2015improving}. Thus we are left to prove that the upper-bound for the runtime is indeed (\ref{eqa:ComputationTimeKNN}).
%
%The fact that the defined Algorithm does indeed solve Problem \ref{pro:KNN} was proved in \cite[Section 7.1.2, Theorem~3]{curtin2015improving}.
%
%From Lemma \ref{lem:dualHeapLookUp} it follows that the running time of the BaseCase() method is $O(\log(k))$ and the complexity of the Score() function is clearly $O(1)$. Due to Theorem \ref{thmm:DualTreeGeneralRunTimeBound} we know that the runtime of the algorithm is bounded by $O(c^4_r |R^{*}|\log(k)(N + i_t(\mathcal{T}_q) + \theta ) )$, where $|R^{*}|$ is the maximum size of the reference set $R^{*}$ at any level during the traversal (Algorithm \ref{alg:StandardCoverTreeTraversal} ). Thus, the only thing that remains is to bound the maximum size $|R^{*}|$.
%
%Assume that at some stage of the standard cover-tree traversal ( Algorithm \ref{alg:StandardCoverTreeTraversal} ) we have encountered $\mathcal{N}_q$ as the query node  and $R^{*}$ as the set of reference nodes. We assume that the maximal level of nodes in set $R^{*}$ is $s^{\max}_r$. Let $d_{\min}$ be the
%metric introduced in Definition \ref{dfn:maxminmetriccover} and let $B$ be as in Defintion \ref{dfn:KNNBound}. Every node $\mathcal{N}_r \in R^{*}$ satisfies the bounding condition $d_{\min}(\mathcal{N}_q, \mathcal{N}_r) \leq B(\mathcal{N}_q)$. Let $p_q$ be the point held in $\mathcal{N}_q$ and let $p_r$ be the point held in $\mathcal{N}_r$. Also, take $\hat{p}_r$ to be the current $k-$nearest neighbor candidate for $p_q$; that is, $D_{p_q}[k] = d(p_q, \hat{p}_r)$ and $N_{p_q}[k] = \hat{p}_r$. Then, \begin{align}
%d_{\min}(\mathcal{N}_q, \mathcal{N}_r) &\leq B(\mathcal{N}_q) \label{eqa:FirstStepLong} \\
%d_{\min}(\mathcal{N}_q, \mathcal{N}_r) &\leq d(p_q, \hat{p}_r) + 2^{s(p_q) + 1}  \label{eqa:BoundExp} \\
%d(p_q, p_r) &\leq d(p_q, \hat{p}_r) + 2^{s(p_q) + 1} + 2^{s(p_r) + 1} + 2^{s(p_q)+1} \label{eqa:QueryReferenceExp}\\
%&\leq d(p_q, \hat{p}_r) + 2(2^{s^{\max}_r + 1}) \label{eqa:TraversalEqa}
%\end{align}
%% i.e. $P = \{p_r \in \mathcal{P}(\mathcal{N}_r) : \mathcal{N}_r \in R^{*}\} $.
%Inequality (\ref{eqa:BoundExp}) follows from expansion of $d_{\min}(\cdot, \cdot)$ and $B(\cdot)$.
%Inequality (\ref{eqa:QueryReferenceExp}) follows from the property of cover tree, which states that the distance between every descendant $p_t$ of covert tree node $p_q$ at level $s_q$ has a bound: $d(p_t, p_q) \leq 2^{s(p_q)+1}$. Thus using the property for both query and reference tree we can bound 
%$d_{\min}(\mathcal{N}_q, \mathcal{N}_r) \leq  2^{s(p_r) + 1} + 2^{s(p_q)+1}$. Last Inequality \ref{eqa:TraversalEqa} follows from inequalities: $s(p_q) + 1 \leq s^{\max}_r$ and $s(p_r) \leq s^{\max}_{r}$. Define the set of points $P$ as the points held in each node in $R^{*}$. Then we can write 
%$$P \subseteq B(p_q, d(p_q, \hat{p}_r) + 2(2^{s^{\max}_r + 1})) \cap S_r.$$
%Suppose that the true $k-$nearest neighbor of $p_q$ is $p_r^{*}$.  The proof is now split into two cases depending on if $d(p_q,p^{*}_r) > 2^{s^{\max}_r+1}$. Let us assume first that this condition is satisfied. We first note that $p^{*}_r$ must be held descendant of some point $\tilde{p}_r \in R^{*}$. Using triangle inequality we deduct:
%$$d(p_q,  \hat{p}_r) \leq d(p_q, \tilde{p}_r) \leq d(p_q, p_r^{*}) + d(\tilde{p}_r, p_r^{*}) \leq d(p_q, p_r^{*}) + 2^{s^{\max}_r + 1}$$
%
%That gives $P \subseteq \bar{B}(p_q, d(p_q, p_r^{*}) + 3(2^{s^{\max}_r + 1})) \cap (S_r \cup \{p_q\})$. The previous step is necessary: to apply the definition of the expansion constant (Definition \ref{dfn:ExpansionConstantOk} ), the ball must be centered at a point in the set; now, the center $(p_q)$ is part of the set. We will now use the definition of expansion constant to bound number of points in set $P$. 
%
%\begin{align}
%|R| &\leq |\bar{B}(p_q, d(p_q, p_r^{*}) + 3(2^{s^{\max}_r + 1})) \cap (S_r \cup \{p_q\})|  \\
%&\leq |\bar{B}(p_q, d(p_q, 4d(p_q, p_r^{*}))) \cap ( S_r \cup \{p_q\} )| \\
%&\leq c_{qr}^{3}|B(p_q, d(p_q, \frac{d(p_q, p_r^{*})}{2})) \cap ( S_r \cup \{p_q\} ) | \leq c_{qr}^{3}k.\label{eqa:lastStepBig}
%\end{align}
%
%We note that the last Equation (\ref{eqa:lastStepBig}) follows from the fact that $p^{*}_r$ was the $k-$nearest neighbor of to $p_q$ in $S_r \cup \{p_q\}$; thus the set $|B_{S_r \cup \{p_q\}}(p_q, d(p_q, \frac{d(p_q, p_r^{*})}{2}))|$ can only contain the $k-1$-nearest neighbors of set $p_q$ and thus is bounded by $k$.  This results into inequality $|R| \leq c_{qr}^{3}k$.
%
%Assume now that $d(p_q, p^{*}_r) \leq 2^{s^{\max}_r}$, which means that $d(p_q, \hat{p}_r) \leq 2^{s^{\max}_r+2}$. Let us denote $\mathcal{T}_r(i)$ to be the set containing all the nodes of cover tree $\mathcal{T}_r$ located on level $i$.
%
%Note that $P \in \mathcal{T}_r(s^{\max}_r)$ and therefore  
%
%\begin{align}
%P &\subseteq \bar{B}(p_q, d(p_q, p^{*}_r) + 3(2^{s^{\max}_r+1})) \cap \mathcal{T}(s^{\max}_r) \cap S_r \\
%&\subseteq \bar{B}(p_q, d(p_q, 4(2^{s^{\max}_r + 1})) \cap \mathcal{T}(s^{\max}_r) \cap S_r
%\end{align}
%
%Every point in $C_{s^{\max}_r}$ is separated by at least $2^{s^{\max}_r}$. Using Lemma \ref{lem:PackingBoundCoverLemma} with $\delta = 2^{s^{\max}_r}$ and $\rho = 8$ yields that $|P| \leq c^5_r$. This gives the result $|R| \leq c_{qr}^5$. And thus by combining the two cases we can deduct  $|R| \leq c_{qr}^{3}(c^2_{qr}k)$. 
%
%%$$d_{\min}(\mathcal{N}_q, \mathcal{N}_r) \leq B(\mathcal{N}_q) $$
%%$$d(p_q, p_r) \leq d(p_q, \hat{p}_r) + 2^{s_q + 1} + 2^{s_r + 1} + $$
%%$$ $$ 
%\end{proof}
%
%
%% alg:StandardCoverTreeTraversal
%\begin{cor}[Complexity of KNN-search, when query set = reference set]
%\label{cor:ComputationTimeKNN}
%The problem \ref{pro:KNN}, where $ X = S_q = S_r$ can be solved by building cover tree $\mathcal{T}$ and running the standard cover tree pruning dual-tree traversal (Algorithm \ref{alg:StandardCoverTreeTraversal}) parameterized by the $k$ nearest neighbor search functions BaseCase() and Score() as given in Algorithms \ref{alg:BaseCaseKNN} and \ref{alg:ScoreKNN}, respectively. Let $c$ be the expansion constant of $X$. Then the running time of the algorithm is bounded by
%%$$ O(c^4_r c^3_{qr}(c^{2}_{qr}+k)\log(k)(N + I(\mathcal{T}_q) + \theta ) ) $$
%
%%%
%\begin{equation}
%\label{eqa:ComputationTimeKNNQR}
%\tag{\ref{cor:ComputationTimeKNN}}
% O(c^{11} k \log(k) |X| \log(|X|) )
%\end{equation}
%\end{cor}
%
%
%% %The proof is similar to the general pro:ComputationTimeKNN cor:DualTreeGeneralRunTimeBoundQR
%
%\begin{proof}
%The required upper bound is obtained by applying Lemma \ref{lem:CoverTreeImbalanceUpperBound} and the fact that $\theta(S,S) = 0$ on Proposition \ref{eqa:ComputationTimeKNN}.
%
%\end{proof}
 %\cite[Definition~3, Lemma~4]{curtin2015plug}. 
\subsection{Bor\r{u}vka's Algorithm}
\label{sec:BoruvkaAlgorithm}

Bor\r{u}vka's algorithm \cite{boruvka1926jistem} is a greedy algorithm that is used for finding a minimum spanning tree of a graph. Given a graph $G$ the running time of this algorithm is $O(|\mathbb{E}(G)|\log(|\mathbb{V}(G)|)) $. Bor\r{u}vka's algorithm can be used to compute a minimum spanning forest of a any graph. In the case, when the input graph $G$ is connected the output of Bor\r{u}vka's algorithm is a minimum spanning tree of a graph. 

 %as we are mainly interested in finding a minimum spanning tree of a connected graph we assume that $G$ is connected in this section.

We assume that all the edges of $G$ have distinct weights (if they are not we can make a small perturbation to the weights of the graph). The basic idea in Bor\r{u}vka's algorithm is to construct a minimum spanning tree iteratively. We start by forming a disconnected graph $F$ consisting of all the vertex points of $G$.
We add edges to the graph in an iterative manner until graph $F$ is connected. During the iteration step, we loop over all the connected components of $R \in F$ and for each of the components we select an edge, that has a minimal weight among all the edges that contain exactly one end point in $R$. All the selected edges are added to the graph $F$. This proccess is repeated until the graph $F$ becomes connected. This idea is formalized in Algorithm \ref{alg:Boruvka}. 

The idea of the Bor\r{u}vka's algorithm can be used, when the input is a point cloud instead of a graph. This idea will be presented in Section \ref{sec:MST}. 
Algorithm \ref{alg:Boruvka} in its current form will be used in Dense-tree data-skeletonization technique presented in Section \ref{sec:dense_tree}. 

%
% we search for each component of $F$ an edge of $G$ having minimal weight and that contains exactly one of the points in the given component. This process is formalized in Algorithm \ref{alg:Boruvka}.

%contract
%simultaneously the minimum weight edges incident on each of the
%vertices in $G$. In a contraction, only the minimum weight
%edge needs to be retained out of any set of multiple edges. The
%process of contracting the minimum weight edge for each vertex in
%the graph is called the \textit{Boruvka phase}.


\begin{algorithm}[H]
\caption{Bor\r{u}vka's Algorithm}
\label{alg:Boruvka}
\begin{algorithmic}[1]
\STATE \textbf{Input: }A connected graph $G$ whose edges have distinct weights
\STATE \textbf{Output: }$F$ is the minimum spanning tree of $G$
%\STATE \textbf{Input} : query point $p_q$, reference point $p_r$, nearest candidate $N(F(p_q))$ and distance $D(F(p_q))$
\STATE Initialize a forest $F$ to be a set of one-vertex trees, one for each vertex of the graph $G$
%\WHILE{$F$ has more than one component}
\WHILE{$F$ is not connected}
\STATE Find a connected components of $F$ and label each vertex of $G$ by its component
%\STATE Initilize the minimal edge for each component to "None.
\FOR{edge $(u,v) \in \mathbb{E}(G)$ }
\IF {$u$ and $v$ are in different components}
\IF {$(u,v)$ has smaller weight than the minimal edge for the component of $u$}
\STATE Set $(u,v)$ as the minimal edge for the component of $u$.
\ENDIF 
\IF {$(u,v)$ has smaller weight than the minimal edge for the component of $v$}
\STATE Set $(u,v)$ as the minimal edge for the component of $v$.
\ENDIF
\ENDIF
\ENDFOR
\FOR {component whose minimal edge is not "None"}
\STATE Add its minimal edge to $F$

\ENDFOR
\ENDWHILE
\end{algorithmic}
\end{algorithm}

\begin{figure}
\begin{tikzpicture}[scale=1.25, auto,swap]
    % Draw a 7,11 network
    % First we draw the vertices
    \foreach \pos/\name in {{(0,2)/a}, {(2,1)/b}, {(3,-0.25)/c},
                            {(0,0)/d}, {(1.0,-1)/e}, {(0,-3)/f}, {(3,-2)/g}}
        \node[vertex] (\name) at \pos {$\name$};
    % Connect vertices with edges and draw weights
    \foreach \source/ \dest /\weight in {b/a/7, c/b/12,d/a/4,d/b/10,
                                         e/b/3, e/c/5,e/d/15,
                                         f/d/6,f/e/8,
                                         g/e/9,g/f/11}
        \path[edge] (\source) -- node[weight] {$\weight$} (\dest);
%    % Start animating the vertex and edge selection. 
%    \foreach \vertex / \fr in {d/1,a/2,f/3,b/4,e/5,c/6,g/7}
%        \path<\fr-> node[selected vertex] at (\vertex) {$\vertex$};
%    % For convenience we use a background layer to highlight edges
%    % This way we don't have to worry about the highlighting covering
%    % weight labels. 
%    \begin{pgfonlayer}{background}
%        \pause
%        \foreach \source / \dest in {d/a,d/f,a/b,b/e,e/c,e/g}
%            \path<+->[selected edge] (\source.center) -- (\dest.center);
%        \foreach \source / \dest / \fr in {d/b/4,d/e/5,e/f/5,b/c/6,f/g/7}
%            \path<\fr->[ignored edge] (\source.center) -- (\dest.center);
%    \end{pgfonlayer}
\end{tikzpicture}
\begin{tikzpicture}[scale=1.25, auto,swap]
    % Draw a 7,11 network
    % First we draw the vertices
  \foreach \pos/\name in {{(0,2)/a}, {(2,1)/b}, {(3,-0.25)/c},
                            {(0,0)/d}, {(1.0,-1)/e}, {(0,-3)/f}, {(3,-2)/g}}
        \node[vertex] (\name) at \pos {$\name$};
    % Connect vertices with edges and draw weights
%    \foreach \source/ \dest /\weight in {b/a/7, c/b/8,d/a/5,d/b/9,
%                                         e/b/7, e/c/5,e/d/15,
%                                         f/d/6,f/e/8,
%                                         g/e/9,g/f/11}
%        \path[edge] (\source) -- node[weight] {$\weight$} (\dest);
	 \path[edge] (b) -- node[weight] {7} (a);
	 \path[edge] (c) -- node[weight] {12} (b);
	 \path[edge,red] (d) -- node[weight] {4} (a);
	 \path[edge] (d) -- node[weight] {10} (b);
	 \path[edge,red] (e) -- node[weight] {3} (b);
	 \path[edge,red] (e) -- node[weight] {5} (c);
	 \path[edge] (e) -- node[weight] {15} (d);
	 \path[edge,red] (f) -- node[weight] {6} (d);
	 \path[edge] (f) -- node[weight] {8} (e);
	 \path[edge,red] (g) -- node[weight] {9} (e);
	 \path[edge] (g) -- node[weight] {11} (f);
        
       
%    % Start animating the vertex and edge selection. 
%    \foreach \vertex / \fr in {d/1,a/2,f/3,b/4,e/5,c/6,g/7}
%        \path<\fr-> node[selected vertex] at (\vertex) {$\vertex$};
%    % For convenience we use a background layer to highlight edges
%    % This way we don't have to worry about the highlighting covering
%    % weight labels. 
%    \begin{pgfonlayer}{background}
%        \pause
%        \foreach \source / \dest in {d/a,d/f,a/b,b/e,e/c,e/g}
%            \path<+->[selected edge] (\source.center) -- (\dest.center);
%        \foreach \source / \dest / \fr in {d/b/4,d/e/5,e/f/5,b/c/6,f/g/7}
%            \path<\fr->[ignored edge] (\source.center) -- (\dest.center);
%    \end{pgfonlayer}


\end{tikzpicture}
\begin{tikzpicture}[scale=1.25, auto,swap]
    % Draw a 7,11 network
    % First we draw the vertices
  \foreach \pos/\name in {{(0,2)/a}, {(2,1)/b}, {(3,-0.25)/c},
                            {(0,0)/d}, {(1.0,-1)/e}, {(0,-3)/f}, {(3,-2)/g}}
        \node[vertex] (\name) at \pos {$\name$};
    % Connect vertices with edges and draw weights
%    \foreach \source/ \dest /\weight in {b/a/7, c/b/8,d/a/5,d/b/9,
%                                         e/b/7, e/c/5,e/d/15,
%                                         f/d/6,f/e/8,
%                                         g/e/9,g/f/11}
%        \path[edge] (\source) -- node[weight] {$\weight$} (\dest);
	 \path[edge,red] (b) -- node[weight] {7} (a);
	 \path[edge] (c) -- node[weight] {12} (b);
	 \path[edge,red] (d) -- node[weight] {4} (a);
	 \path[edge] (d) -- node[weight] {10} (b);
	 \path[edge,red] (e) -- node[weight] {3} (b);
	 \path[edge,red] (e) -- node[weight] {5} (c);
	 \path[edge] (e) -- node[weight] {15} (d);
	 \path[edge,red] (f) -- node[weight] {6} (d);
	 \path[edge] (f) -- node[weight] {8} (e);
	 \path[edge,red] (g) -- node[weight] {9} (e);
	 \path[edge] (g) -- node[weight] {11} (f);
        
       
%    % Start animating the vertex and edge selection. 
%    \foreach \vertex / \fr in {d/1,a/2,f/3,b/4,e/5,c/6,g/7}
%        \path<\fr-> node[selected vertex] at (\vertex) {$\vertex$};
%    % For convenience we use a background layer to highlight edges
%    % This way we don't have to worry about the highlighting covering
%    % weight labels. 
%    \begin{pgfonlayer}{background}
%        \pause
%        \foreach \source / \dest in {d/a,d/f,a/b,b/e,e/c,e/g}
%            \path<+->[selected edge] (\source.center) -- (\dest.center);
%        \foreach \source / \dest / \fr in {d/b/4,d/e/5,e/f/5,b/c/6,f/g/7}
%            \path<\fr->[ignored edge] (\source.center) -- (\dest.center);
%    \end{pgfonlayer}


\end{tikzpicture}
\caption{Bor\r{u}vka's algorithm performed on an example graph weighted by random integers. 
\textbf{Left: } Every node is in its own component , \textbf{Middle: } Two clusters $\{a,d,f\}$ and $\{b,c,e,g\}$, 
\textbf{Right: } All the points are in the same cluster.  
}
\label{fig:BoruvkaClustering}
\end{figure}



The complexity result, Lemma \ref{lem:ComplexityBoruvka} is presented below:

% to produce a quick near-linear time Algorithm, which is capable of computinga minimum spanning tree of a given point-cloud  



\begin{lem}[Complexity of Boruvka algorithm]
\label{lem:ComplexityBoruvka}
The computational complexity of Algorithm \ref{alg:Boruvka} is $O(|\mathbb{E}(G)|\log(|\mathbb{V}(G)|)) $, where $G$ is the input graph.
\end{lem}
\begin{proof}
The idea of the proof is available in \cite{nevsetvril1997few}.
\end{proof}

%A good implementation of a Boruvka phase is the following:
%\begin{list}{}{}
%    \item[1.] mark the edges to be contracted;
%    \item[2.] determine the connected components formed by the marked
%    edges;
%    \item[3.] replace each connected component by a single vertex;
%    \item[4.] finally, eliminate the self-loops and multiple edges
%    created by these contractions.
%\end{list}


\subsection{Minimum spanning tree of a metric space}
\label{sec:MST}
%In this section we present theory related to computation of minimum spanning tree of a metric space.
 In this section we will use notation of \cite{curtin2013tree} to present theory regarding minimum spanning tree algorithm. Recall that $\MST(X,d)$ of a finite metric space $(X,d)$ was defined in Definition \ref{dfn:mst} as minimum spanning tree of the complete graph on $X$ with edge lengths defined by the metric $d$. As usual we start with the problem statement:

\begin{problem}
\label{pro:MST}
Given a finite subset $X$ of Euclidean space $(\R^m,d)$ find a near-linear in size of $X$ algorithm to compute $\MST(X,d)$.
\end{problem} 

In Section \ref{sec:BoruvkaAlgorithm} we have introduced the classical problem of computing minimum spanning tree $T$ of a given graph $G$.  Problem \ref{pro:MST} will be solved by applying general strategy of Algorithm \ref{alg:Boruvka} together with the nearest neighbor method introduced in Section \ref{sec:knn}. In such a way that in each boruvka merging step of Definition \ref{dfn:boruvkaClustering} we apply standard cover tree traversal of Algorithm \ref{alg:StandardCoverTreeTraversal} parameterized by BaseCase() function of Algorithm \ref{alg:BaseCaseMST} and Score() function of Algorithm \ref{alg:ScoreMST} specialized for the $\MST$ computation. We have summarized this procedure in Algorithm \ref{alg:DualTreeBoruvka} . When we use cover tree as the space partioning data structure, it will be shown in Theorem \ref{thmm:MST_time} that running time of the Algorithm \ref{alg:DualTreeBoruvka} is near-linear. 


\begin{dfn}[ Bor\r{u}vka clustering, { \cite[Definition~2]{march2010fast} }]
\label{dfn:boruvkaClustering}
%(? The definition was unclear in the original source: emst paper , this is my interpretation):
Given a finite metric space $(X,d)$, \emph{Boruvka clustering} is an indexed collection of partitions $F_i$. The partition $F_0$ is the trivial partition
$\{ \{p\} \mid p \in X\} $, where each point is contained in a separate collection . Partition $F_{i}$ is obtained from $F_{i-1}$ by merging every
$\mathcal{U} \in F_{i-1}$ with a separate partition $\mathcal{V} \in F_{i-1}$ that minimizes the distance $ \min \{d(x,y) \mid x \in \mathcal{U} \text{ and }y \in \mathcal{V}\}.$
This proccess, illustrated in Figure \ref{fig:BoruvkaClustering} is repeated until $F_i$ becomes a partition consists of one element $\{X\}$. 

% that if $x \sim y$ in $D_j$, then $x \sim y$ in $D_{j+1}$.
\end{dfn}

%
%In Algorithm \ref{alg:DualTreeBoruvka} we start with $F_0$ and after each of iterations of the while-loop (lines 4-8) of Algorithm \ref{alg:DualTreeBoruvka} we update the current $F = F_{i+1}$ as defined in Definition \ref{dfn:boruvkaClustering}. 

Similarly to Definition \ref{dfn:KNNBound}, in order to state usual BaseCase() and Score() methods we need to specify the notation for extra datastructures that will be used. Assume that $(X,d)$ is a finite metric space and assume that $i \in \mathbb{N}$ is fixed. Let $p \in X$ be a point, then:

\begin{itemize}
\item $F_i(p)$ is the be the partition of point $p$ in $F_i$
\item $N_i(p)$ is the current nearest neighboring partition $\mathcal{U} \in F_i$ that minimizes function
\\ $\min \{d(x,y) \mid x \in \mathcal{U} \text{ and }y \in F_i(p)\}.$
\item $D_i(p)$ is the distance to the current nearest neighboring partition $\mathcal{U}$ of $F_i(p)$ 
\item Assume that $\mathcal{T}$ is a space tree built on $X$. Then for every node $\mathcal{N} \in \mathcal{T}$ we denote 
$$B_i(\mathcal{N}) = \max_{p \in \mathcal{D}(\mathcal{N})}D(p),$$
where $\mathcal{D}(\mathcal{N})$ denotes the set of descendants of node $\mathcal{N}$.
\end{itemize}



%\begin{dfn}
%\label{dfn:NotationMST}
%During Algorithm \ref{alg:DualTreeBoruvka}, we maintain a list $F$ made up of $i$ connected components $F_i$. We denote $E_i = \mathbb{E}(F_i) $ and $V_i = \mathbb{V}(F_i)$.  At initialization each element in $F_i$ corresponds to an original point in $S$ i.e. $\mathbb{E}(F_i) = \emptyset$ and $\mathbb{V}(F_i) = \{p_i\}$ for $i \in \{1,...,|S|\}$. For each $p \in S$ we define $F(p) = F_i$ if $F_i$ is the component containing $p$. Similarly to Definition \ref{dfn:KNNBound} of $k$-nearest neighbor search-section we maintain arrays $N$ and $D$, in such a way that $N(F_i)$ and $D(F_i)$ corresponding to the current nearest component of $F_i$ and distance to it, respectively. Let $B$ be the bound function maps every node $\mathcal{N}$ to $\R$ of a tree built on set $X$ as $$B(\mathcal{N}) = \max_{p \in \mathcal{D}(\mathcal{N})}D(F(p)),$$
%where $\mathcal{D}(\mathcal{N})$ denotes the set of descendants of node $\mathcal{N}$.
%\end{dfn}

%It should be noted that we use bound of KNN $B()$ defined in Definition \ref{dfn:KNNBound} in Score() method of $\MST$ computation presented in Algorithm. \ref{alg:ScoreMST}
\begin{algorithm}[H]
\caption{Dual-tree Bor\r{u}vka algorithm for MST}
\label{alg:DualTreeBoruvka}
\begin{algorithmic}[1]
\STATE \textbf{Input: } Root node of tree $\mathcal{N}$ representing finite metric space $(X,d)$.
\STATE \textbf{Output: } Minimum spanning tree $\MST(X,d)$
\STATE Let $G = (V,E)$ satisfying $V = X $ and  $E = \emptyset$, $i = 0$.
\WHILE{$|E| < |X| - 1$}
\STATE Update partition $F_i$ to be the connected components of $G$, Initialize arrays $D_i$, $N_i$. 
\STATE \textbf{Run dual tree-traversal algorithm}  \ref{alg:StandardCoverTreeTraversal} on $\mathcal{N}$, parametrized by  BaseCase($i$) (Algorithm \ref{alg:BaseCaseMST}) and Score($i$) (Algorithm \ref{alg:ScoreMST}) functions of the minimum spanning tree algorithm
\STATE Add all the found edges of line 6 to $E$ i.e. For every $\mathcal{U} \in F_i$ and its nearest component $\mathcal{V} \in F_i$ we 
select $p \in \mathcal{U}$, $q \in \mathcal{V}$ minimizing the distance $d(p,q)$ and add $(p,q)$ to $E$. 
\STATE $i \leftarrow i + 1$
\ENDWHILE
\STATE \textbf{return} G
\end{algorithmic}
\end{algorithm}




\begin{algorithm}[H]
\caption{$\MST$ algorithm BaseCase($i$)}
\label{alg:BaseCaseMST}
\begin{algorithmic}[1]
\STATE \textbf{Input} : query point $p_q$, reference point $p_r$, nearest candidate $N_i(F(p_q))$ and distance $D_i(F(p_q))$
%\STATE \textbf{Output} : distance $d$ between $p_q$ and $p_r$.
%\STATE $ d \leftarrow ||p_q - p_r||$
\IF {$F_i(p_q) \neq F_i(p_r)$ \textbf{and} $d(p_q , p_r ) < D_i(F(p_q)) $}
%\STATE $f_p(p_q) \leftarrow f_p(p_q) + f(d(p_q,p_r))$
\STATE $D_i(F(p_q)) \leftarrow d(p_q , p_r )$
\STATE $N_i(F(p_q)) \leftarrow p_r$
\ENDIF
%\STATE Initialize the heap $H$ consisting of pairs in $\text{Vertices}(G) \times \mathbb{R}$ with the single pair $(p,0)$
%\STATE Dist$(p) \leftarrow 0$, $\NDP(p) \leftarrow \emptyset$
%\WHILE{the heap $H$ is not empty}
%\STATE q $\leftarrow$ H.pop()
%\FOR{\text{each vertex } $r$ \text{ adjacent to $q$ in the graph $G$}}
%\STATE $\leftarrow \text{Dist}(q) + d(r,q)  $
%\IF{Dist$(r) > t$ and $t < \delta$}
%\STATE Dist$(r) \leftarrow t$, $\NDP(r) \leftarrow q$
%\STATE H.push$(r, t)$
%\ENDIF
%\ENDFOR 
%\ENDWHILE
\end{algorithmic}
\end{algorithm}
\begin{algorithm}[H]
\caption{$\MST$ algorithm Score($i$)}
\label{alg:ScoreMST}
\begin{algorithmic}[1]
\STATE \textbf{Input} : query node $\mathcal{N}_q$, reference node $\mathcal{N}_r$
\STATE \textbf{Output} : a score for the node combination $(\mathcal{N}_q, \mathcal{N}_r)$ or $\infty$ if the combination should be pruned
\IF{$d_{\min}(\mathcal{N}_q, \mathcal{N}_r) < B_i(\mathcal{N}_q) $ }
\IF {$F_i(p_q) = F_i(p_r) \forall p_q \in \mathbb{D}(\mathcal{N}), p_r \in \mathbb{D}(\mathcal{N}) $}
\STATE \textbf{return} $\infty$
\ENDIF
\STATE \textbf{return} $d_{\min}(\mathcal{N}_q,\mathcal{N}_r)$
\ENDIF
\STATE \textbf{return} $\infty$

%\STATE $f_p(p_q) \leftarrow f_p(p_q) + f(d(p_q,p_r))$
%\STATE \textbf{return} $f(d(p_q,p_r))$
%\STATE Initialize the heap $H$ consisting of pairs in $\text{Vertices}(G) \times \mathbb{R}$ with the single pair $(p,0)$
%\STATE Dist$(p) \leftarrow 0$, $\NDP(p) \leftarrow \emptyset$
%\WHILE{the heap $H$ is not empty}
%\STATE q $\leftarrow$ H.pop()
%\FOR{\text{each vertex } $r$ \text{ adjacent to $q$ in the graph $G$}}
%\STATE $\leftarrow \text{Dist}(q) + d(r,q)  $
%\IF{Dist$(r) > t$ and $t < \delta$}
%\STATE Dist$(r) \leftarrow t$, $\NDP(r) \leftarrow q$
%\STATE H.push$(r, t)$
%\ENDIF
%\ENDFOR 
%\ENDWHILE
\end{algorithmic}
\end{algorithm}





% we search for nearest neighboring
% Boruvka Algorithm 






\begin{dfn}[Cluster expansion constant, { \cite[Definition~3]{march2010fast} } ]
\label{dfn:ClusterExpansionConstant}
Let $\{F_i\}$ be a Boruvka clustering on a set $X$. Let $q \in X$ be some element and let $r \in \R_{+}$. We define $\bar{B}_i^c(q,r)$ to be the set of all the components in Boruvka clustering $F_i$ which contain a point $p$ such that $d(p,q) \leq r$.
\emph{The cluster expansion constant} is the smallest real number $c_p$ such that
 $$|B^c_i(q,2r)| \leq c_p |B^c_i(q,r)|$$
 for all $q \in X$, distances $r \in \R_{+}$ and all $i \in \mathbb{N}$.
\end{dfn}

\begin{dfn}[Linkage clustering constant, { \cite[Definition~4]{march2010fast} }]
\label{dfn:LinkageClusterConstant}
 Let $C_1$ and $C_2$ be two components in the Boruvka clustering in $F_i$ and let $S_1 \subseteq C_1$ and $S_2 \subseteq C_2 $. We define $\bar{B}^l(S_1,S_2,r)$ to be the set of all pairs $(p,q)$ such that $p \in S_1$, $q \in S_2$ and $d(p,q) \leq r$.
\emph{Linkage clustering constant} is the smallest real number $c_l$ such that $$|\bar{B}^l_i(S_1,S_2,2r)| \leq c_l|\bar{B}^l_i(S_1,S_2,r)|$$ for all $i \in \mathbb{N}$, components $C_1$ and $C_2$ in $F_i$ and subsets $S_1 \subseteq C_1$, $S_2 \subseteq C_2$, and distances $r > 0 $ . 
\end{dfn}


\begin{thmm}
\label{thmm:MST_time}
\cite[Theorem~5.1]{march2010fast} 
For any finite metric space $(X,d)$ a Minimum Spanning Tree $\MST(X,d)$ can be computed in time $O(\max\{c^6,c_p^2c^2_l\}c^{10}|X|\log |X|\,\al(|X|))$ using Algorithm \ref{alg:DualTreeBoruvka} on a cover-tree that is built on set $X$, where 
 $\al(|X|)$ is the inverse Ackermann function, which grows very slowly e.g. $\al(10^{80})\leq 4$. The expansion constant $c$ is introduced in 
Definition \ref{dfn:ExpansionConstantOk}. The cluster expansion constant $c_p$ and the linkage expansion constant $c_l$ depend on $X$ and are defined in Definitions \ref{dfn:ClusterExpansionConstant} and \ref{dfn:LinkageClusterConstant} respectively.
\bs
\end{thmm}

\subsection{Kernel density estimation}
\label{sec:KDETheorySec}

As well as other problems in this section kernel density estimation can be classified as a search problem that has
 quadratic brute-force worst-case time complexity. 
Unlike in previous techniques, it is impossible to find a faster algorithm to compute kernel density estimate for general kernels of functions $K:\R \times \rightarrow \R$. However, a clever technique first developed in \cite{ram2009linearz} and then extended in \cite{curtin2015plug} that allows us to compute an approximation of the kernel density estimation in linear time, when the kernel function $K$ has some constrains.

\begin{dfn}[Shift-invariant Kernel Density Estimate, {\cite[Section~6]{curtin2015plug}}]
\label{dfn:KDE}

Let $(X,d)$ be a metric space and let $S_q$, $S_r$ be its finite subspaces. Let $K: \R \rightarrow \R$ be a function satisfying the following conditions:
\begin{itemize}
\item Function $K$ has a continuous derivative.
\item Function $K:\R \rightarrow \R$ is monotonically decreasing 
\item There exists $h \in \R_{+}$, such that $K$ is concave in interval $[0,h]$ and convex in $[h, +\infty).$
\end{itemize}
Kernel density estimate KDE is a function $f_K:S_q\to\R$, satisfying $f_K(p_q) = \sum_{p_r \in S_r}K(d(p_q,p_r))$.
\end{dfn}

%such as shift-invariance and smoothness. Although kernel density estimation can be defined for general 2-parameter functions $g:\R^2 \rightarrow \R$ we focus only on functions $g$ which have the form $f(d(\cdot, \cdot))$, where $d$ is a metric of the input space. 

%\begin{exa}
%Sigmoid function $f(x) = \frac{1}{1 + e^{ax+b}}$ satisfies the assumption when a > 0.
%\end{exa}

%\end{itemize}



%To prove theoretical results we also assume in this section that $f$ satisfies the following two conditions: 

%absolute value
\begin{dfn}[{\cite[Section~6]{curtin2015plug}}]
\label{dfn:KDE}
We say that $K^{*}_f$ is $\epsilon$-approximation of $K_f$ if for all $p_q \in S_q$ 
$$|K_f(p) - K^{*}_f(p) | < \epsilon$$
\end{dfn}

To define standard BaseCase() and Score() functions, we need extra global parameters. Let $\mathcal{T}_q$ be a space tree that is built on 
set $S_q$. Define $g$ to be an array containing current partial kernel density estimation of all query nodes during the run time.
At the beginning of the algorithm, they are initiated with a value of 0. As the traversal of the algorithms proceeds, the combination of query and reference nodes $\mathcal{N}_q$ and $\mathcal{N}_r$ respectively are pruned if $|K(d_{\max}(\mathcal{N}_q, \mathcal{N}_q))-f(d_{\min}(\mathcal{N}_q, \mathcal{N}_q)|$ is sufficiently small. If the combination is pruned, then partial node estimates are updated. When we reach leafs BaseCase() method is called, which simply updates the partial point estimate with the exact kernel evaluation. 

After the dual tree traversal the value of function $f$ on $p_q$ can be obtained simply by computing 
$$f(p_q) = g(p_q) + \sum_{\mathcal{N}_i \in T}g(\mathcal{N}).$$ This can be done by traversing query tree at most once and thus can be performed in a nearly linear time as proved in Theorem \ref{thmm:KDE_time}




\begin{algorithm}
\caption{Approximate kernel density estimation BaseCase()}
\label{alg:BaseCaseKDE}
\begin{algorithmic}[1]
\STATE \textbf{Input} : query point $p_q$, reference point $p_r$, list of kernel point estimates ${f}_p$
\STATE \textbf{Output} : kernel value $K(d(p_q,p_r))$
\STATE $g(p_q) \leftarrow g(p_q) + K(d(p_q,p_r))$
\STATE \textbf{return} $K(d(p_q,p_r))$
%\STATE Initialize the heap $H$ consisting of pairs in $\text{Vertices}(G) \times \mathbb{R}$ with the single pair $(p,0)$
%\STATE Dist$(p) \leftarrow 0$, $\NDP(p) \leftarrow \emptyset$
%\WHILE{the heap $H$ is not empty}
%\STATE q $\leftarrow$ H.pop()
%\FOR{\text{each vertex } $r$ \text{ adjacent to $q$ in the graph $G$}}
%\STATE $\leftarrow \text{Dist}(q) + d(r,q)  $
%\IF{Dist$(r) > t$ and $t < \delta$}
%\STATE Dist$(r) \leftarrow t$, $\NDP(r) \leftarrow q$
%\STATE H.push$(r, t)$
%\ENDIF
%\ENDFOR 
%\ENDWHILE
\end{algorithmic}
\end{algorithm}

\begin{algorithm}
\caption{Absolute-value approximation kernel density estimation Score()}
\label{alg:ScoreKDE}
\begin{algorithmic}[1]
\STATE \textbf{Input} : query node $\mathcal{N}_q$, reference point $\mathcal{N}_r$, list of node kernel estimates $f_n$
\STATE \textbf{Output} : a score for the node combination $(\mathcal{N}_q, \mathcal{N}_r)$ or $+\infty$ if the combination should be pruned
\IF{$|K(d_{\max}(\mathcal{N}_q, \mathcal{N}_q))-(K(d_{\min}(\mathcal{N}_q, \mathcal{N}_q)| < \epsilon$ }
\STATE $g(\mathcal{N}_q) \leftarrow g(\mathcal{N}_q) + |\mathcal{D}^p(\mathcal{N}_r)|((d_{\min}(\mathcal{N}_q, \mathcal{N}_r) + d_{\max}(\mathcal{N}_q, \mathcal{N}_r))/2 $
\STATE \textbf{return} $+\infty$
\ENDIF
\STATE \textbf{return}  $ |f(d_{\max}(\mathcal{N}_q, \mathcal{N}_q))-f(d_{\min}(\mathcal{N}_q, \mathcal{N}_q)|$

%\STATE $f_p(p_q) \leftarrow f_p(p_q) + f(d(p_q,p_r))$
%\STATE \textbf{return} $f(d(p_q,p_r))$
%\STATE Initialize the heap $H$ consisting of pairs in $\text{Vertices}(G) \times \mathbb{R}$ with the single pair $(p,0)$
%\STATE Dist$(p) \leftarrow 0$, $\NDP(p) \leftarrow \emptyset$
%\WHILE{the heap $H$ is not empty}
%\STATE q $\leftarrow$ H.pop()
%\FOR{\text{each vertex } $r$ \text{ adjacent to $q$ in the graph $G$}}
%\STATE $\leftarrow \text{Dist}(q) + d(r,q)  $
%\IF{Dist$(r) > t$ and $t < \delta$}
%\STATE Dist$(r) \leftarrow t$, $\NDP(r) \leftarrow q$
%\STATE H.push$(r, t)$
%\ENDIF
%\ENDFOR 
%\ENDWHILE
\end{algorithmic}
\end{algorithm}

\begin{thmm}
\label{thmm:KDE_time}
\cite[Theorem~3]{curtin2015plug}
Let $(X,d)$ be a finite metric space and let $S_q, S_r$ be its finite subsets and let $N = \max(S_q,S_r)$. Then the calculation of $\epsilon$-approximation of Kernel Density Estimate $f_K$ on kernel $K: \R \rightarrow \R$ of Definition \ref{dfn:KDE} computed using standard cover tree traversal from Algorithm \ref{alg:StandardCoverTreeTraversal} parametrized by BaseCase() from Algorithm \ref{alg:BaseCaseKDE} and Score() from Algorithm \ref{alg:ScoreKDE} has the asymptotic complexity
 \begin{equation}
\label{eqa:KDE_time}
\tag{\ref{thmm:KDE_time}}
 O(c_r^{8 + \log_2(\zeta)}(N + I + \theta(S_q, S_r))),
 \end{equation}
where $\zeta = -K'(h)K^{-1}(\epsilon)/\epsilon$,  $I$ and $\theta$ are defined in Definition \ref{dfn:DfnNineOfDissertation} and Lemma \ref{lem:FourOfDissertation}.
\bs
\end{thmm}

\begin{cor}
\label{cor:KDE_timeQR}

Assume the conditions of Theorem \ref{thmm:KDE_time} with assumption that $X = S_q = S_r$. Then the run time of standard cover tree traversal of Algorithm \ref{alg:StandardCoverTreeTraversal}  parametrized by BaseCase() from Algorithm \ref{alg:BaseCaseKDE} and Score() from Algorithm \ref{alg:ScoreKDE}
is $$ O(c^{10 + \log_2(\zeta)}\log(|X|) |X|),$$
where $c$ is the expansion constant of set $X$. 

%The problem \ref{pro:KNN}, where $S_q = S_r$ can be solved by building cover tree $\mathcal{T}$ and running the standard cover tree pruning dual-tree traversal (Algorithm \ref{alg:StandardCoverTreeTraversal}) parameterized by the $k$ nearest neighbor search functions BaseCase() and Score() as given in Algorithms \ref{alg:BaseCaseKNN} and \ref{alg:ScoreKNN}, respectively. 
%Assume that $|S| = N$ Let $c$ be the expansion constant of $S$. Then running time of the algorithm is bounded by

\end{cor}
\begin{proof}

The desired bound is obtained from Lemma \ref{lem:CoverTreeImbalanceUpperBound} and the fact that $\theta(S,S) = 0$ that are applied on Equation \ref{eqa:KDE_time}.

\end{proof}


==> chapters/chapterN.tex <==
\chapter{Preliminaries} % Write in your own chapter title
\label{ch:preliminaries} % Add a label in case you want to refer to the chapter.

Some definitions and preliminary results.

==> chapters/chapterNotation.tex <==
\chapter{Notation} % Write in your own chapter title
\label{ch:notation} % Add a label in case you want to refer to the chapter.

Through the thesis the following notation will be used: 

\begin{dfn}
Let $a,b$ the two points in $\mathbb{R}^m $, we denote the line segment by $[a,b]$.  
\end{dfn}
